Boundary Treatment for Variational Quantum Simulations of Partial Differential Equations on Quantum Computers

The paper presents a variational quantum algorithm to solve initial-boundary value problems described by second-order partial differential equations. The approach uses hybrid classical/quantum hardware that is well suited for quantum computers of the current noisy intermediate-scale quantum era. The partial differential equation is initially translated into an optimal control problem with a modular control-to-state operator (ansatz). The objective function and its derivatives required by the optimizer can efficiently be evaluated on a quantum computer by measuring an ancilla qubit, while the optimization procedure employs classical hardware. The focal aspect of the study is the treatment of boundary conditions, which is tailored to the properties of the quantum hardware using a correction technique. For this purpose, the boundary conditions and the discretized terms of the partial differential equation are decomposed into a sequence of unitary operations and subsequently compiled into quantum gates. The accuracy and gate complexity of the approach are assessed for second-order partial differential equations by classically emulating the quantum hardware. The examples include steady and unsteady diffusive transport equations for a scalar property in combination with various Dirichlet, Neumann, or Robin conditions. The results of this flexible approach display a robust behavior and a strong predictive accuracy in combination with a remarkable polylog complexity scaling in the number of qubits of the involved quantum circuits. Remaining challenges refer to adaptive ansatz strategies that speed up the optimization procedure.

==> Container/C_Feb10_Sections/RED-ComputationalStrategy.tex <==
%###########################################
%       Computational Model
%###########################################
\section{Computational Model} \label{sec:Strategy}

%On a Classical Computer (\textsc{CC}), the discrete optimization problem introduced in Sec. \ref{sec:Discretization} can be implemented following the known procures. The solution is encoded by a certain number of bits, which is proportional to the number of grid points $N_\text{p}+1$ and their numerical resolution, i.e. the floating-point arithmetic. On a Quantum Computer \textsc{QC}, the processing of information is executed on qubits, being the bit counterparts. Analogue to the CC, are the qubits again collected in a register. In the scope of this work, we practice the Big-endian standard.
This section outlines the framework for evaluating \Eq{eq:Discrete_Opt_BC} on a QC. %using a Variational Quantum Algorithm (\textsc{VQA}) initially presented by \cite{Lubasch2020}. 
 Sec. \ref{sec:VQA} describes the overall Variational Quantum Algorithm (VQA)
 which shares features with \cite{Lubasch2020}. Subsequently,  the operations used to calculate the different contributions ($j_{L_k}, j_{S_k}, j_{P_k}$) to \Eq{eq:Discrete_Opt_BC} on a QC are described in Sec. \ref{sec:Compilation}. These quantum circuits are also used to approximate the derivative of the objective functional with respect to the parameters in Sec. \ref{sec:Derivative1}, which in turn is required to advance the optimization, cf Sec. \ref{sec:Optimization}.

As outlined by \Eq{eq:discretization_register},
%For the setting covered, 
a register of length $n =\log_2\left(N_\text{p}\right)$ is required to evaluate the objective functional, if ghost-points contributions are represented classically, i.e. on classical hardware. The register is to be realized on a quantum computer using $n$ qubits.
%\trung{From here to the end of the paragraph, I have difficulties to understand the chain of information. We should (a) briefly describe the steps (subsection) needed to implement the equations outlined in II and III + think about ways to avoid duplicate notations - or at least clearly indicate their relations and why we express things differently in this section.} 
Each of the $n$ qubits recovers two distinguishable states, e.g. in the practiced Dirac notation as $\ket{0} = \left(1,0\right)^\intercal$ and $\ket{1}= \left(0,1\right)^\intercal$ \cite{Nielsen2010}. 
%The abbreviation, $\ket{i} = \eb_i$ as the $i$th orthonormal basis of the given vector space \cite{Nielsen2010}, viz. $\ub = u_k \eb_k = \ket{u}$.
%Consequently, a quantum register $\ket{\psi}$ with $n$ qubits contains the basis states $\ket{\psi} = \ket{\psi_1} \otimes \ket{\psi_2} \otimes \hdots \otimes \ket{\psi_n}$, where $\ket{\psi_n} = \alpha_n \ket{0} + \beta_n \ket{1} :~\alpha_n,\beta_n~\in~\mathbb{C}$. 
The $i$th element of orthonormal basis can be expressed with a binary representation $\text{bin}(i)$ as $\ket{\text{bin}(i)} = \eb_i = \ket{i}$, following a \textit{big-endian} convention (left~$\rightarrow$~least-, right~$\rightarrow$~most- significant qubit)
This encoding enables the representation of the discrete $\ub$ by the amplitudes of the quantum register, viz.  $\ub = \sum\limits_{k=1}^{\text{N}_p} u_k \eb_{k-1} = \ket{u} = \sum\limits_{k=1}^{\text{N}_p}u_k \ket{\text{bin}\left(k-1\right)}$, where 
the offset of the indices results from the technical necessity that the basis vectors $\eb_k$  start at $k=0$ but the interior unknowns $u_k$  begin with $k=1$.
%The qubit encoding allows the representation of high resolved function values $u_k \in \mathbb{C},u : \bra{u^*}\ket{u}=1$ at each grid point $x_k \in \O$, represented by the complex amplitudes of the quantum state.
%, as it is intended in \Eq{eq:discretization_register}.
%The numerical resolution of an entity (e.g. $u_k$) at the grid point itself, is independent of the number of qubits $n$. In contrast to a \textsc{CC}, this is one great advantage. However, the normalization condition: the partition of unity (c.f. \Eq{eq:partition_of_unity}), of the quantum physical system must always be fulfilled. Mention that, increasing the number of qubits $n$ to achieve higher resolutions, the amplitudes of $u_k$ are increasingly compressed to conserve the partition of unity. Restricted to single or double precision, this limits the measurement possibilities. Despite, the map $\ket{\text{bin}\left(k\right)}: k \mapsto \ket{\text{binary}\left(k\right)}$, delivers the $k^{th}$ orthonormal basis of the underlying Hilbert space. 
%Accordingly, the values $u_k$ in spatial dimension $x$ can be encoded by $\ket{u} = \sum\limits_{k=1}^{\text{N}_p}u_k \ket{\text{bin}\left(k-1\right)}  \ub = \sum\limits_{k=1}^{\text{N}_p} u_k \eb_{k-1}$.
%, where $u_k$ refers to the amplitude of $u$ at $x_k$. 
Mind that, though complex $u_k$ are generally allowed, we assume real solutions of \Eq{eq:Generic_PDE-TR}, hence $u_k^* =  u_k$, and that the time index is mostly suppressed in this section to improve the readability. 

%\pover{I dont think the normalization cont. needs to be transformed to discrete space -  y= lamb u }
%Since the solution $y(x)$ of \Eq{eq:Generic_PDE} is continuous in space, the discretization affects the normalization. Discretizing the continuous representation of the partition of unity (c.f. \Eq{eq:partition_of_unity}) by the midpoint rule results in 
%\begin{align}
%    1 = \sum \limits_{k=1}^{\text{N}_p} y_k^* y_k\Delta x = \sum \limits_{k=1}^{\text{N}_p}  \lambda_0^2 u_k^* u_k.
%    \label{eq:normalizedf}
%\end{align}

%With the hardware requirements in mind, the following section aims to cover the approximation of the solution to the problem given in \trung{which Equation is that now?:} \Eq{eq:Generic_PDE} using \textsc{VQA} initially presented by \cite{Lubasch2020}. 

%###########################################
%       Variational Quantum Algorithm
\subsection{Variational Quantum Algorithm} \label{sec:VQA}
The \textsc{VQA} methodology aims to minimize an  objective functional $J^{l}$ given in \Eq{eq:Discrete_Opt_BC}, by optimizing the control $\upb^{l}= (\lambda_0^{l}, \lamb_c^{l})^\intercal$ for every time step $l$. The hybrid framework utilizes both classical and quantum hardware, %\pover{restarted every for every discrete $t_l$ step}
 as displayed in \Fig{fig:optimizer}. 
%\pover{In the following, the dependence on the time is dropped for the sake of readability. If necessary it is given explicitly.}
\begin{figure}[htbp]
    \centering
    \input{Figures/communication_opt}
    \caption{Sketch of the hybrid  \textsc{VQA} optimization (time dependence is suppressed for the sake of clarity).}
    \label{fig:optimizer}
\end{figure}

The functional $J^l$ is evaluated on the quantum device, as illustrated by the grey box in Fig. \ref{fig:optimizer}, whereas the optimization process runs on the classical hardware that controls the process and iteratively adjusts the control $\upb$.
%The classical part has full control 
%on the quantum-based parametrization of the objective and thus 
%over the solution, which is parameterized by the ansatz $u(\lamb_c)$. 
For a particular set of ansatz parameters $\lamb_c$, the objective functional is evaluated from dedicated, individual so-called Quantum-Nonlinear-Processing-Units (QNPU, cf. Sec. \ref{sec:Compilation}) for each group of terms in \Eq{eq:Discrete_Opt_BC}, i.e. for $j_{L_k}, j_{P_k}, j_{S_k}$ etc. . An update $\Delta\upb$ is determined by the optimizer as outlined in Sec. \ref{sec:Derivative1} before a new iteration starts.

 Figure \ref{fig:VQA_QNPU} describes the general layout. Grossly speaking, it consists of a measuring  (aka. \textit{Ancilla}) qubit in the upper ''wire''  and a calculation 
 ''wire'' in the lower portion.
  Analogous to classical iterative solution procedures, an initial solution is required to start the calculation. On the quantum device, the qubit registers are initialized to a base state $\ket{0}^{\otimes n}=\ket{0}\otimes\ket{0}\otimes~\hdots~\otimes~\ket{0}$, where $\otimes$ is a dyadic product (cf. \Fig{fig:VQA_QNPU}).
  %, and fed into a quantum circuit composed of a predefined series of quantum operations approximating the PDE dynamics. 
 %The framework is highly dependent on the problem, which determines the layout of the quantum gates, their actions, and the type of measurement needed.
%In addition to this, a gate always requires being unitary to respect the partition of unity (given in \Eq{eq:partition_of_unity}). In classical CFD, this requirement does not exist, which makes unitarization one key discipline in the compilation to quantum hardware. 
\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{0.7\textwidth}
        \centering
        \input{Figures/QNPU.tex}
        \caption{Sketch of a \textsc{VQ} circuit composed of the ansatz $U(\lamb_c)$, the $T_t$ assembly, a specific \textsc{QNPU}, and a measurement qubit (\textit{ancilla} qubit) for indirect measurements. $H$ indicates a Hadamard gate, \textsc{CP} Control Port, \textsc{IP} Input Port, \textsc{OP} Output Port, and $\sigma_z$ provides the expectation value of the measurement operation, cf. \cite{Lubasch2020}.}
        \label{fig:VQA_QNPU}
    \end{subfigure}
    \begin{subfigure}[t]{0.7\textwidth}
         \vspace*{2ex}
        \centering
        \input{Figures/Ansatz.tex}
        \caption{Example of an ansatz circuit $U(\lamb_c)$  composed from  $a=10$ fundamental gates $\Tilde{U}(\lamb_i)$ featuring a bricklayer topology,  parameterized by $\lamb_c = (\lamb_1, \lamb_2,\hdots, \lamb_a)^\intercal$ parameters to encode a test function $\ket{u}$ on $n = 6$ qubits, cf. \cite{Lubasch2020}.}
        \label{fig:VQA_Ansatz}
    \end{subfigure}\\
    \begin{subfigure}[b]{0.7\textwidth}
     \vspace*{2ex}
        \centering
        \input{Figures/SO4_ansatz.tex}
        \caption{Two qubit SO4 ansatz $\Tilde{U}(\lamb_i)$ 
        %\sout{of the \textit{Special Orthogonal 4} Lie Group } 
        to create an optimal variational state \cite{Vatan2004} based on $\lamb_i = \left(\lambda_{i,1},\lambda_{i,2},\hdots,\lambda_{i,6}\right)^\intercal$ individual parameters. In the first layer ($d=1$) the ansatz has only three parameters in $\lamb_i$, the rotation gates corresponding to $\lambda_{i,4}$, $\lambda_{i,5}$, and $\lambda_{i,6}$ are identity gates.}
        \label{fig:quantum_ansatz_SO4}
    \end{subfigure}    
     \vspace*{2ex}
    \caption{Illustration of the employed
    %three fundamental 
     nested VQA circuits.
     %given in \subref{fig:VQA_QNPU},\subref{fig:VQA_Ansatz}\& \subref{fig:quantum_ansatz_SO4}.
     }
    \label{fig:VQA}
\end{figure}
% In this calculation wire, t

  The initial solution is introduced to an ansatz circuit called $U$,
  highlighted in grey. The ansatz $U$ can be denoted by a $N_\text{p} \times N_\text{p}$ matrix. 
 %
 The latter
 follows from an embedded combination of two-qubit-units, i.e. fundamental gates $\tilde U (4 \times 4)$, as illustrated in \Fig{fig:VQA_Ansatz} for the example of 6 qubits. The particular combination employed in this research refers to a scalable depth bricklayer topology and shares some similarities with 
 machine learning topologies. 
 The benefit of the bricklayer topology over alternative topologies has been communicated in \cite{Nakaji2021}. 
 %
 The employed fundamental gate 
  is displayed in dark grey in \Fig{fig:VQA_Ansatz}-\ref{fig:quantum_ansatz_SO4}. 
 It has been suggested by 
 Vatan and Williams \cite{Vatan2004} and is frequently labeled SO4. 
 This gate operates in real and imaginary space which is rather unusual for engineering applications that aim for real-valued results \cite{Sato2021,Leong2022}. Its application promises a richer ansatz function space, which in turn supports the use of shallower depth $d$ in $U$.
 %
 %The circuit implementing the general two-qubit transformation is not a real valued ansatz. 
 As displayed in \Fig{fig:quantum_ansatz_SO4}, the fundamental gate consists of \textsc{R$_y$}, \textsc{R$_z$} and \textsc{CNOT} gates, where \textsc{R$_y$} and \textsc{R$_z$} are parameterized versions of classical Pauli $\sigma_y$ and $\sigma_z$ matrices \cite{Nielsen2010}, and the $(\dots)^\dagger$ symbol indicates the transposed of the conjugate complex. 
 %
 %Additionally mention, that the $R_z(\lambda)$ gates involve imaginary values (c.f.\Fig{fig:quantum_ansatz_SO4}).
 %
 Turning back to \Fig{fig:VQA_QNPU}, the result of the ansatz circuit $U$ is the parameterized state $\ub=\ket{u}$. 
 \pover{Boundary conditions are introduced using a specific matrix $T_t \, (N_\text{p} \times N_\text{p})$ and a specific succeeding gate. The transformation $T_t$ essentially modifies the order of qubits in the register $\ket{u}$. In any other case than the $j_{DN_{1,N_\text{P}}},j_{N_{1,N_\text{P}}}$ contributions, $T_t$ is not required and degenerates to the identity matrix.} 
 \sout{The boundary conditions are subsequently introduced by a specific matrix $T_t \, (N_\text{p} \times N_\text{p})$,  which essentially modifies the order of qubits in the register $\ket{u}$.
 For periodic conditions, $T_t$ simply degenerates to the identity matrix and could be dropped. }
 %
 Through an input port (IP), the result serves as input to the \textsc{QNPU} unit, indicated in light grey in \Fig{fig:VQA_QNPU}, which outputs (OP) the specific objective functional contributions for a group of terms ($j_{L_k}, j_{P_k}$, etc.).
 Different groups require diverse QNPUs, as described in Sec. \ref{sec:Compilation}.
  %
 Rather than assessing the individual contributions at each  grid point $k$, we 
 use a Hadamard test approach \cite{Endo2020} %\pover{May exchange ENDO2020 -  reference to Hardamard test - endo only provides in the appendix} 
 to directly compile the integral, i.e. the sum over all interior grid points, for example $\sum_k j_{L_k}$, and measure its related expectation value denoted by $\sigma_z$
 %= \mathcal{R}\left(\bra{0}U^\dagger  T_t^\dagger \text{ QNPU } T_t U \ket{0}\right)$, where $\mathcal{R}$ denotes the real-part 
 \cite{Nielsen2010}. This is indicated by the upper ''wire'' of \Fig{fig:VQA_QNPU} that connects to the calculation ''wire'' through a control port (CP).
 Mind that experiments with the Hadamard test indicated quantum advantage \cite{Guseynov2023}, which suggests its use.
% \trung{A brief matrix representation of the employed quantum gate/operator symbols if provided in Appendix ?}.
 

%\begin{enumerate}
%     \item \trung{Implementierung der Summe bzw. des Integrals}  The upper qubit, so-called ancilla, is intended for indirect measurements according to the Hadamard test \cite{Endo2020}. The register $\ket{0}^{\otimes n}$ is therefore augmented by another qubit, to $\ket{0}\otimes\ket{0}^{\otimes n}$.
%     One can show that the expectation value results is $\sigma_z = \mathcal{R}\left(\bra{0}U^\dagger\left(\lamb_c\right)  T_t^\dagger \text{ QNPU } T_t U\left(\lamb_c\right)\ket{0}\right)$, where $\mathcal{R}$ denotes the real-part \cite{Nielsen2010}.
%     \trung{Paralleles abgreifen des Outputsignals aus QNPU und streamen über 2x2 Matrix sigma-z was den Erwartungswert des Integrals erzeugt (nicht der einzelenen Beitraege) - durch Spurbildung}
%     The advantage of indirect measurement in contrast to direct measurement is to reduce to a single measurement, instead of multiple measurements $M$, see \Fig{fig:VQA_QNPU}. Secondly, experiments with the Hadamard test showed Quantum advantage in comparison to Classical Computers \textsc{CC} \cite{Guseynov2023}. 
     %Comparing the expectation value given, underlines the similarity of the expressions to that appearing in the bilinear-form $a(\cdot,\cdot)$, c.f. \Eq{equ:weighted_res-2}. 
        
%    \item \pover{Implementierung von der Ansatzfunktion} \trung{Gross U ist generell eine Abbildung zur Erzeugung von klein u. Gross U ist nNp xNp Matrix bestehend aus verschachtelten tilde U die 4 x 4 Matrizen sind  (aus 2 qbits)}
%    The gray filled gate in \Fig{fig:VQA} is the parameterized hardware efficient alternating layer ansatz $U(\lamb_c)$ (ALA). It is the quantum realization of the test function $u$ and spans the normalized ansatz function space, realizing $\ket{u} = U(\lamb_c)\ket{0}^{\otimes n}$. Training the ansatz parameters $\lamb_c$ to transform the initial state $\ket{0}^{\otimes n}$ to approximation $\ket{u}$ is the crucial part of the \textsc{VQA} method. Therefore, one distinguishes between expressibility and trainability in terms of ansatz characterization \cite{Tilly2022}. Both characteristics are comparable well given by the ALA approach \cite{Nakaji2021}.
   % \pover{Why bricklayer ?\cite{Uvarov2021, Tilly2021} -  No check https://quantum-journal.org/papers/q-2021-04-19-434/pdf/ Here they compare ALA Tensor and Leong kind ansatzes and the expressibilty of Bricklayer is greater}. Accordingly, the register $\ket{\psi}$ concludes in $u(\lamb)\ket{0} = u$.
%    The internal structure of the gray $U(\lamb_c)$ is given in \Fig{fig:VQA_Ansatz}. It consists out of $a$ identical building blocks $\Tilde{U}(\lamb_i)$, referred to as base ansatz. With rising depth $d$, more alternating layers of basis ansatz are added. The parameters are kept unique overall $a$ basis ansatz, viz. $\lamb_c = \left(\lamb_1,\lamb_2, \hdots, \lamb_a\right)^\intercal$. One base ansatz is given exemplary in \Fig{fig:quantum_ansatz_SO4}. To achieve the most optimal span in the category of fixed structure and hardware efficient ansatz, we use the advanced two-qubit ansatz as the basis $\Tilde{U}(\lamb_i)$, given by \cite{Vatan2004}. The basis ansatz realizes every two-qubit gate in SO4 \cite{Vatan}.
    %\pover{What is the benefit of SO4 - why is it optimal?}
%    The circuit implementing the general two-qubit transformation is not a real valued ansatz. It consists out of $R_y(\lambda),R_z(\lambda)$ and \textsc{CNOT} gates. Whereas $R_y(\lambda) \, \& \,R_z(\lambda)$ are parameterized versions of the basic $\sigma_y$ and $\sigma_z$ gates. Additionally mention, that the $R_z(\lambda)$ gates involve imaginary values (c.f.\Fig{fig:quantum_ansatz_SO4}). The resulting phase modulation $\varphi = \nicefrac{1}{2}\sum\limits_{\{1,3,4,6\}}\lambda^i$ is to be corrected after the measurement, by multiplication with the corresponding inverse Euler representation.
    %$\exp(- i \, \nicefrac{\sum\limits_{\{1,3,4,6\}}\lambda^i}{2})$.
%    It is a difference in contrast to \cite{Sato2021,Leong2022}, which rely on real valued ansatz to represent real valued results, as it is motivated by \cite{Alghassi2022}.
    %\TODO{ARGUE that we use not a real valued ansatz.} Despite, the experience showed that the expressibility of non-real valued ansatz is greater  \TODO{Show Results regarding expressibility -  It is novel that we use such a advanced ansatz.}

%\item 
%\pover{We do not use ZGR QFT since it ULA outperformes for n<5 \cite{Sarma2023} -  requires many qubits}
%\pover{adapt rho is applidudes flip sign}

%    \item \trung{Tt ist auch eine NpxNp Matrix, die - ähnlich wie U - eine Abbildung erzeugt. Diese erzeugt ein Antidiagonal Matrix. die die Randbedingungen erzeugt   }
%    The transformation $T_t$ modifies the order of the qubits in the register $\ket{u}$, according to the subsequent QNPU. It is a feature, which is not described in \cite{Lubasch2020} and is necessity to represent the novel building blocks of the VQ-assembly. In many cases $T_t= I$, except mentioned separately. 

%    \item The Quantum Nonlinear Processing Unit (\textsc{QNPU}),
%    \trung{erzeugt Laplace Potenzial, Quelle ...} the key element is a succession of quantum gates, representing PDE effects of the system, e.g. in \Fig{fig:VQA_QNPU}. The QNPU takes a prepared state, e.g. $\ket{u}$, on the input port \textsc{IP}. The process ist controlled on the control port \textsc{CP} by the ancilla. The output is then visible on the output port \textsc{OP}. Each QNPU needs to hold these three interfaces. In the current case, the QNPU is required to represent the discretized dynamics, e.g. the Laplace operator, or the source term. Each effect is modelled individually, demanding a library of compiled QNPUs. These are introduced in Sec.\ref{sec:Compilation}.
    
    %of \Eq{eq:Generic_PDE} represented by the functionals $j_i$. Each term $j_i$ of $J$ is evaluated individually.
%\end{enumerate}


Before we discuss the individual QNPUs, the measurement strategy implemented here should be described for the sake of completeness. We rely on the corresponding density matrix of the \textit{ancilla} to approximate the expectation $\sigma_z$ at the measurement gauge in \Fig{fig:VQA_QNPU}. To eliminate stochastic influences, the evaluation of QC-calculated results is usually based on the evaluation of sufficiently large samples. However, if the QC is only emulated, as is the case in the current study, the procedure can be simplified using the trace-out method \cite{Nielsen2010}.  
%
%The measurement method described in sec. \ref{sec:measurement_method} is discarded because it is not capable to calculate an accurate approximation to the solution of the problem. 
The state vector simulation delivers the whole vector state, cf. \Fig {fig:VQA_QNPU}. For an exemplary state $\psi$ this reads 
$\ket{\psi} = \ket{\psi}_\text{ancilla} \otimes \ket{\psi}_\text{\text{QNPU}}$, i.e. \textsc{QNPU} and \textit{ancilla} qubits. As we are only interested in the information collected on the ancilla portion of $\ket{\psi}$, the remainder is traced out and the density operator ${\mbox{$\bm{\rho}$}\xspace}_\text{ancilla}$ of the ancilla remains, viz.
\begin{align}
%    \ket{\psi}  = \ket{\psi}_\text{ancilla} \otimes \ket{\psi}_\text{QNPU}  \quad \text{and} \quad  
    \mbox{$\bm{\rho}$}\xspace = \ket{\psi} \bra{\psi}  \quad \to \quad 
    {\mbox{$\bm{\rho}$}\xspace}_\text{ancilla} = \Tr{\mbox{$\bm{\rho}$}\xspace}_\text{QNPU} = \ket{\psi}_\text{ancilla} \bra{\psi}_\text{ancilla} \Tr{\ket{\psi}_\text{QNPU} \bra{\psi}_\text{QNPU}}.
\end{align}
%\end{document}

%The evaluation of the quantum device is commonly done using $M$ samples, we restrict the information description by tracing out the subsystem “QNPU register”. We rely on the corresponding density matrix of the ancilla, incorporating the partial trace, to approximate the expectation $\sigma_z$ at the measurement gauge, given in \Fig{fig:VQA_QNPU}.  

By this, the result of a state-vector simulation recovers the same effect as intended by the indirect measurement performed on real hardware, without noise and sampling errors \cite{Nielsen2010}. 

%\pover{Wir könnten natürlich auch eine Simulation (Poisson Dir Homo.) mit echter messung machen und dann in der Conclusion diskutieren das hier probleme vorliegen. Wir haben diese Versuche ja gemacht. Die Erfahrung hat gezeigt das es möglich ist die jew. PDE zu lösen, blos die Genauigkeit bleibt wünschenswert.}
%The investigation of the proposed library on NISQ devices, regarding sampling complexity, is motivated for future research. In the following, a library of QNPUs is introduced in detail.
%###########################################
%       Compilation of the Quantum-Nonlinear-Processing-Units
\subsection{Quantum-Nonlinear-Processing-Units}
\label{sec:Compilation}
For the introduction of our library of QNPUs, we use a complex number notation. All QNPUs are highlighted in light gray in the respective figures. They are adjustable to an arbitrary equidistant one-dimensional discretization and have been designed to keep the gate sequence shallow. 
%The set of to-be-presented QNPUs cover dynamics, which commonly occur in PDEs, as in the form of that given in \Eq{eq:Generic_PDE} and as they are common for CFD. 


% EQ 42 - https://quantum-journal.org/papers/q-2022-06-07-730/pdf/
%\pover{Use swap test technqiues to determine initials}
%It follows a detailed overview of the Quantum circuits, each compilation is %sketched in a small example to extract the general pattern.

\medskip
%###########################################
%       Laplace
\subsubsection{Periodic Laplace operator} \label{sec:Compilation:Laplace}
The  Laplacian is given 
%is one of the most frequently differential operators when it comes to PDEs in the context of CFD. Hence, it is a necessity to derive a robust and flexible compilation for the quantum hardware. Inspecting the 
by the finite difference stencil in \Eq{eq:derivatives_space} and partly resembles the classical bit shift operator \cite{Vedral1996,Nielsen2010} due to shifted products, e.g. $u_k^{l*} u_{k+1}^\pover{l}$, $u_k^{l*} u_{k-1}^l$. 
The related QNPU circuit employed herein is based on the adder circuit. In contrast to other approaches, e.g. general decomposition method \cite{Liu2021} or a physically motivated decomposition \cite{Sato2021}, the adder circuit convinces by a  (smaller) polynomial scaling of the gate complexity. Mind that an adder QNPU to
 compute a periodic Laplace operator has previously been reported by Lubasch et al. \cite{Lubasch2020}. 

Using $n\leq 2$ qubits,  a half-adder circuit can be used, which consists of one \textsc{CNOT} ($n=1$) and an additional Toffoli gate ($n=2$). For $n > 2$, additional ($n-2$) carry qubits (auxiliary qubits) are required, which  results in 
%. For the construction of the now-demanded, 
full-adder QNPU circuits, cf. 
%. as well as the theory, the reader is referred to literature on classical computing
\cite{Parhami2010} and \cite{Darper2000,Nielsen2010}. 
%
Assuming a periodic state, it can be shown \cite{Lubasch2020}, that 
%the equation can be reduced to three terms $u_k^* u_{k+1},\; u_k^* u_{k} \;\& \;u_k^* u_{k-1}$, where the first and last request a multiplication by a shifted value. For closure, periodic BC simplifies the expression until a certain point. Accordingly, one can give 
the general structure of the discrete Laplace operator %which
acts like 
\begin{align}
\label{eq:Laplace}
    \sum\limits_{k=1}^{N_\text{p}}u_k \ket{\text{bin}\left(k-1\right)} \to  \sum \limits_{k=1}^{N_\text{p}} u_{k+1}  \ket{\text{bin}\left(k-1\right)} \qquad \text{with} \qquad {1= \sum_{k=1}^{N_\text{p}} u_k^* u_k}.
\end{align}
%\sout{Again, mention that $(u,u)_{L_2}=1.$} 
%\pover{Is the time increment necessary? Where do we want to show ? }
\Fig{fig:Laplace_compiled} depicts an example of the employed Laplace QNPU circuit 
for $n=6$ qubits and $n-2 = 4$ carry bits. The circuit involves $n-2=4$ \textsc{CNOT} gates and $2n-2=10$ Toffoli gates. 

\begin{figure}[htbp]
    \centering
    \input{Figures/Adder.tex}
    \caption{Exemplary quantum circuit of the discrete Laplace in the Hadamard test configuration. The example refers to $n=6$ qubits and  $n-2=4$ carry bits. It requires $n-2=4$ \textsc{CNOT} and $2n-2=10$ Toffoli gates. For $n=2$ qubits, this circuit is exactly implementing a half-adder, cf. \cite{Lubasch2020}.
    }
    \label{fig:Laplace_compiled}
\end{figure}

 %As a proof of concept, mention that the quantum registers for $n=2$ qubits can be decomposed in its complex amplitude as, $\ket{\psi} = \left(c_{00},c_{01},c_{10},c_{11}\right)^\intercal$. It can be shown that the initial state $ \ket{\phi_0} = \ket{0} \otimes \ket{\psi} = \ket{0} \otimes \left(c_{00}\ket{00}+c_{01}\ket{01}+c_{10}\ket{10}+c_{11}\ket{11}\right)$ evaluates to $ \langle\sigma_z\rangle =   \sum\limits_{k=0}^{NP-1}\psi_k\psi_{k+1}$, assuming real function values and periodicity.

%###########################################
%       Boundary Conditions
\subsubsection{Boundary Conditions}\label{sec:Compilation:BC}

\pover{give some more details for each circuit functionality -  to emphasize understandability}
We now introduce an approach to generalize the periodic Laplace implementation for other boundary conditions based on the ghost point approach discussed
in Sec. \ref{sec:Discretization}.%As a benefit of the ghost point implementation introduced in Sec. \ref{sec:Discretization} the adaption to different BC is just a question of finding the corresponding gate sequence for augmentation. In the following, we would like to present another two circuits to adjust the field dynamics to the boundary setting and to link internal and external discretization.
%The suggested method only requires to adjust the field dynamics to the boundary conditions and link the internal and external discretization.

To begin with, we would like to mention the transformation $T_t$ already given by Sato et al. \cite{Sato2021}, which acts using the \textit{Modulo operation} (\textsf{mod}) as
%, like an anti-diagonal matrix on a vector, by the action
\begin{align}
    \label{eq:shift}
    \sum\limits_{k=0}^{N_\text{p}-1} \ket{\text{bin}\big(\left(k+1\right) \textsf{mod} \left(N_\text{p}\right)\big)} \bra{\text{bin}\big(k\big)}.
\end{align}

%\pover{Is the time increment necessary? Where do we want to show ? }
%To correct the discretized dynamics in the previously given QNPU, this transformation is required to align the quantum register for the following modifications. 
An exemplary compilation of the transformation $T_t$ is given in \Fig{fig:Transformation}, which can be implemented as sketched in \Fig{fig:VQA_QNPU}. Note that the transformation $T_t$ inheres a sequence of multi-controlled gates, which can enhance the gate complexity, cf. Sec. \ref{sec:compilation:complexity} . 
\begin{figure}[htbp]
    \centering
    \input{Figures/Transformation}
    \caption{A generic shift operator represented by a sequence of multi-controlled Toffoli gates, exemplary given for $n=4$ qubits. In the following, referred as transformation $T_t$, cf. \cite{Sato2021}.}
    \label{fig:Transformation}
\end{figure}
\pover{Add the newly developed shift operator based on carry actions }
\pover{say explicitly that it is the same as the adder}

In contrast to the approach of Sato et al. \cite{Sato2021} and related studies of Leong et al. \cite{Leong2022}, the corrections for non-periodic conditions are represented as unitary circuits and therefore as quantum gates for an arbitrary number of qubits. In the case of Dirichlet and Neumann BC's, the circuits in \Fig{fig:QNPU_BC} are required as additional QNPUs. {The correction $j_{{DN}_k}$ consists out of $2n-1=7$ \textsc{CNOTS} and $2n=8$ multi-qubit controlled-Z gates. For Neumann boundary conditions and additional sequence of $j_{{N}_k}$ given by $2n-1=7$ \textsc{CNOTS}, one multi-qubits controlled-NOT and $2n=8$ multi-qubit controlled-Z gates come into account.}

\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{0.7\textwidth}
       \centering
        \input{Figures/Dirichlet.tex}
 \caption{Compiled QNPU for the implementation of  $j_{{DN}_{1,N_\text{p}}}$ used to realize both Dirichlet and Neumann conditions, cf. \Eq{eq:Discrete_Opt_BC}.}
        \label{fig:QNPU_BC_Dirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.7\textwidth}
        \centering
        \input{Figures/Neumann}
        \caption{Compiled QNPU for the implementation of  $j_{N_{1,N_\text{p}}}$ used to realize Neumann boundary conditions, cf. \Eq{eq:Discrete_Opt_BC}.}  
        \label{fig:QNPU_BC_Neumann}
    \end{subfigure}  
    \caption{Illustration of the novel boundary correction QNPUs for an exemplary $n=4$ qubits setup.}
    \label{fig:QNPU_BC}
\end{figure}
\medskip

  The complexity of boundary QNPUs illustrated in \Fig{fig:QNPU_BC_Dirichlet} and \Fig{fig:QNPU_BC_Neumann} is considerable, in particular, since their inputs refer to the already 
  more complex transformation $T_t$. Moreover, mind that results of the QNPU illustrated in \Fig{fig:QNPU_BC_Neumann} should also be captured by the QNPU that realizes the potential term, cf. discussion in Sec \ref{sec:Discretization}.
%\end{document}
%###########################################
%       Potential
\subsubsection{External Contributions (potential and source terms)} \label{sec:Compilation:Potential}


The computation of external contributions takes place in two subsequent steps.
%
First, a representation of the external effects on the quantum hardware  -- in this case the representation of the discrete linear source  $\tilde f_k^l$ and potential terms $p_k^l$ -- is assembled to enable computing their contributions to the objective functional in a second step. 
%using the gates outlined in \Fig{fig:QNPU_Potential} (cf. $P$) and  \Fig{fig:overlapp} (cf. $F^\dagger$) in a second step.


For simpler, analytically described terms, e.g. $exp(x)$ or $sin(x)$,  Lubasch et al.  \cite{Lubasch2020} introduced corresponding gate sequences that allow such functions to be represented on a QC. 
Other suggestions intensively deploy Matrix-Product-State  (\textsc{MPS}) techniques, \cite{Oseledets2012,GonzalezConde2023,Oseledets2010}. 
%as a programming paradigm 
%but \trung{... what is there problem - non-unitary? ...}
%.  \TODO{kürzen -> in 1 gibt es beispiele mit gates und wir machen es aber so :  }In this direction, the references \cite{Oseledets2012,GonzalezConde2023} deploy additional compilations for polynomials. For more advanced functions, the subject of \textit{TT-cross approximation techniques} can also be used to approximate the corresponding gate sequences \cite{Oseledets2010}.
%
In our case, however, we first solve a previous optimization problem to represent the external influences by quantum gates, taking the ansatz $U(\lamb)$  into account, viz. 
\begin{align}
     \bar{\lamb_c}=  \min\limits_{\lamb_c} \big(1 -\lambda_0\bra{u(\lamb_c)} \ket{g}\big) \text{ with } \frac{1}{\lambda_0^2}=\sum \limits_1^{N_\text{p}} g_k^{l*} g_k^l \, . 
    \label{eq:OptAnsatz}
\end{align}
%\pover{Double check} \trung{Muss Lambda0 oben nicht genau der Kehrwert der Vektorlänge sein?} \pover{ja}
In \Eq{eq:OptAnsatz} $\gb = \Tilde{\fb}$ or $\gb = \pb$ for the source and the potential term respectively. The benefit of this approach is that it re-uses existing implementations and also supports keeping the depth of the resulting circuits shallow. 
The optimal parameters $\bar{\lamb_c}$ determined in this way result in the required gates $U(\bar{\lamb_c}) = P$ and $U(\bar{\lamb_c}) = F^\dagger$ to be used inside the QNPUs that compute the potential and the source term contributions to $J$ in \eqref{eq:Discrete_Opt_BC}.
%. Therefore, we solve the preliminary problem 

The contribution of the potential term $p(x_k, t^l)$ to $J$ follows from 
%given by an inner product of an external potential $p\left(x\right)$ and the solution $y\left(x\right)=\lambda_0 u(x)$, which can be interpreted as 
$
    \sum\limits_{k=1}^{\text{N}_p} \left[ \lambda_0^2 u_k^*p_k u_k \right]^l 
$. 
%
%\trung{For the hardware shift of the external potential $p\left(x\right)$, requires representation by a corresponding gate sequence $P$.??} 
%In the presented framework, it is achieved solving \Eq{eq:OptAnsatz}, with \pb=\gb. The determined parameters $\bar{\lamb_c}$ yield $U(\bar{\lamb_c}) = P$.}
 The corresponding QNPU circuit is assembled by Toffoli gates according to \Fig{fig:QNPU_Potential} for the example of $N_\text{p}=4, n=2$. Since the multiplication $u_k^* p_k u_k$ is non-unitary, additional $n$ ancilla qubits occur \cite{Sarma2023} in the circuit. %\pover{Note, this circuit mimics an implementation of a diagonal matrix D = diag (p1, p2,p3,....,pn).}
%
\begin{figure}[htbp]
    \centering
    \input{Figures/Potential.tex}
    \caption{Exemplary quantum circuit based on the Hadamard test for a discrete potential function $\pb=( p_1, p_2,p_3, \dots p_{N_\text{p}})^\intercal$ represented by the gate ''$P$''. The displayed example refers to $\text{N}_p=4 \rightarrow n=2$ qubits and outlines the general pattern for $\text{N}_p \ge 4$ discrete points.}
    \label{fig:QNPU_Potential}
\end{figure}
%
%Assuming $n=1$ and $\ket{\theta_0} = \ket{0\psi0}$ as the initial state, a small sketch would deliver the expectation value $ \langle\sigma_z\rangle = \frac{1}{2} \sum \limits_{k=1}^2\psi_k^*v_k\psi_k + \psi_kv_k^*\psi_k^*$, which can be simplified to $\langle\sigma_z\rangle =\sum\limits_{k=1}^{2} \psi_k v_k \psi_k$ assuming real functions.
%
%###########################################
%       Generic Source Terms
%\subsubsection{Generic Source Terms} \label{sec:compilation:source}
%
%Besides the terms above, the \Eq{eq:Generic_PDE} holds a RHS given as $f$, referred to as the source term. It differs a lot from the compilations introduced. 
%\trung{Given the contributions linear in $u$, as they arise in the linear form $F$ of the variational \Eq{eq:variational_eq}, a generalized implementation is given.
%Assuming there is a gate sequence determined, representing the corresponding RHS $f=g$, by solving the problem in \Eq{eq:OptAnsatz}. }
%
Similarly, the gate representation $f = U(\bar{\lamb_c})$ is implemented into the source term QNPU (light gray) given in \Fig{fig:overlapp}. Instead of the uncontrolled ansatz $U(\lamb)$ displayed in 
Fig. \ref{fig:VQA_QNPU}, the linearity of the source term requires that $U(\lamb)$ (gray) is also controlled. 
%This is valid for all linear expressions in \Eq{}. 
\begin{figure}[htbp]
    \centering
    \input{Figures/Overlapp.tex}
    \caption{Evaluation of external source term $f$  by $\bra{u}\ket{f}$, with $T_t = I$.}
    \label{fig:overlapp}
\end{figure}
%
%As already introduced in sec. \ref{sec:Discretization}, requires an inhomogeneous boundary setting the augmentation of the source term $f$ by $f_\text{ghost}$. The additional $f_\text{ghost}$ is simultaneously compiled into a circuit as given above and substituted in the circuit given in \Fig{fig:overlapp}, underlying the modularity of the framework. As a final step, mention that the discretized time derivative, can be written an additional RHS. Thus, using an augmented form allows a direct implementation using the same approach \TODO{adjust time discretization to math sec.}.

%###########################################
%       Gate complexity
%\subsubsection{Gate Complexity} 
\section{Gate Complexity} 
\label{sec:compilation:complexity}
To scrutinize the scalability of the algorithm, the number of single- (\textsc{R$_z$,R$_y$,U,..}) and two-qubit (\textsc{CNOT},..) gates per qubit %for the \textsc{QNPU} circuits 
are outlined in this section.
%
%depicted in \Fig{fig:compilation:GateComplexity}. 
%
The scaling of the number of gates involved in the SO4 ansatz w.r.t. the number of qubits $n$ and the depth $d$ is reported in \Fig{fig:Results:SO4complex}. It is seen, that 
%For the \textsc{SO4} ansatz, 
 the number of gates scales linearly with $n$ and the depth $d$, i.e. $\mathcal{O}(7.5 \, n \, d)$.

\begin{figure}[htbp]
    \begin{subfigure}[t]{0.49\textwidth}
       \centering
        \input{Figures/Complexity/C_Ansatz_SO4.tex}
        \caption{Complexity %per qubit and depth 
        for the \textsc{SO4}-ansatz.} 
        \label{fig:Results:SO4complex}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Complexity/C_QNPU.tex}
        \caption{Complexity %w.r.t. the number of qubits
        for all \textsc{QNPU}s.} 
        \label{fig:Results:QNPUcomplex}
    \end{subfigure}
    \caption{Gate complexity of the employed QNPU and ansatz gate compilations.}
    \label{fig:compilation:GateComplexity}
\end{figure}


Graphs displayed  in \Fig{fig:Results:QNPUcomplex} illustrate the polynomial relation between the number of gates and the number of qubits for 
%the \textsc{SO4} ansatz in \Fig{fig:compilation:GateComplexity}(a) as well as 
the adder ($j_{L_k}$), the source ($j_{S_k}$), the potential circuit ($j_{P_k}$) and the boundary circuits ($j_{DN_{1,N_\text{p}}}, j_{N_{1,N_\text{p}}}$). 
Most QNPUs and the SO4 ansatz depict a linear complexity.
%
The linear complexity of the adder circuit, $\mathcal{O}(32 n)$, is due to the very local reach of the FD stencil for approximating the second derivative. In this case, the resulting circuit conserves the local property. 
%
%\end{document}
An analysis of the source and potential \textsc{QNPU}s also reveals a linear scaling of  $\mathcal{O}(72 n)$ and $\mathcal{O}(15 n)$, respectively, which underlines the importance of an efficient state initialization of generic functions \cite{Chen2021,Kyriienko2021,Creevey2023,Melnikov2023,Araujo2021}.
%
The similarity to the scaling behavior examined for the \textsc{SO4} ansatz is obvious and indicates the strong influence of using $U(\lamb_c)$ to determine $\Tilde{\fb}$ or $\pb$, cf. \Eq{eq:OptAnsatz}. The related overhead in the number of gates w.r.t the ansatz is due to the control operation of the ansatz in both \textsc{QNPU}s and the additional \textsc{CNOT} gates following the $P$ gate for the potential \textsc{QNPU}, see \Fig{fig:QNPU_Potential}.  Note that for the %source and potential \textsc{QNPU} 
values given in \Fig{fig:compilation:GateComplexity} the depth of the ansatz for $j_{P_k}$ and $j_{S_k}$ is assigned to $d=1$. 

The boundary \textsc{QNPU}s ($j_{DN_{1,N_\text{p}}}, j_{N_{1,N_\text{p}}}$), however,  scale exponentially, on the maximum order of $\mathcal{O}(4.8 n^{5})$. This was also observed by other researchers in conjunction with other approaches, for example, \cite{Sato2021,Leong2022,Leong2023}.  The reason for that, is the global property of the boundaries in elliptic \textsc{PDE}s, where the boundary definition influences the solution in the complete domain. The non-locality of the boundary implementation is also reflected by the shape of the circuit, which requires interaction with more than just the nearest neighbor qubits.

%\begin{figure}[htbp]
%\centering
%    \begin{subfigure}[t]{0.7\textwidth}
%       \centering
%        \input{Figures/Dirichlet.tex}
% \caption{Initial QNPU for the implementation of  $j_{{DN}_k}$ used to realize both Dirichlet and Neumann conditions, cf. \Eq{eq:Discrete_Opt_BC} and \Fig{fig:QNPU_BC_Dirichlet-1}.}
%        \label{fig:QNPU_BC_Dirichlet-1}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.7\textwidth}
%        \centering
%        \input{Figures/Neumann}
%        \caption{Modified QNPU for the implementation of  $j_{{DN}_k}$ used to realize both Dirichlet and Neumann conditions, cf. \Eq{eq:Discrete_Opt_BC} \trung{add new figure here}.}
%        \label{fig:QNPU_BC_Dirichlet-2}
%    \end{subfigure}  
%    \caption{Illustration of the modified boundary QNPU for $j_{{DN}_k}$ in an exemplary $n=4$ qubits setup.}
%    \label{fig:QNPU_BC-2}
%\end{figure}
%\medskip


%%% CONTINUE AFTER CALL ... 
In practical applications, e.g. an implementation on NISQ hardware, there is a demand for circuit efficiency. 
%To ensure small de-coherence times, the gate complexity is usually considered critical and shallow circuits are sought. 
%\sbengoechea{An efficient implementation on NISQ hardware demands short decoherence times and low gate complexity.}
To this end, additional carry qubits can be used to achieve the critical and shallow circuits sought. Thereby, intermediate information associated with \textsc{AND}-operations realized by a staggered series of Toffoli gates. The technique is illustrated for the application of a multi-controlled-G Gate (MCG) in \Fig{fig:multicontrol}.
\pover{Write that some hardware is capable of MCG as a native compilation - so it only depends on the hardware to judge the gate complexity  - add a reference \cite{} }
The example consists of $n=6$ qubits and requires $n-1=5$ carry qubits to transform the deep multi-controlled gate on the left of \Fig{fig:multicontrol} into $2n-2$ Toffoli- and one controlled G-gate on the right of \Fig{fig:multicontrol}. 
Mind that after applying G, all carry bits need to be reversed to their initial state, i.e. $\ket{0}$. 
%\pover{Nielsen schows similar approach onpage 183 pdf  \cite{Nielsen2010}}

\begin{figure}[htbp]
    \centering
    \input{Figures/MultiControl}
    \caption{Alternative networks using a  qubit-saving implementation (left) and a shallow circuit depth approach  (right) of a multi-controlled Gate \textsc{G}.}
    \label{fig:multicontrol}
\end{figure}

Applying the same idea to the transformation circuit $T_t$ outlined in \Fig{fig:Transformation} allows to derive the shallower alternative $\Tilde{T}_t$,
%This is illustrated inside the dashed frame in 
cf. \Fig{fig:new-Tt:up}. The illustration features an adder operator which is identical in functionality to the network given in \Fig{fig:Transformation}.
The \Fig{fig:new-Tt:up} also provides the corresponding circuit for the inverted transformation  $\Tilde{T}_{t_\text{inverse}}$  in \Fig{fig:new-Tt:down}. The latter is required for measuring the expectation value $\sigma_z =  \bra{0} U^\dagger T_t^\dagger \; [\text{QNPU}] \; T_t U \ket{0}$ as illustrated by the Hadamard-test based  structure in \Fig{fig:VQA_QNPU}. 
%of $T_t$ by $T_t^\dagger$, 
The inversion of the activity of 
%of ${T}_t$ is 
%due to 
the additional carry qubits follows from an adjoint approach, cf. \Fig{fig:new-Tt}.  
%with the forward and backward transformations given explicitly and  
 Both 
 %\trung{bitte kurz bestaetigen} 
 $\tilde T_t$ and $\tilde T_{t_\text{inv}}$ 
 are controlled by an ancilla qubit,  which follows the same strategy as depicted for the QNPU assembly in \Fig{fig:VQA_QNPU}. 

\begin{figure}
\begin{subfigure}[t]{0.4\textwidth}
      \include{Figures/ShiftUP}
      \caption{Forward Transformation  $\tilde T_t$.}
      \label{fig:new-Tt:up}
\end{subfigure}
\hspace{3cm}
\begin{subfigure}[t]{0.4\textwidth}
      \include{Figures/ShiftDOWN}
      \caption{Backward (adjoint) Transformation $\tilde T_{t_\text{inverse}}$.}
      \label{fig:new-Tt:down}
\end{subfigure}
\caption{Alternative implementations of the forward ($T_t$, $\tilde T_t$) and backward ($T_{t}^\dagger$, $\tilde T_{t_\text{inverse}}$) transformation introduced in \Fig{fig:Transformation}.}
\label{fig:new-Tt}
\end{figure}

%Comparing the network in \Fig{fig:new-Tt:down} with the Laplacian circuit in \Fig{fig:Laplace_compiled}, the similarity between the circuits becomes clear. 
%
%The Laplacian expression is hereby of course only obtained due to the measurement \pover{double check}. 
%above at the end of 
 
As already outlined at the end of Sec. \ref{sec:Discretization}, the QNPU related to the Neumann condition ($j_{N_{1,N_\text{p}}}$) shown in \Fig{fig:QNPU_BC_Neumann} can be casted in terms of the potential $p$ QNPU, depicted in \Fig{fig:QNPU_Potential}. Interestingly, in this case, no substantial change is observed for the scaling of the modified potential circuit ($j_{\tilde P_k}$) as compared to the scaling of $j_{P_k}$ displayed in \Fig{fig:Results:QNPUcomplex}, and remaining issues reduce to the gate complexity of the QNPU for $j_{DN_{1,N_\text{p}}}$. 

Introducing the above-mentioned shallow circuit alternatives to the $j_{DN_{1,N_\text{p}}}$ circuit is straightforward 
%to apply the technique illustrated in \Fig{fig:multicontrol} to the most concerning Dirichlet Neumann  \pover{align name } correction.
and allows replacing the multi-controlled-Z gate by the usage of $n-1$ carry qubits.
%
%This enhancement relates to the same scaling of the Neumann contributions as for the implementation of the polynomial.
%
Finally, a consistent application of shallow circuit (MCG) strategies yields the complexity graph
outlined in \Fig{fig:New-complexity}. Advantageous differences to \Fig{fig:compilation:GateComplexity} are clearly visible, but 
 do of course come at
 the expense 
%. The improved QNPUs are indicated by a $\tilde{(\hdots)}$. Mind that these results come at the expense 
of additional $(n-2)$ carry qubits. The graph exploits a highly efficient scaling superior to $\mathcal{O}(n^2)$. In terms of grid- point $N_\text{p}$ the behavior is of \textit{polylog} complexity. Questions for further improvement are necessary to be asked in the scope of the to-be-used hardware. On this account, further elaboration on the scalability is out of the scope of this publication. 
%, meaning that the number of carry qubits is Pareto optimal to the shallowness of the circuit. 
%the exploit improvements reduces the gate complexity as given in \Fig{fig:New-complexity}. As overhead additional $n-1$ carry qubits remain, which remarks again the Pareto optimal decision to meet by the user.
\begin{figure}[htbp]
    \centering
    \input{Figures/Complexity/C_QNPU_new}
    \caption{Improved gate complexity for all \textsc{QNPU}s.}
    \label{fig:New-complexity}
\end{figure}

 %The strong similarities of the QNPUs  shown in  \Fig{fig:QNPU_BC_Dirichlet} and \Fig{fig:QNPU_BC_Neumann} could provide a way to improve the scaling of $j_{ND_k}$.To reduce the complexity of the $j_{ND_k}$ QNPU we suggest to replace the circuit in \Fig{fig:QNPU_BC_Dirichlet} by the circuit sketched in \Fig{fig:QNPU_BC_Dirichlet-2}

%###########################################
%       Derivative Computation
\section{Optimization Strategy} \label{sec:Optimization}

\pover{Emphasise that Opt strategy is not the main outline of the paper -  it is about the BC}
%\subsection{Optimization Strategy} \label{sec:Optimization}
%\pover{ May take riemian topology on quantum comp into account} %\cite{Wiersema2023}
% do classical example! 
%https://www.researchgate.net/publication/3320516_Steepest_Descent_Algorithms_for_Optimization_Under_Unitary_Matrix_Constraint
%https://arxiv.org/pdf/2112.02572.pdf
% EVIDENCE Given in https://journals.aps.org/pra/abstract/10.1103/PhysRevA.107.062421
The common denominator in \textsc{VQA}s is the implementation of an efficient optimization procedure. As indicated in \cite{Bittel2021}, this is a non-trivial aspect because the problem covered by the VQA is theoretically \textsc{NP}-hard, meaning that optimization is characterized as non-convex.  Problems with multiple local minima
 %The practice unveils the optimization of non-convex functionals, determined by e.g. multiple local stationary points, as faced in
\cite{Sarma2023,Leong2022,Wiersema2023}
and
%Additionally, the effect of \textit{Barren Plateaus}, whereby the
vanishing derivatives impede the efficient update of the control parameters.
%, can occur when using non-shallow quantum circuits \pover{TODO:\cite{ }}. 

%a crucial point and often characterized as a non-trivial task. The publication \cite{Bittel2021} shows that the problem covered in VQA context is theoretically NP-Hard. 

%The use and practicability of zero-/first- or even second-/ order methods therefore highly differentiates with respect to convex optimization.  
%A common approach for optimization problems classified as nonconvex is the use of zero-order evolutionary schemes for initial steps \cite{  }
%, since a good estimate for a starting position is not known in the first glimpse. The main group of these schemes is also known as sampling methods \cite{} Furthermore, has the experience unveiled that, 
%In close vicinity of the stationary point, an efficient updates are realized using a first-order method. 
%Despite this fact, of course, zero-order methods, e.g. the simplex method \cite{Nocedal2006}, as it is done in \cite{Leong2022} can be applied. Wheras, second order approaches require enormous overhead in measuring to construct the Hessian, but of course better results. All in all, they are not practicable \cite{Mari2021}. First-order methods, based on second-order models as given by the Quasi-Newton type algorithms, where the second derivative is estimated by rank-1 or even rank-2 updates \cite{Nocedal2006}, instead find its application for some VQAs \cite{  }. The additional effort for the approximation of the Hessian is here not given, but the requirement for a positive definite Hessian needs to be given as well. 

%In contrast to this presented Euclidean view on the optimization manifold, there are efforts in choosing the descent direction with respect to the underlying Riemannian setting, which is mainly set due to the fact in \Eq{eq:partition_of_unity}. It is observed that, where the Euclidean approaches tend to local stationary points, the Riemannian strategies overcome these \cite{Wiersema2023}. Despite this, we restrict to the emphasized Euclidean setting, but a detailed view on the problem is crucial to achieve an efficient algorithm. 

 To update the controls ($\lambda_0, \lamb_c$) along the route outlined in \Fig{fig:optimizer}, we apply a sequence of a zero- and a first-order method. The combination aims at a wider sampling to address non-convex functionals and higher accuracy in the vicinity of the minima. 
%In this two-fold approach, the initial zero-order step can be interpreted as a starting point estimator for the subsequent first-order optimizer. 
%We implement the update strategy in each iteration $i$ as $\upb_{i+1} = \upb_{i} + \Delta \upb_{i+1}$. 
 The optimization begins with a zero-order step, that employs an evolutionary  \textit{Particle-Swarm Optimization} (\textsc{PSO}) algorithm \cite{Kennedy1995} using $\mathfrak{p}$  particles.
%Taking into account the functional itself, given in \Eq{eq:Discrete_Opt_BC}, it is clear that it is quadratic in $\lambda_0$. In case of the ansatz parameter $\lamb_\text{c}$, it is not so straightforward. 
%\begin{align}
%\Delta \upb_{i+1} =& \underbrace{\omega \Delta \upb_i}_\text{Momentum} + \underbrace{c_1 r_{1_i} %\left(\upb_{\text{best},i}-\upb_i\right)}_\text{Learning}+ \underbrace{c_2 r_{2_i} %\left(\upb_{\text{best},i_\text{swarm}}-\upb_i\right)}_\text{Communication}. 
%\label{eq:PSO}
%\end{align}
The \textsc{PSO} step typically involves O(1000) iterations. The best candidate initializes the control $\upb$ for the subsequent first-order classical \textit{Gradient Descent} (\textsc{GD}) method. The required computation of the objective functional w.r.t. the controls  
%The update is given by a $\alpha$ factored step  
%\begin{align}
%    \Delta \upb_{i+1} = - \alpha \nabla_{\upb} J(\upb_{i}), 
%    \label{eq:GD}
%\end{align}
%being
$\nabla_{\upb} J(\upb_{i})$ is obtained from the QC and follows the expressions given below, cf. \Eq{eq:quantum_derivative_0} and \Eq{eq:quantum_derivative_control}. Convergence is assessed from the absolute change \textsf{ch} of the derivative
\begin{align}
   \textsf{ch}( \nabla J^l_i) = | \nabla J^l_i- \nabla J^l_{i-1}|_{2} % |J^l_i - J^l_{i-1}|_{2} 
   \quad \le 10^{-n} \, , 
   \label{alg:convergence}
\end{align}
 where $n\in[3,6]$ depending on the number of employed qubits, cf. Sec. \ref{sec:Applications}.  
The solution is advanced in time as described in \Fig{fig:discretization_encoding} and the algorithm \ref{alg:VQA}. For time steps $l>1$, the optimal parameters of the previous step $\upb^{l-1}$ serve as an initial guess for the PSO to reduce the efforts, as proposed by \cite{Sato2021,Leong2022}.

%% Alternating direction methods   -  suitable given concept :  
%% Clean up implemented algorithm 
%% Is a spliting of lambda 0 and lambda c convient? 

%% Alternating projection method  - Douglas–Rachfordalternating 

\begin{algorithm}[htbp]
\caption{VQ Algorithm}
\label{alg:VQA}
    \begin{algorithmic}
    \Require $\text{N}_t, \texttt{tol}_\text{P}, \texttt{tol}_\text{G}, f_\text{Ghost}, f, \upb_{0} $
    \State $l$ \gets $1$
    \While{$l \leq \text{N}_t$}  \Comment{Time Evolution}
        \If{$l=1$}
            % initial values
            \State $\Tilde{f}^1$ \gets $\frac{y(x,0,\upb_{0}) }{\Delta t}+ \Tilde{f}^1$ \Comment{Initial setup of the external contribution}
            \State $\upb^1$ \gets $\left(\lambda_0^1,\lamb_c^1\right)^\intercal$  \Comment{Random initialization of $\lambda_0^1\in [0,1]$ and $\lamb_c^1 \in [0,4\pi)$ for all $\mathfrak{p}$ particles}
        \Else
            % next values
            \State $\Tilde{f}^l$ \gets $\frac{y(x, t^l, \upb_{l-1}) }{\Delta t}+ \Tilde{f}^l$ \Comment{Adjust the contributions}
            \State $\upb^l$ \gets $\upb^{l-1}$  \Comment{Propagate previous final control $\upb^{l-1}$}
        \EndIf
        %% PSO
        \State $\upb^{l}$ \gets PSO$(\upb^l)$  \Comment{Iterate until $\texttt{maxit}_{P}$ or $\texttt{tol}_{P}>\textsf{ch}(\nabla J_i^l)$ (c.f. \Fig{fig:optimizer})} \label{alg:VQA:PSO}
        %% GD BASED
        \State $\upb^{l}$ \gets GD$(\upb^{l})$  \Comment{Iterate until $\texttt{maxit}_{G}$ or $\texttt{tol}_{G}>\textsf{ch}(\nabla J_i^l)$ (c.f. \Fig{fig:optimizer})}\label{alg:VQA:GRAD}
        \State $l$ \gets $l+1$
    \EndWhile
    \end{algorithmic}
\end{algorithm}

%Due to the different magnitudes in the derivatives \Eq{eq:quantum_derivative_0} and \Eq{eq:quantum_derivative_control}, the convergence can be accelerated by alternating sequentially the optimization of $\lambda_0$ and $\lambda_c$. With this relaxation, $\lambda_0$ is kept constant in the first step and then whole control is updated. Convergence is determined by a tolerance \texttt{tol} at $ \| \nabla J(\lamb_{i}) \|_2 \leq \texttt{tol}$. The algorithm is given in alg. \ref{alg:VQA}. 

%% Alternating direction methods   -  suitable given concept :  
%% Is a spliting of lambda 0 and lambda c convient? 
%This two-step approach is relaxed by introducing an inner optimization loop, where in the first step $\lambda_0$ is kept constant and in a second step the whole control is updated. 

%With this two-step approach, it is accomplished to cover extensively the unknown solution space. 
%The difficulty of selecting  appropriate initial values for fine-tuning and the nonlinear mapping to the Ansatz parameterization $\lamb_c$ is handled. \sbengoechea{It is accomplished to cover extensively the unknown solution space, to select an appropriate start location for fine-tuning when dealing with nonlinear mappings of the Ansatz parameterization $\lamb_c$.}  
The whole framework is implemented by an in-house 
%\textsc{MPI}-parallel \textsc{PDE} 
toolbox, with \textsc{Qiskit} v.0.42.1 \cite{Qiskit} as a backend. 
\pover{The code is available via .....(codeocean / Gitlab tuhh ? )}
%Inheritance and polymorphism allowed to establish an identical structure to this publication.
%\end{document} 

\subsection{Derivative Computation} \label{sec:Derivative1}
The determination of the gradient to identify the direction of descent can be supported by the QC. To this end, the quantum circuits derived in Sec. \ref{sec:Strategy} are re-used, as outlined below. 
The gradient of the objective functional w.r.t. the scalar 
parameter $\lambda_0$ follows from \Eq{eq:Discrete_Opt_BC} and simply reads
%\Eq{eq:first_order_opt} \trung{man sollte nochmal prüfen, ob man den Kram in Glg 10 etc wirklich benötigt, und nicht direkt auf Glg. 22 verweist} is given by 
\begin{align}
\begin{split}
\nabla_{\lambda_0} J(\lambda_0, \lamb_c) =
   &\sum\limits_{k=1}^{N_\text{p}} \underbrace{ -\left(\frac{2\nu \lambda_{0}}{\Delta x^2}\right) u_k(\lamb_{c}) \bigg(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})+u_{k-1}(\lamb_{c})\bigg) }_{\nabla_{\lambda_0}j_{L_k} } 
   \Delta x \, \\
   & 
    \underbrace{+\left(\frac{2\nu \lambda_{0}}{\Delta x^2}\right) \bigg( u_1(\lamb_{c})u_{N_\text{p}}(\lamb_{c}) + u_1(\lamb_{c}) u_{N_\text{p}}(\lamb_{c})  \bigg)}_{\nabla_{\lambda_0} (j_{DN_1} + j_{ DN_{N_\text{p}}}) } \Delta x \,
     \underbrace{-\left(\frac{2\nu \lambda_{0}}{\Delta x^2}\right) \bigg(  u_1(\lamb_{c})^2 + u_{N_\text{p}}(\lamb_{c}) ^2 \bigg)}_{\nabla_{\lambda_0}(j_{N_1} +j_{N_{N_\text{p}}}) } \Delta x \, \\
   + &\sum\limits_{k=1}^{N_\text{p}} \, \underbrace{ - 2\zeta \lambda_{0} u_k(\lamb_{c}) p_k u_k(\lamb_{c})  }_{\nabla_{\lambda_0} j_{P_k} }  \, \Delta x + \sum\limits_{k=1}^{N_\text{p}} \underbrace{ - 2 u_k(\lamb_{c}) \Tilde{f}_k } _{\nabla_{\lambda_0} j_{S_k}  } \, \Delta x \, . 
   \label{eq:deriv0-a}
\end{split}
\end{align}
Here too, the temporal index has been omitted for better clarity. Comparing  \Eq{eq:deriv0-a} with \Eq{eq:Discrete_Opt_BC}  reveals an equation to be evaluated
 on the QC 
\begin{equation}
\label{eq:quantum_derivative_0}
\nabla_{\lambda_0} J
%(\lambda_0, \lamb_c) 
= \frac{1}{\lambda_0} \bigg[  \sum\limits_{k=1}^{N_\text{p}} 
 \big( 2  j_{L_k}
%(\lambda_0, \lamb_c) 
+ 2 j_{P_k} 
%(\lambda_0, \lamb_c) 
+ j_{S_k} \big)  \; \Delta x \bigg]  
%(\lambda_0, \lamb_c) 
+ \frac{2}{\lambda_0} 
\left[ \bigg(
  j_{DN_1} + j_{DN_{N_\text{p}}}
%(\lambda_0, \lamb_c) 
+ j_{N_1} + j_{N_\text{p}}
%(\lambda_0, \lamb_c) 
 \bigg)
 \, \Delta x \right] \, . 
\end{equation}

Computing the (time-dependent) derivative of $J$ w.r.t. $\lamb_c$ 
%in \Eq{eq:first_order_opt}  
can also be performed on the QC without deriving a new gate sequence. 
Of the methods proposed in the literature, e.g. using \textit{finite differences}, the \textit{parameter shift rule} \cite{Schuld2019,Banchi2021,Crooks2019}, or the \textit{natural gradient} \cite{Stokes2020}, the two former approaches are used in this study. 
Formally, the derivative of the objective function w.r.t the control vector $\lamb_c$ follows from Eqn. (31)
%Using $u_k' = \nabla_{\lamb_c} u_k$, the first-order derivation of the objective function w.r.t the parameter vector $\lamb_c$ follows from \Eq{eq:derivc-a}. However, the equation is not used as such, except for the linear part contained herein related to $j_{S_k}$.
%
%\begin{align} \begin{split}
%\nabla_{\lamb_c} J_k (\lambda_0, \lamb_c) 
%   =
%   &\sum\limits_{k=1}^{N_\text{p}}\underbrace{ - \left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) \left[\Big(u_{k+1}(\lamb_{c})-4u_k(\lamb_{c})+u_{k-1}(\lamb_{c})\Big) u_k'(\lamb_{c})+ u_k(\lamb_{c}) \Big(u_{k-1}'(\lamb_{c}) + u_{k+1}'(\lamb_{c}) \Big) \right]}_{\nabla_{\lamb_c} j_{L_k}  } \Delta x \\
%   &  \underbrace{+2\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) \left(u_1'(\lamb_{c}) \, u_{N_\text{p}}(\lamb_{c}) +  u_{N_\text{p}}' (\lamb_{c})  \, u_1(\lamb_{c}) \right)}_{\nabla_{\lamb_c} (j_{DN_1} +j_{DN_k})  } \Delta x \\
%   &  \underbrace{-2\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) \left( u_1(\lamb_{c}) \, u_1'(\lamb_{c}) + u_{N_\text{p}}(\lamb_{c}) \, u_{N_\text{p}}'(\lamb_{c}) \right)}_{\nabla_{\lamb_c}(j_{N_1} +j_{N_{N_\text{p}}})   }  \,\Delta x \\
%   +&\sum\limits_{k=1}^{N_\text{p}} \, \underbrace{ -2 \zeta \lambda_{0}^2 u_k(\lamb_{c}) p_k   u_k'(\lamb_{c})  }_{\nabla_{\lamb_c}j_{P_k}   }  \, \Delta x + \sum\limits_{k=1}^{N_\text{p}} \underbrace{ -2\lambda_{0}    u_k'(\lamb_{c})  \Tilde{f}_k } _{\nabla_{\lamb_c}j_{S_k}   } \, \Delta x \, .
%   \label{eq:derivc-a}
% \end{split} \end{align}%
\begin{align}
\begin{split}
\nabla_{\lamb_c} J (\lambda_0, \lamb_c) 
   =
   &\sum\limits_{k=1}^{N_\text{p}} \nabla_{\lamb_c} \big( 
j_{L_k} + j_{P_k} + j_{S_k} \big) \Delta x 
   +
   \big( \nabla_{\lamb_c} (j_{DN_1} +j_{DN_{N_\text{p}}}) 
   +
   \nabla_{\lamb_c}(j_{N_1} +j_{N_{N_\text{p}}}) \big)   \,\Delta x  \, .
   \label{eq:derivc-a}
\end{split}
\end{align}


The linear source term $\nabla_{\lamb_c} j_{S_k}$ is approximated with second-order accurate central differences that operate on the complete (linear) objective function contribution, viz.
\begin{equation}
    \nabla_{\lamb_c}j_{S_k}   = -2\lambda_{0} 
%    u_k'(\lamb_{c})  
 \big( \nabla_{\lamb_c} u_k \big)    
\Tilde{f}_k \approx 
  %\sum_{a=1}^c 
  \frac{j_{S_k}(\lambda_0, \lamb_c+h\eb_c)-j_{S_k}(\lambda_0, \lamb_c-h\eb_c)}{2h} %\eb_a 
   + \mathcal{O}(h^2) \, .
   \label{eq:opt-source-FD}
\end{equation}
Mind that \Eq{eq:opt-source-FD} has to be executed for all entries of the
parameter vector $\lamb_c$, and the step size is typically assigned to a constant value of $h\in[10^{-3},10^{-6}]$, depending on the number of employed qubits.
%
For the quadratic terms $j_L, j_P, j_{DN}, j_N$ an exact representation of the derivative is given by the \textit{Parameter Shift Rule}, cf.  \cite{Schuld2019,Banchi2021,Crooks2019}.  The derivative follows using only two additional evaluations of already existing quantum circuits and the nonlinearity is implicitly considered. 
%The parameter of interest, uniquely parameterizing a one qubit gate, is varied by $s = \pm \frac{\pi}{4 r}$, with $ r= \frac{1}{2}$ formulated by \cite{Mitarai2018,Crooks2019}. The perturbed measured expectation values are used for the computation of the relative change, which aligns with the analytical derivative if $s$ is chosen correctly. 
%The product rule concerning the quadratic term is taken care of by this approach inherently.
%According to \cite{Schuld2019,Banchi2021,Crooks2019}, the derivative with the quadratic terms can be evaluated by using the so-called phase shift rule.
%It is based on the assumption that the ansatz $u$ is linear in  control $\lamb_c$ and consists of elementary rotational single parameter gates  \cite{Schuld2019,Crooks2019}. Then, the gate sequences can be reused and no compilation of the derivative needs to be derived.
%Although alternatives to this approach exist, the implementation of the phase shift rule is straightforward, and allows parallelization with respect to the number of parameters. 
%
%The terms, which appear with a linear setting of the trail function, do not follow this straightforward idea. Here the derivative is calculated using a second-order accurate finite difference approach.
%viz %parameterization $g(x)$, given by the central difference scheme using a small perturbation $h$ is
%\begin{align}
%\nabla g(x) =  \frac{g(x+h) - g(x-h)}{2h} + \mathcal{O}(h^2).
%\end{align}
%This numerical derivative is of course an approximation, but only implies another two evaluations and does not require a new gate sequence, as well. 
%Multiple appearances, e.g. cubic or fourth order, of one parameter, need to be treated according to the chain rule  \cite{Mari2021, Schuld2019}. 
Applying these techniques yields an expression for the derivative of the objective functional $J$ 
with respect to the control vector $\lamb_c$ that utilizes the existing circuits, viz.  
\begin{align}
\begin{split}
\nabla_{\lamb_c} J(\lambda_0, \lamb_c) =&  \sum\limits_{k=1}^{N_\text{p}} \frac{1}{2} \bigg(j_{L_k}\big(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c\big) - j_{L_k}\big(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c\big) \bigg) \Delta x\\
&+ \frac{1}{2} \bigg(j_{DN}(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c)- j_{DN}(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c) \bigg) \Delta x \\
&+  \frac{1}{2} \bigg(j_{N}(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c)-j_{N}(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c) \bigg) \Delta x\\
+&\sum\limits_{k=1}^{N_\text{p}} \bigg(\frac{1}{2} \Big( j_{P_k}\big(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c\big)-j_{P_k}\big(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c\big) \Big)  + \nabla_{\lamb_c}j_{S_k} \bigg)\, \Delta x \, .
\end{split}
\label{eq:quantum_derivative_control}
\end{align}


==> Container/C_Feb10_Sections/RED-Conclusion.tex <==
%###########################################
%       Conclusion
%###########################################
\section{Conclusion} \label{sec:Conclusion}

% GENERal Quotes on the framework
   %\item It is shown that the \textsc{VQA} works in principle.  
   %The hybrid optimization approaches delivered satisfactory results to linear \textsc{PDE}s. 
%    \item Quantum4PDE Problems can be cast into optimal control problems.
%   \item We can solve  PDEs with arbitrary boundary conditions implemented in a QNPU structure. Boundary conditions are cast as QNPU elements.
%   \item We have a constant number of contributions to the costfunction if increasing qubits
% \item barenplateaus -  vanishing gradient caused by random initialization and 
%
%    \cite{Wiersema2023}
%    "
%    However, there is evidence
%    that deep quantum circuits can have favorable
%    optimization properties [55, 50, 56]. Perhaps the
%    global convergence guarantees of double bracket
%    flows flows can be used to understand the con-
%    vergence properties of deep quantum circuits and
%    provide deeper insight into the power of VQE op-
%    timization"
%
%


\pover{Include the idea for a convergence criteria based on solutions magnitude}
This study proposes a generic boundary condition extension to solve linear \textsc{PDE}s on a \textsc{QC}, via the \textsc{VQA} presented by Lubasch et al. \cite{Lubasch2020}. To this end, initial-boundary value problems are reformulated as optimal control problems where all terms, including the boundary conditions, are casted into case-independent \textsc{QNPU} elements, assembling the corresponding quantum circuits. This maintains a constant number of contributions to the cost function independent of the number of qubits $n$.
%\trung{The hybrid classical-quantum method based on the \textsc{QNPU}-structure, successfully demonstrates the advantage of the integration feature via ancilla measurements for up to $n=4$ qubits.} 
Proof-of-principle verifications are demonstrated for steady and unsteady heat conduction problems, covering all types of boundary conditions (Dirichlet, Neumann, Mixed Dirichlet/Neumann \trung{CHECK: and Robin}). The obtained VQA-results reveal an excellent alignment with a classical \textsc{FD}-results for two consecutive  discretizations in combination with various steady and transient test cases. 

\smallskip
The novel treatment of the boundaries by the ghost point strategy relaxes the ansatz functions $u(\lamb_c)$, adding cost function contributions that complement the objective functional of the control problem (without using a penalty term). In terms of the boundary conditions, the ansatz $u(\lamb_c)$ needs only to be valid on the internal points, as they are decoupled from the boundary points. The latter are  included in the system through interior corrections and external contributions to the source term. Despite the excellent results of the proposed \textsc{VQA} in implementing the boundaries, the corresponding quantum circuits for the shift operator $T_t$, given by Sato et al. \cite{Sato2021}, scale exponentially with the number of qubits as the multi-controlled Toffoli gates indicate in \Fig{fig:Transformation}. The rising circuit depth, due to the multi-qubit interaction, not only makes the optimization inefficient but also limits the implementation on real hardware \cite{Sato2021,Cerezo2021,Sarma2023}. In the case of Neumann boundaries, an improvement in the scalability is achieved by substituting the Neumann circuit of \Fig{fig:QNPU_BC_Neumann} by a tailor-made mask implemented via the potential circuit, cf. \Fig{fig:QNPU_Potential}. 
%Note that, the exponential scaling in gate complexity does not vanish completely since the $j_{DN}$ contribution is still necessary. This alternative would reduce only the exponential scaling in the case of the $j_N$ contribution.
An alternative option is to measure the state of the single qubit encoding the boundary point, as in \cite{Sato2021}. 

\smallskip 
As for all \textsc{VQA} approaches, the choice of the ansatz is crucial since it defines the underlying functional space for the \textsc{PDE} solution but at the same time also introduces a non-convex property into the optimization. The hardware-efficient bricklayer topology of the applied ansatz shows favorable expressibility, in terms of small $l_2$-norm deviation measures, in noise-less {QC} simulations.
%
However, it also unveils unfavorable scalability in terms of a case dependent increase of the number of control parameters $\lamb_c$ and a related poorer trainability. The combination of challenging  trainability and  non-convex nature of the optimization implies serious convergence issues in tracking the global optimum for $n \ge 8$. 


%Although this idea would correct the exponential scaling, it would also require more measurements and the classical treatment of the boundaries, breaking the full quantum evaluation of the algorithm. 

%Opt more efficient for local H
%https://www.nature.com/articles/s41467-021-21728-w
%n [8], it is proved that the vanishing gradient problem can be avoided if the following conditionsare satisfied; (i) each term of the cost Hamiltonian, H = ∑
%k Hk is local, meaning that each term Hk
%is composed of less than m neighboring qubits, (ii) the ensemble of unitary matrices in each block is
%2-design, and (iii) the number of layers, `, is of the order O(poly(log n)). Note that each block needs
%to be deep enough for the distribution of corresponding unitary matrices to be close to 2-design
%Non local hamiltonians

%non local hamiltonians -  Dirichlet term 
% Non local hamiltonians 
%
%The proposed circuits reproduce that global behavior of the boundaries as indicated by the shape of the gates given in \Fig{fig:Transformation}, \Fig{fig:QNPU_BC_Dirichlet}, and \Fig{fig:QNPU_BC_Neumann} with multi-controlled Toffoli gates. 
%
%Non local hamiltonians \pover{quote on sato section C  .  Quantum circuit for the shift operator
%are already been marked as inefficient by \cite{Sato2021}, claiming the use of multi-controlled Toffoi gates as major bottleneck to create shallow circuits. As alternative may use \cite{Liu2021}  as decomposition approach , but scales less efficient. In terms of our approach only the bilinear form a(,) and the Linear operator F need to be measured. Which is an improve compared to \cite{Liu2021, Sato2021} <- Check }
%
% Non local hamiltonians
%In the case of Neumann boundaries, an improvement in the scalability can be achieved by substituting the Neumann circuit of \Fig{fig:QNPU_BC_Neumann} by a mask implemented via the Potential circuit. For this the potential circuit does no need a state preparation since the task can be split in two with the initialization of $\ket{00...00}$ and $\ket{00...01}$ for the left and right boundary respectively. Note that, the exponential scaling does not vanish completely since the Dirichlet circuit it is still necessary to remove the corners of the antidiagonal, also for the Neumann conditions. This alternative would reduce only the exponential scaling of one of the circuits.  
%Another option is to measure state of the single qubit encoding the boundary point, as Sato does, or in our case the point next to the ghost point. With that information on that point, a mask can be applied to achieve the desired value at the boundary. Although this idea would correct the exponential scaling, it would also require more measurements and classic treatment on the boundaries, breaking the full quantum evaluation of the algorithm. 

%Hardware and ansatz things 
%\pover{Use a real quantum annealer for implementation, due to this you could come around the minimization classically since it converges to the thermodynamic ground state, which coincidences with the optimum of an energy functional. Summarizing you will optimize using a quantum optimizer}

%\pover{Exclude measurement topic}
%Investigations in terms of sampling measurements as well as robustness to shot noise have not been investigated in this publication. We refer the reader to \cite{Lubasch2020} where it is reported that the order of measurements $M$ on the ancilla for the potential is independent of $n$ while for the Laplacian \textsc{QNPU} $M$ increases exponentially with $n$. 

Future research will be devoted to encode first derivatives as a \textsc{QNPU} operator in combination with the non-linearity treatment proposed by \cite{Lubasch2020} 
%will be explored for the representation of 
 to represent convective fluxes.
%in \textsc{CFD} applications such as given by the Burgers equation (Couette flow, Poiseuille Flow, Smith Hutton Case....). 
In view of extending the present algorithm to 2D and 3D spatial problems, the non-convex optimization problem will be addressed by selecting more appropriate (trainable, expressible, shallow) dynamic ansatz strategies. For time evolution, the use of 
%adaptive time stepping schemes as well as 
adaptive ansatz depths seems viable to safe computational cost.
%suitable to efficiently rely on computational resources. 
Furthermore, circuit scalability improvements for the transformation $T_t$ as well as $j_{DN}$ circuits will be addressed to increase the range of applications towards industrial \textsc{NISQ} \textsc{QCFD}. 

%\sbengoechea{\cite{Lubasch2020} provides the possibility of implementing non-linear terms,

%\textbf{OUTLOOK}  2- max 5. senteces
%\begin{itemize}
%\item Develop a first-order derivative (convection) as a QNPU Operator, to solve Burgers equation (Couette flow, Poiseuille Flow, Smith Hutton Case....) . 
%\sbengoechea{\cite{Lubasch2020} provides the possibility of implementing non-linear terms, a scenario that will be explored in future works.}
%
% \item Extend the present to higher dimensions
 
%\item Tightly relax the non-convex opt problem using quadratic programming tech  -  or simply opt :  
% May take riemian topology on quantum comp into account \cite{Wiersema2023}
% do classical example! 
%https://www.researchgate.net/publication/3320516_Steepest_Descent_Algorithms_for_Optimization_Under_Unitary_Matrix_Constraint
%https://arxiv.org/pdf/2112.02572.pdf
% EVIDENCE Given in https://journals.aps.org/pra/abstract/10.1103/PhysRevA.107.062421

%\item \sbengoechea{Ideas on how to improve circuit scalability  - transformation $T_t$ as well as $j_{DN}$}
%\end{itemize}


\pover{Ellaborate on elliptic requirements and Least squares as way out}



==> Container/C_Feb10_Sections/RED-Discretization.tex <==
\section{Discrete Objective Functional and  Boundary Treatment}  \label{sec:Discretization}
\pover{DO we intend to imply the Robin contributions from the internal appendix \ref{sec:internalRobin} for the sake of completeness in this section?}
The objective functional \Eq{eq:Reduced_Opt}  consists of contributions from the Laplace operator $j_L$, the potential $j_P$ and the source term $j_S$. 
%
The integration over the interior domain 
in \Eq{eq:Reduced_Opt} 
is fractioned into sub-integrals around the centrally spaced interior nodes, which are 
 approximated by a 
 second-order accurate midpoint rule, i.e.
\begin{equation}
     J^{l} = \int_\Omega (j_L+ j_P+j_S)^l \,  dx = {\sum_{k=1}^{N_\text{p}}} (j_{L_k} + j_{P_k}+ j_{S_k})^l \, \Delta x \, .
     \label{eq:Reduced_Opt-Disc}
\end{equation} 
Subsequently, the discretized boundary conditions are introduced. These are formulated as corrections to established periodic boundary conditions, which yield augmentations of the discrete objective functional (\ref{eq:Reduced_Opt-Disc}). The approach is compatible for an evaluation on QC hardware and is discussed below using the left boundary ($k=0$) as an example.
 The procedure for the right boundary is analogous and is therefore not discussed in detail. The time index is again deliberately suppressed for the sake of clarity.

The potential and source term contributions $j_{P_k}$, $j_{S_k}$ to \Eq{eq:Reduced_Opt-Disc} are strictly local and therefore do not interact with the ghost point (boundary) values.  
 The contribution of the discrete Laplace operator, however, is non-local (but homogeneous) and interacts with the boundary.
 %\pover{But the Periodic one is local ? \trung{Verstehe ich nicht - diskutieren}}. 
 At the first interior point ($k=1$) the contribution 
%and time $t_l$ 
  reads
\begin{equation}
j_{L_1} =-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x} \right) \; u_1 \bigg( u_0 - 2u_1 +u_2\bigg) \, , 
 \label{eq:Laplace-left}
\end{equation}
where $u_0$ is an unknown that must be closed by the boundary condition. 
%As already mentioned, the strategy follows the work of [\trung{SATO?}]
 As already mentioned, the strategy refers to corrections of periodic boundaries, for which the left ghost point receives the value from the right interior point and the right ghost point gets the value from the left interior point, i.e. $u_0 =  u_{N_\text{p}}$ and  $u_{N_\text{p}+1} =  u_{1}$. 
 The periodic contribution of the left boundary to $J$ reads  
\begin{equation}
    j_{L_1}^P   =-\left(
 \frac{\nu  \, \lambda_{0}^2}{\Delta x^2 }
  \right) \; u_1 \bigg( u_{N_\text{p}} - 2u_1 +u_2\bigg) \, .
  \label{eq:periodic-left}
\end{equation}
On the other hand, a Dirichlet condition $u_0=D$ yields  
\begin{equation}
    j_{L_1}^D  =-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1 \bigg( D - 2u_1 +u_2\bigg) 
%     = 
%     -\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1 \bigg(  - 2u_1 +u_2\bigg)  \underbrace{-u_1  \left(\frac{D \nu  \, \lambda_{0}^2}{\Delta x^2}\right)}_{\text{source term}}
     \, .
     \label{eq:dirichlet-left}
\end{equation}
 Aiming to reconstruct the Dirichlet condition \eqref{eq:dirichlet-left} from the  periodic approach \eqref{eq:periodic-left}, one arrives at 
\begin{equation}
   j_{L_1}^D 
%  = j_{L_1}^P
%  +\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1  u_{N_\text{p}}
%  - \underbrace{u_1  \left( \frac{D \nu  \, \lambda_{0}^2}{\Delta x^2}\right)}_{\text{Source \, Term}}
= j_{L_1}^P
  + u_1 \, \left(\frac{\nu \lambda_0^2}{\Delta x^2} \right) \left( 
   u_{N_\text{p}} - D
  \right)  = j_{L_1}^P \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_1$-contrib.} \, j_{DN_1}} \;   \underbrace{-u_1 D \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{source-term modif.} \, f_1}  \, .
   \label{eq:defcoD-left}
\end{equation}
In the case of Neumann conditions, the prescribed gradient $N= \partial u/\partial x|_0$ first needs to be approximated. The exemplary use of simple first-order finite differences 
%\begin{equation}
 $N \approx (u_1-u_0)/(\Delta x)$ to substitute $u_0 = u_1 - N \Delta x $  
 in \Eq{eq:Laplace-left} 
%\end{equation}
  yields 
\begin{equation}
  j_{L_1}^N   =-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1 \bigg( (u_1 -N \Delta x) - 2u_1 +u_2\bigg) = 
  j_{L_1}^P
   \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_1$-contrib.} \, j_{DN_1}} \; 
     \; \underbrace{- u_1 u_{1} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_1$-contrib.} \, j_{N_1}} \; 
  \underbrace{+ u_1 \, N \left( \frac{\nu \lambda_0^2}{\Delta x} \right)}_{\text{source-term modif.} f_1}
 % =
 % -\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1 \bigg(  - u_1 +u_2\bigg)
 %  \underbrace{+\frac{u_1  \left(N \nu  \, \lambda_{0}^2\right)}{\Delta x}}_{\text{source term}}
  \, .
  \label{eq:defcoN-left}
\end{equation}
 Note that the contribution $j_{DN_1}$ which neutralizes the periodic term occurs for both conditions. 
%The deferred correction of the Neumann condition from a baseline periodic condition %reads
% \begin{equation}
%   j_{L_1}^N
%= j_{L_1}^P
%  + u_1 \, \left( \frac{\nu \lambda_0^2}{\Delta x^2} \right) \left( 
%     N \Delta x - (u_1 -u_{N_\text{p}})
%  \right)  \, .
%\end{equation}
 The technique can also be combined with higher-order, interior-oriented finite differences to approximate the derivative in Neumann or \pover{Check: Robin conditions}. 
 %
 At the right boundary, the corresponding correction terms read
 \begin{equation}
   j_{L_{N_\text{p}}}^D 
= j_{L_{N_\text{p}}}^P
  + u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2} \right) \left( 
   u_{1} - D
  \right) 
  = j_{L_{N_\text{p}}}^P 
   \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_{N_\text{p}}$-contrib.} \, j_{DN_{N_\text{p}}}} \;   \underbrace{-u_{N_\text{p}} D \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{source-term modif.} \, f_{N_\text{p}}}  \, .
   \label{eq:defcoD-right}
\end{equation}
 and 
 \begin{equation}
  j_{L_{N_\text{p}}}^N  
  %=-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_{N_\text{p}} \bigg( u_{N_\text{p}-1} - 2u_{N_\text{p}} + (u_{N_\text{p}} -N \Delta x) \bigg) = 
 = j_{L_{N_\text{p}}}^P
   \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_{N_\text{p}}$-contrib.} \, j_{DN_{N_\text{p}}}} \; 
     \; \underbrace{- u_{N_\text{p}} u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_{N_\text{p}}$-contrib.} \, j_{N_{N_\text{p}}}} \; 
  \underbrace{- u_{N_\text{p}} \, N \left( \frac{\nu \lambda_0^2}{\Delta x} \right)}_{\text{source-term modif.} f_{N_\text{p}}}
  \, .
  \label{eq:defcoN-right}
\end{equation}
% \begin{equation}
%     j_{L_{N_\text{p}}}^N = j_{L_{N_\text{p}}}^P
%  + u_{N_\text{p}} \, \left( \frac{\nu \lambda_0^2}{\Delta x^2} \right) \left(    (u_1 -u_{N_\text{p}})- N \Delta x    \right)  \, .
% \end{equation}
 Again, the contribution $j_{DN_{N_\text{p}}}$ which neutralizes the periodic entries, occurs for both Neumann and Dirichlet conditions, but is also identical for both boundary locations ($j_{DN_{N_\text{p}}}=j_{DN_{1}}$).
 The actual deferred correction implementation is given in \Eq{eq:Discrete_Opt_BC}.  %\pover{MIXED BC -  ad the case of mixed BC as well ? } 
 It employs  three terms, (a) the periodic baseline term, (b) corrections based upon combinations of interior point unknowns ($j_{DN_k}$, $j_{N_k}$) and (c) modifications 
 of the source terms $j_{S_k}$ arising from known boundary condition values ($D$, $N$), viz. 
\begin{align}
\begin{split}
   J(\lambda_0, \lamb_c) =
   &\sum\limits_{k=1}^{N_\text{p}} \underbrace{ -\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) u_k(\lamb_{c}) \big(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})+u_{k-1}(\lamb_{c})\big) }_{j_{L_k}: \; \text{periodic \& interior term}} \Delta x \, \\
    & 
   %\sum\limits_{k=1,N_\text{p}} 
   \underbrace{+\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) \bigg( u_1(\lamb_{c})u_{N_\text{p}}(\lamb_{c}) + u_{1}(\lamb_{c}) u_{N_\text{p}}(\lamb_{c}) \bigg)}_{ j_{DN_1} + j_{ DN_{N_\text{p}} }: \, \text{neutralizing left/right term (Dirichlet \& Neumann)} } \Delta x   \\
    & 
   %\sum\limits_{k=1,N_\text{p}} 
   \underbrace{-\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right)  u_1^2 (\lamb_{c})}_{j_{N_1}:  \, 
   \text{left Neumann cond.}} \Delta x 
   \underbrace{-\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right)    u_{N_\text{p}}^2 (\lamb_{c}) }_{j_{N_{N_\text{p}}}: \,   
   \text{right Neumann cond.}} \Delta x %\pover{\text{Bei den BC term die Sum streichen oder} \sum\limits_{k={1,N_\text{p}}}} 
   \,\\
   + &\sum\limits_{k=1}^{N_\text{p}} \, \underbrace{ -\zeta \lambda_{0}^2 u_k(\lamb_{c}) p_k u_k(\lamb_{c})  }_{{j_{P_k}: \, \text{potential term}}}  \, \Delta x + \sum\limits_{k=1}^{N_\text{p}} \underbrace{- 2\lambda_{0} u_k(\lamb_{c}) \Tilde{f}_k } _{j_{S_k}: \, \text{source term}} \, \Delta x
    \label{eq:Discrete_Opt_BC}
    \end{split}
%    \pover{Dann\,entsprechend\, unten\, drehen}
%\begin{split}
%   &J(\vb)k^l =\\
%   &-\nu\frac{\lambda_{0}^2}{\Delta x^2} \left(\underbrace{\sum\limits_{k=1}^{N_\text{p}}  u_k^l(\lamb_{c}) \left(u_{k+1}^l(\lamb_{c})-2u_k^l(\lamb_{c})+u_{k-1}^l(\lamb_{c})\right) }_{j_1^l : \text{Periodic BC}} - \underbrace{\left( u_1^l(\lamb_{c})u_{N_\text{p}}^l(\lamb_{c}) + u_{N_\text{p}}^l(\lamb_{c}) u_1^l(\lamb_{c}) \right)}_{j_2^l : \text{Dirichlet BC}} + \underbrace{\left(  u_1^l(\lamb_{c})^2 + u_{NP}^l(\lamb_{c})^2 \right)}_{j_3^l : (+j_2^l -> \text{Neumann BC})}\right) \Delta x\\
%   &\quad - \zeta \underbrace{\sum\limits_{k=1}^{N_\text{p}} \lambda_{0}^2 u_k^l(\lamb_{c}) p_k^l u_k^l(\lamb_{c})  \Delta x}_{{j_4^l:\text{Potential}}}  -  2\lambda_{0}\underbrace{\sum\limits_{k=1}^{N_\text{p}}  u_k^l(\lamb_{c}) \Tilde{f}_k  \Delta x}_{j_5^l:\text{Source}}
%    \label{eq:Discrete_Opt_BC}
%    \end{split}
\end{align}
%\end{document}
This approach is applied \trung{in the sense of the desired boundary conditions} for all time steps and can be adapted to various combinations of Dirichlet, Neumann, \pover{Robin} or periodic boundary conditions. \Eq{eq:Discrete_Opt_BC} utilizes a modified source term $\tilde f_k$ which inheres the additional source term contribution given in Eqns. (\ref{eq:defcoD-left}-\ref{eq:defcoN-right}).
%
For the example of a Dirichlet conditions on the left boundary, cf. \Eq{eq:defcoD-left}, the source term contribution modifies 
%from  $j_{S_1} = - 2 \lambda_0 u_1 f_1$ 
to 
   $j_{S_1} = - 2 \lambda_0 u_1 \tilde f_1$, with 
   $\tilde f_1 = f_1 + 0.5  D \nu \lambda_0/\Delta x^2 $.
%  Mind that Dirichlet conditions require $j_{DN_k}$ to be activated and Neumann conditions to activate both,  $j_{DN_k}$ and  $j_{N_k}$.

Before we continue with the  QC implementation of the different objective function contributions, we remark, that the Neumann terms $ j_{N_1}$ and $j_{ N_{N_\text{p}}}$ could also be casted into additional potential term contributions derived from the reciprocal of the diffusive time scale, i.e. 
 $\tilde p_1 = p_1 + \nu/(\zeta \Delta x^2)$ and
 $\tilde p_{N_\text{p}} = p_{N_\text{p}} + \nu/(\zeta \Delta x^2)$.  
%\pover{Neumann can be reformulated into Potential}

%\trung{One could of course also think of doing the j-DN in a linearized version and push that to the source term. Would that resemble the masking?}


==> Container/C_Feb10_Sections/RED-Intro.tex <==
%###########################################
%       Introduction
%###########################################
\section{Introduction}\label{sec:Introduction}
%\pover{
% Contradicting Pub:
%Read this three and see if we need to cite: 
%\cite{Sarma2023}  RECENT ! MENTION!
%\cite{GonzalezConde2022}  %Second ancilla important for  ghost points ...   
%}
%###########################################
%
% --- INTRO TURBULENCE SCALES ---- 
%The large range of spatial and temporal scales in turbulent flows makes its computation very expensive, demanding larger computational centres with high power consumption \cite{Jaksch2023}. 
%
%This posses a problem in the study of flows for industrial and academic, such as, large-scale climate modelling \cite{X}, applications in energy\cite{X}, petrochemical \cite{X}, and transportation industries \cite{X}. but also relevant in the societal impact in biomedical and health research applications such as the development of drug delivery systems \cite{X} and medical devices \cite{X} or the analysis of physiological flows \cite{X}. 
%
% --- INTRO APPLICATIONS ---- 
%\sbengoechea{(the development of drug delivery systems \cite{X} and medical devices \cite{X} or the analysis of physiological flows \cite{X})}, 
%
% --- INTRO for non-Linear ----
%\cite{Berry2014} Despite the computational power of QC, a natural application for QC is linear diff equations, because time evolution under a Hamiltonian corresponds to a linear diff equation. The solution in QMechanics only includes oscillatory terms while general diff equations have solutions that grow or decay exponentially. Classical physics is described by more general diff. equations. Therefore the need of more general (non-linear) Q approaches as in Lubasch et al. 
%
% --- REVIEW QCFD MPS---
%It has recently been shown the benefits of applying quantum-based techniques on CFD calculations \cite{X,X}. This can be intrepreted as a reduced order modes with high  compression data techniques rates. In all these works the last step to from a tensor network to the quantum-gates is omitted. 
%In LiuWu the poisson equation is solve by decomposing the discrete derivative matrix as tensor products, in a quantum-inspired approach. 
%
% --- REVIEW QPDE ---
%The intro of MoawadVanderbauwheSteijl2022 gives a good overview of previous QCFD and QPDE. 
%The review about QC and PDE given in Garcia Molina Rodriguez 2022
%
%###########################################

Partial differential equations (\textsc{PDE}) are ubiquitous for modeling problems in science and engineering. Areas of application include structural and fluid mechanics, electrodynamics, thermodynamics, or quantum physics. Today, sophisticated and dedicated numerical methods are well-established and widely available in all of those areas. However, the increasing demands to resolve wider ranges of spatial and temporal scales with great precision make these simulations very expensive and energy-consuming. 
%
%For industrial and academic applications in large-scale climate forecast \TODO{\cite{} cite NASA vision}, energy \TODO{\cite{} cite}, petrochemical \TODO{\cite{} cite see proposal}, and transportation \TODO{\cite{} cite, see proposal}, as well as in biomedical and health research \TODO{\cite{} cite},
%
%
%supercomputing centers \cite{Jaksch2023}. \pover{NASA VISION 2030 https://ntrs.nasa.gov/citations/20140003093}
%Moreover, chip sizes for classical central processing units (\textsc{CPU}s) are expected to converge in the next decade \cite{Burg2021}, and --due to the related limitations of Moore's Law \cite{Khan2018} --  increasing the computing power with traditional hardware is therefore challenging. 
%
Moreover, chip sizes for classical central processing units (\textsc{CPU}s) are expected to converge in the next decade \cite{Burg2021}, due to the impossibility of reducing the transistor's size further, putting an end to the Moore's Law \cite{Khan2018}. Therefore, the increase of computing power with traditional hardware is challenging.
 
The use of Quantum Computers (\textsc{QC}s) for solving initial or boundary value problems promises to overcome some of the future hardware-related challenges. 
%with a potential not capable of being delivered by their classical counterparts \cite{Jaksch2023}.
%
%The advantage of \textsc{QC} relies on the exponential growth capacity to store and process information by its basic component, the qubit \cite{Jaksch2023}. 
%
%The use of \textsc{QC}s for solving initial or boundary value problems has been attempted previously.
%
Grossly speaking, two categories for QC-supported PDE solutions have been proposed. 
They are either based on the direct encoding of the \textsc{PDE} solution in a large quantum circuit or on the Variational Quantum Algorithm (\textsc{VQA}), which evaluates shallow circuits in combination with classical optimization methods \cite{Suau2021}.
%
%FRIST
For the first category, Quantum Linear Solvers (\textsc{QLS}) are applied to algebraic equation systems derived from the discretization of linear \textsc{PDE}s. 
In a pioneering work \cite{Harrow2009}, Harrow, Hassidim and  Lloyd presented the HHL quantum algorithm to compute the solution of a Linear System of Equations (\textsc{LSE}).
The quantum advantage is achieved by outsourcing the most demanding solution of the LSE part.
%, i.e. $Ax=b$. The approach is exponentially faster than classical algorithms for small condition numbers $k$ of $A$\sout{, between $1/k$ and 1}. 
%The so-called \textsc{HHL} \pover{what is HHl - introduce abbreviation} method can be interpreted as an exponential accelerator for solving \textsc{LSE}. 
In \cite{Montanaro2016} a modification of the HHL algorithm is applied to solve an \textsc{LSE} originating from a Finite-Element Method while the temporal evolution of a linear \textsc{PDE} is approximated in \cite{Berry2014}. 
%
Fluid dynamic applications are reported in \cite{Steijl2018,Gaitan2020,Oz2021,Childs2020,Childs2020a,Cao2013,Chen2021}.
%
 Steijl and Barakos \cite{Steijl2018} %recovers the vorticity for incompressible flows by merging the classical particle-mesh method for the Helmholtz equation with
 used a vortex-in-cell CFD method and 
 employ a quantum Fourier solver for the Poisson equation. 
 %governing the stream function in a vorticity-stream function formulation in 2D. \sbengoechea{Correction: employ a quantum Fourier solver for the Poisson equation governing the vorticity evolution in the Helmholtz equation.}
%At this point, it is also worth mentioning the works of 
In \cite{Gaitan2020} and \cite{Oz2021}
%where the compressible Navier-Stokes and the Burgers' equation for one-dimensional \pover{inviscid -  double check} flows are resolved. In this case,
%the differential form of 
the \textsc{PDE} system is spatially discretized into a system of coupled Ordinary Differential Equations (\textsc{ODE}s) and approximated via a Quantum Amplitude Estimation Algorithm (\textsc{QAEA}) proposed by Kacewicz  \cite{Kacewicz2006}. 
%Another example has also been combined with spectral methods for solving first-order linear Ordinary Differential Equations (\textsc{ODE})s and second-order elliptic \textsc{PDE}s 
 In \cite{Childs2020} and \cite{Childs2020a}, %respectively. Here, 
 the PDE solution is spatially approximated with truncated Fourier or Chebyshev series, in which the unknown coefficients are determined by a \textsc{QLS}. 
%This type of quantum algorithm has also been used
 In the study of Cao et al. \cite{Cao2013}, the \textsc{HHL}  is used to solve the Poisson equation within a predictor-corrector method to solve the incompressible Navier-Stokes equation. 
%\sout{In the case of compressible flows, as in the work of }
%\trung{ what about \cite{Chen2021} ?}
%\sout{, the \textsc{HHL} method can be directly applied as \textsc{QLS} to approximate the \textsc{LSE} resulting from the discretized Navier-Stokes equations with classical Finite Volumes.}
%
%\sout{in the direct method the quantum acceleration is achieved by outsourcing the most computationally demanding part, i.e. solving the \textsc{LSE}, to the \textsc{QC}.} 
%
%To complete efficiently the task of solving the \textsc{PDE} problem, 
The QLS approaches mentioned above mostly require a large number of qubits devoted to error correction.
%, in the quantum computing substep. 
Hence they are more suitable for future fault-tolerant quantum machines and less suitable for QCs of the current Noise Intermediate-Scale Quantum (\textsc{NISQ}) era \cite{Suau2021}. 
%\sout{the quantum sub-step requires \sbengoechea{a large number of} \sout{many} qubits with specific ones devoted to error-correction, making the approach more suitable for future fault-tolerant quantum machines and less appropriate for the current Noise Intermediate-Scale Quantum (\textsc{NISQ}) era }\cite{Suau2021}. 

%SECOND

\smallskip 
 The \textsc{VQA} is an alternative second category to solve PDE problems dedicated to state-of-the-art \textsc{NISQ} devices \cite{Peruzzo2014}. The noise-tolerant procedure is based on the efficient evaluation of a cost function by the \textsc{QC}, while the classical hardware optimizes the parameters of the ansatz circuit that encodes the solution on the QC. 
 %, encoding the solution and avoiding a direct measurement of the quantum register.
As a consequence, the \textsc{PDE} to solve requires to be reformulated as an optimization problem.
A main advantage of the approach is the use of a small number of gate operations, making it more robust to decoherence effects of the quantum registers that compose the circuits. 
%\sbengoechea{Decoherence in gates or register? ask Nis} \pover{Register}

 \textsc{VQA}s are used in many applications such as the identification of ground states \cite{Peruzzo2014}, 
%simulation dynamics of quantum systems \cite{} \TODO{CITE}, 
 or solving \textsc{LSE} \cite{Cerezo2021}. 
 Recent applications to fluid dynamics and related PDEs are
 for example reported in \cite{Demirdjian2022,BravoPrieto2019,Kyriienko2021,Sato2021,Leong2022,Leong2023}. 
%Concerning its application for \sout{\textsc{PDE}s} \sbengoechea{\textsc{CFD}}, the work of \cite{Demirdjian2022} reformulates the 
Burgers advection-diffusion equation is studied in \cite{Demirdjian2022} where the discretized 
%as a \textsc{LSE}, containing the full time and space solutions. 
%The 
sparse matrix problem is 
%can be then
decomposed in a finite series of unitary operators and solved by the variational quantum solver proposed in \cite{BravoPrieto2019}. In \cite{Kyriienko2021}, quantum neural networks are trained with a hybrid \textsc{VQA} to 
solve systems of nonlinear differential equations that
% by optimizing the spectral base function coefficients. 
%The method is tested for the compressible Navier-Stokes equation 
model a supersonic nozzle flow. The work of Sato et al. \cite{Sato2021} is of particular relevance for this study and explores the ability of \textsc{VQA}s to solve the Poisson equation by minimizing the potential energy of an elliptic \textsc{PDE}.
%to find the steady state solution. 
To this end, the dynamics of the Poisson equation can be linearly decomposed in a series of parameterized shallow quantum circuits. The idea of energy minimization from Sato et al. \cite{Sato2021} is extended to time-dependent problems in Leong et al. \cite{Leong2022,Leong2023}.
%by including time domains through the implicit time-stepping of the Laplacian operator for arbitrary right-hand side in \sbengoechea{elliptic \textsc{PDE}s}.
%Additionally, the diffusion parts and the pressure correction of the reaction-diffusion and the incompressible Navier-Stokes equation are treated semi-implicit by the \textsc{VQA} and the non-linear terms with classical approaches. 
%\pover{The above text is very rich in references! I like it. Sometimes I have trouble to read it , it seems like a long enumeration of facts. Maybe when reforming it , we can also shorten it by one paragraph. }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% OUR WORK:
The present joint effort aims to combine  
%is a further step in the collective effort of bringing Computational Fluid Dynamics (\textsc{CFD}) applications to \textsc{QC}s. To this end, 
the quantum framework described in Lubasch et al. \cite{Lubasch2020} with the 
work of Sato et al. \cite{Sato2021}. We focus on 
%(a) the ancillary measurement of results and (b) 
a more flexible treatment of engineering boundary conditions on QCs and deploy
%
%is extended to cover not only \pover{I think they also cover Least square opt in time!} specific eigenvalue problems of quantum mechanics but also elliptic \textsc{PDE}s \pover{with a variational framework derived from the Galerkin and Ritz theories of weighted residuals and variational caclus (given in Sec. \ref{sec:Mathematics}).} \pover{We achived to outline similtudes, between the engineered framework and the version described by \cite{Sato2021}, which closses the loop to common engineering applications.} \sout{with an adapted version of the variational method described by } \cite{Sato2021}. \pover{I would describe our work as a paralell to satos work from engineering point of view, not as a simple repetition.} 
%
%The first aspect is concerned with a special feature of the quantum algorithm that was outlined by Lubasch et al. \cite{Lubasch2020}, namely 
the use of a Hadamard-test-based structure to retain quantum advantage  \cite{Guseynov2023}.
%of theas quantum advantage task described, Hadamard test based structure \cite{Guseynov2023}. 
%This capability of 
The related single-qubit measurements avoid expensive sampling operations for assessing the results encoded in a quantum state and thereby avoid the associated efficiency reductions. 
%\sout{that could} potentially vanish the quantum advantage
\cite{Berry2014,Kyriienko2021,Chen2021}.
%Mind that processing results is particularly expensive in \textsc{VQA} for transient \textsc{CFD}, since \textsc{I/O} between classic and quantum parts occurs in every time step \cite{Chen2021}. 
%Application to elliptic PDEs finalized, an extension to all types of linear PDEs, is achieved with small addition effort. Implicit discretization in time, as the tool for the merge to an elliptic framework, make the framework capable to solve parabolic and hyperbolic PDES, as described in \cite{Leong2022,Leong2023}. \sout{ Furthermore, based on the common Laplacian operator in all types of linear \textsc{PDE}s, the presented quantum algorithm can also be modified to approximate parabolic and hyperbolic \textsc{PDE}s applying implicit time-marching evolution, as described in }\cite{Leong2022,Leong2023}. 

An accurate, flexible and robust treatment of a diverse range of boundary conditions is of crucial importance for engineering applications. 
%\sout{The correct treatment of the boundary conditions is crucial in the solving of \textsc{PDE}s. }
Despite the importance, its rigorous algorithmic implementation in the context of \textsc{QC} is not trivial, as demonstrated by the variety of specific approaches proposed in the literature. 
The works of Cao et al. \cite{Cao2013} and Childs et al. \cite{Childs2020} are restricted to  Dirichlet conditions, while a related study of Childs at al. \cite{Childs2020a} mirrors the solution into the symmetric and antisymmetric sub-spaces for Neumann and Dirichlet cases, respectively. 
The mixed boundary conditions for the Burgers equation suggested in \cite{Oz2021} can only be enforced on classical hardware. 
The algorithm suggested in \cite{Costa2019} imposes Dirichlet or Neumann conditions on the discrete wave equation prior to the derivation of the Hamiltonian operator, i.e. the solutions in the Hilbert space (trial functions)  need to satisfy the boundary conditions. A modification of this approach is presented by \cite{Suau2021} where only Dirichlet boundaries are included. 
For \textsc{VQA} applications, the boundary conditions in \cite{Kyriienko2021} are included either as part of the cost function or as an additional constraint on the ansatz function. 
 The Dirichlet and Neumann boundary condition operators employed by Sato et al. \cite{Sato2021} do not form unitary operators. This  either requires an implementation on classical hardware, due to the required non-unitary corrections, or measuring the whole quantum register, which in turn reduces the efficiency. 
%
%Therefore, a focal point of this study refers to a novel treatment of the boundary conditions specialized to the unique properties of the \textsc{QC} hardware. 
% 
Therefore,  the present paper suggests to combine 
%In particular, 
a classical ghost-point technique 
%from \textsc{CFD} is combined
with a unitary decomposition of the boundary operators along a route suggested in \cite{Sato2021}. The decomposed boundary operators are subsequently  compiled into quantum gates, and finally included in the cost function using a deferred-correction strategy. The proposed approach permits the full-quantum implementation of arbitrary 
 %homogeneous and inhomogeneous  for 
  Dirichlet, Neumann, \pover{Robin} and mixed conditions without putting additional constraints on the trial or ansatz functions.  

%The final goal of this investigation is to address the natural question of how feasible and accurate \textsc{VQA} methods work for homogeneous and inhomogeneous linear \textsc{PDE}s with arbitrary boundary conditions. For that, t

The remainder of the paper is structured as follows: Sec. \ref{sec:Mathematics} introduces the mathematical model. Subsequently, the boundary treatment and the computational model are described in Secs. \ref{sec:Discretization} and \ref{sec:Strategy}. The latter also outlines the QC implementation and the utilized quantum circuits. Section \ref{sec:Optimization} describes the employed optimization procedure, as a by-product of the present study, and section \ref{sec:Applications} is devoted to numerical results. \trung{Applications are concerned with steady and transient heat conduction. Results refer temperature distributions %described by the Poisson and Heat equation 
obtained in combination with various types of boundary conditions which are compared to results of classical Finite-Differences (\textsc{FD}).} Final conclusions and future directions are outlined in Sec. \ref{sec:Conclusion}. 
%
The presented quantum framework is emulated with \textsc{IBM}'s \textsc{Qiskit} environment \cite{Qiskit}. 
%
 Within the publication, 
 %Einstein summation convention is used for lower-case Latin subscripts. V
 vectors and tensors are defined with reference to Cartesian coordinates. 




==> Container/C_Feb10_Sections/RED-Math.tex <==
%###########################################
%       Mathematical Framework
%###########################################
\section{Mathematical Model}  \label{sec:Mathematics}
The mathematical model consists of four steps. First, the considered PDE is introduced and discretized in time. Subsequently, the spatial PDE is casted into an optimization problem, and the objective functional is prepared for being evaluated on QC hardware, before the spatial discretization is outlined.  
%

\subsection{Governing Equation} \label{sec:GoverningEq}
The presented approach is restricted to  unsteady, spatially 1D
problems. An extension to two- or three spatial dimensions $\O$ and its  boundaries $\B$ is straightforward 
%\pover{If the differentiation operators in a dimension are independent of the other dimensions.}
\cite{Lynch1964}. For brevity, we use a \pover{\sout{normalized}} spatial coordinate $x \in [0,1]$ and a time domain $t \in [0,T]$. 
%
The problems considered herein are described by an unsteady reaction/diffusion PDE for an unknown field or state variable $y(x,t)$ 
%\trung{Wave Equations - Decide Later}
\begin{equation}
   \frac{\partial y }{\partial t}-\nu \Delta y -\zeta y \, p   = f \quad \text{in } \O_\text{T} : =  (0,1) \times [0,T] \, . 
   \label{eq:Generic_PDE-TR}
   \end{equation}
In \Eq{eq:Generic_PDE-TR}, the notation  $\Delta y = \nabla \cdot \nabla y$ describes the Laplace operator acting on $y$. 
Moreover, the right-hand side term  $f(x)$ denotes a time-independent source,  $p(x,t)$ is a time-dependent potential that is 
independent of y, 
%wo ist die Nonlinearity geblieben??}\pover{hatte es so verstanden das diese gehn muss. Es würde passen wenn wir diese mit p(x,t,y) wieder holen.}, 
$\zeta$ is a simple (real) coefficient and $\nu$ refers to the inherently positive (real) diffusivity. 
%
In contrast to previous works published in  \cite{Leong2022,Leong2023,Sato2021,Arrazola2019,Cao2013}, the framework to solve \Eq{eq:Generic_PDE-TR} should apply to arbitrary combinations of Dirichlet and Neumann conditions. However, details of the boundary treatment will be outlined in Sec. \ref{sec:Discretization}. 

%\trung{Mind that using a Picard linearization, nonlinearities can be viewed as modifications of the potential  term $p$ in an iterative process.}
\subsection{Temporal Discretization}
 The time horizon $T$ is discretized into $N_\text{t}$ equidistant time instants $t_l$, where $l \in \left[1,N_\text{t}\right]$ and $\Delta t$ marks a constant time step. 
In line with traditional finite approximation strategies,  time derivatives are approximated by implicit backward finite differences, e.g. an implicit first-order Euler scheme or a second-order three time-level scheme
\begin{equation}
 \frac{\partial y(x,t^l)}{\partial t} = \frac{ y(x,t^l) -y(x,t^{l-1}) }{\Delta t} + \mathcal{O}(\Delta t) \, , \quad
 \frac{\partial y(x,t^l)}{\partial t} = \frac{3 y(x,t^l) -4y(x,t^{l-1}) +y(x,t^{l-2}) }{2\Delta t} + \mathcal{O}(\Delta t^2)
 \; .
\label{eq:Generic_time}
\end{equation}
The examples included herein use the implicit Euler scheme. 
This results in the following modifications of the potential term $p\to p + 1/(\zeta \Delta t)$ and the source term $f \to f+ y(x, t^{l-1})/\Delta t$, which yield a spatial PDE at time $t^l$ in residual form 
\begin{equation}
 R(y(x,t^l)) = 
  - \left( \nu \Delta y + \zeta y \, p   + f \right) = 0 \quad \text{in } \O_\text{T} : =  (0,1) \times [0,T] \, . 
   \label{eq:Generic_PDE-TR-2}
   \end{equation}



\subsection{Optimal Control Problem} 
\label{sec:optimal_control}

A weak form of \Eq{eq:Generic_PDE-TR-2} follows from a weighted residual formulation and reads
%\end{document}
\begin{align}
 \int_{\O}  z(x,t^l) \, R(y(x,t^l) \,  dx  = 0 \, , 
  \quad \text{or} \quad  
\underbrace{-\int_{\O} z \big( \nu\Delta y + \zeta y \, p\big) \, dx}_{a(z,y)} 
 - \underbrace{\int_{\O} z \, f \, dx}_{F(z)} = 0  
 \label{equ:weighted_res-2}
\end{align}
 where $z(x,t^l)$ is a weighting function. For $z=y$, the latter evolves into
%  where $y$ is also
a solution to a variational problem  \cite{Grossmann2007,Glowinski2015}
characterized by minimizing an objective functional $\mathcal J$ for 
\begin{align}
    \min\limits_{y} \mathcal{J}(y) \quad  \text{with} \quad \mathcal{J}(y):= a(y,y) - 2F(y).
    \label{eq:Generic_Opt_Approx}
\end{align}
Mind that the equivalence of the PDE solution \eqref{eq:Generic_PDE-TR} and the minimization problem \eqref{eq:Generic_Opt_Approx} restricts the function space $y$ \cite{Grossmann2007}, \pover{May we can include smth. additional to argue with robin. Discuss.. \sout{which will not be discussed further here, and that the computed solution is of course only an approximation to $y$.} In case, that the bilinear term $a(z,y)$, is elliptic and symmetric no restrictions are faced \cite{Grossmann2007}. Furthermore, mention that the computed solution is of course only an approximation to $y$.}
%
 %The state $y$ approximates $y_{\O}$ and is commonly referred to as the ansatz function. It is assumed to be given by a known mapping $u(\lamb_{c}): \mathbb{R}^{c} \to Y$, where $c\in \mathbb{N}$ defines the number of control parameters $\lamb$. 
%
 Due to the limited ability to represent arbitrary states $y$ on QC hardware, $y$ should  ideally fulfill a \textit{partition of unity} constraint 
% by an isoperimetric condition, 
  given by the $L^2$ scalar product as \cite{Troutman1996,Werner2005}
\begin{align}
    (y^*,y)_{L^2} = \int_{\O}  y^*(x,t^l) \, y(x,t^l) \,  dx =  1 \, ,
    \label{eq:partition_of_unity}
\end{align}
where the asterisk indicates the conjugate complex.
%\trung{Wo genau benötigen wir Lie -Gruppen?%\cite{Abrudan2005}} \pover{Die thematik der Lie Gruppen aufzugreifen, galt der darstellung der komplexität bzgl. Optimierung. Des Weiteren ist unserer Ansatz SO4 eine Abbildung der SO4 Lie Gruppe}. 
Turning our attention to the variational framework \eqref{eq:Generic_Opt_Approx}, %into the constraint functional space $(\|y\|_{Y} = 1)$, explicitly given by \textit{Lie groups} \cite{Abrudan2005}. T
the function $y$ is made variable by the control $\upb^l \in \mathbb{R}^{c+1},  \upb^l: = \left(\lambda_0^l, \lamb_c^l\right)^\intercal,$ using the time-dependent ansatz 
\begin{align}
    y(x,t^l, \upb^l) = \lambda_{0}^{l} \, u(x, {t^l}, {\lamb_c^l}) \, , \quad \text{with} \quad 
%    u(x, \trung{?t^l}, \lamb_c) : 
    \big(u^*, u\big)_{L^2} = 1 \, \pover{\text{and} \, c\in \mathbb{N},} %\quad \trung{oder \, besser \, als \, Integral?}
        \label{eq:Generic_Ansatz}
\end{align} 
% where $ u(x,\lamb_c) : \big(u^*, u\big)_{L^2} = 1$ 
 to enforce the normalization restriction \eqref{eq:partition_of_unity}.  
%
Suppressing the temporal index $(...)^l$ and substituting the ansatz \eqref{eq:Generic_Ansatz} into the objective functional, 
%the constraint $J(\upb) : \mathbb{R}^{c+1} \to \mathbb{R}$, 
one obtains (the time-dependent) minimization problem 
%\pover{for each $l \in [1,N_\text{t}]$ timesteps}  
\begin{align}
	\begin{split}
     \min \limits_{\upb} J(\upb)  \quad \text{with} \quad J(\upb) :&= a\big(y(\upb),y(\upb)\big) - 2F(\upb),\\
%     \pover{\text{Correct the rest}}
%			 &=  - \nu  \int_{\O}  \lambda_{0}^2 \;  du(x, \lamb_{c}) \Delta u(x, \lamb_{c}) \, dx - \zeta \int_{\O} \lambda_{0}^2 \;  u(x, \lamb_{c}) \, p(x) \, u(x, \lamb_{c}) \, dx \\
			 &=  - \nu  \, \lambda_{0}^2 \int_{\O}  u(x, \lamb_{c}) \Delta u(x, \lamb_{c}) \, dx - \zeta \, \lambda_{0}^2  \int_{\O} u(x, \lamb_{c}) \, p(x) \, u(x, \lamb_{c}) \, dx \\
        &\quad- 2  \lambda_{0} \int_{\O}  u(x, \lamb_{c}) \, f(x) \, dx \, .
	\end{split}
\label{eq:Reduced_Opt}
\end{align}
For each time step, this minimization is performed using a simple gradient descent method (GD) that requires the derivatives of the objective function with respect to the control. 
% 
The Gâteaux derivative with respect to the control $\upb$
% of the reduced functional $J(\upb)$ 
 provides 
% a condition for a stationary point $\hat{\upb} : J(\upb)  \geq  J(\hat{\upb}) \quad \forall \upb$ can be reformulated as
 a first-order optimality condition \cite{Troutman1996}
\begin{align}
     \frac{\partial J}{\partial \upb} \delta \upb &= {\frac{\partial J}{\partial y} \frac{\partial y}{\partial \upb} \delta\upb} =  \begin{pmatrix}
            \nabla_{\lambda_0} J \\ 
            \nabla_{\lamb_c} J 
        \end{pmatrix}  \cdot \begin{pmatrix}
            \delta \lambda_0\\
            \delta \lamb_c
        \end{pmatrix} =  0 \quad \forall \, \delta\upb.
\end{align}
 The partial derivatives of the objective functional with respect to the control 
 is not discussed in the continuous form herein. Instead, a QC-compatible discretized form is developed in Sec. \ref{sec:Optimization}. 
 
% \begin{align}   \begin{split} 
%       \nabla_{\lambda_0} J &= -2\nu  \, \lambda_{0} \int_{\O}  \big(  u(\lamb_{c}) \, \Delta u(\lamb_{c}) \big)        dx - 2 \zeta \, \lambda_{0} \int_{\O} \big( u(\lamb_{c}) \, p \, u(\lamb_{c}) \big)  dx - 2 \int_{\O} \big( u(\lamb_{c}) \, f \big)        dx \, ,  \\
%       \nabla_{\lamb_c} J  &=         -\nu \,  \lambda_{0}^2 \int_{\O}  \big( u'(\lamb_{c})\, \Delta u(\lamb_{c}) \big)      \, dx        -\nu \, \lambda_{0}^2 \int_{\O} \big(   u(\lamb_{c}) \,       \Delta u'(\lamb_{c})  \big)         \, dx \\
%        &\quad - 2 \zeta \, \lambda_{0}^2  \int_{\O} \big( u(\lamb_{c}) \, p \, u'(\lamb_{c}) \big) \delta\lamb_{c} dx - 2  \lambda_{0} \int_{\O}  \big( u'(\lamb_{c}) \, f \big)         \, dx \, , 
%    \end{split}
%    \label{eq:first_order_opt}
%\end{align}
%where the partial derivative of the ansatz function $u(x, \trung{t^l}, \lamb_c)$ with respect to $\lamb_{c}$ is denoted by 
%$\nabla_{\lamb_c} u = u'$.
%
%Integrating the second term of the Gâteaux derivative  
%$\nabla_{\lamb_c} J$ by parts yields 
%\begin{align}\begin{split}
%\nabla_{\lamb_c} J &= -2 \nu \, \lambda_{0}^2 \int_{\O} \big( u'(\lamb_{c}) \,  \Delta u(\lamb_{c})  \big)  \, dx   - 2 \zeta \, \lambda_{0}^2 \int_{\O} \big(  u(\lamb_{c}) \, p \, u'(\lamb_{c}) \big) \,  dx \\ 
%  &\quad \, - 2  \lambda_{0} \int_{\O} \big( f(x) \, u'(\lamb_{c}) \big) \,  dx -\nu \, \lambda_{0}^2  \oint_{\B} \left( u(\lamb_{c}) \frac{\partial u'(\lamb_{c}) \delta\lamb_{c} }{\partial n}  -  \frac{\partial u(\lamb_{c})}{\partial n} u'(\lamb_{c})   \right)  \,  dS \, .
% \label{eq:continu}
%\end{split} \end{align}
%The last term in (\ref{eq:continu}) denotes a surface integral, with $n$ referring to the outward pointing normal direction of the surface element $dS$. In a periodic boundary setting, the contributions to this surface integral neutralize and the term vanishes. For non-periodic boundaries, the contributions follow from the respective boundary conditions. 
%%%We will, however, not discuss these terms in the continuous form  (\ref{eq:continu}), but introduce the respective boundary contributions to the objective functional in a discretized form in Sec. \trung{???} \ref{sec:Discretization}.  

\subsection{Spatial Discretization}
%###########################################
%       Discretization of the Governing equations
%###########################################
%The discretization employs a simple two-dimensional, spatio-temporal 
%finite difference (FD) discretization, given by the 
% grid, cf. Fig. \ref{fig:discretization_encoding}. % $\mathcal{M} \subset \Bar{\O}_\text{T}$. 
  The spatial discretization of the unit interval $\left[0,1\right]$ is discretized by $N_\text{p}+2$ equidistantly spaced points 
%with spacing $\Delta x$.
%= \nicefrac{1}{N_\text{p}+2}$.
%  The discrete points 
  $x_k$, with $k \in \left[0,N_\text{p}+1\right]$. As alluded to earlier,  the time $t\in [0,T]$ is discretized by $N_\text{t}$ equidistant time instants $t^l$, which  leads to the structured grid depicted in 
  %,  with $l \in \left[1,N_\text{t}\right]$. 
  \Fig{fig:discretization_encoding}. As indicated by the figure, we distinguish between interior points (closed circles) and ghost points (open circles), which serve the introduction of boundary conditions.  
  %shows the structured mesh $\mathcal{M}$.
%  \pover{Do we want to stick to closed circles/open circles or use the tikz graphs in the txt?}
\begin{figure}[htbp]
    \centering
    \input{Figures/Discretization}
    \caption{Illustration of the spatial-temporal discretization %$\mathcal{M}$ of the unit interval given by 
     on an equidistant grid with 
    boundary/ghost nodes indicated by open symbols~(\protect\tikz \protect\draw[thick,black] (1ex,1ex)  circle [radius=0.1];) and ~interior nodes by closed symbols ~(\protect\tikz \protect\draw[fill] (1ex,1ex)  circle [radius=0.1];).}
    \label{fig:discretization_encoding}
\end{figure}
%
%Known from classical CFD techniques, BCs can be realized directly, as a part of the unknowns, or indirectly with the BCs not as part of the system of equations \cite{Ferziger2020}. 
Similar to classical finite approximation schemes, variables located along the spatial boundaries can either be part of the unknowns or separated from the unknowns. 
%
In the latter case, the BCs are represented by 
%interpolating schemes, based on 
the influence of prescribed ghost point variables on the interior point approximations. In the case of Neumann, \pover{Robin,} or mixed boundary conditions, this usually involves the additional discretization of the spatial derivative.   
%
%\trung{What type of BCs were used here? D or N?: A similar idea is emphasized by \cite{GonzalezConde2022}, which suggests a reflection of non-periodic effects at the original domain endpoints.} \pover{Dirichlet} Aiming for a  flexible setting, we introduce a quantum ghost-nodes approach, as a prerequisite for a shift to the quantum hardware. 

%The procedure is as follows: Boundary nodes are assigned to ghost nodes~(\protect\tikz \protect\draw[fill,gray] (1ex,1ex)  circle [radius=0.05];) and the discretized governing equations are evaluated for the internal nodes (\protect\tikz \protect\draw[fill,black] (1ex,1ex)  circle [radius=0.05];) with ghost node values evaluated from the discretized BCs. 

The procedure is as follows: Boundary nodes are assigned to ghost nodes (\protect\tikz \protect\draw[thick,black] (1ex,1ex)  circle [radius=0.1];)  
and the spatially discretized objective function \eqref{eq:Reduced_Opt} is evaluated for the interior nodes (\protect\tikz \protect\draw[fill,black] (1ex,1ex)  circle [radius=0.1];), with the contributions of the ghost nodes arising from discretized BCs.
%
%The degrees of freedom at the boundary  locations are isolated from  interior domain variables. 
Thus, the discrete ansatz function vector $\big(u(x_0,t^l), u(x_1,t^l), \dots, u(x_{N_\text{p}+1},t^l) \big) = \ub^l$ is represented using the orthogonal basis $\eb_k$, viz. 
\begin{align}
    \ub^l = u_0^l \eb_0 +  \underbrace{\sum\limits_{k=1}^{N_\text{p}} u_k^l \eb_k}_\text{Register} + u_{N_\text{p}+1}^l \eb_{N_\text{p}+1} \, ,  
    \label{eq:discretization_register}
\end{align}
with the interior to be stored in a register of length $\log_2(N_\text{p})$. 
%\pover{It would be handy in  sec comp strat if g is replaced by u}
%
%Remark at this point, these changes consequently result in a more flexible numerical framework. Instead of the restrictions by the \textit{Ritz-Method} to the Sobolev space of BC conformal functions $y$, the state $y \in W^{2,2}$ (c.to. \Eq{eq:Generic_Opt_Approx}). As a consequence, the ansatz requires only to ensure $u(\lamb_c) : \mathbb{R^c} \to W^{2,2}$.
%
%On the introduced discretization $\mathcal{M}$, the space collapses down to points-wise constant entities at each $x_k$. 
The derivatives of the Laplace operator required to evaluate the objective functional  (\refeq{eq:Reduced_Opt}) are approximated by
%a second-order approximation of the second derivative, viz. 
\begin{align}
\frac{\partial^2 u^l_k}{\partial x^2} =
%\bigg|_k = 
\frac{u_{k+1}^l-2u_k^l+u_{k-1}^l}{\Delta x^2} +  \mathcal{O}(\Delta x^2) \, , 
\label{eq:derivatives_space}
\end{align}
which is second-order accurate for an equidistant grid. 

==> Container/C_Feb10_Sections/RED-Results.tex <==
%###########################################
%       Numerical Results
%###########################################
\section{Numerical Results} \label{sec:Applications}
\pover{Add reference to UHH hosted experiments data doi.... }

This section describes the application of the 
%presented framework to several boundary-/initial-boundary value problems. The 
\textsc{VQA} to two prototypical \textsc{CFD} problems, i.e. the steady heat conduction 
%\textsc{[P]} 
(Sec. \ref{sec:Application:Poisson}) and the transient heat conduction 
%\textsc{[H]} 
(Sec. \ref{sec:Application:Heat}). Results are discussed for a range of in-/homogeneous Dirichlet and Neumann boundary-condition combinations.
%, ranging from homogenous Dirichlet and Neumann settings to inhomogeneous settings, periodic boundary conditions, as well as Robin  boundary conditions 
%Thereby, the capabilities of the proposed method as a tool for various PDE problems is presented. 
%
%To generalize the complete two-point boundary-value problem in \Eq{eq:Generic_PDE-TR-2}, mention the extension to homogenous and inhomogeneous Dirichlet, Neumann boundary conditions introduced by $D,N$ (c.f. Sec. \ref{sec:Discretization}). As discussed, is the source term adjusted to external contributions, as $\Tilde{\fb}= \fb + \fb_\text{ex}$ given by \Eq{eq:defcoD-left}-\eqref{eq:defcoN-right}. In case of a given value $D_0$ ($D_{N_\text{p}+1}$) as Dirichlet Boundary Conditions at $x=0$ ($x=1$) mention
%\begin{align}
%\fb_\text{ex} = \left(-u_1 D_0 \, \Big(\frac{\nu \lambda_0^2}{\Delta x^2}\Big),0,\hdots,0,-u_{N_\text{p}} D_{N_\text{p}+1} \Big(\frac{\nu \lambda_0^2}{\Delta x^2}\Big)\right)^\intercal.
%\end{align}
%For a Neumann Boundary Condition the analog  is 
%\begin{align}
%\fb_\text{ex} = \left(-u_1 N_0 \, \Big(\frac{\nu \lambda_0^2}{\Delta x}\Big),0,\hdots,0,+u_{N_\text{p}} N_{N_\text{p}+1} \Big(\frac{\nu \lambda_0^2}{\Delta x}\Big)\right)^\intercal.
%\end{align}
%In case of Robin boundary conditions a superposition is used. For periodic boundary condition, no adjustment is required. If an evolution in time space is part of the underlying problem, mention that the additional contributions $\fb \to \fb + \yb(x,t^l)/\Delta t$ and $\pb\to \pb + 1/(\zeta \Delta t)$ are required (c.f. Sec. \ref{sec:GoverningEq}).
%
The validation data is obtained from FD-solutions of the PDE problem. It employs the same discretization as the VQA to approximate the Laplace operator and the temporal derivative, cf. \Eq{eq:Generic_time} and \Eq{eq:derivatives_space}.
%For a quantitative comparison, the discrete solution of the \textsc{PDE} under study is computed classically by solving the linear system of equations arising from the discretization of the variational \Eq{eq:variational_eq} with Finite Differences (\textsc{FD}) and the implicit Euler method.
%

The predictive deviation of the VQA-solution $y^\text{VQA}$ form FD-solutions $y^\text{FD}$ is assessed using either the $l_2$-norm $\varepsilon_{l_2}$ or the frequently employed trace distance  $\varepsilon_{\text{tr}}$, cf.  \cite{BravoPrieto2019,Liu2021,Sato2021}, viz.
\begin{equation}
    \varepsilon_{l_2} = \sqrt{\sum_k (y_k^\text{FD}-y_k^\text{VQA})^2} \, , \qquad
    \varepsilon_{\text{tr}} = \sqrt{\bigg(1- \sum_k \Big|\frac{y_k^\text{FD}}{\sqrt{\sum_j (y_j^\text{FD})^2}}\frac{y_k^\text{VQA}}{\sqrt{\sum_j (y_j^\text{VQA})^2}}\Big|^2 \bigg)} \, .
\end{equation}
%as $ \varepsilon_{l_2} = \sqrt{\sum_k (y_k^\text{FD}-y_k^\text{VQA})^2}$ or the frequently employed trace distance  $\varepsilon_{\text{tr}} = \sqrt{\bigg(1- \sum_k \Big|\frac{y_k^\text{FD}}{\sqrt{\sum_j (y_j^\text{FD})^2}}\frac{y_k^\text{VQA}}{\sqrt{\sum_j (y_j^\text{VQA})^2}}\Big|^2 \bigg)}$, cf.  \cite{BravoPrieto2019,Liu2021,Sato2021}. 
Time-averaged measures are employed to assess the transient heat conduction 
%averaged over the corresponding $N_\text{t}$ timesteps 
and indicated by $ \Bar{\varepsilon}_{l_2}, \Bar{\varepsilon}_{\text{tr}}$. 
The number of control variables $c$  of  $\lamb_c$ is also stated in the results tables.
%, respectively.

% Mind that we restrict the simulations to noise-free idealized quantum devices,  only available via emulation, cf. discussion in Sec. \ref{sec:VQA}. 

%\sbengoechea{The library we present, of course, is subject to scaling effects and robustness when it comes to physical quantum hardware. (Do we need this?)}
%The validation of the variational code is performed by solving variationally the time independent Linear Schrödinger Equation \textsc({LSE}) and comparing the results with those given in the \textsc{QM} textbook of \textit{Griffiths} \cite{Griffiths2018}. 
%Results are given in Appendix \ref{sec:Validaion}. \pover{Suggest that we do not show any LSE results, lets just upload your code}
%To this end, two test cases are selected, the free quantum particle, with only kinetic energy, and two different potentials, infinite square well and the harmonic trap.

\subsection{Steady Heat Conduction (Poisson Equation)}
\label{sec:Application:Poisson}
The first case refers to the Steady Heat Conduction, where the time derivative in \Eq{eq:Generic_PDE-TR} vanishes and $y$ [K] marks the temperature. The physical potential $p(x)$ [1/s] vanishes, the diffusivity is assigned to a unit value $\nu=1$ [m$^2$/s]. In the case of pure Neumann boundary conditions, the source reads $f(x) =1$ for $x<0.5$ and $f(x) =-1$ for $x>0.5$. In all other cases, the unit source responds to  $f(x) \equiv 1$ [K/s]. Mind that singular solutions, e.g. caused by pure Neumann conditions, are fixed by defining a central zero crossing. The application of the \textsc{VQA} framework to this Poisson problem is presented for the following \trung{six} scenarios: in-/homogeneous Dirichlet, in-/homogeneous Neumann, mixed Neumann/Dirichlet conditions and periodic conditions (\trung{perhaps add Robin}). 
%Robin conditions. 
Displayed results are obtained for a coarse grid, featuring $N_\text{p}=4$ interior points ($n=2$ qubits; dashed lines), and a finer grid, featuring $N_\text{p}=16$ interior points ($n=4$ qubits; straight lines). The  \textsc{FD}-results are depicted by open squares ($N_P=16$) and closed circles ($N_P=4$). 

 The periodic case serves as verification reference and is displayed in \Fig{fig:Results:Poisson:periodic}.   
 VQA-results were obtained from shallow circuits $U(\lamb_c)$ using a depth of $d=1$, cf. \Fig{fig:VQA_Ansatz}.
 \Fig{fig:Results:Poisson:periodic:cost} shows the convergence of the cost function with the dotted vertical lines indicating the transition from global (PSO) to local optimization (cf. Alg. \ref{alg:VQA}).
%Vertical dotted lines in \Fig{fig:Results:Poisson:periodic:cost} indicate the switch between \textsc{PSO} and \textsc{GRAD}, c.f. alg. \ref{alg:VQA}. 
%As for all cases, the convergence-trigger is set according the number of employed qubits $n$. The max iterations \texttt{maxit}$_{G,P}=2000$.
%
The VQA-results are compared with  \textsc{FD}-solutions in \Fig{fig:Results:Poisson:periodic:res} and indicate an excellent agreement with the expected solution {$y_k \equiv 0$}. The VQA-result improves as the grid is refined. The latter is also indicated by a reduction of $\varepsilon_{l_2}$ 
 from an already satisfactory value of $10^{-6}$ to $10^{-7}$. This goes hand in hand with lower amplitude but higher frequency wiggles displayed in \Fig{fig:Results:Poisson:periodic:res}, which are reflected by an augmented trace distance $\varepsilon_{\text{tr}}$ and should be viewed with caution due to the vanishing mean value for this case.

%and \Fig{fig:Results:Poisson}. 
 

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \input{Figures/Results/R_Poisson_Cost.tex}
        \vspace{-0.4cm}
        \caption{Evolution of the normalized cost functional over the optimization count $i$. 
        %$J(\upb_i)/J(\upb_0)$ . 
        Dotted vertical lines indicate the transition from global (PSO) to local optimization. %JA!
        }
        %, c.f. alg. \ref{alg:VQA} l.\ref{alg:VQA:PSO} - \ref{alg:VQA:GRAD} respectively.}
        \label{fig:Results:Poisson:periodic:cost}
    \end{subfigure}
    \hspace{0.3cm}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Periodic.tex}
        \caption{Comparisons of VQA- and FD-results, ($n=2$, closed circles; $n=4$, open squares). } 
        \label{fig:Results:Poisson:periodic:res}
    \end{subfigure}
    \caption{Verification results of the \textsc{VQA} application for a periodic steady heat conduction problem  using  $N_\text{p}=4$ ($n=2$, $d=1$; dashed lines) and $N_\text{p}=16$ ($n=4$, $d=1$; straight lines) interior points.}
    \label{fig:Results:Poisson:periodic}
\end{figure}

\begin{figure}[htbp]
\centering
    \input{Figures/Results/Legend_Res.tex}\\
    \vspace{0.2cm}
    \begin{subfigure}[t]{0.49\textwidth}
       \centering
        \input{Figures/Results/R_Poisson_Dirichlet_homogeneous.tex}
        \vspace{-0.4cm}
        \caption{Homogeneous Dirichlet.
        %, at both ends using layer depth $d=1$ and $d=3$ for $n=2$ and $n=4$, respectively.
        }
        \label{fig:Results:Poisson:homoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Neumann_homogeneous.tex}
        \caption{Homogeneous Neumann.
        %using layer depth $d=1$ and $d=3$ for $n=2$ and $n=4$, respectively.
        } 
        \label{fig:Results:Poisson:homoNeumann}
    \end{subfigure}\\
    
     \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Dirichlet_inhomogeneous}
        \vspace{-0.4cm}
        \caption{Inhomogeneous Dirichlet.
        %using layer depth $d=1$ and $d=3$ for $n=2$ and $n=4$, respectively.
        } 
        \label{fig:Results:Poisson:inhomoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
         \input{Figures/Results/R_Poisson_Neumann_inhomogeneous.tex}
        \caption{Inhomogeneous Neumann. 
        %using layer depth $d=1$ and $d=3$ for $n=2$ and $n=4$, respectively.
        }
    \label{fig:Results:Poisson:inhomoNeumann}
    \end{subfigure}\\
   
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Mixed}
        \caption{Mixed.}
        %using layer depth $d=1$ and $d=3$ for $n=2$ and $n=4$, respectively.  
        \label{fig:Results:Poisson:Mixed}    
        \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Robin}
        \caption{Inhomogeneous Robin. \trung{Slightly unfortunate that results for the two grids deviate substantially - Perhaps Dirichlet that matches fine grid solution on the right side}}
        %using layer depth $d=1$ and $d=3$ for $n=2$ and $n=4$, respectively.  
        \TODO{n=4 results update}
        \label{fig:Results:Poisson:Mixed}
    \end{subfigure}\\
    
    \caption{Comparisons of VQA-result (lines) and FD-results (symbols) for the steady heat conduction in combination with different boundary conditions on a grid with $N_\text{p}=4$ ($n=2$; dashed lines \& closed circles) and $N_\text{p}=16$ ($n=4$; straight lines \& open squares) interior points. The depth of the ansatz circuit $U(\lamb_c)$ is $d=1$ for $n=2$ qubits and $d=3$ for $n=4$ qubits, cf. \Fig{fig:VQA_Ansatz}.}
    \label{fig:Results:Poisson}
\end{figure}


As indicated in \Fig{fig:Results:Poisson}, the \textsc{VQA} predictions perfectly agree with the \textsc{FD} reference for all Dirichlet, Neumann or mixed boundary conditions \trung{perhaps Robin} and grid resolutions. 
%\trung{I dont get this: As evident, changes the number of points switching between a periodic or non-periodic boundary setting, cf. \Fig{fig:Results:Poisson:periodic} and \Fig{fig:Results:Poisson}.} 
Furthermore, the first-order accuracy in the discrete approximation of the Neumann conditions is obviously detected in both the VQA- and the FD-results, cf. for example  \Fig{fig:Results:Poisson:homoNeumann}.
 The required depth $d$ increases for non-periodic conditions on the finer mesh. To this end, a depth $d=3$ is sufficient to mimic all boundary investigated conditions in conjunction with the finer grid. 
 %For a more detailed view onto the capabilities \Tab{tab:Results:Poisson:Errors} lists different measures. 

\Tab{tab:Results:Poisson:Errors} quantifies the deviation of the VQA-results from the FD-results 
%in the $l_2$-norm and the trace distance, 
 for all cases depicted in \Fig{fig:Results:Poisson}. The table displays a deviation of approximately $\varepsilon_{l_2} = 10^{-6}$--$10^{-7}$ for two qubits ($N_P=4$), disregarding the imposed boundary conditions. %\trung{Tabelle sagt was anderes: one can observe that this error is kept around $10^{-6}$ despite the boundary setting.} 
 The good agreement of $\varepsilon_{l_2}$ for the periodic case, where no specific boundary condition 
 circuits are required, and the non-periodic cases reveal that no substantial sensitivity of the attainable accuracy is observed when applying the current strategy for a quantum-based implementation of boundary conditions. For the finer discretization associated with $n=4$ qubits, the table %\Tab{tab:Results:Poisson:Errors} 
 shows higher values of $\varepsilon_{l_2} \approx 10^{-3}$ for the non-periodic boundary conditions 
  and thereby a less satisfactory agreement with the periodic arrangement. 
 The latter is attributed to difficulties of finding the global optimum in a non-convex optimization, 
%, ultimately defined by the \textsc{VQA} methodology. This
and highlights a  bottleneck of the VQA in combination with versatile ansatz functions $U(\lamb_c)$, cf. \Fig{fig:VQA}. Moreover, it also outlines that sufficient accuracy of the Ancilla measurements is 
%required not only a necessity to determine the derivative but also 
crucial for detecting the (global) minimum. 

The trace distance $\varepsilon_{\text{tr}}$ is given in the third column of \Tab{tab:Results:Poisson:Errors} and can be interpreted as point-wise correlation between the quantum- and the FD-result. The trace distance is related to the convergence of the global minimum, while the $\varepsilon_{l_2}$ measures the expressibility of the ansatz.
 Since the two measures address different aspects, considering just one of them seems insufficient. Moreover, the trace distance sometimes displays numerical zero values, cf. \Tab{tab:Results:Poisson:Errors}, which does not necessarily guarantee a perfect agreement and also advocates assessing both measures. 
 In addition to the sensors used to assess the VQA-results, the origin of the observed differences in predictive accuracy are also of interest.
 \trung{Check: Should we mention Sato?}  
 Interestingly, the results reported by Sato et al. \cite{Sato2021} -for example- show a much better 
 trace distance compared to the present results for periodic boundaries, although the predictive agreement of the current results appears to be slightly better. For periodic boundaries, a key difference between the current and similar recent efforts,e.g. \cite{Sato2021}, 
 %
 refers to the employed SO4-ansatz illustrated in \Fig{fig:quantum_ansatz_SO4}, which seems to feature an improved ansatz expressibility but is also harder to train. 
 
 %and the quality is assessed by two measures instead of only the trace distance in \cite{Sato2021}.  

Furthermore, the number of control variables $c$ given in 
\Tab{tab:Results:Poisson:Errors} 
roughly scales as $3^{n-1}$, which highlights an unfavorable exponential complexity and suggests room for future improvements in the design of the quantum circuits for the boundary conditions.



%\trung{by means of ... AS REGARDS PURE NEUMANN, I AM ASKING MYSELF, HOW YOU FIXED THE "LEVEL" OF THE SOLUTION (PERHAPS EVEN THROUGH SOMEKIND OF ROBIN ...)}

\begin{table}[htbp]
   \centering
   \caption{Deviations of  VQA- and FD-results in the $l_2$-norm ($\varepsilon_{l_2}$) supplemented by their trace distance ($\varepsilon_{\text{tr}}$) for results depicted in \Fig{fig:Results:Poisson}. The degrees of freedom are  indicated by the number of control variables $c$.}
   \label{tab:Results:Poisson:Errors}
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
Boundary Setting & \multicolumn{2}{c}{$l_2$-Norm $\varepsilon_{l_2}$}  & \multicolumn{2}{c}{trace distance $\varepsilon_{\text{tr}}$}&\multicolumn{2}{c}{DOF $c$} \\ 
\midrule
\multicolumn{1}{r}{interior points}&\multicolumn{1}{l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$   \\
\midrule
Periodic          & \multicolumn{1}{c}{$1.23 \times 10^{-6}$}&\multicolumn{1}{c}{$3.26 \times 10^{-7}$}&\multicolumn{1}{|c}{$9.70 \times 10^{-1}$}&\multicolumn{1}{c}{$1.0 \times 10^{0}$}&\multicolumn{1}{|c}{$3$}&$6$\\
Homog. Dirichlet   & \multicolumn{1}{c}{$1.5 \times 10^{-7}$}&\multicolumn{1}{c}{$6.76\times 10^{-3}$}&\multicolumn{1}{|c}{$0.00$}&\multicolumn{1}{c}{$6.76 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Homog. Neumann   & \multicolumn{1}{c}{$1.37 \times 10^{-8}$
}&\multicolumn{1}{c|}{$5.05 \times 10^{-3}$}&\multicolumn{1}{c}{$6.32 \times 10^{-8}$}&\multicolumn{1}{c}{$5.05 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Inhomog. Dirichlet & \multicolumn{1}{c}{$8.49 \times 10^{-8}$}&\multicolumn{1}{c}{$7.87 \times 10^{-3}$}&\multicolumn{1}{|c}{$4.31 \times 10^{-7}$}&\multicolumn{1}{c}{$7.87 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Inhomog. Neumann  & \multicolumn{1}{c}{$1.68, \times 10^{-6}$}&\multicolumn{1}{c}{$2.55 \times 10^{-3}$}&\multicolumn{1}{|c}{$1.65 \times 10^{-6}$
}&\multicolumn{1}{c}{$2.55 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Mixed   Dirichlet/Neumann          & \multicolumn{1}{c}{$6.01 \times 10^{-8}$
}&\multicolumn{1}{c}{$5.66\times 10^{-4}$
}&\multicolumn{1}{|c}{$0.00$}&\multicolumn{1}{c}{{$5.66
 \times 10^{-4}$}}&\multicolumn{1}{|c}{$3$}&$24$\\ 
Inhomog. Robin          & \multicolumn{1}{c}{$3.32 \times 10^{-9}$
}&\multicolumn{1}{c}{\TODO{$0$}
}&\multicolumn{1}{|c}{{$0.00$}}&\multicolumn{1}{c}{\TODO{$0$}}&\multicolumn{1}{|c}{$3$}&{\TODO{$0$}}\\ 
\bottomrule
\end{tabular}
\end{table}

\subsection{Transient Heat Conduction (Heat Equation)}
\label{sec:Application:Heat}
The second case is concerned with the transient heat conduction where the time derivative in \Eq{eq:Generic_PDE-TR-2} is treated as discussed in Sec. \ref{sec:Mathematics}. The contributions of the potential term $p(x,t)$ [1/s] as well as the physical source term $f(x)$ [K/s] in \Eq{eq:Generic_PDE-TR} are neglected. The diffusivity is again set to a unit value of $\nu=1$ [m$^2$/s]. Four different boundary condition settings are investigated using a constant time step of $\Delta t \nu/\Delta x^2 =0.02/(N_p+1)$ on the same two equidistant grids used in Sec. \ref{sec:Application:Poisson}, 
i.e., a coarse ($N_\text{p}=4$) and a fine grid ($N_\text{p}=16$). 
All cases studied should reach a steady state, and due to the different convergence speeds to the steady state, different time step numbers are shown for different boundary and initial conditions.
%
The convergence of the optimizer is controlled by \Eq{alg:convergence} using a threshold level of 
%$\textsf{ch}( \nabla J^l_i)$, with maximum values of 
$10^{-7}$ for two qubits and $10^{-3}$ for four qubits, respectively. 


\begin{figure}[htbp]
\centering
\input{Figures/Results/Legend_Res.tex}\\
\vspace{0.2cm}
    \begin{subfigure}[t]{0.48\textwidth}
       \centering
        \input{Figures/Results/R_Heat_Dirichlet_f1_homogeneous.tex}
        \caption{Solution obtained for the first 30 time steps with $y(x,t^1)=1$, using homogeneous Dirichlet conditions ($y = 0$) at both ends and $d=1$.
        %and a constant source $f(x,t^1)=1$. 
        %The computation is done for $N_\text{t}=10$ time steps with a depth is $d=1$ \trung{stimmt das?}. 
        \TODO{Improve results and calculate errors}
        }
        \label{fig:Results:Heat:homoDirichlet}
    \end{subfigure}
        \hspace{0.3cm}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Dirichlet_f0_inhomogeneous.tex}
        \caption{Solution obtained for the first 20 time steps with $y(x,t^1)=0$, using inhomogeneous Dirichlet conditions ($y_{0} = 1 ,y_{N_\text{p}+1}=0$) and $d=5$.}
        \label{fig:Results:Heat:inhomoDirichlet}
    \end{subfigure}\\
    
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Mixed_f0_inhomogeneous_nq2.tex}
        \caption{Solution obtained for the first 100 time steps with $y(x,t^1)=0$, using mixed boundaries ($y_{0}=1$, $\nicefrac{\partial y_{N_\text{p}+1}}{\partial x} = 0$)   and 
        %no source $f(x,t)=0$ on $n=2$. The computation is done for $N_\text{t}=100$ time steps with a depth is 
        $d=7$.}
        \label{fig:Results:Heat:mixed_nq2}
    \end{subfigure}
        \hspace{0.3cm}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Mixed_f0_inhomogeneous_nq4.tex}
        \caption{
        \trung{Comparison of coarse and fine grid results for the first ?3? time steps
        with $y(x,t^1)=0$, using mixed boundaries ($y_{0}=1$, $\nicefrac{\partial y_{N_\text{p}+1}}{\partial x} = 0$)   and $d=7$.}
        %Solution of the Heat Equation from $y(x,0)~=~0$ with mixed boundaries ($y_{0}=1$, $\nicefrac{\partial y_{N_\text{p}+1}}{\partial x} = 0$) and no source $f(x,t)=0$ on $n=4$. The computation is done for $N_\text{t}=3$ time steps with a depth is $d=7$.\TODO{UPdate nq = 4 mixed heat}
        }
       \label{fig:Results:Heat:mixed_nq4}
    \end{subfigure}
    \caption{
    Comparisons of VQA-result (lines) and FD-results (symbols) for the transient heat conduction in combination with four different boundary conditions on grids with $N_\text{p}=4$ ($n=2$; dashed lines) and $N_\text{p}=16$ ($n=4$; straight lines) interior points using constant time steps $\Delta t \nu/\Delta x^2 = 0.2/(N_P+1)$.}
    \label{fig:Results:Heat}
\end{figure}
The predicted temperature distributions are depicted in \Fig{fig:Results:Heat}, where arrows indicate the temporal evolution from the initial to the final time step, and  \textsc{FD}-results are again illustrated by open squares (fine grid) and closed circles (coarse grid). Mind that a larger scatter of depth $d$, cf. \Fig{fig:VQA_Ansatz}, is seen for the employed ansatz $U(\lamb_c)$  
which is motivated by the complexity of the initial solution as explained below. %\trung{how can one explain this?}.
%\pover{As far I know is the kind of ansatz group (universal layer ansätze) we employ suitable for the expression for non-smooth solutions \cite{Sarma2023} -  I would expect that a lower depth is sufficient for later time steps. Needs to be checked ... }

\Fig{fig:Results:Heat:homoDirichlet} shows the results obtained for the 
homogeneous Dirichlet problem over the first \trung{10 -- CHECK: To be continued until steady state!} time steps. \trung{Results for the two grids are very similar, hence we mostly confine the discussion to coarse grid results for the sake of brevity}. The initial solution was assigned to a $f(x, t^1)=1$ in the interior, which yields negative heat fluxes at the boundaries in combination with imposed homogeneous Dirichlet boundaries. The figure indicates an excellent agreement between the VQA-results and the FD-results. This also applies to the results obtained for the inhomogeneous Dirichlet problem depicted in  \Fig{fig:Results:Heat:inhomoDirichlet}, where the initial solution refers to  $f(x, t^1)=0$ in the interior domain, and a fairly constant heat flux from the left to the right is predicted at the twentieth time step. An interesting detail refers to the increased depth $d$ of the ansatz circuit $U(\lamb_c)$, cf. \Fig{fig:VQA_Ansatz}. The increase is explained by the different initial conditions and the related steep solution in the initial phase that requires a deeper ansatz circuit, even when using the fairly rich SO4 approach
 for $\tilde U(\lamb_i)$. On the other hand, deeper circuits are afflicted with more parameters to be optimized, and optimization effort could be reduced for lowered depth circuits as the solution advances to the simpler steady state.
%\trung{...explanation ...}.

%The in-/homogenous Dirichlet problem is solved on the coarse discretization using $N_\text{p}=4$ interior points and $N_\text{t} = 20,40$ discrete times, respectively. The results are visualized in the \Fig{fig:Results:Heat:homoDirichlet}- \subref{fig:Results:Heat:inhomoDirichlet}. For the homogeneous case of \Fig{fig:Results:Heat:homoDirichlet}, the initial conditions at $t^0$ are set to constant one. The temporal evolution in this Figure shows the decay of the initial temperature, due to the lower temperature at isothermal boundaries which leads to negative heat flux at the boundaries. On the other hand, the inhomogeneous Dirichlet scenario develops from the initial condition $y(x,t^0) = 0$, as given in \Fig{fig:Results:Heat:inhomoDirichlet}. On the left boundary, heat is pumped into the domain while the right boundary recovers a negative heat flux until linear equilibrium. 

Results obtained for a mixed Dirichlet/Neumann problem are outlined in  \Fig{fig:Results:Heat:mixed_nq2} and \Fig{fig:Results:Heat:mixed_nq4}. The initial temperature distribution is assigned to $y(x,t^1)=0$ in the interior as well as the right side Neumann boundary. The final solution should agree with the left side Dirichlet value $y(0,t)=1$ in the whole domain. For the coarse grid $N_\text{t} = 100$ time steps are displayed in \Fig{fig:Results:Heat:mixed_nq2}. They indicate a remarkable visual agreement between the VQA-results and the FD-results over the entire simulation period. In line with the FD-results, the VQA-results unveil that the temperature on the right increases for the adiabatic condition until the global heat exchange finally vanishes. 
%
\trung{The left figure compares the evolution of the solution for the coarse and the fine mesh for the initial $N_\text{t} = 3$ time steps. Results indicate that the predictive accuracy is similar on both grids.}



%In all experiments, the \textsc{VQA} predictions agree remarkably well with the classical \textsc{FD} benchmark. 
For the sake of clarity, the time evolution of the $\varepsilon_{l_2}$ measure is presented using a log-log visualization in \Fig{fig:Results:Heat:Errors}. For the two Dirichlet cases, the maximum error occurs during the initial time steps and decays as the solution advances in time until approximately $t=0.1$s (5 time steps). Subsequently, the measure remains at a low level ($\varepsilon_{l_2} \approx 10^{-8}$). 
%
 For the mixed Dirichlet/Neumann case, an increase of $\varepsilon_{l_2}$ is seen at $t>0.3$s. Despite the transport of error in time, the implicit numerical scheme stabilizes and ensures no error amplification. %Although the error is transported in this time-marching approach it
 During the final period of time, the error oscillates around a similar magnitude as for the steady heat conduction, cf. Sec. \ref{sec:Application:Poisson}. 
 %The non-adaptive time-stepping scheme leads to small changes in cost functions between consecutive time steps. This permits to restart of the optimization with the previous control parameters which saves computational effort. 


\begin{figure}[htbp]
\centering    
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Errors_nq2.tex}
        \caption{Evolution for coarse-grid results displayed in \Fig{fig:Results:Heat:homoDirichlet}-\subref{fig:Results:Heat:mixed_nq2}.} 
        \label{fig:Results:Heat:Error:nq2}
    \end{subfigure} 
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Errors_Mixed_f0_inhomogeneous_nq4.tex}
        \vspace{-0.42cm}
        \caption{\trung{Comparison of fine- and coarse-grid results}, cf. \Fig{fig:Results:Heat:mixed_nq4}. \TODO{Update nq = 4 mixed heat}}
    \label{fig:Results:Heat:Errors:mixed_nq4}
    \end{subfigure}
    \caption{Temporal evolution of the deviation measure ${\varepsilon^l_{\text{l}_2}}$ for the results displayed in \Fig{fig:Results:Heat}.}
    \label{fig:Results:Heat:Errors}
\end{figure}

\Tab{tab:Results:Heat:Errors}, lists the time averaged
$\Bar{\varepsilon}_{\text{l}_2}$ and the corresponding trace distance measure $\Bar{\varepsilon}_{\text{tr}}$ averaged 
%\sbengoechea{why not the maximum} \TODO{Decide which is more beneficial}. 
As indicated by \Fig{fig:Results:Heat:Error:nq2}, the 
maximum values basically agree with the results of the steady heat conduction case, cf.  \Tab{tab:Results:Poisson:Errors}. However, since the temporal solution changes are small and retarded by the small time steps, both averaged deviations are smaller for the transient than for the steady case due to the favorable restart influences of the time-marching procedure on the optimizer.    

%\pover{Maximum error is of the same magnitude as the steady cases. } Comparing the trace distance in \Tab{tab:Results:Heat:Errors} with the values given in \Tab{tab:Results:Poisson:Errors} one determines smaller values regarding the average as well as the maximum computing transient solutions. This reasons in the fact that the time evolution approach acts like a relaxation in time. Despite the number of control parameters needed to model the mixed boundary setting on the coarse discretization for the $100$ time steps, the exploit approach maintains the same magnitude in trace distance. 
%\trung{The decreasing time derivative acts to catalyze the convergence quality of the \textsc{VQA}. Analyzing the last column of \Tab{tab:Results:Heat:Errors}, the number of ansatz parameters heavily varies between the scenarios. Neglecting the resulting non-shallow quantum circuits, the chosen SO4 ansatz recovers a large bandwidth of ansatz functions. The expressibility is satisfied.}


\begin{table}[htbp]
   \centering
   \caption{Time-averaged deviation measures $\Bar{\varepsilon}_{\text{l}_2}$ and $\Bar{\varepsilon}_{\text{tr}}$ measures for the results depicted in \Fig{fig:Results:Heat}.
   The degrees of freedom are  indicated by the number of control variables $c$.}
    \label{tab:Results:Heat:Errors}
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
Boundary Setting & \multicolumn{2}{c}{2-Norm $\Bar{\varepsilon}_{\text{l}_2}$}  & \multicolumn{2}{c}{Trace distance $\Bar{\varepsilon}_{\text{tr}}$}&\multicolumn{2}{c}{DOF $c$} \\ 
\midrule
\multicolumn{1}{r}{interior points}&\multicolumn{1}{l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$  
\\
\midrule
Homog. Dirichlet  & \multicolumn{1}{c}{\pover{$1.03 \times 10^{-8}$}}&\multicolumn{1}{c|}{-}&\multicolumn{1}{c}{\pover{$7.76 \times 10^{-9}$ }
}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{$3$}&-\\
Inhomog. Dirichlet & \multicolumn{1}{c}{$1.84\times 10^{-8}$
}&\multicolumn{1}{c|}{-}&\multicolumn{1}{c}{$2.77\times 10^{-7}$ }&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{$27$}&-\\
Mixed             & \multicolumn{1}{c}{$8.08 \times 10^{-8}$
}&\multicolumn{1}{c|}{\pover{$3.01 \times 10^{-3}
$}}&\multicolumn{1}{c}{$2.1 \times 10^{-8}$}&\multicolumn{1}{c}{\pover{$8.25 \times 10^{-3}$}}&\multicolumn{1}{|c}{$39$}&$60$\\
    \bottomrule
    \end{tabular}
\end{table}

%\subsection{The Wave Equation}
%\label{sec:Application:Wave}
%Hier einfach auf das framework oben beziehen und knapp skizzeiren 
%obven bleibt alles wie es sit.
% Do similar to : https://people.maths.ox.ac.uk/trefethen/pdectb/wave1d2.pdf
%\begin{itemize}
%    \item 1 . dirac as initial U and 2 hills neumann homo
%    \item  2.  dirac as initial U and 2 hills dirichlet homo
%\end{itemize}
%initial conditions an $e^{-x^2}$
%Additional source terms in the wave eq open the possibilites to model other hyperbolic pdes like Klein Gordon and Sine Gordon equations 


==> Container/C_Feb27/Sections/ComputationalStrategy.tex <==
%###########################################
%       Computational Model
%###########################################
\section{Variational Quantum Algorithm} \label{sec:Strategy}

As outlined above, a quantum register of length $n =\log_2\left(N_\text{p}\right)$ qubits is required to evaluate the objective function on a \textsc{QC}, cf. \Eq{eq:discretization_register}. Each qubit possesses two distinguishable computational states $\ket{0}$ and $\ket{1}$, which form an orthonormal basis of a complex Hilbert space and are frequently identified with basis vectors $\ket{0} = \left(1,0\right)^\intercal$ and $\ket{1}= \left(0,1\right)^\intercal$ \cite{Nielsen2010}.
The $n$ qubit register spans a Hilbert space whose basis is formed by tensor products of the computational basis states of individual qubits, e.g., $\eb_{i=0} = \ket{0}^{\otimes n}=\ket{0}\otimes\ket{0}\otimes~\hdots~\otimes~\ket{0} $, where ${\otimes n}$ indicates an n-fold tensor product. Thus, the $i$-th element of the orthonormal basis can be expressed via the binary representation $\text{bin}(i)$ as $\ket{\text{bin}(i)} = \eb_i$, following the \textit{little-endian} convention where the least-significant qubit corresponds to the right-most register position ($q_1$) and the most-significant qubit corresponds to the left-most register position ($q_n$), i.e., $\ket{q_n~q_{n-1}~\hdots~q_1}$. Furthermore, the least-significant qubit ($q_1$) is drawn as the uppermost qubit in the network figures and the lowermost qubit ($q_n$) indicates the most significant. This encoding enables the representation of the discrete vector $\ub$ by the amplitudes of the quantum register, viz.  $\ub = \sum\limits_{k=1}^{\text{N}_p} u_k \eb_{k-1} =  \sum\limits_{k=1}^{\text{N}_p}u_k \ket{\text{bin}\left(k-1\right)}= \ket{\ub}$, where the offset of the indices results from the technicality that the basis vectors $\eb_k$ start at $k=0$ but the interior unknowns $u_k$  begin with $k=1$. Mind that, though complex $u_k$ are generally allowed, we assume real solutions of \Eq{eq:Generic_PDE-TR}, hence $u_k^* =  u_k$, and that the time index is mostly suppressed in this section to improve the readability. 

%###########################################
%       Variational Quantum Algorithm
\subsection{Variational Quantum Algorithm} \label{sec:VQA}
The \textsc{VQA} methodology aims to minimize an objective function $J^{l}$ given in \Eq{eq:Discrete_Opt_BC}, by optimizing the control parameters $\upb^{l}= (\lambda_0^{l}, \lamb_c^{l})^\intercal$ for every time step $l$. The hybrid framework utilizes both classical and quantum hardware, as displayed in \Fig{fig:optimizer}. 
%
\begin{figure}[htbp]
    \centering
    \input{Figures/communication_opt}
    \caption{Sketch of the hybrid  \textsc{VQA} optimization (time dependencies {in the optimization step} are suppressed for the sake of clarity). 
    }
    \label{fig:optimizer}
\end{figure}
%
The function $J^l$ is evaluated on the quantum device, as illustrated by the shaded box in Fig. \ref{fig:optimizer}, whereas the optimization process runs on the classical hardware that controls the process and iteratively adjusts the control $\upb$. For a particular set of ansatz parameters $\lamb_c$, the objective function is evaluated from dedicated, individual so-called Quantum-Nonlinear-Processing-Units (\textsc{QNPU}) for each group of terms in \Eq{eq:Discrete_Opt_BC}, i.e., for $j_{L_k},{j_{DN}, j_{N}}, j_{P_k}, j_{S_k}$, cf. Sec. \ref{sec:Compilation}. An update $\Delta\upb$ is determined by the optimizer as outlined in Sec. \ref{sec:Derivative1} before a new iteration starts.

Figure \ref{fig:VQA_QNPU} describes two {equivalent} options of the general layout of circuits on the quantum device. Grossly speaking, both options consist of a measuring  (aka. ancilla) qubit in the upper ''wire''  and calculation qubits in the lower ''wires''. In general, the qubits are initialized to the base state $\ket{0}$.
%{In general, the qubit register is initialized to the base state $\ket{0}^{\otimes n}$.$=\ket{0}\otimes\ket{0}\otimes~\hdots~\otimes~\ket{0}$, where ${\otimes n}$ indicates an n-fold tensor product (cf. \Fig{fig:VQA_QNPU}).}
The calculation qubits are then introduced to an ansatz circuit called $U$, highlighted in grey in \Fig{fig:VQA_QNPU}. The ansatz $U$ can be denoted by a $N_\text{p} \times N_\text{p}$ matrix composed by an embedded combination of two-qubit units, i.e., fundamental gates $\tilde U (4 \times 4)$, as illustrated in \Fig{fig:VQA_Ansatz} for six qubits. The particular combination employed in this research refers to a scalable depth bricklayer topology and shares some similarities with machine learning topologies. The benefit of the bricklayer topology over alternative topologies has been communicated in \cite{Nakaji2021}.

\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \input{Figures/QNPU.tex}
        \caption{Sketch of two \textsc{VQ} circuits composed of the ansatz $U(\lamb_c)$, the $T_t$ or $\tilde T_t (\tilde T^\dagger_{t})$ transformation, a specific \textsc{QNPU}, and a measurement qubit (ancilla qubit) for indirect measurements. $H$ indicates a Hadamard gate, \textsc{CP} denotes a control port, \textsc{IP} marks the input port \& \textsc{OP} the output port, and $\langle \sigma_z \rangle$ provides the expectation value of the measurement operation, cf. \cite{Lubasch2020}. 
        }
        \label{fig:VQA_QNPU}
    \end{subfigure}
    \begin{subfigure}[t]{1.0\textwidth}
         \vspace*{2ex}
        \centering
        \input{Figures/Ansatz.tex}
        \caption{Example of an ansatz circuit $U(\lamb_c)$  composed from  $a=10$ fundamental gates $\Tilde{U}(\lamb_i)$ featuring a bricklayer topology,  parameterized by $\lamb_c = (\lamb_1, \lamb_2,\hdots, \lamb_a)^\intercal$ parameters to encode a test function $\ket{\ub}$ on $n = 6$ qubits, cf. \cite{Lubasch2020}. }
        \label{fig:VQA_Ansatz}
    \end{subfigure}\\
    \begin{subfigure}[b]{1.0\textwidth}
     \vspace*{2ex}
        \centering
        \input{Figures/SO4_ansatz.tex}
        \caption{Two qubit \textsc{\it SO4} ansatz $\Tilde{U}(\lamb_i)$ 
        to create an optimal variational state \cite{Vatan2004} based on $\lamb_i = \left(\lambda_{i,1},\lambda_{i,2},\hdots,\lambda_{i,6}\right)^\intercal$ individual parameters. In the first layer ($d=1$) the ansatz has only three parameters in $\lamb_i$, the rotation gates corresponding to $\lambda_{i,4}$, $\lambda_{i,5}$, and $\lambda_{i,6}$ are identity gates.}
        \label{fig:quantum_ansatz_SO4}
    \end{subfigure}\\    
     %\vspace*{2ex}
     
    \caption{Illustration of the employed nested \textsc{VQA} circuits.}
    \label{fig:VQA}
\end{figure}
The employed fundamental gate is displayed in dark grey in Figs. \ref{fig:VQA_Ansatz}-\ref{fig:quantum_ansatz_SO4}. It has been suggested by Vatan and Williams \cite{Vatan2004} and is frequently labeled \textsc{\it SO4}. This gate operates in real and imaginary space, which is rather unusual for engineering applications that aim for real-valued results \cite{Sato2021,Leong2022}. Its application promises a richer ansatz function space that, in turn, supports the use of shallower depth $d$ in $U$.
%
As displayed in \Fig{fig:quantum_ansatz_SO4}, the fundamental gate consists of \textsc{R$_y$}, \textsc{R$_z$} and \textsc{CNOT} gates, where \textsc{R$_y$} and \textsc{R$_z$} are parameterized versions of classical Pauli $\sigma_y$ and $\sigma_z$ matrices \cite{Nielsen2010}, cf. App.~\ref{app:Fundamentals}, and the $(\dots)^\dagger$ symbol indicates the transposed of the complex conjugate. 

Turning back to \Fig{fig:VQA_QNPU}, the result of the ansatz circuit $U$ is the parameterized state $\ket{\ub}$. 
Subsequently, a particular transformation matrix $T_t$ or $\tilde T_t$ is introduced
in case of boundary contributions $j_{DN}$ and $j_{N}$ before the data enters a  boundary-specific \textsc{QNPU}. 
The transformation essentially modifies the order of qubits in the register $\ket{\ub}$ where necessary. 
%%
As will be shown in Sec.~\ref{sec:compilation:complexity}, two implementations are conceivable, cf. \Fig{fig:VQA_QNPU}, by either using highly complex multi-controlled gates, or by employing additional ''carry qubits''. 

The prepared state ($T_t \ket{\ub}$ or $\tilde T_t \ket{\ub}$) inputs to the main \textsc{QNPU} gate, indicated in light grey in \Fig{fig:VQA_QNPU}, through the input port (\textsc{IP}) and outputs the specific objective function contributions for a group of terms ($j_{L_k},j_{DN}, j_{N}, j_{P_k}, j_{S_k}$) through and output port (\textsc{OP}). 
%
%The main gate, the \textsc{QNPU} unit indicated in light grey in \Fig{fig:VQA_QNPU}, is fed with a prepared state through an input port (IP) and outputs (OP) the specific objective function contributions for a group of terms ($j_{L_k}, j_{P_k}$, etc.)
%
Finally, the register is reversed to its initial order after applying the boundary-specific \textsc{QNPU}. To this end, the  Hadamard test method inherently reverses the  gates in the upper variant of \Fig{fig:VQA_QNPU}. In contrast, the implementation example at the bottom of \Fig{fig:VQA_QNPU} requires the explicit application of $\tilde T^\dagger_{t}$. 
%
Note that for periodic conditions, where neither $j_{DN}$ nor $j_{N}$ contributions occur, no transformation is needed and $T_t$ simply degenerates to the identity matrix $I$ in line with the upper part of \Fig{fig:VQA_QNPU}. 
%%%%%%%%%%
%
The use of the Hadamard test \cite{Endo2020} is motivated by previous studies \cite{Guseynov2023}, which indicated quantum advantage with this approach. Here, rather than assessing the individual contributions at each grid point $k$ \cite{Endo2020},  
the integral over all interior points is directly compiled, for example $\sum_k j_{L_k}$, and measured statistically on the upper ''wire'' by the expectation value denoted by $\langle \sigma_z \rangle$ \cite{Nielsen2010}. This is indicated by the upper ''wire'' of \Fig{fig:VQA_QNPU} that connects to the calculation ''wires'' through a control port (\textsc{CP}). 

Before we discuss the individual \textsc{QNPU}s in Sec.~\ref{sec:Compilation}, the measurement strategy implemented here should be described for the sake of completeness. We rely on the density (or autocorrelation) matrix $\rho_\text{ancilla}$ of the ancilla qubit to approximate the expectation $\langle \sigma_z \rangle$ at the measurement gauge in \Fig{fig:VQA_QNPU}. To eliminate stochastic influences, evaluating \textsc{QC}-calculated results is usually based on evaluating sufficiently large samples. However, if the \textsc{QC} is only emulated, as in the current study, the procedure can be simplified using the trace-out method \cite{Nielsen2010}. 
%
First, the whole system state $\ket{\psib}$ (ancilla and calculation qubits) is computed by a state-vector simulation. As we are only interested in the information contained in the ancilla portion of the state $\ket{\psib}$, the remainder is traced out, and the density operator $\rho_\text{ancilla}= \text{Tr}_\text{QNPU}\{ \ket{\psib}\bra{\psib}\}$ of the ancilla remains. The state-vector simulation thus yields the same result as the measurement of the ancilla performed on real hardware, without noise and sampling errors \cite{Nielsen2010}. 

%###########################################
%       Compilation of the Quantum-Nonlinear-Processing-Units
\section{Quantum-Nonlinear-Processing-Units}
\label{sec:Compilation}
For the introduction of our library of {Quantum-Nonlinear-Processing-Units} (\textsc{QNPU}s), we use a complex number notation. All \textsc{QNPU}s are highlighted in light grey in the respective figures, which links them to the \textsc{VQ} circuits depicted in \Fig{fig:VQA_QNPU}. They are adjustable to an arbitrary equidistant one-dimensional discretization and have been designed to keep the gate sequence shallow. Quantum gates are often associated with matrices or matrix operations. Therefore, the interested reader is referred to App.~\ref{app:MatrixGateConversion} for a brief introduction to converting gate sequences into matrices. 

%###########################################
%       Laplace
\subsection{Periodic Laplace operator} \label{sec:Compilation:Laplace}

The Laplacian is given by the {\textsc{FD}} stencil in \Eq{eq:derivatives_space} and partly resembles the classical bit shift operator \cite{Nielsen2010,Vedral1996} due to shifted products, e.g. $u_k^{l*} u_{k+1}^l$, $u_k^{l*} u_{k-1}^l$. 
In contrast to other approaches \cite{Sato2021,Liu2021} the \textsc{QNPU} circuit employed herein is based on the adder circuit with a polynomial scaling of the gate complexity, cf. Sec. \ref{sec:compilation:complexity}. 
%
Using $n=2$ qubits,  a half-adder circuit can be used, which consists of one \textsc{CNOT} and an additional Toffoli gate. For $n > 2$, additional ($n-2$) ''carry qubits'' (auxiliary qubits) are required, which results in a full-adder 
circuit, cf. \cite{Parhami2010, Draper2000}. 
%
Assuming a periodic state, it can be shown \cite{Lubasch2020} that the general structure of the discrete Laplace operator is represented by  
\begin{align}
\label{eq:Laplace}
    \sum\limits_{k=1}^{N_\text{p}}u_k \ket{\text{bin}\left(k-1\right)} \to  \sum \limits_{k=1}^{N_\text{p}} u_{k+1}  \ket{\text{bin}\left(k-1\right)} \, , \qquad \text{with} \qquad {1= \sum_{k=1}^{N_\text{p}} u_k^* u_k}.
\end{align}

Mind that an adder \textsc{QNPU} to compute a periodic Laplace operator has previously been reported by Lubasch et al. \cite{Lubasch2020}.  \Fig{fig:Laplace_compiled} depicts an example of the employed Laplace QNPU circuit 
for $n=6$ qubits and $n-2 = 4$ carry bits. The circuit involves $n-2=4$ \textsc{CNOT} gates and $2n-2=10$ Toffoli gates. 

\begin{figure}[htbp]
    \centering
    \input{Figures/Adder.tex}
    \caption{Exemplary quantum circuit of the discrete Laplacian in the Hadamard test configuration. The example refers to $n=6$ qubits and  $n-2=4$ carry bits. It requires $n-2=4$ \textsc{CNOT} and $2n-2=10$ Toffoli gates. For $n=2$ qubits, this circuit is exactly implementing a half-adder, cf. \cite{Lubasch2020}.
    }
    \label{fig:Laplace_compiled}
\end{figure}

%###########################################
%       Potential
\subsection{External Contributions (potential and source terms)} \label{sec:Compilation:Potential}

The computation of external contributions follows from two subsequent steps.
First, the representation of the discrete linear source  $\tilde f_k^l$ and potential terms $p_k^l$  are assembled. This enables computing their contributions to the objective function {($j_S$,$j_P$)} in a second step. 

For simple, analytically described terms, e.g., $exp(x)$ or $sin(x)$,  Lubasch et al.  \cite{Lubasch2020} introduced corresponding gate sequences that allow such functions to be represented on a \textsc{QC}. Other suggestions intensively deploy Matrix-Product-State (\textsc{MPS}) techniques, \cite{Oseledets2012,GonzalezConde2023,Oseledets2010}. 
In our case, however, we first solve a prior optimization problem to represent arbitrary external contributions by quantum gates, taking the ansatz $U(\lamb)$ into account, viz. 
\begin{align}
     \bar{\lamb}_c =  \min\limits_{\lamb_c} \big(1 -\lambda_0\bra{\ub(\lamb_c)} \ket{\gb}\big) \text{ with } \frac{1}{\lambda_0^2}=\sum \limits_1^{N_\text{p}} g_k^{l*} g_k^l \, . 
    \label{eq:OptAnsatz}
\end{align}

In \Eq{eq:OptAnsatz} $\gb = \Tilde{\fb}$ or $\gb = \pb$ for the source and the potential term, respectively. The benefit of this approach is that it re-uses existing implementations and also supports keeping the depth of the resulting circuits shallow. 
The optimal parameters $\bar{\lamb}_c$ determined in this way result in the required gates $U(\bar{\lamb}_c) = P$ and $U(\bar{\lamb}_c) =  {F}$ to be used inside the \textsc{QNPU}s that compute the potential and the source term contributions to $J$ in \eqref{eq:Discrete_Opt_BC}.

The contribution of the potential term $p(x_k, t^l)$ to $J$ follows from $\sum\limits_{k=1}^{\text{N}_p} \left[ \lambda_0^2 u_k^*p_k u_k \right]^l $. The corresponding \textsc{QNPU} circuit is assembled by Toffoli gates according to \Fig{fig:QNPU_Potential}. Since the product $u_k^* p_k u_k$ is non-unitary, additional $n$ ancilla qubits occur in the circuit \cite{Sarma2023}. 
%
Similarly, the representation of $\ket{\fb} = U(\bar{\lamb}_c)\ket{0}$ is implemented into the source term \textsc{QNPU} (light grey) given in \Fig{fig:overlapp}. Note that thanks to the versatility of the \textsc{\it SO4} ansatz, the minimum depth $d=1$ is usually sufficient to reconstruct $\fb$ and $\pb$. 
Instead of the uncontrolled ansatz $U(\lamb)$ displayed in Fig. \ref{fig:VQA_QNPU}, the linearity of the source term requires that $U(\lamb)$  is also controlled. 

\begin{figure}[htpb]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Potential.tex}
        \caption{Exemplary quantum circuit for a discrete potential function $\pb=( p_1, p_2,p_3, \dots p_{N_\text{p}})^\intercal$ represented by the gate ''$P$''. }
        \label{fig:QNPU_Potential}
    \end{subfigure}
    \hspace{0.2cm}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Overlapp.tex}
        \caption{Evaluation of external source term $f$  by $\bra{\ub}\ket{\fb}$, with $T_t = I$.}
        \label{fig:overlapp}
    \end{subfigure}
    \caption{External contributions on the Hadamard test. The displayed example refers to $\text{N}_p=64$, $n=6$ qubits.}
    \label{fig:externals}
\end{figure}

%###########################################
%       Boundary Conditions
\subsection{Boundary Conditions}\label{sec:Compilation:BC}
With the intention of developing a quantum equivalent of the ghost point approach discussed in Sec. \ref{sec:Discretization}, we first elaborate on a matrix-based representation to facilitate the understanding of the quantum implementation. Subsequently, the novel \textsc{QNPU}s for the boundary treatment in variational quantum simulations are introduced. 
\medskip

The implementation of boundary conditions is based on the correction of the periodic contributions in the derivative matrix. To outline the transfer of \Eq{eq:Discrete_Opt_BC} into quantum-inspired or true quantum computations, we restrict ourselves to Dirichlet conditions imposed for a simple Laplace equation $-\nu \Delta u=0$ in the 2-qubit case. 
%
Next, let's recover a slightly reduced version of \Eq{eq:Discrete_Opt_BC} for this problem in a matrix-based approach, assuming $\ub \in \mathbb{C}^{N_p}$ and $A \in \mathbb{R}^{N_p \text{x} N_p}$. For the sake of clarity, we also define $(\nu \lambda_0^2/\Delta x) = 1$, viz. 
\begin{align}
\begin{split}
    \ub^{\dagger} \cdot A \cdot \ub &= \begin{pmatrix} u_{1}^* & u_{2}^* & u_{3}^* & u_{4}^* \end{pmatrix} \cdot \begin{pmatrix} 2 & -1 & 0 & -1 \\ -1 & 2 & -1 & 0 \\ 0 & -1 & 2 & -1 \\ -1 & 0 & -1 & 2 \end{pmatrix} \cdot \begin{pmatrix} u_{1} \\ u_{2} \\ u_{3} \\ u_{4} \end{pmatrix} \\ 
    & = 2 u^{*}_1 u_1 - u_1^*u_2 - u_2^* u_1 + 2 u_2 u_2^* - u_2^*u_3 - u_3^*u_2 \\
    &\quad + 2 u_3 u_3^* - u_3^*u_4 - u_4^*u_{3} + 2 u_4^* u_4 - \underbrace{u_1^*u_4 - u_4^*u_1}_{\text{periodic boundary}}.
\end{split}
\label{eq:Expect_perio}
\end{align}

The sum on the right-hand side of \Eq{eq:Expect_perio} distinguishes between regular interior contributions and periodic boundary contributions. In line with \Eq{eq:Discrete_Opt_BC}, the periodic contributions of $-u_1^*u_4 - u_4^*u_1$ need to be eliminated by another term in the cost function, viz. $J = \sum\limits_{k=1}^4 j_{L_k} + j_{DN_1} + j_{DN_4}$. 
%Following the example of \Eq{eq:Expect_perio}, 
This is achieved by 
\begin{align}
\begin{split}
    J_{DN} = j_{DN_1} + j_{DN_4} = \ub^{\dagger} \cdot D \cdot \ub &= \begin{pmatrix} u_{1}^* & u_{2}^* & u_{3}^* & u_{4}^* \end{pmatrix} \cdot \begin{pmatrix}0 & 0 & 0 & 1 \\ 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 \end{pmatrix} \cdot \begin{pmatrix} u_{1} \\ u_{2} \\ u_{3} \\ u_{4} \end{pmatrix} \\ 
    & = \underbrace{u_1^*u_4 + u_4^*u_1}_{\text{boundary}}. 
\end{split}
\label{eq:Bound_J}
\end{align}

The matrix $D \in \mathbb{R}^{N_p \text{x} N_p}$ needs to be unitary for its representation by quantum gates. This distinguishes the quantum-inspired approaches from true \textsc{QC} methods. A \textsc{QC}-compatible representation of $D$ follows from a modification with the basis of its null space removing the zero eigenvalues and intuitively matching the boundary contributions of \Eq{eq:Bound_J}. Accordingly, the unitary matrix $C \in \mathbb{R}^{N_p \text{x} N_p}$ is  proposed as 
\begin{align}
\begin{split}
    J_{DN} = \ub^{\dagger} \cdot C \cdot \ub &= \begin{pmatrix} u_{1}^* & u_{2}^* & u_{3}^* & u_{4}^* \end{pmatrix} \cdot \begin{pmatrix}0 & 0 & 0 & 1 \\ 0 & 0 & -1 & 0 \\ 0 & 1 & 0 & 0 \\ 1 & 0 & 0 & 0 \end{pmatrix} \cdot \begin{pmatrix} u_{1} \\ u_{2} \\ u_{3} \\ u_{4} \end{pmatrix} \\ 
    & = \underbrace{ u_1^*u_4 -u_2^*u_3 + u_3^* u_2 + u_4^*u_1 }_{\text{if } \bm{u} \in \mathbb{R}^n}  = \underbrace{2u_1u_4}_{\text{boundary}} \, . 
\end{split}
\label{eq:Bound_J_unit}
\end{align}

The unitary matrix $C$ only inheres nonzero entries on the antidiagonal. The upper and lower corners must have the same sign to neutralize the periodic contributions of matrix $A$. The other terms need to change sign with respect to the main diagonal for these contributions to be canceled when the expectation value $\langle \sigma_z \rangle$ is measured. Note that for the summation of the interior antidiagonal elements, one obtains zero only if $\ub \in \mathbb{R}^n$. 

The remaining task is to design the circuits that implement the transformation described by the matrix $C$. To this end, the heuristic approach requires another decomposition, i.e., $C = T_t^{-1} \cdot B \cdot T_t$, where  $T_t$ relates to a permutation operator and $B$ to a boundary \textsc{QNPU}, which both directly translate into quantum gates, cf. \Fig{fig:matrix2gate}. 


%
%\begin{align}
%\label{eq:shift2}
%    \sum\limits_{k=1}^{N_\text{p}}u_k \ket{\text{bin}\left(k-1\right)} \to  \sum \limits_{k=1}^{N_\text{p}} u_{k-1}  \ket{\text{bin}\left(k-1\right)} \qquad \text{with} \qquad {1= \sum_{k=1}^{N_\text{p}} u_k^* u_k}.
%\end{align}
%
%

In general, deriving the gate sequence corresponding to a given matrix is neither trivial nor unique. 
The application of heuristic approaches leads to the gate-level implementation for two qubits outlined in \Fig{fig:matrix2gate:shift} and \Fig{fig:matrix2gate:dir}. 

\begin{figure}[htpb]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \begin{equation*}
        T_t = \begin{pmatrix}0 & 0 & 0 & 1 \\ 1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 & 1 & 0 \end{pmatrix}
        \end{equation*}
        \caption{Matrix representation of $T_t$.}
        \label{fig:matrix2gate:MatrixT}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \begin{equation*}
        B = \begin{pmatrix}0 & 1 & 0 & 0 \\ 1 & 0 & 0 & 0 \\ 0 & 0 & 0 & -1 \\ 0 & 0 & 1 & 0 \end{pmatrix}
        \end{equation*}
        \caption{Matrix representation of $B$.}
        \label{fig:matrix2gate:MatrixB}
    \end{subfigure}

    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Transformation_n2}
        \caption{Gate representation of $T_t$ \cite{Sato2021}.}
        \label{fig:matrix2gate:shift}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Dirichlet_n2}
        \caption{Gate representation of $B$.}
        \label{fig:matrix2gate:dir}
    \end{subfigure}
    \caption{Matrices and their corresponding circuits for 2-qubits.}
    \label{fig:matrix2gate}
\end{figure}

In contrast to the method of Sato et al. \cite{Sato2021} and the related studies of Leong et al. \cite{Leong2022}, the proposed boundary corrections are represented as unitary circuits and, therefore, as quantum gates. Further insight into the conversion between matrix and circuit representation is given in App.~\ref{app:MatrixGateConversion}. For the sake of completeness, the four qubit version of the circuits in \Fig{fig:matrix2gate:shift} and \Fig{fig:matrix2gate:dir} with the corresponding unitary matrix $C$ are also included in App.~\ref{app:BoundaryMatrixGate}. 

\begin{figure}[htbp]
    \centering
    \input{Figures/Transformation}
    \caption{Six qubit example of the permutation  operator $T_t$ represented by a sequence of multi-controlled Toffoli gates cf. \cite{Sato2021}.}
    \label{fig:Transformation}
\end{figure}

\bigskip

The extension to a $n$ qubit framework implies the multi-qubit implementation of the transformation $T_t$ with a sequence of $n-2$ multi-controlled \textsc{NOT} gates, cf. \Fig{fig:Transformation}. Similarly, the boundary corrections $j_{DN}$ and $j_{N}$ consist of $2n-1$ \textsc{CNOTS} and controlled-\textsc{Z} gates for an arbitrary number of qubits. Furthermore, one $n$ multi-qubit controlled-\textsc{Z} gate for both circuits and one $n$ multi-controlled \textsc{NOT} gate for $j_{DN}$ complete the circuits, as illustrated in \Fig{fig:QNPU_BC} for $n=6$ qubits. Both circuits shown in \Fig{fig:QNPU_BC_Dirichlet} and \Fig{fig:QNPU_BC_Neumann} use operations that only manipulate the dynamics at the boundaries. In the interior domain, the effect of the operator neutralizes for the expectation value $\langle \sigma_z \rangle$. 

\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{1.0\textwidth}
       \centering
        \input{Figures/Dirichlet.tex}
        \caption{Compiled \textsc{QNPU} for the implementation of  $j_{DN}$ used to realize both Dirichlet and Neumann conditions, cf. \Eq{eq:Discrete_Opt_BC}.}
        \label{fig:QNPU_BC_Dirichlet}
    \end{subfigure}\\
    \vspace*{2ex}
    
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \input{Figures/Neumann}
        \caption{Compiled \textsc{QNPU} for the implementation of  $j_{N}$ used to realize Neumann boundary conditions, cf. \Eq{eq:Discrete_Opt_BC}.}  
        \label{fig:QNPU_BC_Neumann}
    \end{subfigure}\\
    
    \caption{Illustration of the novel boundary correction \textsc{QNPU}s for $n=6$ qubits setup.}
    \label{fig:QNPU_BC}
\end{figure}
\medskip

The resulting circuits for $T_t$, $j_{DN}$, and $j_N$ in \Fig{fig:Transformation} and \Fig{fig:QNPU_BC} 
inhere sequences of multi-controlled gates, which substantially deteriorate the gate complexity. In this regard, the most efficient implementation depends on the available \textsc{QC} hardware and its support for multi-controlled gates. Alternatively, additional carry qubits can be used to obtain more shallow circuits. These carry qubits implement intermediate information associated with \textsc{AND} operations by a staggered series of Toffoli gates. This technique is illustrated in more detail in Sec. \ref{sec:compilation:complexity}.


%###########################################
%       Gate complexity
%\subsubsection{Gate Complexity} 
\section{Gate Complexity} 
\label{sec:compilation:complexity}
To scrutinize the scalability of the algorithm, the number of single- (\textsc{R$_z$,R$_y$,U},...) and two-qubit (\textsc{CNOT},...) gates per qubit are outlined in this section. For this purpose, multi-qubit gates are decomposed using known identities, which are available, for example, in \textsc{Qiskit} \cite{Qiskit}. The scaling of the number of gates involved in the \textsc{\it SO4} ansatz with respect to the number of qubits $n$ and the depth $d$ is reported in \Fig{fig:Results:SO4complex}.  It is observed that the number of gates scales linearly with $n$ and $d$, i.e., $\mathcal{O}(n \, d)$.

\begin{figure}[htbp]
    \begin{subfigure}[t]{0.49\textwidth}
       \centering
        \input{Figures/Complexity/C_Ansatz_SO4.tex}
        \caption{Complexity for the \textsc{\it SO4} ansatz.} 
        \label{fig:Results:SO4complex}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Complexity/C_QNPU.tex}
        \caption{Complexity for all \textsc{QNPU}s.} 
        \label{fig:Results:QNPUcomplex}
    \end{subfigure}
    \caption{Gate complexity of the employed \textsc{QNPU}s and ansatz gate compilations.}
    \label{fig:compilation:GateComplexity}
\end{figure}

The graphs displayed in \Fig{fig:Results:QNPUcomplex} illustrate the polynomial relation between the number of gates and the number of qubits for the adder ($j_{L}$), the source ($j_{S}$), the potential ($j_{P}$) and the boundary circuits -- the latter using either multi-controlled gates ($j_{DN}, j_{N}$) described in Sec. \ref{sec:Compilation:BC} or the corresponding modifications described below ($\tilde j_{DN}, \tilde j_{N}$). 
 
Most \textsc{QNPU}s in \Fig{fig:Results:QNPUcomplex} depict a favorable complexity. The linear complexity of the adder circuit, $\mathcal{O}( n)$, is due to the very local reach of the \textsc{FD} stencil for approximating the second derivative. In this case, the resulting circuit conserves the local property. An analysis of the source and potential \textsc{QNPU}s also reveals a linear scaling of  $\mathcal{O}( n)$, respectively, which underlines the importance of an efficient state initialization for arbitrary generic functions \cite{Chen2021,Kyriienko2021,Creevey2023,Melnikov2023,Araujo2021}, cf. Sec. \ref{sec:Compilation:Potential}. The similarity to the scaling behavior examined for the \textsc{\it SO4} ansatz is obvious and indicates the strong influence of the prior optimization of $U(\lamb_c)$ to determine $\Tilde{\fb}$ or $\pb$, cf. \Eq{eq:OptAnsatz}. The related overhead in the number of gates with respect to the ansatz is due to the control operation of the ansatz in both \textsc{QNPU}s ($j_S$,$j_P$) and the additional \textsc{CNOT} gates following the $P$ gate for the potential \textsc{QNPU}, see \Fig{fig:QNPU_Potential}.  Note that for the values given in \Fig{fig:compilation:GateComplexity}, the depth of the ansatz for $j_{P}$ and $j_{S}$ is assigned to $d=1$. 

The boundary \textsc{QNPU}s ($j_{DN}, j_{N}$), however, scale polynomially, on the maximum order of $\mathcal{O}(n^{5})$. This was also observed by other researchers when using multi-controlled quantum gates, for example, \cite{Sato2021,Leong2022,Leong2023}. The reason for that is the non-locality of the implementation and the multi-controlled feature, which yields interaction with more than just the nearest neighbor qubits. 
%
In practical applications, e.g., an implementation on \textsc{NISQ} hardware, there is a demand for circuit efficiency. To obtain more shallow circuits, additional carry qubits are used. As mentioned above, they implement intermediate information associated with \textsc{AND} operations by a staggered series of Toffoli gates. The technique is illustrated for a multi-controlled-\textsc{G} Gate (\textsc{MCG}) in \Fig{fig:multicontrol}.

The example consists of $n=6$ qubits and requires $n-2=4$ carry qubits to transform the deep multi-controlled gate on the left of \Fig{fig:multicontrol} into $n+2$ Toffoli- and one controlled G-gate on the right of \Fig{fig:multicontrol}. Mind that after applying \textsc{G}, all carry bits need to be reversed to their initial state, i.e., $\ket{0}$. 

\begin{figure}[htbp]
    \centering
    \input{Figures/MultiControl}
    \caption{Equivalent networks using a deep qubit-saving implementation (left) and a shallow circuit depth approach (right) to realize a multi-controlled gate \textsc{G}.}
    \label{fig:multicontrol}
\end{figure}

Applying this concept to the transformation circuit $T_t$ outlined in \Fig{fig:Transformation} allows to derive a shallower alternative $\Tilde{T}_t$ resulting in a permutation operator, cf. \Fig{fig:new-Tt:up}. 
This figure also provides the corresponding circuit for the inverted transformation  $\Tilde{T}^\dagger_{t}$  in \Fig{fig:new-Tt:down}. The latter is required for measuring the expectation value $\langle \sigma_z \rangle = \bra{0} U^\dagger T_t^\dagger \; [\text{QNPU}] \; T_t U \ket{0}$ as illustrated by the Hadamard-test based  structure in \Fig{fig:VQA_QNPU}. Both $\tilde T_t$ and $\tilde T^\dagger_{t}$ are controlled by an ancilla qubit,  which follows the same strategy as depicted for the \textsc{QNPU} assembly in \Fig{fig:VQA_QNPU}. 

\begin{figure}
\begin{subfigure}[t]{0.4\textwidth}
      \include{Figures/ShiftUP}
      \caption{Forward transformation $\tilde T_t$.}
      \label{fig:new-Tt:up}
\end{subfigure}
\hspace{3cm}
\begin{subfigure}[t]{0.4\textwidth}
      \include{Figures/ShiftDOWN}
      \caption{Backward (adjoint) transformation $\tilde T^\dagger_{t}$.}
      \label{fig:new-Tt:down}
\end{subfigure}
\caption{Alternative implementations of the forward ($T_t$, $\tilde T_t$) and backward ($T_{t}^\dagger$, $\tilde T^\dagger_{t}$) transformation introduced in \Fig{fig:Transformation}.}
\label{fig:new-Tt}
\end{figure}

Introducing the above-mentioned shallow circuit alternatives to the $j_{DN}$ circuit is straightforward and allows replacing the multi-controlled-\textsc{Z} gate by the usage of $n-2$ carry qubits. As already outlined at the end of Sec. \ref{sec:Discretization}, the \textsc{QNPU} related to the Neumann condition ($j_{N}$) shown in \Fig{fig:QNPU_BC_Neumann} can be cast in terms of the potential $p$-\textsc{QNPU}, depicted in \Fig{fig:QNPU_Potential}. A consistent application of shallow circuit (\textsc{MCG}) strategies yields the complexity graphs for $\tilde j_N$, $\tilde j_{DN}$ marked by symbols in \Fig{fig:compilation:GateComplexity}. Advantageous differences to the initial implementation
$j_N, j_{DN}$, given by lines in \Fig{fig:compilation:GateComplexity}, are clearly visible but do, of course, come at the expense of additional $(n-2)$ carry qubits. The graph displays an efficient scaling below $\mathcal{O}(n^2)$. In terms of grid-point $N_\text{p}$ behavior, the complexity is of \textit{polylog} scaling. We again emphasize that the chosen reduction in complexity, i.e., the number of carry qubits used, depends on the capabilities of the \textsc{QC} hardware. 

%###########################################
%      Optimization Strategy
\section{Optimization Strategy} \label{sec:Optimization}

A common denominator of all \textsc{VQA}s is the efficiency of the optimization process. As stated in \cite{Bittel2021}, this is non-trivial since the problem covered by \textsc{VQA} is theoretically \textsc{NP}-hard, meaning that the optimization is often characterized as non-convex and features multiple local minima and/or vanishing derivatives \cite{Leong2022,Sarma2023,Wiersema2023}. 
To update the controls ($\lambda_0, \lamb_c$) along the route outlined in \Fig{fig:optimizer}, we apply the sequence of a zero- and a first-order method. The combination aims at a larger sample size to address non-convex functionss and higher accuracy in the vicinity of the minima and might be replaced by a more sophisticated strategy. The optimization starts with the zero-order approach and employs an evolutionary \textit{Particle-Swarm Optimization} (\textsc{PSO}) algorithm \cite{Kennedy1995} using $\mathfrak{p}$ particles. The \textsc{PSO} step typically involves $\mathcal{O}(1000)$ iterations, where around $\mathfrak{p} \approx 100\,n$ particles are employed. The best candidate initializes the control $\upb$ for the subsequent first-order classical \textit{Gradient Descent} (\textsc{GD}) method. The required derivative of the objective function with respect to the controls $\nabla_{\upb} J(\upb_{i})$ is obtained from the \textsc{QC} and follows the expressions given below, cf. \Eq{eq:quantum_derivative_0} and \Eq{eq:quantum_derivative_control}. Convergence is assessed from the absolute change \textsf{ch} of the derivative
\begin{align}
   \textsf{ch}( \nabla J^l_i) = | \nabla J^l_i- \nabla J^l_{i-1}|_{2} % |J^l_i - J^l_{i-1}|_{2} 
   \quad \le 10^{-m}  \, , 
   \label{alg:convergence}
\end{align}
where $m\in[3,7]$ depending on the number of employed qubits, cf. Sec. \ref{sec:Applications}.  
The solution is advanced in time as described in \Fig{fig:discretization_encoding} and the algorithm \ref{alg:VQA}. For time steps $l>1$, the optimal parameters of the previous step $\upb^{l-1}$ serve as an initial guess for the \textsc{PSO} to reduce the efforts, as proposed by \cite{Sato2021,Leong2022}.

\begin{algorithm}[htbp]
\caption{VQ Algorithm}
\label{alg:VQA}
    \begin{algorithmic}
    \Require $N_\text{t}, \texttt{tol}_\text{P}, \texttt{tol}_\text{G}, f_\text{Ghost}, f, \upb_{0} $
    \State $l \gets 1$
    \While{$l \leq N_\text{t}$}  \Comment{Time Evolution}
        \If{$l=1$}
            % initial values
            \State $\Tilde{f}^1 \gets \frac{y(x,0,\upb_{0}) }{\Delta t}+ \Tilde{f}^1$ \Comment{Initial setup of the external contribution}
            \State $\upb^1 \gets \left(\lambda_0^1,\lamb_c^1\right)^\intercal$  \Comment{Random initialization of $\lambda_0^1\in [0,1]$ and $\lamb_c^1 \in [0,4\pi)$ for all $\mathfrak{p}$ particles}
        \Else
            % next values
            \State $\Tilde{f}^l \gets \frac{y(x, t^l, \upb_{l-1}) }{\Delta t}+ \Tilde{f}^l$ \Comment{Adjust the contributions}
            \State $\upb^l \gets \upb^{l-1}$  \Comment{Propagate previous final control $\upb^{l-1}$}
        \EndIf
        %% PSO
        \State $\upb^{l} \gets$ \textsc{PSO}$(\upb^l)$  \Comment{Iterate until $\texttt{maxit}_{P}$ or $\texttt{tol}_{P}>\textsf{ch}(\nabla J_i^l)$ (cf. \Fig{fig:optimizer})} \label{alg:VQA:PSO}
        %% GD BASED
        \State $\upb^{l} \gets$ \textsc{GD}$(\upb^{l})$  \Comment{Iterate until $\texttt{maxit}_{G}$ or $\texttt{tol}_{G}>\textsf{ch}(\nabla J_i^l)$ (cf. \Fig{fig:optimizer})}\label{alg:VQA:GRAD}
        \State $l \gets l+1$
    \EndWhile
    \end{algorithmic}
\end{algorithm}

The whole framework is implemented by an in-house toolbox, with \textsc{Qiskit} v.0.42.1 \cite{Qiskit} as a quantum backend. 

%###########################################
%      Derivative Computation
\subsection{Derivative Computation} \label{sec:Derivative1}
The determination of the descent direction is supported by the \textsc{QC}. To this end, the quantum circuits derived in Secs. \ref{sec:Compilation} and \ref{sec:Strategy} are re-used, as outlined below. The gradient of the objective function with respect to the scalar parameter $\lambda_0$ follows from \Eq{eq:Discrete_Opt_BC} and simply reads
\begin{align}
\begin{split}
\nabla_{\lambda_0} J(\lambda_0, \lamb_c) =
   &\sum\limits_{k=1}^{N_\text{p}} \underbrace{ -\left(\frac{2\nu \lambda_{0}}{\Delta x^2}\right) u_k(\lamb_{c}) \bigg(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})+u_{k-1}(\lamb_{c})\bigg) }_{\nabla_{\lambda_0}j_{L_k} } 
   \Delta x \, \\
   & 
    \underbrace{+\left(\frac{2\nu \lambda_{0}}{\Delta x^2}\right) \bigg( u_1(\lamb_{c})u_{N_\text{p}}(\lamb_{c}) + u_1(\lamb_{c}) u_{N_\text{p}}(\lamb_{c})  \bigg)}_{\nabla_{\lambda_0} (j_{DN_1} + j_{ DN_{N_\text{p}}}) } \Delta x \,
     \underbrace{-\left(\frac{2\nu \lambda_{0}}{\Delta x^2}\right) \bigg(  u_1(\lamb_{c})^2 + u_{N_\text{p}}(\lamb_{c}) ^2 \bigg)}_{\nabla_{\lambda_0}(j_{N_1} +j_{N_{N_\text{p}}}) } \Delta x \, \\
   + &\sum\limits_{k=1}^{N_\text{p}} \, \underbrace{ - 2\zeta \lambda_{0} u_k(\lamb_{c}) p_k u_k(\lamb_{c})  }_{\nabla_{\lambda_0} j_{P_k} }  \, \Delta x + \sum\limits_{k=1}^{N_\text{p}} \underbrace{ - 2 u_k(\lamb_{c}) \Tilde{f}_k } _{\nabla_{\lambda_0} j_{S_k}  } \, \Delta x \, . 
   \label{eq:deriv0-a}
\end{split}
\end{align}
Again, the temporal index has been omitted for better clarity. Comparing \Eq{eq:deriv0-a} with \Eq{eq:Discrete_Opt_BC} reveals
\begin{equation}
\label{eq:quantum_derivative_0}
\nabla_{\lambda_0} J
%(\lambda_0, \lamb_c) 
= \frac{1}{\lambda_0} \bigg[  \sum\limits_{k=1}^{N_\text{p}} 
 \big( 2  j_{L_k}
%(\lambda_0, \lamb_c) 
+ 2 j_{P_k} 
%(\lambda_0, \lamb_c) 
+ j_{S_k} \big)  \; \Delta x \bigg]  
%(\lambda_0, \lamb_c) 
+ \frac{2}{\lambda_0} 
\left[ \bigg(
  j_{DN_1} + j_{DN_{N_\text{p}}}
%(\lambda_0, \lamb_c) 
+ j_{N_1} + j_{N_\text{p}}
%(\lambda_0, \lamb_c) 
 \bigg)
 \, \Delta x \right] \, ,
\end{equation}
which can be evaluated on the \textsc{QC}. The derivative of $J$  with respect to $\lamb_c$ can also be computed on the \textsc{QC} without deriving a new gate sequence. The derivative of the objective function with respect to the control vector $\lamb_c$ follows from 
\begin{align}
\begin{split}
\nabla_{\lamb_c} J (\lambda_0, \lamb_c) 
   =
   &\sum\limits_{k=1}^{N_\text{p}} \nabla_{\lamb_c} \big( 
j_{L_k} + j_{P_k} + j_{S_k} \big) \Delta x 
   +
   \big( \nabla_{\lamb_c} (j_{DN_1} +j_{DN_{N_\text{p}}}) 
   +
   \nabla_{\lamb_c}(j_{N_1} +j_{N_{N_\text{p}}}) \big)   \,\Delta x  \, .
   \label{eq:derivc-a}
\end{split}
\end{align}

The linear source term $\nabla_{\lamb_c} j_{S_k}$ is approximated with second-order accurate central differences that operate on the complete (linear) objective function contribution \cite{Nocedal2006}, viz.
\begin{align}
    \nabla_{\lamb_c}j_{S_k}   = -2\lambda_{0} 
%    u_k'(\lamb_{c})  
 \big( \nabla_{\lamb_c} u_k \big)    
\Tilde{f}_k \approx 
  %\sum_{a=1}^c 
  \frac{j_{S_k}(\lambda_0, \lamb_c+h\eb_c)-j_{S_k}(\lambda_0, \lamb_c-h\eb_c)}{2h} %\eb_a 
   + \mathcal{O}(h^2) \, .
   \label{eq:opt-source-FD}
\end{align}
Mind that \Eq{eq:opt-source-FD} has to be executed for all entries of the parameter vector $\lamb_c$, and the step size is typically assigned to a constant value of $h\in[10^{-3},10^{-6}]$, depending on the number of employed qubits. For the quadratic terms $j_L, j_P, j_{DN}, \text{ and } j_N$, an exact representation of the derivative is given by the \textit{Parameter Shift Rule}, cf.  \cite{Schuld2019,Banchi2021,Crooks2019}. The derivative follows using only two additional evaluations of existing quantum circuits, and the nonlinearity is implicitly considered. Applying these techniques yields an expression for the derivative of the objective function $J$ with respect to the control vector $\lamb_c$ that utilizes the existing circuits, viz.  
\begin{align}
\begin{split}
\nabla_{\lamb_c} J(\lambda_0, \lamb_c) =&  \sum\limits_{k=1}^{N_\text{p}} \frac{1}{2} \bigg(j_{L_k}\big(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c\big) - j_{L_k}\big(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c\big) \bigg) \Delta x\\
&+ \frac{1}{2} \bigg(j_{DN}(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c)- j_{DN}(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c) \bigg) \Delta x \\
&+  \frac{1}{2} \bigg(j_{N}(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c)-j_{N}(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c) \bigg) \Delta x\\
+&\sum\limits_{k=1}^{N_\text{p}} \bigg(\frac{1}{2} \Big( j_{P_k}\big(\lambda_0, \lamb_c+\frac{\pi}{2}\eb_c\big)-j_{P_k}\big(\lambda_0, \lamb_c-\frac{\pi}{2}\eb_c\big) \Big)  + \nabla_{\lamb_c}j_{S_k} \bigg)\, \Delta x \, .
\end{split}
\label{eq:quantum_derivative_control}
\end{align}

==> Container/C_Feb27/Sections/Conclusion.tex <==
 %###########################################
%       Conclusion
%###########################################
\section{Conclusion} \label{sec:Conclusion}

The study presents a flexible and general boundary condition treatment for the numerical solution of \textsc{PDE}s on a \textsc{QC}. The strategy is based on the \textsc{VQA} approach by Lubasch et al. \cite{Lubasch2020}. To this end, initial-boundary value problems are reformulated as optimal control problems where all terms, including the boundary conditions, are cast into case-independent \textsc{QNPU}s. The boundary treatment combines ghost points with boundary cost function contributions that complement the objective function of the control problem. The method relaxes the requirements for the ansatz functions $U(\lamb_c)$, which must only be valid for the interior points that remain decoupled from the boundary points, and avoids the use of penalty terms. Verification studies are performed for steady and unsteady heat conduction problems, covering a variety of boundary conditions. 

\smallskip

The obtained \textsc{VQA}-results reveal an excellent agreement with a classical \textsc{FD}-results. 
The increase of the circuit depth could attenuate the optimization efficiency due to multi-controlled gates, limiting the implementation on \textsc{QC} hardware \cite{Cerezo2021,Sato2021,Sarma2023}. Analogously to the implementation of Laplacian and potential terms, improvements in this regard are achieved by replacing the multi-controlled gates with additional carry qubits. 
%The most efficient implementation ultimately depends on the available \textsc{QC} hardware and its support for multi-controlled gates.
The remarkable flexibility and accuracy of the proposed approach is thereby complemented by a favorable scaling of the quantum circuits with the number of qubits.
%-----Alternative

%\rule{10cm}{1mm}
 
\smallskip 
As for all \textsc{VQA} approaches, the choice of the ansatz is crucial since it defines the underlying function space for the \textsc{PDE} solution. At the same time, the approach can introduce a non-convex property into the optimization. The hardware-efficient bricklayer topology of the employed ansatz shows favorable expressibility in terms of small deviations from \textsc{FD} solutions in noise-less \textsc{QC} simulations. 
%
 The richer expressibility of the \textsc{\it SO4} ansatz in combination with shallow depths $d$ is advantageous, for example, to express general source terms. 
%
However, the strategy also unveils unfavorable with regard to the case-dependent increase of control parameters $\lamb_c$ and depth $d$, and the related poorer trainability. The combination of challenging trainability and the non-convex nature of the optimization can imply serious convergence issues in tracking the global optimum for larger numbers of qubits. 

Future research will be devoted to encode first derivatives as a \textsc{QNPU} operator to represent convective fluxes. In view of extending the present algorithm to \textsc{2D} and \textsc{3D} spatial problems, the non-convex optimization problem will be addressed by selecting more appropriate (trainable, expressible, shallow) dynamic ansatz strategies. For instance, strategies for avoiding barren plateaus in the cost function \cite{Ragone2023} include utilizing classical shadows \cite{Sack2022} and convolutional neural networks \cite{Pesah2021}. For the time evolution, the use of adaptive ansatz depths and circuit re-compilation techniques \cite{Jaderberg2020} seem promising ways to save computational cost and increase the range of applications towards industrial \textsc{QCFD} in the current \textsc{NISQ} era. 

==> Container/C_Feb27/Sections/Container-Chap4.tex <==
\bigskip
START NEW
\rule{10cm}{1mm}\\  %Does not like hline unfortunatly ...
%for the application of a multi-controlled-G Gate (MCG) in \Fig{fig:multicontrol} BITTE MODIFIZIEREN!.}
\pover{The example consists of $n=6$ qubits and requires $n-1=5$ carry qubits to transform the deep multi-controlled gate on the left of \Fig{fig:multicontrol} into $2n-2$ Toffoli- and one controlled G-gate on the right of \Fig{fig:multicontrol}.} 
Mind that all carry qubits finally need to be reversed to their initial state, i.e., $\ket{0}$. 

\begin{figure}[htbp]
    \centering
    \input{Figures/MultiControl}
    \caption{Alternative networks using a  qubit-saving implementation (left) and a shallow circuit depth approach  (right) of a multi-controlled Gate \textsc{G}.}
    \label{fig:multicontrol}
\end{figure}

%The decision for the most beneficial implementation is required to meet in knowledge of the to-be-used hardware. Experimental implementations regarding the native compilation of a multi-controlled gate have been exploited in \cite{McDonnell2022}, where the implementation in \Fig{fig:Transformation} is preferable. 
\pover{For this reason, we are carrying out both ideas and apply the idea of \Fig{fig:multicontrol} to the transformation circuit $T_t$ outlined in \Fig{fig:Transformation}. This allows us to derive the shallower alternative $\Tilde{T}_t$, cf. \Fig{fig:new-Tt:up}. 

\begin{figure}
\begin{subfigure}[t]{0.4\textwidth}
      \include{Figures/ShiftUP}
      \caption{Forward Transformation  $\tilde T_t$.}
      \label{fig:new-Tt:up}
\end{subfigure}
\hspace{3cm}
\begin{subfigure}[t]{0.4\textwidth}
      \include{Figures/ShiftDOWN}
      \caption{Backward (adjoint) Transformation $\tilde T_{t_\text{inverse}}$.}
      \label{fig:new-Tt:down}
\end{subfigure}
\caption{Alternative implementations of the forward ($T_t$, $\tilde T_t$) and backward ($T_{t}^\dagger$, $\tilde T_{t_\text{inverse}}$) transformation introduced in \Fig{fig:Transformation}.}
\label{fig:new-Tt}
\end{figure}

The illustration again features two adder operators, realizing the same effect as the network $T_t$ in \Fig{fig:Transformation} (left) and its inverse $T_t^\dagger$ (left). The inversion of the activity of the additional carry qubits follows from an adjoint approach, cf. \Fig{fig:new-Tt}.  Both  $\tilde T_t$ and $\tilde T_{t_\text{inv}}$ are controlled by an ancilla qubit,  which follows the strategy as depicted for the QNPU assembly in \Fig{fig:VQA_QNPU}.  The latter is required for measuring the expectation value $\sigma_z =  \bra{0} U^\dagger T_t^\dagger \; [\text{QNPU}] \; T_t U \ket{0}$ as illustrated by the Hadamard-test based  structure in \Fig{fig:VQA_QNPU}.  
 }

 %%%%%%%%%%%%%%%%%%%%%%


 %pover%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Hier steht das alte : 
\bigskip
START OLD
\rule{10cm}{1mm}\\
We now introduce an approach to generalize the periodic Laplace implementation for other boundary conditions based on the ghost point approach discussed
in Sec. \ref{sec:Discretization}.%As a benefit of the ghost point implementation introduced in Sec. \ref{sec:Discretization} the adaption to different BC is just a question of finding the corresponding gate sequence for augmentation. In the following, we would like to present another two circuits to adjust the field dynamics to the boundary setting and to link internal and external discretization.
%The suggested method only requires to adjust the field dynamics to the boundary conditions and link the internal and external discretization.

To begin with, we would like to mention the transformation $T_t$ already given by Sato et al. \cite{Sato2021}, which acts using the \textit{Modulo operation} (\textsf{mod}) as

%, like an anti-diagonal matrix on a vector, by the action
\begin{align}
    \label{eq:shift}
    \sum\limits_{k=0}^{N_\text{p}-1} \ket{\text{bin}\big(\left(k+1\right) \textsf{mod} \left(N_\text{p}\right)\big)} \bra{\text{bin}\big(k\big)}.
\end{align}

%\pover{Is the time increment necessary? Where do we want to show ? }
%To correct the discretized dynamics in the previously given QNPU, this transformation is required to align the quantum register for the following modifications.
An exemplary compilation of the transformation $T_t$ is given in \Fig{fig:Transformation}, which can be implemented as sketched in \Fig{fig:VQA_QNPU}. Note that the transformation $T_t$ inheres a sequence of multi-controlled gates, which can enhance the gate complexity, cf. Sec. \ref{sec:compilation:complexity} . 

\begin{figure}[htbp]
    \centering
    \input{Figures/Transformation}
    \caption{Four qubit example of a  generic shift operator $T_t$  represented by a sequence of multi-controlled Toffoli gates
    %. In the following, referred as transformation $T_t$,
    cf. \cite{Sato2021}.}
    \label{fig:Transformation}
\end{figure}


%pover%%%%%%%%%%%%%%%%%%%%%%%%%%%%% < - Hier steht das alte 
\bigskip
END OLD
\rule{10cm}{1mm}\\

==> Container/C_Feb27/Sections/Container-Matrix.tex <==
\section{Matrix-based Objective Function Representation}
The implementation of boundary conditions is based on the correction of the periodic contributions in the derivative matrix. To outline the transfer of \Eq{eq:Discrete_Opt_BC} into quantum-inspired or true quantum computations we restrict ourselves to  Dirichlet conditions imposed for a simple Laplace equation $\nu \Delta u=0$ in the simple 2-qubit case.
%
Let us try to recover a slightly reduced version of \Eq{eq:Discrete_Opt_BC} for this problem in a matrix-based approach for 4 points (two qubits) assuming $u \in \mathbb{C}^n$ \pover{Assuming real solutions would not restrict us here}. For the sake of clarity, we also assume $(\nu \lambda_0/\Delta x^2) = 1$, viz.
%
\begin{equation}
\begin{split}
    u^{\dagger} \cdot \Ab \cdot u &= \begin{pmatrix} u_{1}^* & u_{2}^* & u_{3}^* & u_{4}^* \end{pmatrix} \cdot \begin{pmatrix} -2 & 1 & 0 & 1 \\ 1 & -2 & 1 & 0 \\ 0 & 1 & -2 & 1 \\ 1 & 0 & 1 & -2 \end{pmatrix} \cdot \begin{pmatrix} u_{1} \\ u_{2} \\ u_{3} \\ u_{4} \end{pmatrix} \\ 
    & = -2 u^{*}_1 u_1 + u_1^*u_2 + u_2^* u_1 - 2 u_2 u_2^* + u_2^*u_3 + u_3^*u_2 \\
    &- 2 u_3 u_3^* + u_3^*u_4 + u_4^*u_{3} - 2 u_4^* u_4 + \underbrace{u_1^*u_4 + u_4^*u_1}_{\text{periodic boundary}}.
\end{split}
\label{eq:Expect_perio}
\end{equation}

The sum on the RHS of \Eq{eq:Expect_perio} distinguishes between regular interior contributions and periodic boundary contributions. In line with \eqref{eq:Discrete_Opt_BC},
the periodic contributions of $u_1^*u_4 + u_4^*u_1$ need to be eliminated by another term in the cost function given by  $J_{DN}$, viz. $J = \sum_1^4 j_L + j_{DN_1} + j_{DN_4}$. Following the classical computing example of Eqn. (\ref{eq:Expect_perio}), this is achieved by 
\begin{equation}
\begin{split}
    J_{DN}=  -(j_{DN_1} + j_{DN_4}) = u^{\dagger} \cdot \Db \cdot u &= \begin{pmatrix} u_{1}^* & u_{2}^* & u_{3}^* & u_{4}^* \end{pmatrix} \cdot \begin{pmatrix}0 & 0 & 0 & 1 \\ 0 & 0 & 0 & 0 \\ 0 & 0 & 0 & 0 \\ 1 & 0 & 0 & 0 \end{pmatrix} \cdot \begin{pmatrix} u_{1} \\ u_{2} \\ u_{3} \\ u_{4} \end{pmatrix} \\ 
    & = \underbrace{u_1^*u_4 + u_4^*u_1}_{\text{boundary}}. 
\end{split}
\label{eq:Bound_J}
\end{equation}

\noindent
However, matrix $\Db$ needs to be unitary for its representation by quantum gates. This distinguishes the quantum-inspired approaches from true QC methods. To this end, a unitary matrix $\Cb_2$ -- where the index refers to the number of qubits -- is proposed \sbengoechea{by us} \trung{by Sato et al.?} \cite{} as 

\begin{equation}
\begin{split}
    J_{DN} = u^{\dagger} \Cb u &= \begin{pmatrix} u_{1}^* & u_{2}^* & u_{3}^* & u_{4}^* \end{pmatrix} \cdot \begin{pmatrix}0 & 0 & 0 & 1 \\ 0 & 0 & 1 & 0 \\ 0 & -1 & 0 & 0 \\ 1 & 0 & 0 & 0 \end{pmatrix} \cdot \begin{pmatrix} u_{1} \\ u_{2} \\ u_{3} \\ u_{4} \end{pmatrix} \\ 
    & = u_1^*u_4 + \underbrace{u_2^*u_3 - u_3^* u_2}_{\text{if } u \in \mathbb{R}^n} + u_4^*u_1 = \underbrace{2u_1u_4}_{\text{boundary}} \, . 
\end{split}
\label{eq:Bound_J_unit}
\end{equation}

The unitary matrix $\Cb_2$ is constructed exclusively with nonzero entries on the antidiagonal. The upper and lower corners are required to have the same sign and correspond to the periodic contributions of matrix $\Ab$. While the other terms need to change the sign w.r.t. the main diagonal for these contributions to be canceled when the expectation value is measured. Note that for the summation of interior elements of the antidiagonal, one obtains zero only if $u \in \mathbb{R}^n$. 


The remaining task now is to design the circuits that implement the transformation described by the matrix $\Cb_2$. 
To this end, the approach is \trung{quite heuristic / not trivial ... } and requires \pover{always} another fractioning, i.e., $\Cb_2 = \Pb^{-1} \cdot \Bb \cdot \Pb$, where  $\Pb$ relates to a shift operator \cite{Sato2021} and $\Bb$ to a boundary circuit, which both directly translate into quantum gates. 
 \begin{equation}
     \Pb = \begin{pmatrix}0 & 0 & 0 & 1 \\ 0 & 0 & 1 & 0 \\ 1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \end{pmatrix} \quad 
     \Bb = \begin{pmatrix}0 & 0 & 1 & 0 \\ 0 & 0 & 0 & -1 \\ 1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \end{pmatrix}
     \label{eq:PBmatrix}
\end{equation}         

Perhaps more on more qubits ...

\pover{
\begin{itemize}
    \item Elaborate on the extension to higher numbers of qubits ...  $C_4$, $C_6$,... 
    \item Generalization is not unique and not only thus non-trivial 
    \item Kazeev Publication  - addresses strategy for Toeplitz matrices to gates/MPSs
    \item According to Nis, MPS is not a general approach -  heuristics essential    
    \item SVD, heuristics
\end{itemize}
}

\sbengoechea{
\begin{itemize}
    \item For nq >2 complex matrices, no unique solution show C4 in Appendix, maybe C6
    \item Remark that this part is to outline the steps towards gate level: by 2 steps
    \item 1) decomposition PBP
    \item 2) Find the gates for the matrix
    \item From gates to Matrix straightforward but from Matrix to gate hard, it is an inverse problem, the solution is not unique.  
    \item One possible route is MPS and citatons. 
\end{itemize}
}

% Now, let's shift to a more practical viewpoint. Assume we have two spring-mass systems in 1D. The velocity state-space is given by $\dot{x}_1\in \mathbb{R} \times \dot{x}_2 \in \mathbb{R} : = \mathbb{R}_1^2$. The velocity state vector is $\psi = (\dot{x}_1,\dot{x}_2)^\intercal$. In the following, the masses are in a steady state with certain $\dot{x}_1,\dot{x}_2$. One of them is in equilibrium. Let's assume $\dot{x}_1 = 0$, which relates to a state vector equal to the multiple of $\ket{1}$. Thus, this state is referred to as state-1 or $\ket{1}$ in the following. The state $\dot{x}_1 \neq 0 ,\dot{x}_2 = 0 $ named analogue $\ket{0}$.

==> Container/C_Feb27/Sections/Discretization.tex <==
\section{Discrete Objective Function and  Boundary Treatment}  \label{sec:Discretization}
The objective function \Eq{eq:Reduced_Opt} consists of contributions from the Laplace operator $j_L$, the potential $j_P$, and the source term $j_S$. The integration over the interior domain 
in \Eq{eq:Reduced_Opt} is fractioned into sub-integrals around the centrally spaced interior nodes, which are approximated by a  second-order accurate midpoint rule, i.e.
\begin{equation}
     J^{l} = \int_\Omega (j_L+ j_P+j_S)^l \,  dx = {\sum_{k=1}^{N_\text{p}}} (j_{L_k} + j_{P_k}+ j_{S_k})^l \, \Delta x \, .
     \label{eq:Reduced_Opt-Disc}
\end{equation} 
Subsequently, the discretized boundary conditions are introduced. These are formulated as corrections to established periodic boundary conditions, which yield augmentations of the discrete objective function \eqref{eq:Reduced_Opt-Disc}. The approach is compatible for an evaluation on \textsc{QC} hardware and is discussed below using the left boundary ($k=0$) as an example. The procedure for the right boundary is analogous and is therefore not discussed in detail. The time index is again deliberately suppressed for the sake of clarity.

The potential and source term contributions $j_{P_k}$, $j_{S_k}$ to \Eq{eq:Reduced_Opt-Disc} are strictly local and therefore do not interact with the ghost point (boundary) values. The contribution of the discrete Laplace operator, however, is non-local (but homogeneous) and interacts with the boundary. At the first interior point ($k=1$), the contribution reads
\begin{equation}
j_{L_1} =-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x} \right) \; u_1 \bigg( u_0 - 2u_1 +u_2\bigg) \, , 
 \label{eq:Laplace-left}
\end{equation}
where $u_0$ is an unknown that must be closed by the boundary condition. As already mentioned, the strategy refers to corrections of periodic boundaries, for which the left ghost point receives the value from the right interior point and the right ghost point gets the value from the left interior point, i.e., $u_0 =  u_{N_\text{p}}$ and  $u_{N_\text{p}+1} =  u_{1}$. The periodic contribution of the left boundary to $J$ reads 
\begin{equation}
    j_{L_1}^P   =-\left(
 \frac{\nu  \, \lambda_{0}^2}{\Delta x^2 }
  \right) \; u_1 \bigg( u_{N_\text{p}} - 2u_1 +u_2\bigg) \, .
  \label{eq:periodic-left}
\end{equation}
On the other hand, a Dirichlet condition $u_0=D$ yields  
\begin{equation}
    j_{L_1}^D  =-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1 \bigg( D - 2u_1 +u_2\bigg) \, .
     \label{eq:dirichlet-left}
\end{equation}
 Aiming to reconstruct the Dirichlet condition \eqref{eq:dirichlet-left} from the periodic approach \eqref{eq:periodic-left}, one arrives at 
\begin{equation}
   j_{L_1}^D = j_{L_1}^P
  + u_1 \, \left(\frac{\nu \lambda_0^2}{\Delta x^2} \right) \left( 
   u_{N_\text{p}} - D
  \right)  = j_{L_1}^P \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_1$-contrib.} \, j_{DN_1}} \;   \underbrace{-u_1 D \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{source-term modif.} \, f_1}  \, .
   \label{eq:defcoD-left}
\end{equation}
In the case of Neumann conditions, the prescribed gradient $N= \partial u/\partial x\rvert_0$ first needs to be approximated. The exemplary use of simple first-order \textsc{FD} $N \approx (u_1-u_0)/(\Delta x)$ to substitute $u_0 = u_1 - N \Delta x $ in \Eq{eq:Laplace-left} yields 
\begin{align}
\begin{split}
    j_{L_1}^N   &=-\left(\frac{\nu  \, \lambda_{0}^2}{\Delta x^2}\right) \; u_1 \bigg( (u_1 -N \Delta x) - 2u_1 +u_2\bigg) \\
    &= 
  j_{L_1}^P
   \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_1$-contrib.} \, j_{DN_1}} \; 
     \; \underbrace{- u_1 u_{1} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_1$-contrib.} \, j_{N_1}} \; 
  \underbrace{+ u_1 \, N \left( \frac{\nu \lambda_0^2}{\Delta x} \right)}_{\text{source-term modif.} f_1}
  \, .
\end{split}
  \label{eq:defcoN-left}
\end{align}
Note that the contribution $j_{DN_1}$, which neutralizes the periodic term, occurs for any conditions. The technique can be combined with higher-order \textsc{FD} to approximate derivative expressions in Neumann or Robin conditions. At the right boundary, the corresponding correction terms read
 \begin{align}
   j_{L_{N_\text{p}}}^D 
= j_{L_{N_\text{p}}}^P
  + u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2} \right) \left( 
   u_{1} - D
  \right) 
  = j_{L_{N_\text{p}}}^P 
   \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_{N_\text{p}}$-contrib.} \, j_{DN_{N_\text{p}}}} \;   \underbrace{-u_{N_\text{p}} D \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{source-term modif.} \, f_{N_\text{p}}} \,
   \label{eq:defcoD-right}\\
   \text{ and } \qquad  j_{L_{N_\text{p}}}^N   = j_{L_{N_\text{p}}}^P
   \; \underbrace{+ u_1 u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_{N_\text{p}}$-contrib.} \, j_{DN_{N_\text{p}}}} \; 
     \; \underbrace{- u_{N_\text{p}} u_{N_\text{p}} \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{new J$_{N_\text{p}}$-contrib.} \, j_{N_{N_\text{p}}}} \; 
  \underbrace{- u_{N_\text{p}} \, N \left( \frac{\nu \lambda_0^2}{\Delta x} \right)}_{\text{source-term modif.} f_{N_\text{p}}}
  \, .
  \label{eq:defcoN-right}
\end{align}

Again, the contribution $j_{DN_{N_\text{p}}}$, which neutralizes the periodic entries, occurs for both Neumann and Dirichlet conditions, and it is identical for both boundary locations ($j_{DN_{N_\text{p}}}=j_{DN_{1}}$). 
The actual correction implementation is given in \Eq{eq:Discrete_Opt_BC}. 
It employs three terms: (a) the periodic baseline term, (b) corrections based upon combinations of unknown interior points ($j_{DN_k}$, $j_{N_k}$), and (c) modifications of the source terms $j_{S_k}$ arising from known boundary condition values ($D$, $N$), viz. 
\begin{align}
\begin{split}
   J(\lambda_0, \lamb_c) =
   &\sum\limits_{k=1}^{N_\text{p}} \underbrace{ -\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) u_k(\lamb_{c}) \big(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})+u_{k-1}(\lamb_{c})\big) }_{j_{L_k}: \; \text{periodic \& interior term}} \Delta x \, \\
    & \underbrace{+\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right) \bigg( u_1(\lamb_{c})u_{N_\text{p}}(\lamb_{c}) + u_{1}(\lamb_{c}) u_{N_\text{p}}(\lamb_{c}) \bigg)}_{ j_{DN_1} + j_{ DN_{N_\text{p}} }: \, \text{neutralizing left/right term (Dirichlet \& Neumann)} } \Delta x   \\
    & \underbrace{-\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right)  u_1^2 (\lamb_{c})}_{j_{N_1}:  \, 
   \text{left Neumann cond.}} \Delta x 
   \underbrace{-\left(\frac{\nu \lambda_{0}^2}{\Delta x^2}\right)    u_{N_\text{p}}^2 (\lamb_{c}) }_{j_{N_{N_\text{p}}}: \,   
   \text{right Neumann cond.}} \Delta x \,\\
   + &\sum\limits_{k=1}^{N_\text{p}} \, \underbrace{ -\zeta \lambda_{0}^2 u_k(\lamb_{c}) p_k u_k(\lamb_{c})  }_{{j_{P_k}: \, \text{potential term}}}  \, \Delta x + \sum\limits_{k=1}^{N_\text{p}} \underbrace{- 2\lambda_{0} u_k(\lamb_{c}) \Tilde{f}_k } _{j_{S_k}: \, \text{source term}} \, \Delta x.
    \label{eq:Discrete_Opt_BC}
    \end{split}
\end{align}

This approach is applied {in the sense of the desired boundary conditions} for all time steps and can be adapted to combinations of Dirichlet, Neumann, {Robin} or periodic conditions. \Equ{eq:Discrete_Opt_BC} utilizes a modified source term $\tilde f_k$ which inheres the additional  sources  given in Eqns. (\ref{eq:defcoD-left}-\ref{eq:defcoN-right}). For the example of a Dirichlet conditions on the left boundary, cf. \Eq{eq:defcoD-left}, the source term 
modifies to $j_{S_1} = - 2 \lambda_0 u_1 \tilde f_1$, with $\tilde f_1 = f_1 + 0.5  D \nu \lambda_0/\Delta x^2 $.

\medskip
The following two sections outline the framework for evaluating \Eq{eq:Discrete_Opt_BC} on a QC. 
Sec. \ref{sec:Strategy} describes the Variational Quantum Algorithm (VQA) framework, which shares features with \cite{Lubasch2020}. Subsequently,  the quantum circuits used to calculate the different contributions ($j_{L_k}, j_{S_k}, j_{P_k}$) to \Eq{eq:Discrete_Opt_BC} on a QC are described in Sec. \ref{sec:Compilation}. The gate
complexity of these circuits is optimized in Sec. \ref{sec:compilation:complexity} before they will be used to approximate the derivative of the objective function with respect to the parameters in Sec. \ref{sec:Optimization}, which in turn is required to advance the optimization.

\medskip
Before we continue with the \textsc{QC} implementation of the different objective function contributions, we remark that the Neumann terms $ j_{N_1}$ and $j_{ N_{N_\text{p}}}$ could also be cast into potential term contributions derived from the reciprocal of the diffusive time scale, i.e. $\tilde p_1 = p_1 + \nu/(\zeta \Delta x^2)$ and $\tilde p_{N_\text{p}} = p_{N_\text{p}} + \nu/(\zeta \Delta x^2)$. 

==> Container/C_Feb27/Sections/Intro.tex <==
%###########################################
%       Introduction
%###########################################
\section{Introduction}\label{sec:Introduction}

Partial differential equations (\textsc{PDE}) are ubiquitous for modeling problems in science and engineering. Areas of application include structural and fluid mechanics, electrodynamics, thermodynamics, and quantum physics. Today, sophisticated and dedicated numerical methods are well-established and widely available in all of those areas. However, the increasing demands to resolve wider ranges of spatial and temporal scales with great precision make these simulations expensive and energy-consuming. 
%
Furthermore, chip sizes for classical central processing units (\textsc{CPU}s) are expected to converge over the next decade \cite{Burg2021} due to the limits of reducing the transistor's size further, putting an end to Moore's Law \cite{Khan2018}. 
In regard of increasing computing power, Quantum Computers (\textsc{QC}s) promise to address some future hardware challenges.
%Therefore, the increase of computing power with traditional hardware is challenging. In this regard,  Quantum Computers (\textsc{QC}s) promise to overcome some of the future hardware-related challenges. 
%Grossly speaking, 
Two categories for \textsc{QC}-supported \textsc{PDE} solutions have been proposed. They are either based on the direct encoding of the \textsc{PDE} solution in a large quantum circuit or on a Variational Quantum Algorithm (\textsc{VQA}), which evaluates shallow circuits in combination with classical optimization methods \cite{Suau2021}. 

%FIRST
For the first category, Quantum Linear Solvers (\textsc{QLS}) are applied to solve the algebraic equation systems derived from the discretization of linear \textsc{PDE}s. In a pioneering work \cite{Harrow2009}, Harrow, Hassidim, and Lloyd presented the \textsc{HH}L quantum algorithm to compute the solution of a Linear System of Equations (\textsc{LSE}). 
The \textsc{HHL} algorithm promises an exponential speedup, provided that the state preparation and information readout can efficiently be performed on the \textsc{QC}, which is by no means self-evident.
 The algorithm works best for non-stiff \textsc{LSE}, but scales worse than classical methods for stiff problems.
%The quantum advantage is achieved by outsourcing the most demanding solution of the LSE. 
%
In \cite{Montanaro2016}, a modification of the \textsc{HHL} algorithm is applied to solve an \textsc{LSE} originating from a Finite-Element Method while the temporal evolution of a linear \textsc{PDE} is approximated in \cite{Berry2014}. 
%
Computational Fluid Dynamic (\textsc{CFD}) applications are reported in \cite{Steijl2018,Gaitan2020,Oz2021,Childs2020,Childs2020a,Cao2013,Chen2021}.
Steijl and Barakos \cite{Steijl2018} used a vortex-in-cell \textsc{CFD} method and employed a quantum Fourier solver for the Poisson equation. In \cite{Gaitan2020} and \cite{Oz2021} the \textsc{PDE} system is spatially discretized into a system of coupled Ordinary Differential Equations (\textsc{ODE}s) and approximated via a Quantum Amplitude Estimation Algorithm (\textsc{QAEA}) proposed by Kacewicz  \cite{Kacewicz2006}. In \cite{Childs2020} and \cite{Childs2020a}, the \textsc{PDE} solution is spatially approximated with truncated Fourier or Chebyshev series, in which the unknown coefficients are determined by a \textsc{QLS}. In the study of Cao et al. \cite{Cao2013}, the \textsc{HHL} is used to solve the Poisson equation within a predictor-corrector method to solve the incompressible Navier-Stokes equation. 
%
The \textsc{QLS} approaches mentioned above mostly require a large number of qubits devoted to error correction, and the number of operations associated with the \textsc{HHL} exceeds the capabilities of current \textsc{QC} hardware. Hence, \textsc{QLS} methods are more suitable for future fault-tolerant quantum machines and less suitable for \textsc{QC}s of the current Noise Intermediate-Scale Quantum (\textsc{NISQ}) generation \cite{Suau2021}. 

%SECOND
\smallskip 
The \textsc{VQA} is an alternative category to solve \textsc{PDE} problems and is dedicated to state-of-the-art \textsc{NISQ} devices~\cite{Peruzzo2014}. The noise-tolerant procedure is based on the efficient evaluation of a cost function by the \textsc{QC}, while the classical hardware optimizes the parameters of the ansatz circuit that encodes the solution on the \textsc{QC}. As a consequence, the \textsc{PDE} to solve must be reformulated as an optimization problem. The main advantage of this approach is the use of a small number of gate operations, making it more robust to decoherence effects of the quantum registers that compose the circuits. 

\textsc{VQA}s are used in many applications such as the identification of ground states \cite{Peruzzo2014}, or solving \textsc{LSE} \cite{Cerezo2021}. 
Recent applications to fluid dynamics and related \textsc{PDE}s are, for example, reported in \cite{Demirdjian2022,BravoPrieto2019,Kyriienko2021,Sato2021,Leong2022,Leong2023}. Burgers' advection-diffusion equation is studied in \cite{Demirdjian2022} where the discretized sparse matrix problem is decomposed in a finite series of unitary operators and solved by the variational quantum solver proposed in \cite{BravoPrieto2019}. In \cite{Kyriienko2021}, quantum neural networks are trained with a hybrid \textsc{VQA} to solve systems of nonlinear differential equations that model a supersonic nozzle flow. The work of Sato et al. \cite{Sato2021} is of particular relevance for this study and explores the ability of \textsc{VQA}s to solve the Poisson equation by minimizing the potential energy of an elliptic \textsc{PDE}. To this end, the dynamics of the Poisson equation can be linearly decomposed in a series of parameterized shallow quantum circuits. The idea of energy minimization from Sato et al. \cite{Sato2021} is extended to time-dependent problems in Leong et al. \cite{Leong2022,Leong2023}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% OUR WORK:
The present effort aims to combine the quantum framework described in Lubasch et al. \cite{Lubasch2020} with the work of Sato et al. \cite{Sato2021}. We focus on a flexible treatment of engineering boundary conditions on \textsc{QC}s and deploy a Hadamard-test-based structure to gain quantum advantage \cite{Guseynov2023}. The related single-qubit measurements reduce expensive sampling operations to evaluate the results encoded in a quantum state and thus the associated loss of efficiency \cite{Berry2014,Kyriienko2021,Chen2021}.
%
An accurate, flexible, and robust treatment of diverse boundary conditions is crucial for engineering applications. Despite the importance, a rigorous algorithmic implementation in the context of \textsc{QC} is not trivial, as demonstrated by the variety of specific approaches proposed in the literature. The works of Cao et al. \cite{Cao2013} and Childs et al. \cite{Childs2020} are restricted to Dirichlet conditions, while a related study of Childs et al. \cite{Childs2020a} mirrors the solution into the symmetric and antisymmetric sub-spaces for Neumann and Dirichlet cases, respectively. 
The mixed boundary conditions for the Burgers' equation suggested in \cite{Oz2021} can only be enforced on classical hardware. 
The algorithm suggested in \cite{Costa2019} imposes Dirichlet or Neumann conditions on the discrete wave equation prior to the derivation of the Hamiltonian operator, i.e., the solutions in the Hilbert space (trial functions) need to satisfy the boundary conditions. Suau et al. \cite{Suau2021} present a modification of this approach, where only Dirichlet boundaries are included. 
For \textsc{VQA} applications, the boundary conditions in \cite{Kyriienko2021} are included either as part of the cost function or as an additional constraint on the ansatz function. 
The Dirichlet and Neumann boundary operators employed by Sato et al. \cite{Sato2021} do not form unitary operators. This either requires implementation on classical hardware due to the necessary non-unitary corrections or measuring the whole quantum register, which in turn reduces the efficiency. 

The paper suggests combining a classical CFD ghost-point technique with a unitary decomposition of the boundary operators by modifying the route proposed in \cite{Sato2021}. The decomposed boundary operators are subsequently compiled into quantum gates and finally included in the cost function using a deferred correction strategy. The proposed approach permits the full-quantum implementation of arbitrary Dirichlet, Neumann, and Robin conditions without additional constraints on the trial or ansatz functions. 

The remainder of the paper is structured as follows: Sec. \ref{sec:Mathematics} introduces the mathematical model and the boundary treatment is described in Sec. \ref{sec:Discretization}. Subsequently Secs. \ref{sec:Strategy} and \ref{sec:Compilation} outline the computational model. The latter also addresses the \textsc{QC} implementation and the quantum circuits. Section \ref{sec:compilation:complexity} discusses means to reduce the gate complexity of the utilized quantum circuits. Section \ref{sec:Optimization} describes the employed optimization procedure in brief 
%as a by-product of the present study,
and Sec. \ref{sec:Applications} is devoted to numerical results. The applications are concerned with steady and transient heat conduction. Particular emphasis is given to temperature distributions obtained with various types of boundary conditions, which are compared to results of classical Finite-Differences (\textsc{FD}). Final conclusions and future directions are outlined in Sec. \ref{sec:Conclusion}. 
%
The presented quantum framework is emulated with \textsc{IBM}'s \textsc{Qiskit} environment \cite{Qiskit}. 
%
Within the publication, vectors and tensors are defined with reference to Cartesian coordinates. Note that binary representations follow the \textit{little-endian} convention.


==> Container/C_Feb27/Sections/Math.tex <==
%###########################################
%       Mathematical Framework
%###########################################
\section{Mathematical Model}  \label{sec:Mathematics}
%The mathematical model consists of four steps. 
%First, the considered \textsc{PDE} is introduced and discretized in time. Subsequently, the spatial \textsc{PDE} is cast into an optimization problem, and the objective function is prepared for being evaluated on \textsc{QC} hardware before the simple spatial discretization is outlined. 

The considered \textsc{PDE} is first introduced and discretized in time. Subsequently, the \textsc{PDE} is cast into an optimization problem, and the objective function is prepared for being evaluated on \textsc{QC} hardware before the spatial discretization is outlined. 

\subsection{Governing Equation} \label{sec:GoverningEq}
The presented approach is restricted to unsteady, spatially \textsc{1D} problems.
An extension to two- or three spatial dimensions is straightforward \cite{Lynch1964}. For brevity, we use a {normalized} spatial coordinate {$x \in [0,1]$} 
%$x \in \Bar{\O}$} 
and a time domain $t \in [0,T]$. 
%
The problems considered herein are described by an unsteady reaction/diffusion \textsc{PDE} for an unknown field or state variable $y(x,t)$, viz. 
\begin{align}
   \frac{\partial y }{\partial t}-\nu \Delta y -\zeta y \, p   = f \quad \text{in } \O_\text{T} : =  (0,1) \times (0,T] \, . 
   \label{eq:Generic_PDE-TR}
\end{align}
In \Eq{eq:Generic_PDE-TR}, the notation $\Delta y = \nabla \cdot \nabla y$ describes the Laplace operator acting on $y$. 
Moreover, the right-hand side term  $f(x)$ denotes a time-independent source,  $p(x,t)$ is a time-dependent potential that is 
independent of $y$, $\zeta$ is a simple (real) coefficient and $\nu$ refers to the inherently positive (real) diffusivity. 
%
In contrast to previous works published in  \cite{Cao2013,Sato2021,Leong2022,Leong2023,Arrazola2019}, the proposed framework to solve \Eq{eq:Generic_PDE-TR} applies to arbitrary combinations of Dirichlet and Neumann conditions. The details of the boundary treatment will be outlined in Sec. \ref{sec:Discretization}. 

\subsection{Temporal Discretization}
The time horizon $T$ is discretized into $N_\text{t}$ equidistant time instants $t_l$, where $l \in \left[0,N_\text{t}\right]$  and $\Delta t$ marks a constant time step. 
In line with traditional finite approximation strategies,  time derivatives are approximated by implicit backward \textsc{FD}, e.g., an implicit first-order Euler scheme or a second-order three-time-level scheme
\begin{align}
\begin{split}
     \frac{\partial y(x,t^l)}{\partial t} &= \frac{ y(x,t^l) -y(x,t^{l-1}) }{\Delta t} + \mathcal{O}(\Delta t) \, ,\\
 \frac{\partial y(x,t^l)}{\partial t} &= \frac{3 y(x,t^l) -4y(x,t^{l-1}) +y(x,t^{l-2}) }{2\Delta t} + \mathcal{O}(\Delta t^2)
 \; .
\end{split}
\label{eq:Generic_time}
\end{align}
The examples included herein use the implicit Euler scheme. 
This results in the following modifications of the potential term $p\to p + 1/(\zeta \Delta t)$ and the source term $f \to f+ y(x, t^{l-1})/\Delta t$, which yields a spatial \textsc{PDE} at time $t^l$ in residual form 
\begin{equation}
 R(y(x,t^l)) = 
  - \left( \nu \Delta y + \zeta y \, p   + f \right) = 0 \quad \text{in } \O_\text{T} : =  (0,1) \times (0,T] \, . 
   \label{eq:Generic_PDE-TR-2}
\end{equation}

\subsection{Optimal Control Problem} 
\label{sec:optimal_control}

A weak form of \Eq{eq:Generic_PDE-TR-2} follows from a weighted residual formulation and reads
\begin{align}
 \int_{\O}  z(x,t^l) \, R(y(x,t^l)) \,  dx  = 0 \, , 
  \quad \text{or} \quad  
\underbrace{-\int_{\O} z \big( \nu\Delta y + \zeta y \, p\big) \, dx}_{a(z,y)} 
 - \underbrace{\int_{\O} z \, f \, dx}_{F(z)} = 0  
 \label{equ:weighted_res-2}
\end{align}
where $z(x,t^l)$ is a weighting function. For $z=y$, \Eq{equ:weighted_res-2} evolves into the solution of a variational problem \cite{Grossmann2007,Glowinski2015} characterized by minimizing an objective function $\mathcal J$ for 
\begin{align}
    \min\limits_{y} \mathcal{J}(y) \quad  \text{with} \quad \mathcal{J}(y):= a(y,y) - 2F(y).
    \label{eq:Generic_Opt_Approx}
\end{align}
Mind that the equivalence between the \textsc{PDE} solution \eqref{eq:Generic_PDE-TR} and the minimization problem \eqref{eq:Generic_Opt_Approx} restricts the function space $y$ to an elliptic $a(z,y)$ \cite{Grossmann2007} and that the computed solution is, of course, only an approximation to $y$.

The limited ability to represent arbitrary states $y$ on \textsc{QC} hardware, yields the \textit{partition of unity} constraint 
given by the $L^2$ scalar product as \cite{Troutman1996,Werner2005}
\begin{align}
    (y^*,y)_{L^2} = \int_{\O}  y^*(x,t^l) \, y(x,t^l) \,  dx =  1 \, ,
    \label{eq:partition_of_unity}
\end{align}
where the asterisk indicates the complex conjugate. Turning our attention to the variational framework \eqref{eq:Generic_Opt_Approx}, the function $y$ is made variable by the control $\upb^l \in \mathbb{R}^{c+1},  \upb^l: = \left(\lambda_0^l, \lamb_c^l\right)^\intercal$ ($c \in \mathbb{N}$), using the time-dependent ansatz 
\begin{align}
    y(x,t^l, \upb^l) = \lambda_{0}^{l} \, u(x, {t^l}, {\lamb_c^l}) \, , \quad \text{with} \quad 
    \big(u^*, u\big)_{L^2} = 1 \, 
        \label{eq:Generic_Ansatz}
\end{align} 
to enforce the normalization restriction \eqref{eq:partition_of_unity}.  Suppressing the temporal index $(...)^l$ and substituting the ansatz \eqref{eq:Generic_Ansatz} into the objective function, one obtains the (time-dependent) minimization problem 
\begin{align}
	\begin{split}
     \min \limits_{\upb} J(\upb)  \quad \text{with} \quad J(\upb) :&= a\big(y(\upb),y(\upb)\big) - 2F(\upb),\\
			 &=  - \nu  \, \lambda_{0}^2 \int_{\O}  u(x, \lamb_{c}) \Delta u(x, \lamb_{c}) \, dx - \zeta \, \lambda_{0}^2  \int_{\O} u(x, \lamb_{c}) \, p(x) \, u(x, \lamb_{c}) \, dx \\
        &\quad- 2  \lambda_{0} \int_{\O}  u(x, \lamb_{c}) \, f(x) \, dx \, .
	\end{split}
\label{eq:Reduced_Opt}
\end{align}
For each time step, this minimization is performed using a simple gradient descent method (\textsc{GD}) that requires the derivatives of the objective function with respect to the control. The Gâteaux derivative with respect to the control $\upb$ provides a first-order optimality condition \cite{Troutman1996}
\begin{align}
     \frac{\partial J}{\partial \upb} \delta \upb &= {\frac{\partial J}{\partial y} \frac{\partial y}{\partial \upb} \delta\upb} =  \begin{pmatrix}
            \nabla_{\lambda_0} J \\ 
            \nabla_{\lamb_c} J 
        \end{pmatrix}  \cdot \begin{pmatrix}
            \delta \lambda_0\\
            \delta \lamb_c
        \end{pmatrix} =  0 \quad \forall \, \delta\upb.
\end{align}
The partial derivatives of the objective function with respect to the control 
are not discussed in the continuous form here. Instead, a \textsc{QC}-compatible discretized form is developed in Sec. \ref{sec:Optimization}. 
 
\subsection{Spatial Discretization}
%###########################################
%       Discretization of the Governing equations
%###########################################
The unit interval is discretized by $N_\text{p}+2$ equidistantly spaced points  $x_k$, with $k \in \left[0,N_\text{p}+1\right]$. As alluded to earlier,  the time $t\in [0,T]$ is discretized by $N_\text{t}+1$ equidistant time instants $t^l$, which leads to the structured grid depicted in \Fig{fig:discretization_encoding}. As indicated by the figure, we distinguish between interior points (closed circles) and ghost points (open circles), which serve to introduce boundary conditions. 
\begin{figure}[htbp]
    \centering
    \input{Figures/Discretization}
    \caption{Illustration of the spatial-temporal discretization on an equidistant grid with 
    boundary/ghost nodes indicated by open symbols~(\protect\tikz \protect\draw[thick,black] (1ex,1ex)  circle [radius=0.1];) and interior nodes by closed symbols~(\protect\tikz \protect\draw[fill] (1ex,1ex)  circle [radius=0.1];).}
    \label{fig:discretization_encoding}
\end{figure}
Similar to classical finite approximation schemes, variables located along the spatial boundaries can either be part of the unknowns or separated from the unknowns. In the latter case, the boundary conditions are represented by the influence of prescribed ghost point variables on the interior point approximations. In the case of Neumann or Robin conditions, this usually involves the additional discretization of the spatial derivative.   

The procedure is as follows: Boundary nodes are assigned to ghost nodes (\protect\tikz \protect\draw[thick,black] (1ex,1ex)  circle [radius=0.1];)  and the spatially discretized objective function \eqref{eq:Reduced_Opt} is evaluated for the interior nodes (\protect\tikz \protect\draw[fill,black] (1ex,1ex)  circle [radius=0.1];), with the contributions of the ghost nodes arising from discretized boundary conditions. Thus, the discrete ansatz function vector $\big(u(x_0,t^l), u(x_1,t^l), \dots, u(x_{N_\text{p}+1},t^l) \big) = \ub^l$ is represented using the orthogonal basis $\eb_k$, viz. 
\begin{align}
    \ub^l = u_0^l \eb_0 +  \underbrace{\sum\limits_{k=1}^{N_\text{p}} u_k^l \eb_k}_\text{register} + u_{N_\text{p}+1}^l \eb_{N_\text{p}+1} \, ,  
    \label{eq:discretization_register}
\end{align}
with the interior to be stored in a register of length $\log_2(N_\text{p})$ qubits as shown in Sec.~\ref{sec:Strategy}. The derivatives of the Laplace operator required to evaluate the objective function (\refeq{eq:Reduced_Opt}) are approximated by
\begin{align}
\frac{\partial^2 u^l_k}{\partial x^2} =
\frac{u_{k+1}^l-2u_k^l+u_{k-1}^l}{\Delta x^2} +  \mathcal{O}(\Delta x^2) \, , 
\label{eq:derivatives_space}
\end{align}
which is second-order accurate for an equidistant grid. 

==> Container/C_Feb27/Sections/Results.tex <==
%###########################################
%       Numerical Results
%###########################################
\section{Numerical Results} \label{sec:Applications}
This section describes the application of the \textsc{VQA} to two prototypical \textsc{CFD} problems, i.e., the steady heat conduction (Sec. \ref{sec:Application:Poisson}) and the transient heat conduction (Sec. \ref{sec:Application:Heat}). Results are discussed for a range of Dirichlet, Neumann, and Robin boundary-condition combinations. The validation data is obtained from \textsc{FD}-solutions of the \textsc{PDE} problem. It employs the same discretization as the \textsc{VQA} to approximate the Laplace operator and the temporal derivative, cf. \Eq{eq:Generic_time} and \Eq{eq:derivatives_space}.

The predictive deviation of the \textsc{VQA}-solution $y^\text{VQA}$ from \textsc{FD}-solutions $y^\text{FD}$ is assessed using either the $l_2$-norm $\varepsilon_{l_2}$ or the frequently employed trace distance $\varepsilon_{\text{tr}}$, cf.  \cite{Sato2021,BravoPrieto2019,Liu2021}, viz.
\begin{align}
    \varepsilon_{l_2} = \sqrt{\sum_k (y_k^\text{FD}-y_k^\text{VQA})^2} \, , \qquad
    \varepsilon_{\text{tr}} = \sqrt{\Bigg(1- \sum_k \bigg|\frac{y_k^\text{FD}}{\sqrt{\sum_j (y_j^\text{FD})^2}}\frac{y_k^\text{VQA}}{\sqrt{\sum_j (y_j^\text{VQA})^2}}\bigg|^2 \Bigg)} \, .
\end{align}

Time-averaged measures are employed to assess the transient heat conduction and indicated by $ \Bar{\varepsilon}_{l_2}, \Bar{\varepsilon}_{\text{tr}}$. The number of control variables $c$  of  $\lamb_c$ is also stated in the results tables. A full dataset of the performed experiments is available via \cite{data}.

\subsection{Steady Heat Conduction (Poisson Equation)}
\label{sec:Application:Poisson}
The first case refers to the Steady Heat Conduction, where the time derivative in \Eq{eq:Generic_PDE-TR} vanishes, and $y$ [K] marks the temperature. The physical potential $p(x)$ [1/s] vanishes, and the diffusivity is assigned to a unit value $\nu=1$ [m$^2$/s]. In the case of pure Neumann boundary conditions, the source reads $f(x) =1$ for $x<0.5$ and $f(x) =-1$ for $x>0.5$. In all other cases, the unit source responds to $f(x) \equiv 1$ [K/s]. Mind that singular solutions, e.g., caused by pure Neumann conditions, are fixed by defining a central zero crossing. The application of the \textsc{VQA} framework to this Poisson problem is presented for the following seven scenarios: in-/homogeneous Dirichlet, in-/homogeneous Neumann, mixed Neumann/Dirichlet conditions, Robin conditions, and periodic conditions. 
Displayed results are obtained for a coarse grid, featuring $N_\text{p}=4$ interior points ($n=2$ qubits; dashed lines), and a finer grid, featuring $N_\text{p}=16$ interior points ($n=4$ qubits; straight lines). The  \textsc{FD}-results are depicted by closed circles ($N_\text{p}=4$) and open squares ($N_\text{p}=16$). 

The periodic case serves as a verification reference and is displayed in \Fig{fig:Results:Poisson:periodic}. \textsc{VQA}-results were obtained from shallow circuits $U(\lamb_c)$ using a depth of $d=1$, cf. \Fig{fig:VQA_Ansatz}.
\Fig{fig:Results:Poisson:periodic:cost} shows the convergence of the objective function with the dotted vertical lines indicating the transition from global (\textsc{PSO}) to local ({\textsc{GD}) optimization (cf. Alg. \ref{alg:VQA}). The \textsc{VQA}-results are compared with \textsc{FD}-solutions in \Fig{fig:Results:Poisson:periodic:res} and indicate an excellent agreement with the expected solution {$y_k \equiv 0$}. The \textsc{VQA}-result improves as the grid is refined. The latter is also indicated by a reduction of $\varepsilon_{l_2}$ from an already satisfactory value of $10^{-6}$ to $10^{-7}$, cf. \Tab{tab:Results:Poisson:Errors}. The reduction goes hand in hand with lower amplitude but higher frequency wiggles displayed in \Fig{fig:Results:Poisson:periodic:res}, which are reflected by an augmented trace distance $\varepsilon_{\text{tr}}$ and should be viewed with caution due to the vanishing mean value for this case.
 
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \input{Figures/Results/R_Poisson_Cost.tex}
        \caption{Evolution of the normalized objective function over the optimization count $i$. Dotted vertical lines indicate the transition from global (\textsc{PSO}) to local (GD) optimization. }
        \label{fig:Results:Poisson:periodic:cost}
    \end{subfigure}
    \hspace{0.3cm}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Periodic.tex}
        \caption{Comparisons of \textsc{VQA}- and \textsc{FD}-results, ($n=2$, closed circles; $n=4$, open squares). } 
        \label{fig:Results:Poisson:periodic:res}
    \end{subfigure}
    \caption{Verification results of the \textsc{VQA} application for a periodic steady heat conduction problem  using  $N_\text{p}=4$ ($n=2$, $d=1$; dashed lines) and $N_\text{p}=16$ ($n=4$, $d=1$; straight lines) interior points.}
    \label{fig:Results:Poisson:periodic}
\end{figure}

\begin{figure}[htbp]
\centering
    \hspace{0.5cm}\input{Figures/Results/Legend_Res.tex}\\
    \vspace{0.2cm}
    \begin{subfigure}[t]{0.49\textwidth}
       \centering
        \input{Figures/Results/R_Poisson_Dirichlet_homogeneous.tex}
        \vspace{-0.4cm}
        \caption{Homogeneous Dirichlet.}
        \label{fig:Results:Poisson:homoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Neumann_homogeneous.tex}
        \caption{Homogeneous Neumann.} 
        \label{fig:Results:Poisson:homoNeumann}
    \end{subfigure}\\
    \smallskip
     \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Dirichlet_inhomogeneous}
        \vspace{-0.4cm}
        \caption{Inhomogeneous Dirichlet.} 
        \label{fig:Results:Poisson:inhomoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
         \input{Figures/Results/R_Poisson_Neumann_inhomogeneous.tex}
        \caption{Inhomogeneous Neumann.}
    \label{fig:Results:Poisson:inhomoNeumann}
    \end{subfigure}\\
    \smallskip
    \begin{subfigure}[t]{0.49\textwidth}
        \centering       
        \input{Figures/Results/R_Poisson_Mixed}
        \caption{Mixed.}
        \label{fig:Results:Poisson:Mixed}    
        \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Robin}
        \caption{Inhomogeneous Robin.}
        \label{fig:Results:Poisson:Robin}
    \end{subfigure}\\
    
    \caption{Comparisons of \textsc{VQA}-result (lines) and \textsc{FD}-results (symbols) for the steady heat conduction in combination with different boundary conditions on a grid with $N_\text{p}=4$ ($n=2$; dashed lines \& closed circles) and $N_\text{p}=16$ ($n=4$; straight lines \& open squares) interior points. The depth of the ansatz circuit $U(\lamb_c)$ is $d=1$ for $n=2$ qubits and $d=3$ for $n=4$ qubits, cf. \Fig{fig:VQA_Ansatz}.}
    \label{fig:Results:Poisson}
\end{figure}

As indicated in \Fig{fig:Results:Poisson}, the \textsc{VQA} predictions perfectly agree with the \textsc{FD} reference for all Dirichlet, Neumann, Robin, or mixed boundary conditions and grid resolutions. Furthermore, the first-order accuracy in the discrete approximation of the Neumann conditions is obviously detected in both the \textsc{VQA}- and the \textsc{FD}-results, cf. for example \Fig{fig:Results:Poisson:homoNeumann}. The required depth $d$ increases for non-periodic conditions on the finer mesh. To this end, a depth $d=3$ is sufficient to mimic all investigated boundary conditions in conjunction with the finer grid. 

\Tab{tab:Results:Poisson:Errors} quantifies the deviation of the \textsc{VQA}-results from the \textsc{FD}-results for all cases depicted in \Fig{fig:Results:Poisson}. The table displays a deviation of $\varepsilon_{l_2} \approx 10^{-6}$--$10^{-7}$ for two qubits ($N_\text{p}=4$), disregarding the imposed boundary conditions.

The good agreement of $\varepsilon_{l_2}$ for the periodic case, where no specific boundary condition circuits are required, and the non-periodic cases reveal that no substantial sensitivity of the attainable accuracy is observed when applying the current strategy for a quantum-based implementation of boundary conditions. For the finer discretization associated with $n=4$ qubits, the table shows higher values of $\varepsilon_{l_2} \approx 10^{-3}$ for the non-periodic boundary conditions and thereby a less satisfactory agreement with the periodic arrangement. The latter is attributed to difficulties of finding the global optimum in non-convex optimization and highlights a bottleneck of the \textsc{VQA} in combination with versatile ansatz functions $U(\lamb_c)$, cf. \Fig{fig:VQA}. Moreover, it also outlines that sufficient accuracy of the ancilla measurements is crucial for detecting the (global) minimum. 

The trace distance $\varepsilon_{\text{tr}}$ is given in the third column of \Tab{tab:Results:Poisson:Errors} and can be interpreted as point-wise correlation between the quantum- and the \textsc{FD}-result. The trace distance is related to the convergence to the global minimum, while the $\varepsilon_{l_2}$ measures the expressibility of the ansatz. Since the two measures address different aspects, considering just one of them seems insufficient. Moreover, the trace distance sometimes displays numerical zero values, cf. \Tab{tab:Results:Poisson:Errors}, which does not necessarily guarantee a perfect agreement and also advocates assessing both measures. In addition to the error measures used to assess the \textsc{VQA}-results, the origin of the observed differences in predictive accuracy are also of interest. 
%\trung{Check: Should we mention Sato?}  
Interestingly, the results reported by Sato et al. \cite{Sato2021} -for example- show a much better trace distance compared to the present results for periodic boundaries, although the predictive agreement of the current results appears to be slightly better.  A key difference between the current and similar recent efforts, e.g., \cite{Sato2021}, refers to the employed \textsc{\it SO4} ansatz illustrated in \Fig{fig:quantum_ansatz_SO4}, which seems to feature an improved ansatz expressibility but is also harder to train. 
Furthermore, the number of control variables $c$ given in \Tab{tab:Results:Poisson:Errors} roughly scales as $\mathcal{O}(n \, d)$, which 
%highlights an unfavorable complexity and 
suggests room for future improvements, in the design of the quantum ansatz circuits towards more problem specific strategies \cite{Holmes2022}. 

\begin{table}[htbp]
   \centering
    \begin{tabular}{@{}lcccccc@{}}
\toprule
Boundary Setting & \multicolumn{2}{c}{$l_2$-norm $\varepsilon_{l_2}$}  & \multicolumn{2}{c}{trace distance $\varepsilon_{\text{tr}}$}&\multicolumn{2}{c}{\textsc{DOF} $c$} \\ 
\midrule
\multicolumn{1}{r}{interior points}&\multicolumn{1}{l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$   \\
\midrule
Periodic          & \multicolumn{1}{c}{$1.23 \times 10^{-6}$}&\multicolumn{1}{c}{$3.26 \times 10^{-7}$}&\multicolumn{1}{|c}{$9.70 \times 10^{-1}$}&\multicolumn{1}{c}{$1.0 \times 10^{0}$}&\multicolumn{1}{|c}{$3$}&$6$\\
Homog. Dirichlet   & \multicolumn{1}{c}{$1.5 \times 10^{-7}$}&\multicolumn{1}{c}{$6.76\times 10^{-3}$}&\multicolumn{1}{|c}{$0.00$}&\multicolumn{1}{c}{$6.76 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Homog. Neumann   & \multicolumn{1}{c}{$1.37 \times 10^{-8}$
}&\multicolumn{1}{c|}{$5.05 \times 10^{-3}$}&\multicolumn{1}{c}{$6.32 \times 10^{-8}$}&\multicolumn{1}{c}{$5.05 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Inhomog. Dirichlet & \multicolumn{1}{c}{$8.49 \times 10^{-8}$}&\multicolumn{1}{c}{$7.87 \times 10^{-3}$}&\multicolumn{1}{|c}{$4.31 \times 10^{-7}$}&\multicolumn{1}{c}{$7.87 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Inhomog. Neumann  & \multicolumn{1}{c}{$1.68 \times 10^{-6}$}&\multicolumn{1}{c}{$2.55 \times 10^{-3}$}&\multicolumn{1}{|c}{$1.65 \times 10^{-6}$
}&\multicolumn{1}{c}{$2.55 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&$24$\\
Mixed   Dirichlet/Neumann          & \multicolumn{1}{c}{$6.01 \times 10^{-8}$
}&\multicolumn{1}{c}{$5.66\times 10^{-4}$
}&\multicolumn{1}{|c}{$0.00$}&\multicolumn{1}{c}{{$5.66
 \times 10^{-4}$}}&\multicolumn{1}{|c}{$3$}&$24$\\ 
Inhomog. Robin          & \multicolumn{1}{c}{$3.32 \times 10^{-9}$
}&\multicolumn{1}{c}{$3.7 \times 10^{-3}$
}&\multicolumn{1}{|c}{{$0.00$}}&\multicolumn{1}{c}{$3.7 \times 10^{-3}$}&\multicolumn{1}{|c}{$3$}&{$24$}\\ 
\bottomrule
\end{tabular}
\caption{Deviations of \textsc{VQA}- and \textsc{FD}-results in the $l_2$-norm ($\varepsilon_{l_2}$) supplemented by their trace distance ($\varepsilon_{\text{tr}}$) for results depicted in \Fig{fig:Results:Poisson}. The degrees of freedom (\textsc{DOF}) are indicated by the number of control variables~$c$.}
\label{tab:Results:Poisson:Errors}
\end{table}

\subsection{Transient Heat Conduction (Heat Equation)}
\label{sec:Application:Heat}
The second case deals with the transient heat conduction where the time derivative in \Eq{eq:Generic_PDE-TR-2} is treated as discussed in Sec. \ref{sec:Mathematics}. The contributions of the potential term $p(x,t)$ [1/s] as well as the physical source term $f(x)$ [K/s] in \Eq{eq:Generic_PDE-TR} are neglected. The diffusivity is again set to a unit value of $\nu=1$ [m$^2$/s]. Four different boundary condition settings are investigated using a constant time step of $\Delta t \nu/\Delta x^2 =1/(2^{\abs{n-3}}(N_p-n))$ in each of the four cases. The discretizations are the same two equidistant grids used in Sec. \ref{sec:Application:Poisson}, i.e., a coarse ($N_\text{p}=4$) and a fine grid ($N_\text{p}=16$). All cases studied should reach a steady state, and due to the different convergence speeds to the steady state, different time step numbers are shown for different boundary and initial conditions. The convergence of the optimizer is controlled by \Eq{alg:convergence} using a threshold level of $10^{-7}$ for two qubits and $10^{-4}$ for four qubits, respectively. 

The predicted temperature distributions are depicted in \Fig{fig:Results:Heat}, where arrows indicate the temporal evolution from the initial to the final time step, and  \textsc{FD}-results are again illustrated by open squares (fine grid) and closed circles (coarse grid). Mind that a larger scatter of depth $d$, cf. \Fig{fig:VQA_Ansatz}, is seen for the employed ansatz $U(\lamb_c)$  
which is motivated by the complexity of the initial solution as explained below. 
\begin{figure}[htbp]
\centering
\hspace{0.5cm}\input{Figures/Results/Legend_Res.tex}\\
\vspace{0.2cm}
    \begin{subfigure}[t]{0.48\textwidth}
       \centering
        \input{Figures/Results/R_Heat_Dirichlet_f1_homogeneous.tex}
        \caption{Solution obtained for the first 30 time steps with $y(x_k,t^0)=1$, using homogeneous Dirichlet conditions ($y = 0$) at both ends and $d=1$.}
        \label{fig:Results:Heat:homoDirichlet}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Dirichlet_f0_inhomogeneous.tex}
        \caption{Solution obtained for the first 20 time steps with $y(x_k,t^0)=0$, using inhomogeneous Dirichlet conditions ($y_{0} = 1, y_{N_\text{p}+1}=0$) and $d=5$.}
        \label{fig:Results:Heat:inhomoDirichlet}
    \end{subfigure}\\
    \smallskip
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Mixed_f0_inhomogeneous_nq2.tex}
        \caption{Solution obtained for the first 100 time steps with $y(x_k,t^0)=0$, using mixed boundaries ($y_{0}=1$, $\nicefrac{\partial y_{N_\text{p}+1}}{\partial x} = 0$) and $d=7$.}
        \label{fig:Results:Heat:mixed_nq2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Mixed_f0_inhomogeneous_nq4.tex}
        \caption{Comparison of coarse and fine grid results for the first seven time steps
        with $y(x_k,t^0)=0$ and $\Delta t = 1.67\times10^{-3}$[s], using mixed boundaries ($y_{0}=1$, $\nicefrac{\partial y_{N_\text{p}+1}}{\partial x} = 0$)  and $d=7$.} 
       \label{fig:Results:Heat:mixed_nq4}
    \end{subfigure}
    \caption{
    Comparisons of \textsc{VQA}-result (lines) and \textsc{FD}-results (symbols) for the transient heat conduction in combination with four different boundary conditions on grids with $N_\text{p}=4$ ($n=2$; dashed lines) and $N_\text{p}=16$ ($n=4$; straight lines) interior points.} %using constant time steps $\Delta t \nu/\Delta x^2 =1/(2^{\abs{n-3}}(N_p-n))$.}
    \label{fig:Results:Heat}
\end{figure}

\Fig{fig:Results:Heat:homoDirichlet} shows the results obtained for the 
homogeneous Dirichlet problem over the first 30  time steps. Since the results for the two grids are very similar, we mostly confine the discussion to coarse grid results for the sake of brevity. The initial solution was assigned to $f(x_k, t^0)=1$ in the interior, which yields negative heat fluxes at the boundaries in combination with imposed homogeneous Dirichlet boundaries. The figure indicates an excellent agreement between the \textsc{VQA}-results and the \textsc{FD}-results. This also applies to the results obtained for the inhomogeneous Dirichlet problem depicted in  \Fig{fig:Results:Heat:inhomoDirichlet}, where the initial solution refers to $f(x_k, t^0)=0$ in the interior domain, and a constant heat flux from the left to the right is predicted at the twentieth time step. An interesting detail refers to the increased depth $d$ of the ansatz circuit $U(\lamb_c)$, cf. \Fig{fig:VQA_Ansatz}. The increase is explained by the different initial conditions and the related steep solution in the initial phase that requires a deeper ansatz circuit, even when using the fairly rich \textsc{\it SO4} approach for $\tilde U(\lamb_i)$. On the other hand, deeper circuits are afflicted with more parameters to be optimized, and optimization effort could be reduced for lowered depth circuits as the solution advances to the simpler steady state.

Results obtained for a mixed Dirichlet/Neumann problem are outlined in \Fig{fig:Results:Heat:mixed_nq2} and \Fig{fig:Results:Heat:mixed_nq4}. The initial temperature distribution is assigned to $y(x_k,t^0)=0$ in the interior as well as the right side Neumann boundary. The final solution should agree with the left side Dirichlet value $y(0,t^l)=1$ in the whole domain. For the coarse grid, $N_\text{t} = 100$ time steps are displayed in \Fig{fig:Results:Heat:mixed_nq2}. They indicate a remarkable visual agreement between the \textsc{VQA}-results and the \textsc{FD}-results over the entire simulation period. In line with the \textsc{FD}-results, the \textsc{VQA}-results unveil that the temperature on the right increases for the adiabatic condition until the global heat exchange finally vanishes. 
%
{Figure \ref{fig:Results:Heat:mixed_nq4} compares the evolution of the solution on the coarse and the fine mesh for the initial $N_\text{t} = 7$ time steps. Results indicate that the predictive accuracy is similar on both grids.}

The time evolution of the $\varepsilon_{l_2}$ measure is displayed, using a \textit{log-log} representation in \Fig{fig:Results:Heat:Error:nq2} and a \textit{semi-log} representation in \Fig{fig:Results:Heat:Errors:mixed_nq4}. For the inhomogeneous Dirichlet and the mixed boundary condition, the maximum error occurs during the initial time steps and decays as the solution advances in time until approximately $t=0.1$s (5 time steps).
Subsequently, the measure remains at a low level for these cases. For the homogeneous Dirichlet case with $d=1$, displayed in \Fig{fig:Results:Heat:homoDirichlet}, the error increases significantly after approximately 10 time steps but remains small. 
In contrast, the ansatz with $d=7$ that was used to compute the homogeneous steady state solution depicted in \Fig{fig:Results:Heat:mixed_nq2} outperforms the trainability in the homogeneous Dirichlet setting ($d=1$).  

Despite a general temporal error transport, the implicit numerical scheme remains stable and does not indicate any amplification of the error, which is in the range of the error of the steady-state solution, cf. Sec. \ref{sec:Application:Poisson}. 


\begin{figure}[htbp]
\centering    
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Errors_nq2.tex}
        \caption{Evolution for coarse-grid results displayed in \Fig{fig:Results:Heat:homoDirichlet}-\subref{fig:Results:Heat:mixed_nq2}.} 
        \label{fig:Results:Heat:Error:nq2}
    \end{subfigure} 
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Errors_Mixed_f0_inhomogeneous_nq4.tex}

        \caption{Evolution of fine-grid results displayed \Fig{fig:Results:Heat:mixed_nq4}.}
    \label{fig:Results:Heat:Errors:mixed_nq4}
    \end{subfigure}
    \caption{Temporal evolution of the deviation measure ${\varepsilon^l_{\text{l}_2}}$ for the results displayed in \Fig{fig:Results:Heat}.}
    \label{fig:Results:Heat:Errors}
\end{figure}

As indicated by \Fig{fig:Results:Heat:Error:nq2}, the 
maximum values agree with the results of the steady heat conduction case provided by  \Tab{tab:Results:Poisson:Errors}. The corresponding 
\Tab{tab:Results:Heat:Errors} lists the time-averaged values of the $l_2$-norm $\Bar{\varepsilon}_{\text{l}_2}$ and the trace distance measure $\Bar{\varepsilon}_{\text{tr}}$.   Since the changes of the solution over time are small, maximum values of $\Bar{\varepsilon}_{\text{l}_2}$ and $\Bar{\varepsilon}_{\text{tr}}$ are bounded, and the averaged values remain within the range of the steady state results.
%er for the transient than for the steady case due to the favorable restart influences of the time-marching procedure on the optimizer. {Despite this, the alluded agreement of the transient homogeneous Dirichlet and the periodic case is again clearly visible by the trace distance $\Bar{\varepsilon}_{\text{tr}}$.}   

\begin{table}[htbp]
   \centering
    %%Table caption below according C&F Guide
    \begin{tabular}{@{}lcccccc@{}}
    \toprule
Boundary Setting & \multicolumn{2}{c}{$l_2$-norm $\Bar{\varepsilon}_{\text{l}_2}$}  & \multicolumn{2}{c}{trace distance $\Bar{\varepsilon}_{\text{tr}}$}&\multicolumn{2}{c}{DOF $c$} \\ 
\midrule
\multicolumn{1}{r}{interior points}&\multicolumn{1}{l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$& \multicolumn{1}{|l}{$N_\text{p}=4$}& $N_\text{p}=16$  
\\
\midrule
Homog. Dirichlet  & \multicolumn{1}{c}{{$6.70 \times 10^{-6}$}}&\multicolumn{1}{c|}{-}&\multicolumn{1}{c}{{$4.63
 \times 10^{-5}$ }
}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{$3$}&-\\
Inhomog. Dirichlet & \multicolumn{1}{c}{$1.84\times 10^{-8}$
}&\multicolumn{1}{c|}{-}&\multicolumn{1}{c}{$2.77\times 10^{-7}$ }&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{$27$}&-\\
Mixed             & \multicolumn{1}{c}{$8.08 \times 10^{-8}$
}&\multicolumn{1}{c|}{{$2.42 \times 10^{-3}
$}}&\multicolumn{1}{c}{$2.1 \times 10^{-8}$}&\multicolumn{1}{c}{{$1.71 \times 10^{-3}$}}&\multicolumn{1}{|c}{$39$}&$60$\\
    \bottomrule
    \end{tabular}
   \caption{Time-averaged deviation measures $\Bar{\varepsilon}_{\text{l}_2}$ and $\Bar{\varepsilon}_{\text{tr}}$ for the results depicted in \Fig{fig:Results:Heat}. The degrees of freedom (\textsc{DOF}) are indicated by the number of control variables $c$.}
    \label{tab:Results:Heat:Errors}
\end{table}

==> Container/C_Feb27/highlights.tex <==
\begin{center}
    {\Large
Highlights
}
\end{center}

%Highlights should be submitted in a separate editable file in the online submission system. Please use 'Highlights' in the file name and include 3 to 5 bullet points (maximum 85 characters, including spaces, per bullet point).

\begin{itemize}
    \item Variational Quantum algorithm to solve initial-boundary value problems. 
    
    \item Quantum Computing-ready implementations of Dirichlet, Neumann, and Robin conditions.
    
    \item Robust boundary treatment, without additional ansatz or framework requirements. 
    
    \item Excellent agreement with classical finite differences results for heat transfer. 
    
    \item A remarkable \textit{polylog} complexity in the number of grid points or corresponding qubits. 
\end{itemize}


==> Container/C_OldSections/ComputationalStrategy.tex <==
%###########################################
%       Computational Strategy
%###########################################
\section{Computational Strategy} \label{sec:Strategy}
On a Classical Computer (\textsc{CC}), the discrete optimization problem introduced in Sec. \ref{sec:Discretization} can be implemented following the known procures. The solution is encoded by a certain number of bits, which is proportional to the number of grid points $N_\text{p}+2$ and their numerical resolution, i.e. the floating-point arithmetic. On a Quantum Computer \textsc{QC}, the processing of information is executed on qubits, being the bit counterparts. Analogue to the CC, are the qubits again collected in a register. In the scope of this work, we practice the Big-endian standard.

For the discretization introduced, a quantum register, assembled with $n$ qubits to represent $N_\text{p} = 2^n$ discrete points, is required. The ghost-points values are represented classically. Each of the $n$ qubits recovers two distinguishable states, e.g. in Dirac notation as $\ket{0}$ and $\ket{1}$. The abbreviation, $\ket{0}$ and $\ket{1}$, refer to the first and second orthonormal basis of the given vector space \cite{Nielsen2010}. Straightforward, a quantum register $\ket{\psi}$ with $n$ qubits contains the basis states $\ket{\psi} = \ket{\psi_1} \otimes \ket{\psi_2} \otimes \hdots \otimes \ket{\psi_n}$, where $\ket{\psi_n} = \alpha_n \ket{0} + \beta_n \ket{1} :~\alpha_n,\beta_n~\in~\mathbb{C}$. 
This encoding allows the representation of high resolved function values $u_k \in \mathbb{C},u : \bra{u}\ket{u}=1$ at each $x_k \in \O$, represented by the complex amplitudes of the quantum state, as it is given in \Eq{eq:discretization_register}. \pover{Is this a Carleman embedding?} The numerical resolution of an entity (e.g. $u_k$) at the grid point itself, is independent of the number of qubits $n$. In contrast to a \textsc{CC}, this is one great advantage. However, the normalization condition: the partition of unity (c.f. \Eq{eq:partition_of_unity}), of the quantum physical system must always be fulfilled. Mention that, increasing the number of qubits $n$ to achieve higher resolutions, the amplitudes of $u_k$ are increasingly compressed to conserve the partition of unity. Restricted to single or double precision, this limits the measurements possibilities. Despite, the map $\ket{\text{bin}\left(k\right)}: k \mapsto \ket{\text{binary}\left(k\right)}$, delivers the $k^{th}$ orthonormal basis of the underlying Hilbert space. Accordingly, the values $u_k$ in spatial dimension $x$ can be encoded by $\ket{u} = \sum\limits_{k=1}^{\text{N}_p}u_k \ket{\text{bin}\left(k-1\right)}$, where $u_k$ refers to the amplitude of $u$ at $x_k$. Mention, that the complex conjugate amplitude $u_k^* =  u_k$, assuming only real solutions of \Eq{eq:Generic_Opt}.

\pover{I dont think the normalization cont. needs to be transformed to discrete space -  y= lamb u }
Since the solution $y(x)$ of \Eq{eq:Generic_PDE} is continuous in space, the discretization affects the normalization. Discretizing the continuous representation of the normalization condition by the midpoint rule results in 
\begin{align}
    1 = \sum \limits_{k=1}^{\text{N}_p} y_k^* y_k\Delta x = \sum \limits_{k=1}^{\text{N}_p}  \lambda_0^2 u_k^* u_k.
    \label{eq:normalizedf}
\end{align}

With the hardware requirements in mind, the following section aims to cover the approximation of the solution to the problem given in \Eq{eq:Generic_PDE} using \textsc{VQA} initially presented in the same structure by \cite{Lubasch2020}. 

%###########################################
%       Variational Quantum Algorithm
\subsection{Variational Quantum Algorithm}
The \textsc{VQA} methodology is to minimize an underlying objective $J$, by variationally optimizing a control $\upb$. For the variational method, a qubit registers $\ket{\psi}$ is initialized with the computational basis state $\ket{0}$ and is used as an input to a quantum circuit composed of a predefined series of quantum operations, so-called gates, modulating the PDE dynamics. The framework is highly dependent on the problem, which determines the arrangement of the gates, their actions, and the type of measurement. In addition to this, a gate always requires being unitary to respect the partition of unity (given in \Eq{eq:partition_of_unity}). In classical CFD, this requirement does not exist, which make unitarization one key discipline in the compilation to quantum hardware. With respect, it is possible to structure the compiled quantum circuits into the following four parts, see \Fig{fig:VQA}:

\begin{enumerate}
     \item The upper qubit, so-called ancilla, is intended for indirect measurements according to the Hadamard test \cite{Endo2020}. The register $\ket{\psi}$ is therefore augmented by another qubit, to the whole register $\ket{0}\otimes\ket{\psi}$. One can show that the expectation value results in $\mathcal{R}\left(\bra{\psi}U\ket{\psi}\right)$, where $\mathcal{R}$ denotes the real-part \cite{Nielsen2010}. Comparing the expectation value given, with the expression in \Eq{eq:Generic_Opt}, underlines the similarity of the expressions to that appearing in the bilinear-form $a(\cdot,\cdot)$. The advantage of indirect measurement in contrast to direct measurement is to reduce to a single measurement, instead of multiple measurements $M$, see \Fig{fig:VQA_QNPU}. Secondly, experiments with the Hadamard test showed Quantum supremacy in comparison to CC \cite{Guseynov2023}.
        
    \item The parameterized ansatz $u(\lamb)$ spans the normalized ansatz function space $Y :  \| Y\|=1$.  $u$, and thus is crucial to express a qualitative approximation to the true solution $y_\Omega$. Training the ansatz parameters to transform the initial state $\ket{\psi}$ to the best approximation $y$ is the  a crucial part of the \textsc{VQA} method. Therefore, one distinguishes between expressibility and trainability in terms of ansatz characterization \cite{Tilly2022}.   To achieve a most optimal span in the category of fixed structure and hardware efficient ansatz, we rely on the advanced SO4 two-qubit Ansatz, given by \cite{Vatan2004}. It is visualized in \Fig{fig:quantum_ansatz_SO4}. The gates are $S_1 =R_z(\nicefrac{\pi}{2})$, $R_1=R_y(\nicefrac{\pi}{2})$, $A=R_z(\lambda_1)R_y(\lambda_2)R_z(\lambda_3)$, and $B=R_z(\lambda_4)R_y(\lambda_5)R_z(\lambda_6)$. By using the whole assembly, the parameterization $\lamb$ refers to a subset in the control $\upb$ in \Eq{eq:Reduced_Opt} and thus for the  SO4  ansatz in $\lamb=(\lambda_1,\lambda_2,\hdots,\lambda_6)^\intercal$. To modulate the capabilities of the base ansatz, the depth $d$ of the ansatz circuit can be scaled. With rising depth $d$, more revolutions of a basis ansatz are added and structured in a bricklayer fashion. The parameters are kept unique. \pover{Why bricklayer ?\cite{Uvarov2021, Tilly2021}}. Accordingly, the register $\ket{\psi}$ concludes in $u(\lamb)\ket{0} = u$.

    The use of $R_z(\cdot) \in \mathbb{C}^{2\times 2}$ involves imaginary values, which is the cost to pay for a more complex space encoding. It is a difference in contrast to \cite{Sato2021,Leong2022}. The resulting phase modulation requires to be corrected after the measurement. By choosing the ansatz in Lie Group \textit{Special-Orthogonal-4} the problem characteristic as optimization under unitary matrix constraint gets again clear.    
\pover{adapt rho is applidudes flip sign}
\pover{Parameter scale to [0, 2pi)}
 
    \item The transformation $T_t$ aligns the order of the amplitudes in the register $\ket{\psi}$, according to the subsequent QNPU. It is a feature, which is not described in \cite{Lubasch2020} and modularizes the building blocks of the VQ-assembly even more. In many cases $T_t= I$, expect the cases where it is mentioned separately. 

    \item The Quantum Nonlinear Processing Unit (\textsc{QNPU}) is a succession of quantum gates, representing PDE effects of the system, e.g. in  \Fig{fig:VQA_QNPU}. In the current case, the QNPU is required to represent the discretized dynamics of \Eq{eq:Generic_PDE} represented by the functionals $j_i$. Each term $J_i$ of $J$ is evaluated individually. Based on the order of nonlinearity $\xi$ of \Eq{eq:Generic_PDE}, the number of inputs $r$ is increased to point-wise multiply various copies. 
\end{enumerate}

\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \input{Figures/QNPU.tex}
        \caption{Schematic sketch of a \textsc{VQ} circuit composed by the \pover{Ansätze ? } $^ru(\lamb)$, the $T_t$ assembly, a specific \textsc{QNPU}, and a measurement qubit (ancilla qubit) for indirect measurement technique. $H$ indicates a Hadamard gate, \textsc{CP}$_i$ Control Port, \textsc{IP}$_i$ Input Port, \textsc{OP}$_i$ Output Port, and $\sigma_z$ the expectation value at the measurement operation, c.f. \cite{Lubasch2020}.}
        \label{fig:VQA_QNPU}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \input{Figures/Ansatz.tex}
        \caption{Exemplary topology for one $u(\lamb)$ Ansatz circuit composed out of $g$ fundamental gates structured in a bricklayer fashion and parameterized by $\lamb = (\lamb_1, \lamb_2,\hdots, \lamb_g)^\intercal$ parameters encoding a test function on $n = 6$ qubits, c.f. \cite{Lubasch2020}.}
        \label{fig:VQA_Ansatz}
    \end{subfigure}  \\
    \begin{subfigure}[c]{0.45\textwidth}
        \centering
        \input{Figures/SO4_ansatz}
        \caption{Two qubit Ansatz to create an optimal variational state \cite{Vatan2004}.}
        \label{fig:quantum_ansatz_SO4}
    \end{subfigure}    
    \caption{Visualization of fundamental VQA elements for the implementation of the exploit paradigm.}
        \label{fig:VQA}
\end{figure}

The quantum circuit given, the minimization of the cost function $J$ can be realized in a hybrid classical-quantum algorithm, which is common to all VQA methodologies. \Fig{fig:optimizer} sketches the hybrid quantum-classical framework, extending the structure given in \Fig{fig:VQA}.



The objective $J$ is evaluated mainly on the quantum device, which is controlled by the outer classical counterpart. The classical part has in both cases full control on the quantum-based parametrization of the objective and thus over the solution, which is parameterized by the Ansatz $ u(\lamb)$. The objective is evaluated individually for each larger summand $j_l$ of \Eq{eq:Discrete_Opt_BC}. The evaluation of the quantum device is commonly done using $M$ samples. The number of samples determines the accuracy of the expectation value. Here the sampling complexity gives an insight. In the following, we restrict the information description by tracing out the subsystem “QNPU register” and using the corresponding density matrix of the ancilla, incorporating the partial trace, to approximate the expectation at the measurement gauge, given in \Fig{fig:VQA_QNPU}.  By this, the result of a state-vector simulation recovers the same effect as intended by the indirect measurement performed on real hardware, without noise and sampling errors \cite{Nielsen2010}. The investigation of the proposed library on NISQ devices is motivated for future research. The Ansatz and parameters $\lamb$ are kept identical for each term $j_l$. In the outer classical loop, the determined value is scaled and assembled to $J$. Consequently, an update $\delta\upb$ is to be determined, to update the parameters $\upb$ for the next iteration $i$. To efficiently update, knowledge about a descent direction is necessary. As known from optimal control theory and the subject of optimization, first-order methods outperform zero-order optimization methods quickly. 

Since the derivative, follows the chain and product rule, taking the derivative of the ansatz and thereby the gate sequence cannot be bypassed. The ideas presented in \cite{Stokes2020,Bittel2022,Schuld2019} can be used to obtain an approximation to the derivative of $J$ on the quantum hardware, without deriving a new gate sequence. The ideas follow some finite difference approximation of the derivative in the quantum framework. The application of the idea to the framework realized is introduced in the Sec. \ref{sec:Derivative}. In the following, a library of QNPUs for application in the VQA assembly is introduced in detail

\subsection{Compilation of the Quantum-Nonlinear-Processing-Units}
\label{sec:Compilation}
With the availability of quantum tools, namely indirect measurement and function space encoding, it is possible to derive a quantum compilation. For the introduction of our library of QNPUs we use a complex number notation. All QNPUs are extendable to arbitrary fine one-dimensional discretization and have been designed to keep the gate sequence shallow. The set of to-be-presented QNPUs cover dynamics, which commonly occur in PDEs, as in the form of that given in \Eq{eq:Generic_PDE} and as they are common for CFD. Despite the fact, that $\xi = \zeta = 0$, we will introduce two QNPUs for the case  $\xi \neq 0, \zeta \neq 0$.  
In the cases of external effects as by an external source $f$ or, the potential $p$ the compilation to quantum hardware needs to be available. In terms of trigonometric contributions, the publication by \cite{Lubasch2020} introduces gate sequences for $e(x)$, $sin(\kappa x)$ and their superpositions based on the Matrix-Product-State formalism as a programming paradigm. In this direction, the references \cite{Oseledets2012,GonzalezConde2023} deploy additional compilations for polynomials. For more advanced functions, the subject of TT-cross approximation techniques can also be used to approximate the corresponding gate sequences \cite{Oseledets2010}. To give the reader a detailed overview of the Quantum circuits, each compilation is sketched in a small example to extract the general pattern.

\pover{ADD a comment on higher dimensions  :  Check Sato P 4}

\subsubsection{The Laplace} \label{sec:Compilation:Laplace}
The Laplacian is one of the most frequently differential operators when it comes to PDEs in the context of CFD. Hence, it is a necessity to derive a robust and flexible compilation for the quantum hardware. Inspecting the finite difference stencil in \Eq{eq:derivatives_space}, a similitude to the classical bit shift operator can be stated. With a discretization of $n\leq 2$ the half-adder circuit is used. Beyond, it is limited, and additional carry bits become a necessity. For the construction of the now-demanded, full adder circuits as well as the theory, the reader is referred to literature on classical computing \cite{Parhami2010} and \cite{Lubasch2020,Darper2000,Nielsen2010}. The full adder as used in the QNPU for the Laplace operator has already been developed in the work of \cite{Lubasch2020}. \pover{ofcourse there are other approaches, \cite{Liu2021} presents a general decomposition method. \cite{Sato2021} shows a decomposition splitting the QNPU for the periodic terms into two....  }For the sake of completeness, it is introduced by starting at the \Eq{eq:derivatives_space}. It can be shown, that the equation can be reduced to three terms $u_k^* u_{k+1},\; u_k^* u_{k} \;\& \;u_k^* u_{k-1}$, where the first and last request a multiplication by a shifted value. For closure, periodic BC simplifies the expression until a certain point. Accordingly, one can give the general structure of the discretized Laplace operator which acts on a state-like, \cite{Lubasch2020} 
\begin{align}
\label{eq:Laplace}
    \sum\limits_{k=1}^{N_\text{p}}u_k \ket{\text{bin}\left(k-1\right)} \to  \sum \limits_{k=1}^{N_\text{p}} u_{k+1} \ket{\text{bin}\left(k-1\right)}.
\end{align}
The final circuit is shown in \Fig{fig:Laplace_compiled} e.g. $n=6$.

\begin{figure}[htbp]
    \centering
    \input{Figures/Adder.tex}
    \caption{Quantum circuit for the Laplacian term for $n=6$, in the Hadamard test configuration. In practice, the input $\ket{\psi}$ is given by an ansatz, e.g. as introduced in \Fig{fig:quantum_ansatz_SO4}. For $n=2$ qubits, this circuit is exactly implementing a half-adder, c.f. \cite{Lubasch2020}.}
    \label{fig:Laplace_compiled}
\end{figure}

 %As a proof of concept, mention that the quantum registers for $n=2$ qubits can be decomposed in its complex amplitude as, $\ket{\psi} = \left(c_{00},c_{01},c_{10},c_{11}\right)^\intercal$. It can be shown that the initial state $ \ket{\phi_0} = \ket{0} \otimes \ket{\psi} = \ket{0} \otimes \left(c_{00}\ket{00}+c_{01}\ket{01}+c_{10}\ket{10}+c_{11}\ket{11}\right)$ evaluates to $ \langle\sigma_z\rangle =   \sum\limits_{k=0}^{NP-1}\psi_k\psi_{k+1}$, assuming real function values and periodicity.
 
\paragraph{Boundary Conditions}\label{sec:Compilation:BC}
Given the Laplacian for a periodic setting, we now introduce the novel approach to generalize the implementation to a more general setting, which is mandatory for the transformation to industrial application. 

As a benefit of the ghost point implementation introduced in Sec. \ref{sec:Discretization} the adaption to different BC is just a question of finding the corresponding gate sequence. Furthermore, as mentioned above in the derivation of the Laplace operator, is the assumption of periodic BC's crucial. This fact needs to be given for the Laplacian, but of course, can be corrected by another QNPU. In the following, we would like to present another two circuits to adjust the field dynamics to the boundary setting and to link internal and external discretization.

As a prelude, to mention the transformation $T_t$, given by \cite{Sato2021}, acting on $u_k$, like an anti-diagonal matrix on a vector, by the action
\begin{align}
    \label{eq:shift}
    \sum\limits_{k=1}^{N_\text{p}}u_k \ket{\text{bin}\left(k-1\right)} \to  \sum \limits_{k=1}^{N_\text{p}} u_{k} \ket{\text{bin}\left(k \text{ mod } N_\text{p} \right)}.
\end{align}
To correct the discretized dynamics in the previously given operator, this transformation is required to align the quantum register for the following modifications. An exemplary compilation of the transformation $T_t$ is given in \Fig{fig:Transformation}, which can be implemented as sketched in \Fig{fig:VQA_QNPU}. 

\begin{figure}[htbp]
    \centering
    \input{Figures/Transformation}
    \caption{A generic shift operator represented by a sequence of multi-controlled Toffoli gates, exemplary given for $n=4$ qubits. In the following, referred as transformation $T_t$, c.f. \cite{Sato2021}.}
    \label{fig:Transformation}
\end{figure}

With the transformed register available, the implemented actions of the Laplace operator can be transformed. In contrast to the approach of \cite{Sato2021} and \cite{Leong2022}, the BC correction on the periodicity can be represented as unitary circuits and therefore as quantum gates for an arbitrary number of qubits. In the case of Dirichlet (\Fig{fig:QNPU_BC_Dirichlet}) and Neumann BC's (\Fig{fig:QNPU_BC_Neumann}), the circuits in \Fig{fig:QNPU_BC} are required as additional QNPUs.

\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{0.49\textwidth}
       \centering
        \input{Figures/Dirichlet.tex}
        \caption{Compiled QNPU for the implementation of Dirichlet boundary conditions by realization of $j_2$ in \Eq{eq:Discrete_Opt_BC}}
        \label{fig:QNPU_BC_Dirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Neumann}
        \caption{Compiled QNPU for the implementation of Neumann boundary conditions by realization of $j_3$ in \Eq{eq:Discrete_Opt_BC}. It is required to be used together with the Dirichlet QNPU.}        \label{fig:QNPU_BC_Neumann}
    \end{subfigure}  
    \caption{Visualization of the novel Boundary Correction QNPU elements in an exemplary $n=4$ qubits setup as augmentation to the Laplace QNPU.}
    \label{fig:QNPU_BC}
\end{figure}

\subsubsection{The Potential} \label{sec:Compilation:Potential}
This section covers the quantum computational evaluation of the bi-linear term covering the potential $p(x)$. After application of the discretization technique according to \Fig{fig:discretization_encoding}, can the bi-linear term be written as
\begin{align}
    \sum\limits_{k=1}^{\text{N}_p} \lambda_0^2 u_k^*p_k u_k.          
    \label{eq:P_dis}
\end{align}

The potential contribution is modeled by an inner product of an external potential $p\left(x\right)$ and the solution $y\left(x\right)=\lambda_0 u(x)$, which can be interpreted as a discrete point-wise multiplication over space. To encode the external potential  $p\left(x\right)$ on the quantum hardware, multiple approaches exist to derive the corresponding gate sequence $P$. References are given in Sec. \ref{sec:Compilation}. The compiled QNPU circuit assembled by multi-controlled NOT gates is given in \Fig{fig:potential_measuremment}. 

\begin{figure}[htbp]
    \centering
    \input{Figures/Potential.tex}
    \caption{The quantum circuit based on the Hadamard test for the discrete potential function $\pb=( p_1, p_2,p_3, p_4)^\intercal$, e.g. given in a $\text{N}_p=4 \rightarrow n=2$ qubit setup, which shows the pattern for a full extension to a $\text{N}_p$ point discretization.}
    \label{fig:potential_measuremment}
\end{figure}

%Assuming $n=1$ and $\ket{\theta_0} = \ket{0\psi0}$ as the initial state, a small sketch would deliver the expectation value $ \langle\sigma_z\rangle = \frac{1}{2} \sum \limits_{k=1}^2\psi_k^*v_k\psi_k + \psi_kv_k^*\psi_k^*$, which can be simplified to $\langle\sigma_z\rangle =\sum\limits_{k=1}^{2} \psi_k v_k \psi_k$ assuming real functions.

\subsubsection{Generic Source Terms} \label{sec:compilation:source}
Besides the terms above, the \Eq{eq:Generic_PDE} holds a RHS given as $f$, referred to as the source term. It differs a lot from the compilations introduced.  Given in the linear form $F$ of the variational \Eq{eq:variational_eq}, it is only multiplied by the test function ones, resulting in a linear expression. Compared to the other operators above, which are quadratic in the test function, this is an important difference. Again, for the derivation of special gate compilations, the reader is referred to \cite{Oseledets2012,Lubasch2020,GonzalezConde2023}, the detailed description is given in sec. \ref{sec:Compilation}. Assuming there is a gate sequence representing $f$, the RHS can be implemented by using the QNPU given in \Fig{fig:overlapp}. Instead of the uncontrolled ansatz $u_1(\lamb)$, the linearity of the source terms, requires that the ansatz  $u_1(\lamb)$ is controlled, analog to $u_2(\lamb)$ in \Fig{fig:VQA_QNPU}.

\begin{figure}[htbp]
    \centering
    \input{Figures/Overlapp.tex}
    \caption{The implementation of the external source $f$ is realized by the overlapp $\ket{u}\bra{f}$. In the common case $T_t = I$.}
    \label{fig:overlapp}
\end{figure}
 
As already introduced in sec. \ref{sec:Discretization}, requires an inhomogeneous boundary setting the augmentation of the source term $f$ by $f_\text{ghost}$. The additional $f_\text{ghost}$ is simultaneously compiled into a circuit as given above and substituted in the circuit given in \Fig{fig:overlapp}, underlying the modularity of the framework. As a final step, mention that the discretized time derivative, can be written an additional RHS. Thus, using an augmented form allows a direct implementation using the same approach.
\pover{scalar product phase shift correction -  expectation value in code L. 231 source/objectives \TODO{Do we still need this correction?}}

\subsubsection{Gate complexity}
To investigate on the scalability of our algorithm, we illustrate the relations of qubits with the number of gates for all the circuits composing the QNPU and the SO4 ansatz. Note that the gate complexity of the ansatz depends on the type and depth selected, and is case dependent. However, we have included the gate complexity of the used SO4 ansatz w.r.t to depth and $n$ to give the reader a comprehensive view on the total complexity of the VQA used in this work. 

The results are depicted in \Fig{fig:compilation:GateComplexity}. The right-hand-side of this figure shows the polynomial of order x \sbengoechea{(linear?) to find out the polynom order)} relation of the number of gates of the ansatz w.r.t. to the number of qubits. The same polynomial \sbengoechea{(to check the order)} behavior is found for the Laplacian QNPU as can be seen in the left-hand side of the same figure. This complexity of the Laplacian circuits is due to the local effect of the discrete stencil for approximating the second space derivative, in this case the resulting circuit conserves this local property. On the other hand, the QNPUs for the boundaries show an exponential increase in the number of gates w.r.t. the number of qubits. 

%\pover{Of cource , boundary conditions sclae expontially, as it is observed in \cite{Sato2021,Leong2022,Leong2023}, hence the effect of them is not bind to a local behaviour and thus requires a multi quibit interaction, which scales naturally with the number of sites. The compiled circuit we show nevertheless, allows to represent this non hermtian effect in a robust manner on quantum hardware. A mask can be used or as sato does , a measurement on only a single quibit can be done..\textbf{}\textbf{}} 

\sbengoechea{The non-unitary approach/Matrix to BC proposed by Sato is here adapted to unitary.}

Hence, the effect of the BC is not bind to a local behavior and thus requires a multi qubit interaction, which scales naturally with the number of sites. The compiled circuit we show, nevertheless, allows representing this non-unitary effect of the BC robust on quantum hardware. 
The circuits reproduce the global property of the boundaries for elliptic PDEs, namely the BC influence affects the complete domain. This conclusion can also be observed in the shape of the gates given in \Fig{fig:Transformation}, \Fig{fig:QNPU_BC_Dirichlet}, and \Fig{fig:QNPU_BC_Neumann} where multi-controlled Toffoli gates scale with the number of qubits. The same behavior is found in the approaches used in \cite{Sato2021,Leong2022,Leong2023}. 

\pover{I would remove the idea how to improve the scalability  - lets move it to the outlook. }
In the case of Neumann boundaries, an improvement in the scalability can be achieved by substituting the Neumann circuit of \Fig{fig:QNPU_BC_Neumann} by a mask implemented via the Potential circuit. For this time the potential circuit does no need a state preparation since the task can be split in two with the initialization of $\ket{00...00}$ and $\ket{00...01}$ for the left and right boundary respectively. Note that, the exponential scaling does not vanish completely since the Dirichlet circuit it is still necessary to remove the corners of the antidiagonal, also for the Neumann conditions. This alternative would reduce only the exponential scaling of one of the circuits.  
Another option is to measure state of the single qubit encoding the boundary point, as Sato does, or in our case the point next to the ghost point. With that information on that point, a mask can be applied to achieve the desired value at the boundary. Although this idea would correct the exponential scaling, it would also require more measurements and classic treatment on the boundaries, breaking the full quantum evaluation of the algorithm. 

For the two remaining QNPUs, Source and Potential, the same exponential scaling is observed. The reasoning, is the realization of the external contributions $f,p$. The QNPU given, scales linearly in the number of controlled-CNOT gates and underlines the importance of an efficient implementation of $f,p$.  Although necessary, this step is reported to be expensive and non-efficient \cite{Chen2021,Kyriienko2021,Creevey2023} and work is being invested in this topic \cite{Creevey2023,Melnikov2023,Araujo2021}. 

\begin{figure}[htbp]
    \centering
    %\includegraphics[width=0.45\textwidth]{Figures/Gate_complexity_QNPU.png}
    %\includegraphics[width=0.45\textwidth]{Figures/Gate_complexity_Ansatz.png}
    \TODO{Uncomment files}
    \caption{Gate complexity for all used QNPUs w.r.t he number of qubits. The circuits are first decompose in single qubits gates (Rz,Ry, u, u3) and two qubits gates (cx) and then added. For  the sake of completeness, the number of gates per qubits for the ansatz SO4 is also reported.}
    \label{fig:compilation:GateComplexity}
\end{figure}

\TODO{Gate complexity with sinus as f in source and potential. Remove exponential curves for potential and source. Give only the complexity curve for circuits w/o state vector preparation.}

\sbengoechea{As for the laplacian it is easy to see that the circuits for overlap and potential are efficient up to the shape of the function to be read. We do not include in this analysis the state vector preparation costs. However, in our study we have applied the state vector preprataion to encode the generic functions in the PDE which leads to an exponential scaling in many cases. We have concentrated in to algorithmic point of view. }

Another important aspect is the algorithm behavior w.r.t. shot noise. In our case, the use of the measurement approach explained in Sec. \ref{sec:Compilation}) avoids the shot measurement to recover the expectation value. Therefore, the stability/robustness against shot noise of the approach has not been investigated in this publication. We refer the reader to \cite{Lubasch2020} where it is reported that the order of measurements $M$ on the ancilla for the potential is independent of $n$ while for the Laplacian QNPU \pover{and non-linear term} $M$ increases exponentially with $n$. 

\pover{quote on sato section C  .  Quantum circuit for the shift operator
are already been marked as inefficient by \cite{Sato2021}, claiming the use of multi-controlled Toffoi gates as major bottleneck to create shallow circuits. As alternative may use \cite{Liu2021}  as decomposition approach , but scales less efficient. In terms of our approach only the bilinear form a(,) and the Linear operator F need to be measured. Which is an improve compared to \cite{Liu2021, Sato2021} <- Check }


\subsection{Derivative Computation} \label{sec:Derivative}
%Section \ref{sec:Mathematics} finalized by stating the first-order optimality condition. To complete the shift to quantum hardware, this detail is the only missing. Therefore, multiple techniques for the computation of the derivative exist. 
%Since the derivative, follows the chain and product rule, taking the derivative of the ansatz and thereby the gate sequence cannot be bypassed. The ideas presented in \cite{Stokes2020,Bittel2022,Schuld2019} can be used to obtain an approximation to the derivative of $J$ on the quantum hardware, without deriving a new gate sequence.

%The ideas follow some finite difference approximation of the derivative in the quantum framework. The application of the idea to the framework realized is introduced in the Sec. \ref{sec:Derivative}.

Computing the derivative, introduced in \Eq{eq:first_order_opt}, on quantum hardware without deriving a new gate sequence is possible using either the straightforward \textit{Numerical Derivative}, the \textit{Parameter Shift Rule} \cite{Schuld2019,Banchi2021,Crooks2019}, or the \textit{Natural Gradient} \cite{Stokes2020}. In the case of higher order derivatives, additional techniques come into account, as they are presented in \cite{Mari2021}. 
%If measuring effect, e.g. noise, comes into account the reader is referred to \cite{Sweke2020}, which elaborates on stochastic gradient descent techniques in uncertain environments. 


With quantum circuits presented in \Fig{fig:VQA_QNPU} available, an evaluation of \Eq{eq:Discrete_Opt_BC} is realizable on the quantum hardware. Accordingly, an approximation to \Eq{eq:first_order_opt} can be evaluated in the following manner. \pover{Due to the ghost point strategy, the boundary term in \Eq{eq:first_order_opt} vanishes and the discrete derivative is given as }
\TODO{ADAPT THE DERIVATIVE HERE when Sec 1 is done.}
\begin{align}
\begin{split}
\nabla_{\lamb_c} J(\upb) &= -2\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \sum\limits_k  
\left(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})-u_{k-1}(\lamb_{c})\right)  \nabla_{\lamb_c}u_k(\lamb_{c})\\
%&\quad +\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \left( u_1(\lamb_{c}) \frac{\partial \nabla_{\lamb_c}u_1(\lamb_{c})}{\partial n} -  \frac{\partial u_1(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_1(\lamb_{c}) - u_{NP}(\lamb_{c}) \frac{\partial \nabla_{\lamb_c} u_{NP}(\lamb_{c})}{\partial n} -  \frac{\partial u_{NP}(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_{NP}(\lamb_{c})\right)\\
&\quad - 2\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \left(\left( u_1(\lamb_{c}) \nabla_{\lamb_c}u_{NP}(\lamb_{c}) +    u_{NP}(\lamb_{c}) \nabla_{\lamb_c}u_1(\lamb_{c}) \right) +\left( u_1(\lamb_{c})\nabla_{\lamb_c}u_1(\lamb_{c}) + u_{NP}\nabla_{\lamb_c}u_{NP} \right) \right)\\
&\quad - 2  \lambda_{0}   \sum\limits_k \Tilde{f}_k \nabla_{\lamb_c} u_k(\lamb_{c}) . 
\end{split}
\end{align}

%It is clear to observe that the derivative would require manipulation of the implemented gate sequence for some terms. Despite the derivative with respect to $\lambda_0$. 
As indicated in the equation above, can the gate sequences for $j_l$ be used for an analytical evaluation of the derivative. For the derivatives with respect to the vector $\lamb_\text{c}$, the picture looks different. Here it needs to be distinguished between the terms where $u(\lamb_\text{c})$ appears quadratically and the rest. 

For the quadratic terms, the derivative is given by the \textit{Phase Shift Rule}. The parameter of interest, uniquely parameterizing a one qubit gate, is varied by $s = \pm \frac{\pi}{4 r}$, with $ r= \frac{1}{4}$ formulated by \cite{Mitarai2018,Crooks2019}. The perturbed measured expectation values are used for the computation of the relative change, which aligns with the analytical derivative if $s$ is chosen correctly. The product rule concerning the quadratic term is taken care of by this approach inherently.
%According to \cite{Schuld2019,Banchi2021,Crooks2019}, the derivative with the quadratic terms can be evaluated by using the so-called phase shift rule.
%It is based on the assumption that the ansatz $u$ is linear in  control $\lamb_c$ and consists of elementary rotational single parameter gates  \cite{Schuld2019,Crooks2019}. Then, the gate sequences can be reused and no compilation of the derivative needs to be derived.
The derivative follows using only two additional evaluations. 
%Although alternatives to this approach exist, the implementation of the phase shift rule is straightforward, and allows parallelization with respect to the number of parameters. 

The terms, which appear with a linear setting of the trail function, do not follow this straightforward idea. Here the derivative is calculated using a second-order accurate finite difference approach, e.g. for a parameterization $g(x)$, given by the central difference scheme using a small perturbation $h$ is
\begin{align}
\nabla g(x) =  \frac{g(x+h) - g(x-h)}{2h} + \mathcal{O}(h^2).
\end{align}
This numerical derivative is of course an approximation, but only implies another two evaluations and does not require a new gate sequence. 
%Multiple appearances, e.g. cubic or fourth order, of one parameter, need to be treated according to the chain rule  \cite{Mari2021, Schuld2019}. 

\TODO{CHECk AGAIN if top is done}
Applying the techniques above allow to approximate the derivatives given by 
\begin{align}
&\nabla_{\lambda_0} J(\upb) = 
-2\nu\frac{\lambda_{0}}{\Delta x^2} \left(J_1(\lamb_\text{c}) + J_2(\lamb_\text{c}) + J_3(\lamb_\text{c}) \right) - 2 J_4 (\lamb_\text{c}) ,\\
\begin{split}
\nabla_{\lamb_c} J(\upb) &= -\frac{ \nu \lambda_{0}^2}{\Delta x^2 } r \left(\left(J_1(\lamb_\text{c}+s) - J_1(\lamb_\text{c}-s)\right) - \left(J_2(\lamb_\text{c}+s) - J_2(\lamb_\text{c}-s)\right) +\left(J_3(\lamb_\text{c}+s) - J_3(\lamb_\text{c}-s)\right) \right) \\
&\quad - 2  \lambda_{0}  \frac{(J_4(\lamb_\text{c}+h) - (J_4(\lamb_\text{c}+h)}{2h} + \mathcal{O}(h^2).\\
%&\quad +\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \left( u_1(\lamb_{c}) \frac{\partial \nabla_{\lamb_c}u_1(\lamb_{c})}{\partial n} -  \frac{\partial u_1(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_1(\lamb_{c}) - u_{NP}(\lamb_{c}) \frac{\partial \nabla_{\lamb_c} u_{NP}(\lamb_{c})}{\partial n} -  \frac{\partial u_{NP}(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_{NP}(\lamb_{c})\right).
\end{split}
\label{eq:quantum_derivative}
\end{align}
\pover{Check Derivative dimensions  - make sure scalar/vector match!}



\subsection{Optimization methodology} \label{sec:optimization}

\pover{ May take riemian topology on quantum comp into account} \cite{Wiersema2023}
% do classical example! 
%https://www.researchgate.net/publication/3320516_Steepest_Descent_Algorithms_for_Optimization_Under_Unitary_Matrix_Constraint
%https://arxiv.org/pdf/2112.02572.pdf
% EVIDENCE Given in https://journals.aps.org/pra/abstract/10.1103/PhysRevA.107.062421

As common for VQAs is the classical realized optimization, a crucial point. It is often characterized as a non-trivial task. The publication \cite{Bittel2021} shows that the problem covered in VQA context is theoretically NP-Hard. The practice unveils the optimization of nonconvex functional, determined by e.g. multiple local stationary points as faced in \cite{Sarma2023,Leong2022,Wiersema2023}. Additional to this, the effect of Barrett Plateaus can occur for high layer depths, whereby the vanishing derivative, an efficient update is impossible \cite{}. The use and practicability of zero-/first- or even second-/ order methods therefore highly differentiates with respect to convex optimization.  

A common approach for optimization problems classified as nonconvex is the use of zero-order evolutionary schemes for initial steps, since a good estimate for a starting position is not known in the first glimpse. The main group of these schemes is also known as sampling methods \cite{} Furthermore, has the experience unveiled that, in close vicinity of the stationary point, the necessity for an efficient number of iterations demands a first-order method. Despite this fact, of course, zero-order methods, e.g. the simplex method \cite{Nocedal2006}, as it is done in \cite{Leong2022} can be applied. Second order approaches require enormous overhead in measuring to construct the Hessian, but of course better results. All in all, they are not practicable \cite{Mari2021}. First-order methods, based on second-order models as given by the Quasi-Newton type algorithms, where the second derivative is estimated by rank-1 or even rank-2 updates \cite{Nocedal2006}, instead find its application for some VQAs \cite{  }. The additional effort for the approximation of the Hessian is here not given, but the requirement for a positive definite Hessian needs to be given as well. 

In contrast to this presented Euclidean view on the optimization manifold, there are efforts in choosing the descent direction with respect to the underlying Riemannian setting, which is mainly set due to the fact in \Eq{eq:partition_of_unity}. It is observed that, where the Euclidean approaches tend to local stationary points, the Riemannian strategies overcome these \cite{Wiersema2023}. Despite this, we restrict to the emphasized Euclidean setting, but a detailed view on the problem is crucial to achieve an efficient algorithm. 

Sticking to a Euclidean setting, we use a evolutionary algorithm coupled with a first-order method, to combine robustness in terms of the nonconvexity and high accuracy at the close vicinity of stationary points. We keep our algorithmic strategies to local updates. For the derivation of the update for the first order methods, mention the quantum compiled expression for the derivative in \Eq{eq:quantum_derivative}. Taking into account the functional itself, given in \Eq{eq:Discrete_Opt_BC}, it is clear that it is quadratic in $\lambda_0$. In case of the ansatz parameter $\lamb_\text{c}$, it is not so straightforward. For an evolution in time, the corresponding problem is solved iteratively, as emphasized in \Fig{fig:discretization_encoding}.

The numerical strategy to address the variational problem in \Eq{eq:Discrete_Opt_BC}, compiled as described in Sec. \ref{sec:Compilation}, is two-folded. First, a Monte Carlo-based optimization, sampling method, so-called particle-swarm optimization \cite{Kennedy1995} is used, in order to determine a suitable initial parameter position. The algorithm is based on the next parameter $\lamb$ update
 \begin{align}
\lamb_{i+1} =& \lamb_{i}+\Delta \lamb_{i+1}\\
\Delta \lamb_{i+1} =& \underbrace{\omega \Delta \lamb_i}_\text{Momentum} + \underbrace{c_1 r_{1_i} \left(\lamb_{\text{best},i}-\lamb_i\right)}_\text{Learning}+ \underbrace{c_2 r_{2_i} \left(\lamb_{\text{best},i_\text{swarm}}-\lamb_i\right)}_\text{Communication}.
\end{align}
\pover{convergence criteria}
Once the Particle swarm is terminated, the obtained parameter setting is provided to the second method, namely a gradient descent method. Here the choice is the classical Gradient Descent given as $ \lamb_{i+1} = \lamb_{i} - \alpha \nabla J(\lamb_{i}) $
Convergence is determined by a tolerance \texttt{tol} at $ \| \nabla J(\lamb_{i}) \|_2 \leq \texttt{tol}$. This two-step approach is relaxed by introducing an inner optimization loop, where in the first step $\lambda_0$ is kept constant and in a second step the whole control is updated. \textbf{}With this two-step approach, it is accomplished to cover extensively the unknown solution space. The difficulty of selecting an appropriate start location for fine-tuning and the nonlinear mapping to the Ansatz parameterization $\lamb$ is handled. For time step $t> 0$ and higher steps of inner iterations the previous optimal parameter are taken as initial guess as proposed by \cite{Sato2021,Leong2022}
The whole library given is made available by the in-house MPI-parallel PDE toolbox, with \textsc{qiskit} as an interface and backend. Inheritance and polymorphism allowed to establish an identical structure as presented here. As a summary, the complete algorithm is given in Alg. \ref{alg:VQA}.

\begin{algorithm}[htbp]
\caption{VQ Algorithm}
\label{alg:VQA}
    \begin{algorithmic}
    \Require $\text{N}_t, \text{N}_p, \texttt{tol}, \lamb_0$
    \While{$t \leq T $}
        \While{$i\leq 10$}
            \If{i==0 or t==0}
                \State $\lamb_i$ \gets PSO$(\lamb_0)$
            \Else
                \State $\lamb_{\text{c}_i}$ \gets GD$(\lamb_i)$
            \EndIf
             \If{i==0 or t==0}
                \State $\lambda_i$ \gets GD$(\lamb_i)$
            \Else
                \State $\lamb_i$ \gets GD$(\lamb_i)$
            \EndIf
            \State $\texttt{tol}$ \gets \texttt{tol}/inner
            \State inner \gets inner+1
        \EndWhile
        \State $t$ \gets $t+1$
    \EndWhile
    \end{algorithmic}
\end{algorithm}

==> Container/C_OldSections/ComputationalStrategy_old.tex <==
%###########################################
%       Computational Strategy
%###########################################

\section{Computational Strategy} \label{sec:Strategy}
References
\cite{Dennis1996}
\cite{Nocedal2006}
\cite{Press2007}
\sbengoechea{Encoding the continuous function values in the complex amplitudes of the quantum state vector}.
On a Classical Computer (\textsc{CC}), the discrete optimization problem introduced in Sec. \ref{sec:Discretization} and derived in \Eq{eq:Discrete_Opt} can be implemented following the known procures. The information is encoded by a certain number of bits, which is proportional to the number of grid points $NP$ and their numerical resolution, i.e. the floating-point arithmetic. On a Quantum Computer \textsc{QC}, the processing of information is executed on qubits, being the bit counterparts. Analogue to the CC, are the qubits again collected in a register.

\pover{We use BigEdian for all computations and the models }
For the discretization introduced, a quantum register, assembled with $n$ qubits to represent $NP = 2^n$ number of discrete points $NP$ is required. Each of the $n$ qubits recovers two distinguishable states, e.g. in Dirac notation as $\ket{0}$ and $\ket{1}$. Maintaining the Dirac notation, a quantum register $\ket{\psi}$ with $n$ qubits contains the basis states $\ket{\psi} = \ket{\psi_1} \otimes \ket{\psi_2} \otimes \hdots \otimes \ket{\psi_n}$, where $\ket{\psi_n} = \alpha_n \ket{0} + \beta_n \ket{1} :~\alpha_n,\beta_n~\in~\mathbb{C}$. The abbreviation, $\ket{0}$ and $\ket{1}$, refer to the first and second orthonormal basis of the given vector space \cite{Nielsen2010}. 
Based on this encoding, it allows the representation of high resolved function values $g_k \in \mathbb{C}$ at each $x_k \in \Omega$. This enables a more general encoding, compared to bits, where an integer value goes from $0$ to $2^n-1$ assuming $n$ classical bits are available \sbengoechea{(another n for classical bits)}. Accordingly, the numerical resolution of an entity (e.g. $g_k$) at the grid point itself, is independent of the number of qubits $n$. In contrast to a \textsc{CC}, this is one great advantage. 
However, the normalization condition: the partition of unity $\bra{\psi}\ket{\psi}=1$ (c.f. \Eq{eq:partition_of_unity}), of the quantum physical system must always be fulfilled. This is an essential requirement for QC and a consequence of the probabilistic nature of Quantum Mechanics (\textsc{QM}) and is respected by the already introduced control parameter $\lambda_0$.

With this in mind, mention the map $\ket{\text{bin}\left(k\right)}: k \mapsto \ket{\text{binary}\left(k\right)}$, which delivers the $k^{th}$ orthonormal basis of the underlying Hilbert space $H^n$. Consequently, the spatial dimension $x$ can be encoded by $\ket{\psi} = \sum\limits_{k=0}^{2^n-1} \psi_k \ket{\text{bin}\left(k\right)}$, where $\psi_k$ refers to the amplitude of $\psi_k$ at $x_k$. For a discretized function $g_k \in \mathbb{C}$, the encoding thus is $g_k = \Tilde{\lambda}_0 \psi_k$, where $\Tilde{\rho}$ \sbengoechea{(use $\lamb_0$ or $\rho$, is that needed?)} is implied to satisfy the partition of unity $\sum \limits_{k=0}^{N-1} |\psi_k|^2 =1 = \frac{1}{\rho} \sum \limits_{k=0}^{N-1}g_k^* g_k$.

Since the solution $y(x)$ of \Eq{eq:Generic_PDE} is continuous in space, the discretization affects the normalization. Discretizing the continuous representation of the normalization condition  by the trapezoidal rule results in 
\begin{align}
    1 = \sum \limits_{k=0}^{N-1} y_k^* y_k\Delta x = \sum \limits_{k=0}^{N-1}  \lambda_0^2 \psi_k^* \psi_k.
    \label{eq:normalizedf}
\end{align}
\sbengoechea{$\rho_0$ needs to be 1 in 33}
At this point, it is important to mention that this relation between discretization and normalization is defined by the quantum properties of the vector states and, in particular, by their probability amplitudes. This has a major impact on the numerical resolution of the trial functions $y(x)$. As the number of qubits increases to achieve higher resolutions, the amplitudes of $y(x)$ are increasingly compressed to conserve the partition of unity.

With the hardware requirements in mind, the following section aims to cover the approximation of the solution to the problem given in \Eq{eq:Generic_PDE} using \textsc{VQA} initially presented in the same structure by \cite{Lubasch2020}. 

\subsection{Variational Quantum Algorithm}
\pover{
Cite for Hadamard test use and achieve Q supremacy:
\cite{Guseynov2023} MENTION!   Exploits the why to hardamard test! see conclusion
}

The \textsc{VQA} is a methodology to minimize the underlying objective $J$, by variationally optimizing a control $\upb$ (set of parameters) and thereby varying the amplitudes of the state $\ket{\psi}$. The optimal value of the functional $J$ is prescribed by the variational method of QM, which shows other parallels between classical PDE problems and QM applications \cite{Tilly2022}. For the variational method, a qubit registers $\ket{\psi}$ is initialized with the computational basis state $\ket{0}$ and is used as an input to a quantum circuit composed of a predefined series of quantum operations modulating the PDE dynamics, the so-called gates. The chosen approach is highly dependent on the problem, which determines the arrangement of the gates, their actions, and the type of measurement. In addition to this, a gate always requires being unitary to respect the partition of unity. In classical CFD, this requirement is most often violated and needs to be unitarized, which is one key discipline in the compilation to quantum hardware. Despite this difficulty, it is possible to structure the compiled quantum circuit into the following three parts, see \Fig{fig:VQA}:
\begin{enumerate}
     \item The upper qubit, so-called ancilla, is intended for indirect measurements according to the Hadamard test, or the swap test methodology \cite{Endo2020}. The advantage of this technique is to reduce to a single measurement, instead of multiple measurements, \sbengoechea{see \Fig{fig:VQA_QNPU}}. The register $\ket{\psi}$ is therefore augmented by another qubit, to the whole register $\ket{0} \otimes\ket{\psi}$. As introduced, the size of the register depends on the number of points $NP$.
        
%%

    
    \item The parameterized Ansatz $U_r(\lamb)$ spans the trail function space of the test-functions $\ket{\psi}$. All of them are available to be evaluated. Therefore, the Ansatz must be capable of modelling the underlying physical effects of the problem covered, making the Ansatz, and its arrangement, a crucial part of the \textsc{VQA} method. 
    A set of parameters, the control $\upb$, determines the shape of the resulting test function $\ket{\psi}$. In the mathematical framework, exploit in Sec. \ref{sec:Mathematics}, the control refers to the vector $\upb$ in \Eq{eq:Generic_OptimalControlProblem}. The mapping of the control to a collection of trail functions is advantageous. However, as indicated in \Fig{fig:VQA_Ansatz}, the depth $d$ of the Ansatz circuit defines the number of sequential quantum operations and affects the level of entanglement \pover{entanglement? knowledge assumed} in $\ket{\psi}$ and thus the capabilities regarding the test functions. With rising depth $d$ more revolutions of the Ansatz are added and structured in a bricklayer fashion. \pover{Why bricklayer ?\cite{Uvarov2021}}.
    
    \item The transformation $T_t$ aligns the order of the amplitudes in the register of $\psi$, according to the subsequent QNPU. It is a feature, which is not described in \cite{Lubasch2020} and modularizes the building blocks of the VQ-assembly even more.
    It allows to reuse multiple QNPU compilations, where the same technique only appears with another $T_t$. Nevertheless, in many cases $T_t= I$, expect the cases where it is mentioned separately. 

    \item The Quantum Nonlinear Processing Unit (\textsc{QNPU}) is a succession of quantum gates, representing PDE effects of the system, e.g. in  \Fig{fig:VQA_QNPU}. In the current case, the QNPU is required to represent the discretized dynamics of \Eq{eq:Generic_PDE} represented by the functionals $J_i$. Based on the order of nonlinearity $\xi$ \sbengoechea{of \Eq{eq:Generic_PDE}}, the number of inputs $r$ is increased to point-wise multiply various copies. 
\end{enumerate}

\begin{figure}[h]
\centering
    \begin{subfigure}[b]{0.9\textwidth}
        \centering
        \input{Figures/QNPU.tex}
        \caption{Schematic sketch of a \textsc{VQ} circuit composed by the \pover{Ansätze ? } $u_r(\lamb)$, the $T_t$ assembly, a specific \textsc{QNPU}, and a measurement qubit (ancilla qubit) for indirect measurement technique. $H$ indicates a Hadamard gate, \textsc{CP}$_i$ Control Port, \textsc{IP}$_i$ Input Port, \textsc{OP}$_i$ Output Port, and $\sigma_z$ the expectation value at the measurement operation, c.f. \cite{Lubasch2020}.}
        \label{fig:VQA_QNPU}
    \end{subfigure}
    \begin{subfigure}[b]{0.9\textwidth}
        \centering
        \input{Figures/Ansatz.tex}
        \caption{Exemplary topology for one $u(\lamb)$ Ansatz circuit composed out of $g$ fundamental gates structured in a bricklayer fashion and parameterized by $\lamb = (\lamb_1, \lamb_2,\hdots, \lamb_g)^\intercal$ parameters encoding a test function on $n = 6$ qubits, c.f. \cite{Lubasch2020}.}
        \label{fig:VQA_Ansatz}
     \end{subfigure}  
    \caption{Visualization of fundamental VQA elements for the implementation of the exploit paradigm.}
    \label{fig:VQA}
\end{figure}

With the layout of quantum compilation given, the minimization of the cost function $J$ can be realized in a hybrid classical-quantum algorithm, which is common to all VQA methodologies. \Fig{fig:optimizer} sketches the hybrid quantum-classical framework, extending the structure given in \Fig{fig:VQA}.

\begin{figure}[h]
    \centering
    \input{Figures/communication_opt}
    \caption{Sketch of the hybrid classic-quantum VQA optimization procedure. \sbengoechea{Clarify better Classic and Q parts of the optimization box.}}
    \label{fig:optimizer}
\end{figure}

The objective $J$ is evaluated mainly on the quantum device, which is controlled by the outer classical counterpart. The classical part hereby has full control of the quantum-based parametrization of the objective and thus over the solution, which is parameterized by the Ansatz $ u(\lamb)$. The objective is evaluated individually for each larger summand of \Eq{eq:Discrete_Opt}. The Ansatz and parameters $\lamb$ are kept identical for each term. In the outer classical loop, the determined value is scaled and assembled to $J$. Consequently, an update $\delta\upb$ is to be determined, to update the parameters $\upb$ for the next iteration $i$. To efficiently update, the knowledge about a descending direction is necessary. As known from optimal control theory and the subject of optimization, first-order methods outperform zero-order optimization methods quickly. 
Since the derivative, follows the chain and product rule, taking the derivative of the ansatz and thereby the gate sequence cannot be bypassed. The ideas presented in \cite{Stokes2020,Bittel2022,Schuld2019} can be used to obtain an approximation to the derivative of $J$ on the quantum hardware, without deriving a new gate sequence.  The ideas follow some finite difference approximation of the derivative in the quantum framework. The application of the idea to the framework realized is introduced in the Sec. \ref{sec:Derivative}. In the following, each part of the VQA assembly is introduced in detail. 



\subsection{Measurement techniques}\label{sec:measurement}
\pover{Exclude chapter and mention trace out at application}
\sbengoechea{I would leave this section here and not moved to numerical experiments}
The indirect measurement in contrast to the direct measurement has multiple advantages. We would like to present them quickly. Therefore, mention both of the techniques, presented in \Fig{fig:quantum_measurement}.
\begin{figure}[htbp]
\centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering        
         \input{Figures/direct_meas}
         \caption{Direct measurement technique}
         \label{fig:quantum_measurement_direct}
     \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \input{Figures/indirect_meas}
         \caption{Indirect measurement technique}
         \label{fig:quantum_measurement_indirect}
     \end{subfigure}  
    \caption{Comparison of direct and indirect measurement for quantum circuits.}
    \label{fig:quantum_measurement}
\end{figure}

Instead of $n$ measurements per experiment, whereby the quantum register is affected by the non-reversible operation, an indirect measurement is introduced. This technique reduces the measuring operation to just one measurement on the ancilla (measurement qubit) (given in fig. \ref{fig:quantum_measurement_indirect}). This avoids the measuring of the probabilities for all $n$ qubits in the register (e.g. fig. \ref{fig:quantum_measurement_direct}). In a more general form, the ancilla qubit in the Hadamard test can be understood as a tracker of all possible computing scenarios, ending up in a summation of information. 
Assuming the initial state to be 
\begin{align*}
     \ket{\phi_0} &= \ket{0} \otimes \ket{\psi}.
\end{align*}
One can show that the final state is \sbengoechea{(citation, Nielsen?)}
\begin{align}
    \ket{\phi_3} &= \frac{1}{2}\left(\ket{0}\otimes \underbrace{\left(I+U\right)\ket{\psi}}_{\rightarrow P(0)}+\ket{1}\otimes \underbrace{\left(I-U\right)\ket{\psi}}_{\rightarrow P(1)}\right).
\end{align}
For the measurement of the probabilities $P(0)$ and $P(1)$, the inner product of the state vector with its complex conjugate at the measurement is calculated. \sbengoechea{(Why is the next sentence important?)} Furthermore, for $z\in \mathcal{C} : z=x+iy \rightarrow  z+z^* = x+iy + x-iy = 2\mathcal{R}\left(z\right)$. Based on the probabilities $P(0)$ and $P(1)$ the expectation value $\langle\sigma_z\rangle$ can be calculated as 
    \begin{align}
    \langle\sigma_z\rangle &= \bra{\phi_3}^\dagger\sigma_z\ket{\phi_3} \notag\\
    &= \underbrace{\bra{\phi_3}^\dagger\ket{0}\bra{0}\ket{\phi_3}}_{P\left(0\right)}-\underbrace{\bra{\phi_3}^\dagger\ket{1}\bra{1}\ket{\phi_3}}_{P\left(1\right)} 
    \end{align}
The measurement on the basis of $\sigma_z = \ket{0}\bra{0}-\ket{1}\bra{1}$, hereby refers to a measurement in a positional basis. Each state is measured according to its projection onto the z-axis of the Bloch sphere. For further information, the reader is referred to \cite{Nielsen2010}. The real part $\mathcal{R}$ is 
\begin{align}
\begin{split}
    \langle \sigma_z \rangle=&\frac{1}{2} \left(1+\mathcal{R}\left(\bra{\psi}U\ket{\psi}\right)\right)\\
    &\quad- \frac{1}{2} \left(1-\mathcal{R}\left(\bra{\psi}U\ket{\psi}\right)\right)
    \end{split}\notag\\
    =&\mathcal{R}\left(\bra{\psi}U\ket{\psi}\right).
    \end{align}
    \label{eq:expectation_hadamard}

Comparing the expectation value given, with the expression in \Eq{eq:Generic_Opt}, underlines the similarity of the expressions to that appearing in the bilinear-form $a(\cdot,\cdot)$, \sbengoechea{(when a(psi,psi))}. However, the expectation value is still depending on the number of samples and only represents a weighted average. Thus, it requires a robust measurement technique with multiple experiment executions ($N$ experiments). In summary, this concept is an essential prerequisite for using quantum devices, and it conforms to the application of indirect measurements by the Hadamard test methodology. 

According to the statistical and probabilistic effect, \sbengoechea{the practice has shown that it can become challenging to maintain industrial accuracy using this measurement technique on real devices. (I would be a bit more open in what the problem is. The measurement is based on vector state projection on $\sigma_z$ and as the mixture in the states increases the length of the vector reduces, limiting the measurement accuracy. This is part of the measurement issue in QC, how to improve accuracy of projection measurements.) Ask Kiffner?} Hence, we like to restrict to the implementation and realization of the classical CFD known techniques for this publication. We use a so-called trace-out technique to emulate the integration effect of the ancilla measurement on a state vector simulation signal. Therefore, assume to have a composite “quantum” system of subsystems $A$ and $B$ such that $A\cup B$ with $a\in A, b \in B$. A system reduction, without information loss, can be then archived by the application of the partial trace. This is defined for the subsystem $B$ as \cite{Nielsen2010} 
\begin{align}
    \Tr{\ket{a}\bra{a}\otimes \ket{b}\bra{b}}_B \equiv \ket{a} \bra{a} \Tr{\ket{b}\bra{b}}.
    \label{eq:partial_trace}
\end{align}.
Taking the ancilla as subsystem $A$ and the QNPU register as subsystem $B$, the application of the partial trace is straightforward. By this, the result of a state-vector simulation recovers the same effect as intended by the indirect measurement performed on real hardware, without noise and shoot errors. With the setting of the Measurement exploit, the first key element follows. The role of the ansatz is given in the next section. 

\subsection{Ansatz- TODO} \label{sec:ansatz}
\pover{SO4,SATO, LEONG}
\pover{Hilber space in relation to parms }
\sbengoechea{Here, I would mention briefly only the ansätze we use. If we finally use only one we could remove this section and plot the ansatz in Fig. 3b}

\pover{Assume the solution Is in the set of the ansatz}

\pover{introduce what y the state  and z the testfunction is in our setting and define the Hilbert space $H$ -  compare to inital framework at mathematicall sec. 1}
As already mentioned above, the Ansatz needs to be chosen according to the problem at hand. It defines the span of the test function/ solution space, where all feasible functions $\psi$ can be determined. A basic exemplary Ansatz is given in \Fig{fig:quantum_basic_ansatz}. Here, the Ansatz creates an entangled state, without an introduction of phase delay. The employed parameterized gates $R_y(\lambda)$ are identical and parameterized by a single parameter $\lambda$ only. The ansatz is taken from \cite{Lubasch2020}. 

\begin{figure}[htbp]
\centering
\input{Figures/ODRY_ansatz}
\caption{Quantum Ansatz to create a variational state, $R_y\left(\lambda\right) = exp(-i\lambda\nicefrac{\sigma_y}{2}): \lambda \in \left[0;2\pi\right)$ \cite{Lubasch2020}.}
\label{fig:quantum_basic_ansatz}
\end{figure}

Taking more advanced Ansätze into account enables to span a greater function space. The Ansatz in \Fig{fig:quantum_ansatz_SO4} is such an Ansatz. It is called optimal SO4 two-qubit Ansatz and is given by \cite{Vatan2004}.

\begin{figure}[htbp]
\centering
\input{Figures/SO4_ansatz}
\caption{Two qubit Ansatz to create an optimal variational state $\psi \in \mathbb{C}  : \lamb \in \mathbb{R}^3$ \cite{Vatan2004}.}
\label{fig:quantum_ansatz_SO4}
\end{figure}

The gates are $S_1 =R_z(\nicefrac{\pi}{2})$, $R_1=R_y(\nicefrac{\pi}{2})$, $A=R_z(\lambda_1)R_y(\lambda_2)R_z(\lambda_3)$, and $B=R_z(\lambda_4)R_y(\lambda_5)R_z(\lambda_6)$, whereby $B$ is not always required. By using the whole assembly, it results in $\lamb=(\lambda_1,\lambda_2,\hdots,\lambda_6)^\intercal$ for each Ansatz gate. The use of $R_z(\cdot) \in \mathbb{C}^{2\times 2}$ involves imaginary values, which is the cost to pay for a more complex space encoding. The resulting phase modulation about $SO4\_phase$ should thus be corrected after the measurement. This is done according to 
\begin{align}
    \mathcal{R}(\ket{\psi}) =  \mathcal{R}(\ket{\psi} \exp(- i \, \frac{SO4\_phase}{2}).
    \label{eq:phase_corr}
\end{align}
Attention, the phase modulation deflects the measurement in $\sigma_z$ by an offset. 

Using this parameterization of the function space, it follows the mapping $U(\lamb) \text{ where }\lamb : \mathbb{R}^{\#Par}\mapsto \mathbb{C}^{2^n}$. Accordingly, the $\ket{\psi}$ encoding by $U(\lambda)$ concludes in $\ket{\psi} = U(\lamb)\ket{0}$ with $\hat{\Bar{L}}(\psi) = \hat{\Bar{L}}(\psi(\lamb))$. 

\pover{Number of lambdas should be at most polynomial ideal linear in n :  point}
\pover{adapt rho is applidudes flip sign}
\pover{Parameter scale to [0, 2pi)}

\pover{Also give Leong and Sato ?  Comment on the differnces?}

\subsection{Compilation of the Quantum-Nonlinear-Processing-Units}
\label{sec:Compilation}
References: \cite{GonzalezConde2023}
https://arxiv.org/abs/2307.10917

With the availability of quantum tools, namely indirect measurement and function space encoding, it is possible to derive a quantum compilation of the second key element \sbengoechea{(the QNPU box)}. We want to introduce our library of QNPUs. All of them are extendable to arbitrary fine one-dimensional discretization and have been designed to keep the gate sequence shallow. The application to equidistantly spaced finite difference discretization, as given in \Fig{fig:discretization_encoding}, is possible without any additional effort. The set of to-be-presented QNPUs cover dynamics, which commonly occur in PDEs, as in the form of that given in \Eq{eq:Generic_PDE} and as they are common for CFD. \sbengoechea{(We use the potential for the mixed BC. I would take out the non-linear term since we do not use it.)} Despite the fact, that \sbengoechea{$\xi = \zeta = 0$ ()}, we will introduce two QNPUs for the case  $\xi \neq 0, \zeta \neq 0$. To give the reader a direct overview of the Quantum circuits, each compilation is finalized with a $n=2$ \sbengoechea{and 4} qubit example as well as a general expression.

\subsubsection{The Laplace}\label{sec:Compilation:Laplace}
The Laplacian is one of the most often appearing differential operators when it comes to PDEs in the context of CFD. Hence, it is a necessity to derive a robust and flexible compilation for the quantum hardware. Inspecting the finite difference stencil in \Eq{eq:derivatives_space}, a similitude to the classical bit shift operator can be stated. With a discretization of $n\leq 2$ the half-adder circuit is used beyond it is limited and additional carry bits become a necessity. For the construction of the now-demanded, full adder circuits as well as the theory, the reader is referred to literature on classical computing \cite{Parhami2010} and \cite{Lubasch2020,Darper2000,Nielsen2010}. The full adder as used in the QNPU for the Laplace operator has already been developed in the work of \cite{Lubasch2020}. For the sake of completeness, it is nevertheless introduced. 

Starting at the \Eq{eq:derivatives_space}, it can be shown, that the equation can be reduced to three terms $\psi_k^* \psi_{k+1},\;\psi_k^* \psi_{k} \;\& \;\psi_k^* \psi_{k-1}$, where the first and last request a multiplication by a shifted value. For a closure, the periodic boundary condition simplifies the expression until a certain point. This needs to be corrected as mentioned above. Accordingly, one can give the general structure of the discretized Laplace operator which acts on a state-like, \cite{Lubasch2020} 
\begin{align}
\label{eq:Laplace}
    \sum \limits_{k=0}^{NP-1} \psi_k \text{binary} \to  \sum \limits_{k=0}^{NP-1} \psi_{k+1} \text{binary}.
\end{align}
The final circuit is shown in \Fig{fig:Laplace_compiled} e.g. $n=6$.

\begin{figure}[h]
    \centering
    \input{Figures/Adder.tex}
    \caption{Quantum circuit for the Laplacian term for $n=6$, in the Hadamard test configuration. In practice, the input $\ket{\psi}$ is given by an ansatz, as those introduced in sec. \ref{sec:ansatz}. For $n=2$ qubits, this circuit is exactly implementing a half-adder, c.f. \cite{Lubasch2020}.}
    \label{fig:Laplace_compiled}
\end{figure}

As a proof of concept, mention that the quantum registers for $n=2$ qubits can be decomposed in its complex amplitude as, $\ket{\psi} = \left(c_{00},c_{01},c_{10},c_{11}\right)^\intercal$. It can be shown that the initial state $ \ket{\phi_0} = \ket{0} \otimes \ket{\psi} = \ket{0} \otimes \left(c_{00}\ket{00}+c_{01}\ket{01}+c_{10}\ket{10}+c_{11}\ket{11}\right)$ evaluates to $ \langle\sigma_z\rangle =   \sum\limits_{k=0}^{NP-1}\psi_k\psi_{k+1}$, assuming real function values and periodicity. 

\sbengoechea{I would put BC as subsection too}
\paragraph{Boundary Conditions}\label{sec:Compilation:BC}
\sbengoechea{Note that the special treatment for mixed BC. Because the mixed combination is not unitary, one needs to use mask function with the potential term TOINCLUDE}
Given the Laplacian for a periodic setting, we now introduce the novel approach to generalize the implementation to a more general setting, which is required for the transformation to industrial application. 

As a benefit, the ghost point implementation introduced in Sec. \ref{sec:Discretization} the adaption to different boundary conditions is just a question of finding the corresponding gate sequence. Furthermore, as mentioned above in the derivation of the Laplace operator, is the assumption of periodic boundary conditions crucial. This fact needs to be given for the Laplacian, but of course, can be corrected by another QNPU. In the following, we would like to present another two circuits to adjust the field dynamics to the boundary setting and to link internal and external discretization.

As a prelude, mention the transformation $T_t$, given by \cite{Sato2021}. To correct the discretized dynamics in the previously given operator, this transformation is required to align the quantum register to fit the following compiled correction. The transformation $T_t$ is given in \Fig{fig:Transformation}, and is implemented as sketched in \Fig{fig:VQA_QNPU} \sbengoechea{(maybe the BC circuits for nq = 4. We don't use 3 qubits)}. \sbengoechea{In contrast to the approach of \cite{Sato2021} and \cite{Leong2022}, here the BC correction on the periodicity can be represented as unitary circuits and therefore as quantum gates for an arbitrary number of qubits.}

\begin{figure}[h]
    \centering
    \input{Figures/Transformation}
    \caption{Transforamtion $T_t$}
    \label{fig:Transformation}
\end{figure}

With the transformed register available, the implemented actions of the Laplace operator can be transformed. In the case of Dirichlet boundary conditions, the circuit in \Fig{fig:QNPU_Dirichlet} needs to be used as an QNPU.

\begin{figure}[htbp]
    \centering
    \input{Figures/Dirichlet.tex}
    \caption{Dirichlet Circuit}
    \label{fig:QNPU_Dirichlet}
\end{figure}


For Neumann Boundary conditions, it is given by  \Fig{fig:QNPU_Neumann}

\begin{figure}[h]
    \centering
    \input{Figures/Neumann}
    \caption{Neumann BC}
    \label{fig:QNPU_Neumann}
\end{figure}

\subsubsection{The Potential}\label{sec:Compilation:Potential}
This section covers the quantum computational evaluation of the bi-linear term covering the potential $p(x)$. After application of the discretization technique according to \Fig{fig:discretization_encoding}, can the bi-linear term be written as
\begin{align}
    \sum\limits_{k=0}^{NP-1} \psi_k^*p_k \psi_k.          
    \label{eq:P_dis}
\end{align}

In the following, the compilation is given, and its basic functionality will be emphasized in a $NP=4 \rightarrow n=2$ qubit setup, which shows the pattern for a full extension to a $NP$ point representation. The potential contribution is modeled by an inner product of an external potential $p\left(x\right)$ and the solution $y\left(x\right)$, which can be interpreted as a discrete point-wise multiplication over space. To encode the external potential on the quantum hardware, multiple approaches exist to derive the corresponding gate sequence. In terms of trigonometric contributions, the publication by \cite{Lubasch2020} introduces gate sequences for $e(x), sin(\kappa x)$ and some superposition of fundamental functions based on the Matrix-Product-State formalism as a programming paradigm. In this direction, the references \cite{Oseledets2012,GonzalezConde2023} \pover{give some more references who encode functions} deploy additional compilations. \pover{TT cross techniques can also be used to approx non continues potentials} Despite, the compilation of external potential, e.g. polynomials or trigonometric functions, the corresponding quantum circuit interfaces to all and is given for $n=2$ qubits in \Fig{fig:potential_measuremment}. 

\begin{figure}[h]
    \centering
    \input{Figures/Potential.tex}
    \caption{The quantum circuit based on the Hadamard test for the discrete potential function $p_k=( p_0, p_1,p_2, p_3)^\intercal$.}
    \label{fig:potential_measuremment}
\end{figure}

Assuming $n=1$ and $\ket{\theta_0} = \ket{0\psi0}$ as the initial state, a small sketch would deliver the expectation value $ \langle\sigma_z\rangle = \frac{1}{2} \sum \limits_{k=1}^2\psi_k^*v_k\psi_k + \psi_kv_k^*\psi_k^*$, which can be simplified to $\langle\sigma_z\rangle =\sum\limits_{k=1}^{2} \psi_k v_k \psi_k$ assuming real functions.

\subsubsection{The Nonlinearities}\label{sec:Compilation:Nonlinearities}
\pover{Reference 
Towards Cosmological Simulations of Dark Matter on Quantum Computers
Philip Mocz (Princeton), Aaron Szasz (Perimeter Institute)}
%https://arxiv.org/abs/2101.05821


\sbengoechea{I would remove this part}
To create non-linearities, multiple copies are related via point-wise multiplication. As a result, the quantum circuit is again enhanced to accommodate the nonlinear terms. As evident, is the modular structure of the library based on a few fundamentals, such that the circuit for the last two terms in \Eq{eq:Generic_PDE} is substantially the same. In the following derivation, a more simplified view is given again, where the spatial dimension is discretized with two points, i.e. one qubit. According to the expression, the nonlinear exponent should sum up to $r$.
To address non-linearities, the definition $f^2(x) = \Tilde{p}(x)$ is introduced. Underlining the modularity of the exploit framework, the resulting circuit is straightforward, similar to \Fig{fig:potential_measuremment}. For the sake of consistency, we pull out the substituted $\Tilde{p(x)}$ and derive the structure given in \Fig{fig:VQA_QNPU}. For now, just to mention that 
\begin{align}
\psi_k^*\Tilde{p}_k \psi_k  = \psi_k^* \psi_k^2 \psi_k .
      \label{eq:I_dis}
\end{align}
 \pover{introduce another exponent } For the derivation, it is essential to take into account the controlled Ansatz's gates $U$, $\ket{\psi_i}= U_i\ket{0} = \left(\psi_{i1},\psi_{i2}\right)^{\intercal}$ of the copies. The figure below, \Fig{fig:nonlinear_measurement}, illustrates the underlying quantum circuit. 

\begin{figure}[htbp]
    \centering
    \input{Figures/Nonlinear.tex}
    \caption{Hadamard test configuration of the quantum circuit for the evaluation of the nonlinear interaction term $\hat{I}$. $n=1$ and number of copies $r=3$. The dashed red lines indicate intermediate quantum states.}
    \label{fig:nonlinear_measurement}
\end{figure}
Again, it is easy to show that, defining $\ket{\theta_0} = \ket{0}\ket{0}\ket{0}\ket{0} = \ket{0000}$ as an input for the quantum circuit of \Fig{fig:nonlinear_measurement} evolves in the outcome $\langle \sigma_z \rangle  = \sum \limits_{i=1}^3\sum\limits_{k=0}^{NP-1} \psi_{ik}^4$.

\subsubsection{Generic Source Terms} \label{sec:compilation:source}
Besides the terms above, the \Eq{eq:Generic_PDE} holds a RHS given as $f$, referred to as the source term. It differs a lot from the compilations introduced. Instead of a dynamic, it represents effects on the dynamical system. A classical source term is an e.g. hotspot given by a defined temperature in the domain $\Omega$. Given in the linear form $F$ of the variational \Eq{eq:variational_eq}, it is only multiplied by the test function ones, resulting in a linear expression. Compared to the other operators above, which are quadratic in the test function, this is an important difference. Additionally, the RHS is restricted to fit in the QNPU framework, the RHS must be given as an invertible gate sequence. Again, for the derivation of special gate compilations, the reader is referred to \cite{Oseledets2012,Lubasch2020,GonzalezConde2023}, the detailed description given in sec. \ref{sec:Compilation:Potential}. Assuming there is a gate sequence representing $f$, the RHS can be implemented by using the QNPU given in \Fig{fig:overlapp}. 

\begin{figure}[h]
    \centering
    \input{Figures/Overlapp.tex}
    \caption{The overlapp. \sbengoechea{Include the whole circuit with u controlled.}}
    \label{fig:overlapp}
\end{figure}

Instead of the uncontrolled ansatz $u_1(\lamb)$, the linearity of the source terms, requires that the ansatz  $u_1(\lamb)$ is controlled, analog to $u_2(\lamb)$ in \Fig{fig:VQA_QNPU}. 

As already introduced in sec. \ref{sec:Discretization:BC}, requires an inhomogeneous boundary setting the augmentation of the source term $f$. The additional $f_\text{ghost}$ is compiled to a gate and simultaneously compiled into a circuit as given above, to just mention the similarities in the framework. 

\pover{scalar product phase shift correction -  expectation value in code L. 231 source/objectives \TODO{Do we still need this correction?}}

%\subsubsection{Time derivative}
As a final step, mention the discretized time derivative given in \Eq{eq:elliptic_heat_eq}. The RHS appears in an augmented form and thus can easily be implemented using the technique given in Sec. \ref{sec:compilation:source}. The inner product of the state $\psi$ with itself is always summing up to one, stated by \Eq{eq:partition_of_unity}.

\subsubsection{Gate complexity}
In order to investigate the scalability of our algorithm, we show the relation of nq with the number of gates for all the circuits composing the QNPU and the SO4 ansatz. Note that the gate complexity of the ansatz depends on the type and depth selected and it is case dependant. However, we have included the gate complexity of the used SO4 ansatz w.r.t to depth and nq to give the reader a comprehensive view of how is the total complexity of the VQA used in this work. 

The results are depicted in \Fig{fig:compilation:GateComplexity}. The right-hand-side of this figure 
shows the polynomic of order x \sbengoechea{(linear?) to find out the polynom order)} relation of the number of gates of the ansatz w.r.t. the number of qubits. The same polynomic \sbengoechea{(to check the order)} behavior is found for the Laplacian QNPU as can be seen in the left-hand side of the same figure. This complexity of the Laplacian circuits is due to the local effect of the discrete stencil for approximating the second space derivative, in this case the resulting circuit conserves this local property. On the other hand, the QNPUs for the boundaries show an exponential increase in the number gates w.r.t. the number of qubits. 

%\pover{Of cource , boundary conditions sclae expontially, as it is observed in \cite{Sato2021,Leong2022,Leong2023}, hence the effect of them is not bind to a local behaviour and thus requires a multi quibit interaction, which scales naturally with the number of sites. The compiled circuit we show nevertheless, allows to represent this non hermtian effect in a robust manner on quantum hardware. A mask can be used or as sato does , a measurement on only a single quibit can be done..\textbf{}\textbf{}} 

\sbengoechea{The non-unitary approach/Matrix to BC proposed by Sato is here adapted to unitary.}

Hence the effect of the BC is not bind to a local behaviour and thus requires a multi quibit interaction, which scales naturally with the number of sites. The compiled circuit we show nevertheless, allows to represent this non unitary effect of the BC in a robust manner on quantum hardware. 
The circuits reproduce the global property of the boundaries for elliptic PDEs, namely the BC influence affects the complete domain. This conclusion can also be observed in the shape of the gates given in \Fig{fig:Transformation}, \Fig{fig:QNPU_Dirichlet}, and \Fig{fig:QNPU_Neumann} where multi-controlled toffoli gates scale with the number of qubits. 
The same behavior is found in the approaches used in \cite{Sato2021,Leong2022,Leong2023}. 

In the case of Neumann boundaries an improvement in the scalability can be achieve by substituting the Neumann circuit of \Fig{fig:QNPU_Neuman} by a mask implemented via the Potential circuit. For this time the potential circuit does no need a state preparation since the task can be split in two with the initialization of $\ket{00...00}$ and $\ket{00...01}$ for the left and right boundary respectively. Note that, the exponential scaling does not vanish completely since the Dirichlet circuit it is still necessary to remove the corners of the antidiagonal, also for the Neumann conditions. This alternative would reduce only the exponential scaling of one of the circuits.  
Another option is to measure state of the single qubit encoding the boundary point, as Sato does, or in our case the point next to the ghost point. With that information on that point a mask can be applied to achieve the desired value at the boundary. Although this idea would correct the exponential scaling it would also require more measurments and classic treatment on the boundaries, breaking the full quantum evaluation of the algorithm. 

For the two remaining QNPUs, Source and Potential, the same exponential scaling is observed. This is explained by the initilization of the multi-qubit statevector to an arbritrary state. Although necessary, this step is reported to be expensive and non-efficient \cite{Chen2021,Kyriienko2021,Creevey2023} and work is been invested in this topic \cite{Creevey2023,Melnikov2023,Araujo2021}. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/Gate_complexity_QNPU.png}
    \includegraphics[width=0.45\textwidth]{Figures/Gate_complexity_Ansatz.png}
    \caption{Gate complexity for all used QNPUs w.r.t he number of qubits. The circuits are first decompose in single qubits gates (Rz,Ry, u, u3) and two qubits gates (cx) and then added. For completeness the number of gates per qubits for the ansatz SO4 is also reported.}
    \label{fig:compilation:GateComplexity}
\end{figure}

\TODO{Gate complexity with sinus as f in source and potential. Remove exponential curves for potential and source. Give only the complexity curve for circuits w/o state vector preparation.}

\sbengoechea{As for the laplacian it is easy to see that the circuits for overlap and potential are efficient up to the shape of the function to be read. We do not include in this analysis the state vector preparation costs. However, in our study we have applied the state vector preprataion to encode the generic functions in the PDE which leads to an exponential scaling in many cases. We have concentrated in to algorithmic point of view. }

Another important aspect is the algorithm behavior w.r.t. shotnoise. In our case the use of the measurement approach explained in Sec. \ref{sec:measurement}) avoids the shot measurement to recover the expectation value. Therefore, the stability/robutsness against shotnoise of the approach has not been investigated in this publication. We refer the reader to \cite{Lubasch2020} where it is reported that the order of measuremnts M on the ancilla for the potential is independent of nq while for kinetic and non-lienar term M increases exponentially with nq. 


\subsection{Derivative Computation}
\label{sec:Derivative}
Section \ref{sec:Mathematics} finalized by stating the first-order optimality condition. To complete the shift to quantum hardware this detail is the only missing. Therefore, multiple techniques for the computation of the derivative exist. They are separated into the straightforward Numerical derivative, the Parameter shift rule \cite{Schuld2019,Banchi2021,Crooks2019}, and the Natural Gradient \cite{Stokes2020}. In the case of higher order derivatives, additional techniques come into account, as they are presented in \cite{Mari2021}. If measuring effect, e.g. noise, comes into account the reader is referred to \cite{Sweke2020}, which elaborates on stochastic gradient descent techniques in uncertain environments. 

However, assume to have the circuits above available, so that an evaluation of \Eq{eq:Discrete_Opt_BC} is realizable on the quantum hardware. Accordingly, the discretized expression of \Eq{eq:first_order_opt} can be evaluated in the following manner.
Due to the ghost point strategy, the boundary term in \Eq{eq:first_order_opt} vanishes and the discrete derivative is given as 
\begin{align}
\begin{split}
    \nabla_{\lambda_0} J(\upb) &= 
-2\nu\frac{\lambda_{0}}{\Delta x^2} \left(\underbrace{\sum\limits_k  u_k(\lamb_{c}) \left(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})-u_{k-1}(\lamb_{c})\right) }_{J_1 : \text{Periodic BC}} - 2\underbrace{\left( u_1(\lamb_{c})u_{NP}(\lamb_{c}) \right)}_{J_2 : \text{Dirichlet BC}} - \underbrace{\left(  u_1(\lamb_{c})^2 + u_{NP}^2 \right)}_{J_3 : \text{Neumann BC}}\right)\\
   &\quad- 2\underbrace{\sum\limits_k  u_k(\lamb_{c}) \Tilde{f}_k}_{J_4:\text{Source}}
   ,
\end{split}\\
\begin{split}
\nabla_{\lamb_c} J(\upb) &= -2\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \sum\limits_k  
\left(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})-u_{k-1}(\lamb_{c})\right)  \nabla_{\lamb_c}u_k(\lamb_{c})\\
%&\quad +\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \left( u_1(\lamb_{c}) \frac{\partial \nabla_{\lamb_c}u_1(\lamb_{c})}{\partial n} -  \frac{\partial u_1(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_1(\lamb_{c}) - u_{NP}(\lamb_{c}) \frac{\partial \nabla_{\lamb_c} u_{NP}(\lamb_{c})}{\partial n} -  \frac{\partial u_{NP}(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_{NP}(\lamb_{c})\right)\\
&\quad - 2\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \left(\left( u_1(\lamb_{c}) \nabla_{\lamb_c}u_{NP}(\lamb_{c}) +    u_{NP}(\lamb_{c}) \nabla_{\lamb_c}u_1(\lamb_{c}) \right) +\left( u_1(\lamb_{c})\nabla_{\lamb_c}u_1(\lamb_{c}) + u_{NP}\nabla_{\lamb_c}u_{NP} \right) \right)\\
&\quad - 2  \lambda_{0}   \sum\limits_k \Tilde{f}_k \nabla_{\lamb_c} u_k(\lamb_{c}) . 
\end{split}
\end{align}

It is clear to observe that the derivative would require manipulation of the implemented gate sequence for some terms. Despite the derivative with respect to $\lambda_0$. As indicated in the equation above, can the gate sequences for $J_i$ be used for an analytical evaluation of the derivative. For the derivatives with respect to the vector $\lamb_\text{c}$, the picture looks different. Here it needs to be distinguished between the terms where $u(\lamb_\text{c})$ appears quadratically and the rest. According to \cite{Schuld2019,Banchi2021,Crooks2019}, the derivative with the quadratic terms can be evaluated by using the so-called phase shift rule. It is based on the assumption that the ansatz $u$  is linear in each control $\lamb_i$ and consists of elementary rotational single parameter gates  \cite{Schuld2019,Crooks2019}. Then, the gate sequences can be reused and no compilation of the derivative needs to be derived. The analytic derivative follows using only 2 additional evaluations. Although alternatives to this approach exist, the implementation of the phase shift rule is straightforward, and it allows parallelization with respect to the number of parameters. For application, each parameter, when parameterized by one qubit gate, is varied by $s = \pm \frac{\pi}{4 r}$, with $ r= \frac{1}{4}$ formulated by \cite{Mitarai2018,Crooks2019}. The perturbed measured expectation values are used for the computation of the relative change, which aligns with the analytical derivative if $s$ is chosen correctly.  The product rule concerning the quadratic term is taken care of by this approach inherently. 

The terms, which appear with a linear setting of the trail function, do not follow this straightforward idea. Here the derivative is calculated using a second-order accurate finite difference approach, e.g. for a parameterization $g(x)$, given by the central difference scheme using a small perturbation $h$ is
\begin{align}
\nabla g(x) =  \frac{g(x+h) - g(x-h)}{2h} + \mathcal{O}(h^2).
\end{align}

This numerical derivative is of course an approximation, but only implies another 2 evaluations and does not require deriving a new gate sequence for evaluation of the derivative, which would only be 1 evaluation cheaper. 
Multiple appearances, e.g. cubic or fourth order, of one parameter, need to be treated according to the chain rule  \cite{Mari2021, Schuld2019}. In practical terms, the Ansatz of \Fig{fig:quantum_basic_ansatz} would require a chain rule adaption, whereby the Ansatz of \Fig{fig:quantum_ansatz_SO4} not because it is just linear in each $\lambda$. 

Applying the techniques above allows to approximate the derivatives given by 
\begin{align}
&\nabla_{\lambda_0} J(\upb) = 
-2\nu\frac{\lambda_{0}}{\Delta x^2} \left(J_1(\lamb_\text{c}) + J_2(\lamb_\text{c}) + J_3(\lamb_\text{c}) \right) - 2 J_4 (\lamb_\text{c}) ,\\
\begin{split}
\nabla_{\lamb_c} J(\upb) &= -\frac{ \nu \lambda_{0}^2}{\Delta x^2 } r \left(\left(J_1(\lamb_\text{c}+s) - J_1(\lamb_\text{c}-s)\right) - \left(J_2(\lamb_\text{c}+s) - J_2(\lamb_\text{c}-s)\right) +\left(J_3(\lamb_\text{c}+s) - J_3(\lamb_\text{c}-s)\right) \right) \\
&\quad - 2  \lambda_{0}  \frac{(J_4(\lamb_\text{c}+h) - (J_4(\lamb_\text{c}+h)}{2h} + \mathcal{O}(h^2).\\
%&\quad +\frac{ \nu \lambda_{0}^2}{\Delta x^2 } \left( u_1(\lamb_{c}) \frac{\partial \nabla_{\lamb_c}u_1(\lamb_{c})}{\partial n} -  \frac{\partial u_1(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_1(\lamb_{c}) - u_{NP}(\lamb_{c}) \frac{\partial \nabla_{\lamb_c} u_{NP}(\lamb_{c})}{\partial n} -  \frac{\partial u_{NP}(\lamb_{c})}{\partial n} \nabla_{\lamb_c}u_{NP}(\lamb_{c})\right).
\end{split}
\label{eq:quantum_derivative}
\end{align}

\pover{Check Derivative dimensions  - make shure scalar/vector match!}
\subsection{Optimization methodology}
\pover{barenplateaus -  vanishing gradient caused by random initialization and non local hamiltonians }
\pover{ May take riemian topology on quantum comp into account} \cite{Wiersema2023}
% do classical example! 
%https://www.researchgate.net/publication/3320516_Steepest_Descent_Algorithms_for_Optimization_Under_Unitary_Matrix_Constraint
%https://arxiv.org/pdf/2112.02572.pdf
% EVIDENCE Given in https://journals.aps.org/pra/abstract/10.1103/PhysRevA.107.062421

As common for VQAs is the classical realized optimization, a crucial point. It is often characterized as a non-trivial task. The publication \cite{Bittel2021} shows that the problem covered in VQA context is theoretically NP-Hard. The practice unveils the optimization of nonconvex functional, determined by e.g. multiple local stationary points as faced in \cite{Sarma2023,Leong2022,Wiersema2023}.  Additional to this, the effect of Barrett Plateaus can occur for high layer depths, whereby the vanishing derivative, an efficient update is impossible \cite{}. The use and practicability of zero-/first- or even second-/ order methods therefore highly differentiates with respect to convex optimization.  

A common approach for optimization problems classified as nonconvex is the use of zero-order evolutionary schemes for initial steps, since a good estimate for a starting position is not known in the first glimpse. The main group of these schemes is also known as sampling methods \cite{} Furthermore, has the experience unveiled that, in close vicinity of the stationary point, the necessity for an efficient number of iterations demands a first-order method. Despite this fact, of course, zero-order methods, e.g. the simplex method \cite{Nocedal2006}, as it is done in \cite{Leong2022} can be applied. Second order approaches require enormous overhead in measuring to construct the Hessian, but of course better results. All in all, they are not practicable \cite{Mari2021}. First-order methods, based on second-order models as given by the Quasi-Newton type algorithms, where the second derivative is estimated by rank-1 or even rank-2 updates \cite{Nocedal2006}, instead find its application for some VQAs \cite{  }. The additional effort for the approximation of the Hessian is here not given, but the requirement for a positive definite Hessian needs to be given as well. 

In contrast to this presented Euclidean view on the optimization manifold, there are efforts in choosing the descent direction with respect to the underlying Riemannian setting, which is mainly set due to the fact in \Eq{eq:partition_of_unity}. It is observed that, where the Euclidean approaches tend to local stationary points, the Riemannian strategies overcome these \cite{Wiersema2023}. Despite this, we restrict to the emphasized Euclidean setting, but a detailed view on the problem is crucial to achieve an efficient algorithm. 

Sticking to a Euclidean setting, we use a evolutionary algorithm coupled with a first-order method, to combine robustness in terms of the nonconvexity and high accuracy at the close vicinity of stationary points. We keep our algorithmic strategies to local updates. For the derivation of the update for the first order methods, mention the quantum compiled expression for the derivative in \Eq{eq:quantum_derivative}. Taking into account the functional itself, given in \Eq{eq:Discrete_Opt_BC}, it is clear that it is quadratic in $\lambda_0$. In case of the ansatz parameter $\lamb_\text{c}$, it is not so straightforward. For an evolution in time, the corresponding problem is solved iteratively, as emphasized in \Fig{fig:discretization_encoding}

The numerical strategy to address the variational problem in \Eq{eq:Discrete_Opt_BC}, compiled as described in Sec. \ref{sec:Compilation}, is two-folded. First, a Monte Carlo-based optimization, sampling method, so-called particle-swarm optimization \cite{Kennedy1995} is used, in order to determine a suitable initial parameter position. The algorithm is based on the next parameter $\lamb$ update
 \begin{align}
\lamb_{i+1} =& \lamb_{i}+\Delta \lamb_{i+1}\\
\Delta \lamb_{i+1} =& \underbrace{\omega \Delta \lamb_i}_\text{Momentum} + \underbrace{c_1 r_{1_i} \left(\lamb_{\text{best},i}-\lamb_i\right)}_\text{Learning}+ \underbrace{c_2 r_{2_i} \left(\lamb_{\text{best},i_\text{swarm}}-\lamb_i\right)}_\text{Communication}.
\end{align}
\pover{convergence criteria}
Once the Particle swarm is terminated, the obtained parameter setting is provided to the second method, namely a gradient descent method. Here the choice is the classical Gradient Descent given as
\begin{align}
        \lamb_{i+1} =& \lamb_{i} - \alpha \nabla J(\lamb_{i})
\end{align}

Convergence is determined by a tolerance \texttt{tol} at
\begin{align}
        \| \nabla J(\lamb_{i}) \|_2 \leq \texttt{tol}.
\end{align}
This two-step approach is relaxed by introducing an inner optimization loop, where in the first step $\lambda_0$ is kept constant and in a second step the whole control is updated. \textbf{}With this two-step approach, it is accomplished to cover extensively the unknown solution space. The difficulty of selecting an appropriate start location for fine-tuning and the nonlinear mapping to the Ansatz parameterization $\lamb$ is handled. For time step $t> 0$ and higher steps of inner iterations the previous optimal parameter are taken as initial guess as proposed by \cite{Sato2021,Leong2022}
The whole library given is made available by the in-house MPI-parallel PDE toolbox, with qiskit as an interface and backend. Inheritance and polymorphism allowed to establish an identical structure as presented here. As a summary, the complete algorithm is given in Alg. \ref{alg:VQA}.

\begin{algorithm}
\caption{VQ Algorithm}
\label{alg:VQA}
    \begin{algorithmic}
    \Require $NT, NP, \texttt{tol}, \lamb_0$
    \While{$t \leq T2 $}
        \While{$i\leq 10$}
            \If{i==0 or t==0}
                %\State $\lamb_i$ \gets PSO$(\lamb_0)$
            \Else
                %\State $\lamb_{\text{c}_i}$ \gets GD$(\lamb_i)$
            \EndIf
             \If{i==0 or t==0}
                %\State $\lambda_i$ \gets GD$(\lamb_i)$
            \Else
                %\State $\lamb_i$ \gets GD$(\lamb_i)$
            \EndIf
             %\State $\texttt{tol}$ \gets \texttt{tol}/inner
             %\State inner \gets inner+1
        \EndWhile
        %\State $t$ \gets $t+1$
    \EndWhile
    \end{algorithmic}
\end{algorithm}
\clearpage

==> Container/C_OldSections/Conclusion.tex <==
%###########################################
%       Conclusion
%###########################################
\section{Conclusion} \label{sec:Conclusion}
\pover{barenplateaus -  vanishing gradient caused by random initialization and non local hamiltonians }
\pover{ May take riemian topology on quantum comp into account} \cite{Wiersema2023}
% do classical example! 
%https://www.researchgate.net/publication/3320516_Steepest_Descent_Algorithms_for_Optimization_Under_Unitary_Matrix_Constraint
%https://arxiv.org/pdf/2112.02572.pdf
% EVIDENCE Given in https://journals.aps.org/pra/abstract/10.1103/PhysRevA.107.062421

\pover{We have a constant number of contributions to the costfunction if increasing qubits}


\trung{DO WE NEED THIS?: Choosing problem appropriate $u(x,\lamb_c)$'s shifts the problem \Eq{eq:Reduced_Opt} into a nonconvex setting, which of course is elaborated in detail given sec. \ref{sec:optimization} \cite{Bittel2021,Symons2023}. 
\pover{May add https://doi.org/10.1007/978-3-031-00832-0} -TO BE SHIFTED TO RESULTS SECTION}


\TODO{We simulate with  n noiseless ansatz qubits }
\pover{Convergence reseasons : }
%https://www.nature.com/articles/s41467-021-21728-w
%n [8], it is proved that the vanishing gradient problem can be avoided if the following conditionsare satisfied; (i) each term of the cost Hamiltonian, H = ∑
%k Hk is local, meaning that each term Hk
%is composed of less than m neighboring qubits, (ii) the ensemble of unitary matrices in each block is
%2-design, and (iii) the number of layers, `, is of the order O(poly(log n)). Note that each block needs
%to be deep enough for the distribution of corresponding unitary matrices to be close to 2-design
\pover{compare so4 with real value ansätze ?  }






\pover{Shift below to conclusion:
The proposed circuits reproduce that global behavior of the boundaries as indicated by the shape of the gates given in \Fig{fig:Transformation}, \Fig{fig:QNPU_BC_Dirichlet}, and \Fig{fig:QNPU_BC_Neumann} with multi-controlled Toffoli gates. These circuits, nevertheless, allows the robust representation of boundary conditions by adapting the non-unitary boundary matrix given by Sato et al. \cite{Sato2021} to the \textsc{QC} developed by Lubasch et al. \cite{Lubasch2020}. 
}

\pover{Imply correction of Neumann  by another ghost to get a higher resolution for small grids, evident in the low res poisson results}

\begin{itemize}
    \item It is shown that the \textsc{VQA} works in principle. However, the problem scales wrongly with the number of qubits $n$, making it very difficult to solve the optimization problem for $n \ge 8$. 
    \item The choice of the Ansatz is crucial. It defines the Hilbert space $\mathcal{H}$ where the solution is approximated.
    \item The measurement in the $\sigma_z$ basis is problematic. The found errors for highly entangled states are too big and constitute the Achilles heel of the approach. Alternatives such as \textsc{POVM} and \textsc{QST} need to be explored. For the time being, the trace-out method is used for the measurements. 
    \item The approach is still limited to Hamiltonian formulations in the form of $\psi H \psi $. For a more general application, it requires adaptation to $\psi H \theta$ with arbitrary trail functions $\psi$ and $\theta$. 
    \item The validation of the \textsc{VQCFD} code with textbook references is accomplished \cite{Griffiths2018}.
    \item The whole optimization approach can be enhanced by the application of the second Phase-Shift-Rule, to calculate the second-order derivative for the descent approach. 
    \item The hybrid optimization approaches delivered satisfactory results. Nevertheless, the cause of the fluctuations in the objective function and the derivative need to be clarified. 
    \item The current parallelization is a preliminary one and future work needs to be invested into a more extensive parallelization strategy. 
    \item The current setup is limited to periodic boundary conditions. This limitation needs to be overcome for the simulation of more realistic cases. 
    \item In a state simulation, the number of qubits is limited by the computational resources. Since the dimensions increase exponentially, the technique of Matrix Product State \textsc{MPS} is more suitable to work with a higher number of qubits and is a must-have for future implementations. 
    \item \sbengoechea{\cite{Lubasch2020} provides the possibility of implementing non-linear terms, a scenario that will be explored in future works.}
    \item \pover{Use a real quantum annealer for implementation , due to this you could come around the mininization calssically since it converges to the thermodynamic ground state , which coincidences with the optimum of an energy functional. Summarizing you will optimize using a quantum optimizer}
    \item Tightly relax the non-convex opt problem using quadratic progromming tech
\end{itemize}


\begin{itemize}
    \item We can solve all types of PDEs with arbitrary boundary conditions implemented in a QNPU structure.
    \vspace{0.5cm}
    \item The ghost point approach relaxes the requirements on the Ansatz functions $\psi(\pmb \lambda)$, especially in terms of the boundary conditions.
    \item The structure of the control-to-state operator $\psi(\pmb \lambda)$, the Ansatz, is affecting the optimization problem majorly. 
    \item The decomposition of non-unitary operations to gate-level ready tasks is non-trivial. 
    \item Boundary conditions are cast as QNPU elements.
    \item The ghost point approach relaxes the requirements on the Ansatz functions $\psi(\pmb \lambda)$, especially in terms of the boundary conditions.
    \item Quantum4PDE Problems can be cast into optimal control problems.
\end{itemize}

\textbf{OUTLOOK}
\begin{itemize}
    \item Proof of concept for the wave equation: 
    \begin{align*}
    \frac{\partial^2 u}{\partial^2 t} = \nu \frac{\partial^2 u\left(x\right)}{\partial x^2} + f\left(x\right)  \qquad \qquad \text{in \;} \Omega
    \end{align*}
 \item Develop a first-order derivative (convection) as a QNPU Operator, to solve Burgers equation. 
 \begin{align*}
      \frac{\partial u}{\partial  t}  + \pmb{u \frac{\partial u}{\partial x}}= \nu \frac{\partial^2 u\left(x\right)}{\partial x^2}+ f\left(x\right)  \qquad \qquad \text{in \;} \Omega
 \end{align*}
 \item Investigate mixed boundary conditions to enhance the industrial application,
 Dirichlet/Neumann (non-/homogeneous) 
\end{itemize}

\sbengoechea{Ideas on how to improve circuit scalability}

\pover{quote on sato section C  .  Quantum circuit for the shift operator
are already been marked as inefficient by \cite{Sato2021}, claiming the use of multi-controlled Toffoi gates as major bottleneck to create shallow circuits. As alternative may use \cite{Liu2021}  as decomposition approach , but scales less efficient. In terms of our approach only the bilinear form a(,) and the Linear operator F need to be measured. Which is an improve compared to \cite{Liu2021, Sato2021} <- Check }

In the case of Neumann boundaries, an improvement in the scalability can be achieved by substituting the Neumann circuit of \Fig{fig:QNPU_BC_Neumann} by a mask implemented via the Potential circuit. For this time the potential circuit does no need a state preparation since the task can be split in two with the initialization of $\ket{00...00}$ and $\ket{00...01}$ for the left and right boundary respectively. Note that, the exponential scaling does not vanish completely since the Dirichlet circuit it is still necessary to remove the corners of the antidiagonal, also for the Neumann conditions. This alternative would reduce only the exponential scaling of one of the circuits.  
Another option is to measure state of the single qubit encoding the boundary point, as Sato does, or in our case the point next to the ghost point. With that information on that point, a mask can be applied to achieve the desired value at the boundary. Although this idea would correct the exponential scaling, it would also require more measurements and classic treatment on the boundaries, breaking the full quantum evaluation of the algorithm. 

\sbengoechea{Comment on shot noise}
The robustness against shot noise has not been investigated in this publication. We refer the reader to \cite{Lubasch2020} where it is reported that the order of measurements $M$ on the ancilla for the potential is independent of $n$ while for the Laplacian QNPU \pover{and the non-linear term} $M$ increases exponentially with $n$. 

\cite{Wiersema2023}
"
However, there is evidence
that deep quantum circuits can have favorable
optimization properties [55, 50, 56]. Perhaps the
global convergence guarantees of double bracket
flows flows can be used to understand the con-
vergence properties of deep quantum circuits and
provide deeper insight into the power of VQE op-
timization.
"

\textbf{Validation}
In the appendix we have include two test cases for solving the time independent NLSE in order to validate our code. For that purpose we have taken the Free particle (only kinetic energy) and two different potentials, infinite sqr well and Harmonic trap. Our results are compared with the results given in the QM textbooks with excellent results. We can be certain that our code is validated.  







==> Container/C_OldSections/Discretization.tex <==
%###########################################
%       Discretization of the Governing equations
%###########################################
\section{Discretization of the Governing equations}  \label{sec:Discretization}
The variational setting, introduced in \Eq{eq:Reduced_Opt}, is sketched for spatial dynamics only. Yet is time evolution, as is the case for the heat equation or the wave equation, an important property of many PDE problems. The problems distinguish from the initially described elliptic setting in \Eq{eq:Generic_PDE}, hence the heat equation is parabolic, and the wave equation is characterized as a hyperbolic PDE. Nonetheless, we want to outline a consistent discretization to cast various PDE problems into the variational framework which is derived for elliptic PDEs. A technique for elliptic relaxation of the non-elliptic problems is introduced in the end of this section. As a sub-step, the discretization of each term in \Eq{eq:Generic_PDE} follows.

The dynamics are evaluated on a two-dimensional finite difference (FD) discretization, given by the mesh $\mathcal{M} \subset \Bar{\O}_\text{T}$. The spatial dimension $x$ in the interval $\left[0,1\right]$ is discretized by $N_\text{p}$ equality-spaced points, with spacing $\Delta x = \nicefrac{1}{N_\text{p}+1}$ \sbengoechea{(-1 or +1 to check dx)}. The discrete points $x_k$ are indexed with $k \in \left[0,N_\text{p}+1\right]$. The time $t\in [0,T]$ is discretized accordingly, given by $N_\text{t}$ points spaced with $\Delta t$ and indexed by $l \in \left[1,N_\text{t}\right]$. For exemplary reasons, \Fig{fig:discretization_encoding} shows the encoding of a complex valued scalar function $g(x,t): \mathbb{R} \times [0,T]\to \mathbb{C}$, where the discrete $g_k^l = g(x_k,t_l) : \forall k,l$ and consequently $\gb^l = \left(g_0^l, g_1^l, \hdots, g_{N_\text{p}+1}^l\right)^\text{T} = g_i^l \eb_i^l$ on the structured mesh $\mathcal{M}$.
\begin{figure}[htbp]
    \centering
    \input{Figures/Discretization}
    \caption{Encoding of the continuous function $g(x,t)$ on the discrete $x_k^l$ represented by $\mathcal{M}$.
    Boundary-/ Ghost-nodes:~(\protect\tikz \protect\draw[fill,gray] (1ex,1ex)  circle [radius=0.05];),~Internal-nodes:~(\protect\tikz \protect\draw[fill,black] (1ex,1ex)  circle [radius=0.05];) \sbengoechea{(indicate x,t point in the center as g(xk,t))}}
    \label{fig:discretization_encoding}
\end{figure}

Known from classical CFD techniques, BCs can be realized directly, as a part of the unknowns, or indirectly with the BCs not as part of the system of equations \cite{Ferziger2020}. In the latter, the BCs are represented by interpolating schemes, based on ghost points. A similar idea is emphasized by \cite{GonzalezConde2022}, which suggests a reflection of non-periodic effects at the original domain endpoints.
Aiming for a more flexible setting, we want to introduce quantum novelty, the so-called quantum ghost-nodes approach, as a prerequisite for the shift to the quantum hardware. 

The procedure is as follows, the boundary nodes must be taken as ghost nodes~(\protect\tikz \protect\draw[fill,gray] (1ex,1ex)  circle [radius=0.05];). For the internal nodes (\protect\tikz \protect\draw[fill,black] (1ex,1ex)  circle [radius=0.05];), the governing equations are solved and the values at the ghost nodes are obtained by the discretized BCs. The degrees of freedom at the two outer node locations are subtracted from free variables in the domain. Thus, the discrete function $\gb^l$, to be implemented in a register with length $n=\log_2(N_\text{p})$, is represented by 
\begin{align}
    \gb^l = g_0^l \eb_0 +  \underbrace{\sum\limits_{k=1}^{NP} g_k^l \eb_k}_\text{Register} + g_{N_\text{p}+1}^l \eb_{N_\text{p}+1}. 
    \label{eq:discretization_register}
\end{align}

Remark at this point, these changes consequently result in a more flexible numerical framework. Instead of the restrictions by the \textit{Ritz-Method} to the Sobolev space of BC conformal functions $y$, the framework is open to $W^{2,2}$. As a consequence, the ansatz requires only to be $u(\lamb_c) : \mathbb{R^c} \to W^{2,2}$. Of course, it is important to adapt the definition of the BCs in the whole problem description as well. At the end of this section, we emphasize this.

In the idea of FDs, the terms given in \Eq{eq:Generic_PDE}, need to be translated into a discrete analog to derive a consistent, converge, and robust framework. On the introduced discretization $\mathcal{M}$, the space collapses down to points-wise entities, which are taken to be constant at each $x_k$. With the equidistant and orthonormal discretization ($\Delta x =$ const.) and the Taylor expansion for $g$ in the close vicinity of $k$, an expression for a first-order approximation of the first derivative and a second-order accurate approximation of the second derivative is derived, \cite{Ferziger2020}, 
\begin{align}
\frac{\partial g^l}{\partial x} \bigg|_k  = \frac{g_{k+1}^l-g_k^l}{\Delta x} + \mathcal{O}(\Delta x^2)
, \quad
\frac{\partial^2 g^l}{\partial x^2}\bigg|_k = \frac{g_{k+1}^l-2g_k^l+g_{k-1}^l}{\Delta x^2} +  \mathcal{O}(\Delta x^3).
\label{eq:derivatives_space}
\end{align}
For the approximation of the integral operators, a first-order accurate midpoint rule is implied. For the introduced equidistant time discretization, it is straightforward to write an Euler backward rule, \cite{Ferziger2020} 
\begin{align}
    \frac{\partial g(x,t)}{\partial t} = \frac{g(x)^{l}-g(x)^{l-1}}{\Delta t} + \mathcal{O}(\Delta t^2).
    \label{eq:derivative_time}
\end{align}

Returning to the spatial implementation for $k=0$ and $k={N_\text{p}}$, exemplary derived for \Eq{eq:Generic_PDE}. The Dirichlet BCs defined need to be implied in the discrete non-conforming implementation of the functional $J(\upb)$, \cite{Grossmann2007}. The neglected effect of the Dirichlet BC by the ghost-points onto the internal domain is replaced by an additional term on the RHS. The corresponding RHS source term is given as
\begin{align}
\text{Dirichlet}: 
          f_\text{ghost} = \begin{pmatrix}
            a/\Delta x^2 \\
           \pmb 0 \\
            b/\Delta x^2
         \end{pmatrix}
         ,  \qquad \text{Neumann: }      
         f_\text{ghost} = \begin{pmatrix}
            -a/\Delta x \\
           \pmb 0 \\
            -b/\Delta x
         \end{pmatrix}.
         \label{eq:Ghost}
\end{align}
The two variables $a,b$ quantify Neumann and Dirichlet values, respectively. In the case of Neumann BC, the derivative is approximated with the first order approximation of the normal derivative $\nicefrac{\partial y(x)}{\partial n}$ on $\B$. If mixed BCs occur, the two definitions can of course be used in a superposition. If Periodic BCs are required, the ghost points are neglected and only the solution on the inner domain is taken into account. Accordingly, no modification of the RHS is required. 
Completed the modification of the linear operator $F(y)$, mention the changes on the bilinear term $a(y,y)$ discretizing the functional $J(\upb)$ in \Eq{eq:Generic_Opt_Approx}. In the case of periodic BCs, the summation is closed over $k = 1$ and $k={N_\text{p}}$, such that $u_0(\lamb_{c})=u_{N_\text{p}+1}(\lamb_{c})$ and then solved only on the internal domain.  In the case of Dirichlet BCs, using the ghost-point approach, the factors in front of $u_1(\lamb_{c})u_{N_\text{p}}(\lamb_{c})$ \sbengoechea{the periodic entries at the antidiagonal corners} need to vanish. In the case of the Neumann boundaries, the factors at the same location need to vanish as well. Additionally, the factors at $u_1(\lamb_{c})^2,u_{N_\text{p}}(\lamb_{c})^2$ need to be manipulated according to a forward/backward finite difference step \cite{Ferziger2020}. As a result, the factors are scaled to $\nicefrac{1}{\Delta x^2}$ \sbengoechea{(Where did 1/dx**2 come from? To check again)}. We have developed additional terms, which augment the discretized cost functional to achieve the described setting. The corrections are presented in \Eq{eq:Discrete_Opt_BC}, viz $j_2, \, j_3$  and $j_4$. Instead of modifying the stencils directly, \sbengoechea{(we do not have access to the differentiation matrices)}, the manipulations are introduced as additional terms visible as $j_2$ and $j_3$ (given in Sec. \ref{sec:Compilation:BC}). As evident from above, The term $j_4$ holds $\Tilde{f} = f + f_\text{ghost}$, incorporating non-homogeneous BCs (given in sec. \ref{sec:compilation:source}). Given in this general layout, the framework can be applied to all problems given by \Eq{eq:Generic_PDE} subject to various combinations of Dirichlet, Neumann, or Periodic BCs.


Time implicit formulation, using the stencil in \Eq{eq:derivative_time} for time depending PDEs, allows rewriting the PDE to a set of $l \in \left[1,N_\text{t}\right]$ problems, identical in the structure of \Eq{eq:Generic_PDE}. For $t=\Delta t,l=1$, the required reference is given by the previously defined initial conditions $y(x,0)$ of the initial boundary value problem. The subsequent steps $N_\text{t}$ steps are realized by another RHS $f_\text{time}$, taking into account the evolution in time. A similar approach has been presented by \cite{Leong2022}, analogically each time step requires solving one optimization problem $J^l$. With this, we can extend the framework based on elliptic PDE to approximate discrete-time parabolic and hyperbolic problems. With all terms given, any differential equation of the form \Eq{eq:Generic_PDE} can be treated. As a preliminary estimation, the time step $\Delta t$ determines by the Courant-number (Diffusion) $CO_\text{D} = \nicefrac{\nu \Delta t}{\Delta x^2}$ or Courant-number (Convection) $CO_\text{C}= \nicefrac{\nu \Delta t}{\Delta x}$ \cite{Ferziger2020}.

For the space $x\in[0,1]$, the time $t\in[0,T]$ and the assumption of a given discrete $y_k^l \rightarrow u_k^l$, the above-introduced discretization techniques can be applied to the continuous functional given in \Eq{eq:Reduced_Opt}. The RHS $f(x)$ is given by $\fb = \left(f_1, f_2,  \dots, f_k\right)^\intercal$, which holds the values of $f(x)$ as a vector constant over time. The RHS finally assembles as $\Tilde{f}= f + f_\text{ghost} + f_\text{time}$. For each cost contribution, a compiled expression is derived in section \ref{sec:Compilation}, which enables a quantum evaluation of the generalized functional $J(\upb)$ 
\begin{align}
\begin{split}
   J(\upb)^l &=  -\nu\frac{\lambda_{0}^2}{\Delta x^2} \left(\underbrace{\sum\limits_k  u_k^l(\lamb_{c}) \left(u_{k+1}^l(\lamb_{c})-2u_k^l(\lamb_{c})-u_{k-1}^l(\lamb_{c})\right) }_{j_1^l : \text{Periodic BC}} - 2\underbrace{\left( u_1^l(\lamb_{c})u_{N_\text{p}}^l(\lamb_{c}) \right)}_{j_2 : \text{Dirichlet BC}} - \underbrace{\left(  u_1^l(\lamb_{c})^2 + u_{NP}^l(\lamb_{c})^2 \right)}_{j_3 : \text{Neumann BC}}\right)\\
   &\quad- 2\lambda_{0}\underbrace{\sum\limits_k  u_k^l(\lamb_{c}) \Tilde{f}_k}_{j_4:\text{Source}}
    \label{eq:Discrete_Opt_BC}
    \end{split}
\end{align}
 \clearpage

==> Container/C_OldSections/Discretization_old.tex <==
%###########################################
%       Discretization of the Governing equations
%###########################################
\section{Discretization of the Governing equations}  \label{sec:discretization}
References: \cite{Ferziger2020}
%https://doi.org/10.1007/978-3-319-99693-6

\pover{Ghost point : Coppied from:
Further, non-periodic functions can be transformed into periodic functions by extending the
domain and reflecting the function about one of the original domain’s endpoints, to create a new function which is now
symmetric, as in Ref. [21], 
Simulating option price dynamics with exponential quantum speedup
Javier Gonzalez-Conde, Ángel Rodríguez-Rozas, Enrique Solano, Mikel Sanz
}

For the implementation of the above given, the continuous problem given in \Eq{eq:Reduced_Opt}, a consistent discretization technique on space is applied first.  Once the discretization is available, the compilation of the given problem \Eq{eq:Reduced_Opt} to the quantum hardware is done. As a sub-step, the terms in \Eq{eq:Generic_PDE} follow. For each of the terms, a compiled expression is derived, which allows evaluation of the functional $J(\upb)$ on quantum hardware.

The dynamics represented in the \Eq{eq:Generic_PDE} are evaluated on a one-dimensional finite difference discretization, given by the mesh $\mathcal{M} \subset \Omega$. The spatial dimension $x$ on the interval $\left[0,1\right]$ is discretized by $NP+1$ equality-spaced points, with spacing $\Delta x = \nicefrac{1}{NP+1}$. The abbreviation $NP$ \pover{Another abbreviation for Number of Points} refers to the “number of points”. The discrete points $x_k$ are indexed by $k \in \left[0,NP+1\right]$. The structured mesh $\mathcal{M}$ to the described setting is given in \Fig{fig:discretization_encoding}.

\begin{figure}[htbp]
    \centering
     \def\svgwidth{0.5\textwidth} 
    \input{Figures/Discretization}
    \caption{Encoding of the continuous function $g(x)$ on the discrete $x_k$ represented by $\mathcal{M}$. \sbengoechea{(Reduce labels Ghost ....)}}
    \label{fig:discretization_encoding}
\end{figure}

For exemplary reasons, \Fig{fig:discretization_encoding} shows the encoding of the complex valued scalar function $g(x)$, where the discrete $g_k = g(x_k) : \forall k$ and consequently $\gb = \left(g_0, g_1, \hdots, g_{NP+1}\right)^\text{T}$.
Known from classical numerical \sbengoechea{(CFD)} techniques, the boundary conditions can be realized directly as a part of the unknowns or indirectly where the boundary conditions are not part of the system of equations but are respected by interpolating schemes, taking the ghost points into the space dynamics. In addition, the dynamics of the internal space of course need to be adapted to include the information from the BC. Furthermore, constraints on the hardware the choice of the ansatz such that we suggest relying on the so-called ghost-point approach as a prerequisite for the shift to the underlying hardware\cite{Ferziger2020}. 
Therefore, the boundary nodes are required to be taken as ghost nodes. For the internal nodes, the governing equations are solved and the values at the ghost points are obtained by the discretized boundary conditions. 
The degrees of freedom at the two outer node locations are subtracted from free variables in the domain. As a consequence, the discrete function $\gb$ can now be represented by 
\begin{align}
    \gb = g_0 \pmb e_0 +  \underbrace{\sum\limits_{k=1}^{NP} g_k e_k}_\text{Register} + g_{NP+1} \pmb e_{NP+1},
\end{align}
where $e_i$ refers to an orthogonal basis in the corresponding discrete space. As indicated, can the sum, now be implemented in a register with length $n=\log_2({NP})$. These changes consequently result in a more flexible numerical framework, regarding the requirements of the ansatz. Initially, given by the theory of the Ritz-Method, the requirements for the choice of the test function are $y\in Y \subset H^2_0$. Instead of restricting the Hilbert space to boundary condition conformal functions, the framework is now $H^2$. As a consequence, the ansatz $u(x)$  requires only to be $u(\lamb_c) :  \mathbb{R^c} \to H^2$. Of course, it is important to adapt the definition of the boundary conditions as well. The Sec. \ref{sec:Discretization:BC} emphasizes this. 


Following the idea of finite differences, the terms given in \Eq{eq:Generic_PDE}, need to be translated into a discrete analog to derive a consistent, converge, and robust framework. As a basis, the introduced discretization $\mathcal{M}$ is used. On this finite difference approximation, the space collapses down to points-wise entities, which are taken to be constant at each $x_k$. 
For the derivation of the approximations mentioned, the Taylor expansion for $g$ in the close vicinity of $k$ is defined as, \cite{Ferziger2020},
\begin{align}
\begin{split}
        g_{k+1} &= g_k + \Delta x \frac{\partial g}{\partial x}\bigg|_k+\frac{\Delta x^2}{2!}\frac{\partial^2 g}{\partial x^2}\bigg|_k+ \frac{\Delta x^3}{3!}\frac{\partial^3 g}{\partial x^3}\bigg|_k + \mathcal{O}^4
\end{split}
\end{align}
\pover{checkspell : Recursing} the above equation, an expression for a first-order approximation of the derivative is derived 
\begin{align}
    \frac{\partial g}{\partial x} \bigg|_k  &= \frac{g_{k+1}-g_k}{\Delta x} + \mathcal{O}^2.
\label{eq:Upwind_FD}
\end{align}
The one-dimensional discrete Laplacian operator is derived by two Taylor expansions. To this end, the first derivative approximation in \Eq{eq:Upwind_FD} at position $k-1/2$ and $k+1/2$ is used in a central differencing approach, c.f. \cite{Ferziger2020},
\begin{align}
    \frac{\partial^2 g}{\partial x^2}\bigg|_k \approx \frac{\frac{\partial g}{\partial x}\big|_{k+\frac{1}{2}} + \frac{\partial g}{\partial x}\big|_{k-\frac{1}{2}}}{\Delta x}.
    \label{eq:second_derivative}
\end{align} 
Simplifying the expression above based on the equidistant and orthonormal discretization ($\Delta x =$ const.) of $\mathcal{M}$ results in 
\begin{align}
    \frac{\partial^2 g}{\partial x^2}\bigg|_k = \frac{g_{k+1}-2g_k+g_{k-1}}{\Delta x^2} +  \mathcal{O}(\Delta x^2).
\end{align}
For the approximation of the integral operators, a second-order accurate midpoint rule is implied. The integral expression simplifies to a summation weighted by $\Delta x$. Recall, that the midpoint rule is defined as \cite{Ferziger2020}
\begin{align}
    \int_a^b \square dx = (b-a) \sum\limits_x \square + \mathcal{O}^2.
\end{align}

 \TODO{Fit the eq in one line}
For the interval $x\in[0,1]$ and assumption of a given discrete $u_k$, the above-introduced discretization techniques can be applied to the continuous functional given in \Eq{eq:Reduced_Opt}. The RHS $f(x)$ is given by $\fb = \left(f_1, f_2,  \dots, f_k\right)^\intercal$, which holds the values of $f(x)$ as a vector. With all terms in the PDE in \Eq{eq:Generic_PDE} given, mention that for $k=0$ and $k={NP}$ the Dirichlet Boundary conditions must be taken into account. Respecting this, the analog discrete non-conforming implementation of the functional $J(\upb)$ is, \cite{Grossmann2007}
\begin{align}
    J(\upb) =  -\nu\frac{\lambda_{0}^2}{\Delta x^2}\sum\limits_k  u_k(\lamb_{c}) \left(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})+u_{k-1}(\lamb_{c})\right)  - 2\lambda_{0} \sum\limits_k  u_k(\lamb_{c}) f_k dx.
    \label{eq:Discrete_Opt}
\end{align}
Mention here that the discretization techniques are valid for all problems covered by \Eq{eq:Generic_PDE}  ($\zeta, \, \xi \in \mathbb{R}$). 

\subsection{Handling of Boundary Conditions} \label{sec:Discretization:BC}

As a preparation step before shifting to quantum hardware, the adaption of the Boundary Conditions to the above-introduced discretization is mandatory. In the case of the Dirichlet boundary conditions, as given in \Eq{eq:Generic_PDE}, the value at the ghost point is known. The neglected effect of the Dirichlet boundary condition onto the internal domain is replaced by an additional term on the RHS. The new augmented source $\Tilde{f}= f + f_\text{ghost}$. In the case of homogeneous Dirichlet boundary conditions $a=b=0$. For the sake of completeness, mention the similar approach applied in the case of Neumann boundary conditions. In contrast to a Dirichlet setting instead, a derivative is given as a boundary condition. The two corresponding RHS source terms are given as
\begin{align}
\text{Dirichlet}: 
          f_\text{ghost} = \begin{pmatrix}
            a/\Delta x^2 \\
           \pmb 0 \\
            b/\Delta x^2
         \end{pmatrix}
         ,  \qquad \text{Neumann: }      
         f_\text{ghost} = \begin{pmatrix}
            -a/\Delta x \\
           \pmb 0 \\
            -b/\Delta x
         \end{pmatrix}.
         \label{eq:Ghost}
\end{align}


The two variables $a,b$ quantify the \sbengoechea{first order derivative approximation} of the normal derivative $\nicefrac{\partial y(x)}{\partial n}$ on $\B$ in case of the Neumann boundary conditions. If mixed boundary conditions occur, the two definitions can of course be used in a superposition. 
If Periodic Boundary conditions are required, following the ghost point approach, introduces difficulties. In this case, the ghost points are neglected and only the solution on the inner domain is taken into account. Accordingly, no modification of the RHS is required. 

Instead of the discretized functional $J(\upb)$ given in \Eq{eq:Discrete_Opt}, the balance of the outer summands ($k = 1$ \& $k={NP}$) needs to be adapted for all types of boundary conditions. 
In the case of periodic boundary conditions, the summation is closed over $k = 1$ and $k={NP}$, such that $u_0(\lamb_{c})=u_{NP+1}(\lamb_{c})$ and then solved only on the internal domain. 
In the case of Dirichlet boundary conditions, using the ghost point approach, the factors in front of $u_1(\lamb_{c})u_{NP}(\lamb_{c})$ \sbengoechea{the periodic entries at the antidiagonal corners} need to vanish. In the case of the Neumann boundaries, the factors at the same location need to vanish as well. Additionally, the factors at $u_1(\lamb_{c})^2,u_{NP}(\lamb_{c})^2$ need to be manipulated according to a forward/backward finite difference step \cite{Ferziger2020}. As a result, the factors are scaled to $\nicefrac{1}{\Delta x^2}$ \sbengoechea{(Where did 1/dx**2 come from? To check again)}. 

Presenting a general framework, of course, requires adapting to any kind of boundary setting in small a turnaround time. Therefore, we have developed additional terms, which augment the discretized cost functional in \Eq{eq:Discrete_Opt} to achieve the indented setting. The generalized functional reads
\begin{align}
\begin{split}
   J(\upb) &=  -\nu\frac{\lambda_{0}^2}{\Delta x^2} \left(\underbrace{\sum\limits_k  u_k(\lamb_{c}) \left(u_{k+1}(\lamb_{c})-2u_k(\lamb_{c})-u_{k-1}(\lamb_{c})\right) }_{J_1 : \text{Periodic BC}} - 2\underbrace{\left( u_1(\lamb_{c})u_{NP}(\lamb_{c}) \right)}_{J_2 : \text{Dirichlet BC}} - \underbrace{\left(  u_1(\lamb_{c})^2 + u_{NP}^2 \right)}_{J_3 : \text{Neumann BC}}\right)\\
   &\quad- 2\lambda_{0}\underbrace{\sum\limits_k  u_k(\lamb_{c}) \Tilde{f}_k}_{J_4:\text{Source}}
    \label{eq:Discrete_Opt_BC}
    \end{split}
\end{align}
Instead of modifying the stencils directly, \sbengoechea{(we do not have access to the differentiation matrices)}, the manipulations are introduced as additional terms here visible as $J_2$ and $J_3$. As evident from above, the term $J_4$ now holds the tilde version of $f$, incorporating non-homogeneous boundary conditions. Given in this general layout, the framework can be applied to all problems given by \Eq{eq:Generic_PDE} subject to various combinations of Dirichlet, Neumann, or Periodic boundary conditions. One next step towards industrial application is prepared. \sbengoechea{Note that the special treatment for mixed BC. Because the mixed combination is not unitary, one needs to use mask function with the potential term. See next TODO}

\TODO{Just reference all the compilation sections comming downwards, to make it more readable }

\subsection{Time Dependecy}
The discretization of the variational setting introduced in \Eq{eq:Generic_OptimalControlProblem} could cover time evolution as well. In the case of the heat equation or the wave equation, the time derivative (first and second order) is crucial. In the same glimpse, these temporal terms are the difference to the initially described elliptic setting, hence the heat equation is parabolic and the wave equation is a hyperbolic PDE problem. Despite this, we want to outline a strategy to cast various PDE problems into the variational framework derived. Therefore consider a heat distribution $\vartheta(x,t) \in \mathbb{R}$ on the domain given one-dimensional bounded domain $\Bar{\O}$ with boundary $\B$ and the time $(T_1,T_2)$. Mention the heat equation, on $\O_T : = (T_1,T_2) \times \O , \; \BT : = (0,T) \times \B$ for the classical partial differential equation (\textsc{PDE}) given in the strong form, $\vartheta(x,t), f(x,t):\mathbb{R} \times (T_1,T_2) \to \mathbb{R}$ \sbengoechea{I would take the same solution letter as in Eq.1, $y$}
\begin{align}
\begin{split}
    \frac{\partial \vartheta(x,t)}{\partial t} -\Delta \vartheta(x,t) &= f(x,t) \quad \text{in} \quad \Omega_T,\\
    \qquad \vartheta(x,t) &= \vartheta_0 \quad \quad \text{on} \quad \B, \\
   \qquad  \vartheta(x,0) &= \vartheta_{t_0}           \quad \quad \text{on} \quad \BT.
    \label{eq:Heateq}
\end{split}
\end{align}

Now, in addition to the discretization in space as given in \Fig{fig:discretization_encoding}, \Fig{fig:discretization_time} introduces a discretization in time.

\begin{figure}[h]
    \centering
    \input{Figures/Discretization_time.tex}
    \caption{Time Discretization \TODO{merge with FIg. 1 in 3D}}
    \label{fig:discretization_time}
\end{figure}

Using this equidistant time discretization is straightforward to write an Euler backward rule, 
\begin{align}
    \frac{\partial \vartheta(x,t) }{\partial t} \approx \frac{\vartheta(x)^{t}-\vartheta(x)^{t-1}}{\Delta t}.
\end{align}
Implicit formulation, using the stencil in the above given PDE, allows rewriting the PDE to a set of NT problems of the form
\begin{align}
\begin{split}
   -\Delta t \Delta \vartheta(x)^{t} &=  \underbrace{\Delta t f(x)^{t} + \vartheta(x)^{t-1} - \vartheta(x)^{t}}_{f(x,\vartheta(x)^t)^{t}} \quad \text{in} \quad \O,\\
    \qquad \vartheta(x)^0 &= \vartheta_0 \quad \quad \text{in} \quad \B, \\
   \qquad  \vartheta(x) &= \vartheta_{t_0} \quad \quad\text{on} \quad \BT.
    \label{eq:elliptic_heat_eq}
\end{split}
\end{align}

For $t=1$, the required reference is given by the previously defined initial conditions $ \vartheta_0$ of the initial boundary value problem. The subsequent steps $NT$ steps are now described in the form of the second-order equation given initially in \Eq{eq:Generic_PDE}. Consequently, each timestep requires solving of one optimization problem $J_t$ covered analog to \Eq{eq:Discrete_Opt}. With this, we can extend the framework based on elliptic PDE to approximate discrete-time parabolic and hyperbolic problems.

In the following, the hardware requirements are introduced and the basic setting of the quantum framework used is given. Proceeding to this, the problem given in \Eq{eq:Discrete_Opt_BC} is compiled for the hardware. The derivation for each summand is shown in Sec. \ref{sec:Compilation}.

\clearpage

==> Container/C_OldSections/Introduction.tex <==
%###########################################
%       Introduction
%###########################################
\section{Introduction}\label{sec:Introduction}
\TODO{2 max 2.5 Pages}
\pover{
% Contradicting Pub:
Read this three and see if we need to cite: 
\cite{Sarma2023}  RECENT ! MENTION!
\cite{GonzalezConde2022}  %Second ancilla important for  ghost points ...   
\pover{Reference  Schrödinger Poisson
Towards Cosmological Simulations of Dark Matter on Quantum Computers
Philip Mocz (Princeton), Aaron Szasz (Perimeter Institute)}
%https://arxiv.org/abs/2101.05821
\cite{Mocz2021}
}
%###########################################
%
% --- INTRO TURBULENCE SCALES ---- 
%The large range of spatial and temporal scales in turbulent flows makes its computation very expensive, demanding larger computational centres with high power consumption \cite{Jaksch2023}. 
%
%This posses a problem in the study of flows for industrial and academic, such as, large-scale climate modelling \cite{X}, applications in energy\cite{X}, petrochemical \cite{X}, and transportation industries \cite{X}. but also relevant in the societal impact in biomedical and health research applications such as the development of drug delivery systems \cite{X} and medical devices \cite{X} or the analysis of physiological flows \cite{X}. 
%
% --- INTRO APPLICATIONS ---- 
%\sbengoechea{(the development of drug delivery systems \cite{X} and medical devices \cite{X} or the analysis of physiological flows \cite{X})}, 
%
% --- INTRO for non-Linear ----
%\cite{Berry2014} Despite the computational power of QC, a natural application for QC is linear diff equations, because time evolution under a Hamiltonian corresponds to a linear diff equation. The solution in QMechanics only includes oscillatory terms while general diff equations have solutions that grow or decay exponentially. Classical physics is described by more general diff. equations. Therefore the need of more general (non-linear) Q approaches as in Lubasch et al. 
%
% --- REVIEW QCFD MPS---
%It has recently been shown the benefits of applying quantum-based techniques on CFD calculations \cite{X,X}. This can be intrepreted as a reduced order modes with high  compression data techniques rates. In all these works the last step to from a tensor network to the quantum-gates is omitted. 
%In LiuWu the poisson equation is solve by decomposing the discrete derivative matrix as tensor products, in a quantum-inspired approach. 
%
% --- REVIEW QPDE ---
%The intro of MoawadVanderbauwheSteijl2022 gives a good overview of previous QCFD and QPDE. 
%The review about QC and PDE given in Garcia Molina Rodriguez 2022
%
%###########################################

Partial Differential Equations (\textsc{PDE})s are ubiquitous in science and engineering, modeling numerous phenomena ranging from classical mechanics, such as electrodynamics, thermodynamics, and fluid dynamics, to quantum physics. 
For industrial and academic applications in large-scale climate forecast \TODO{\cite{} cite NASA vii
sion}, energy \TODO{\cite{} cite}, petrochemical \TODO{\cite{} cite see proposal}, and transportation \TODO{\cite{} cite, see proposal}, as well as in biomedical and health research \TODO{\cite{} cite}, there are interests to resolve wide ranges of spatial and temporal scales making the computations very expensive and demanding energy-intensive supercomputing centers \cite{Jaksch2023}. \pover{NASA VISION 2030 https://ntrs.nasa.gov/citations/20140003093}
Moreover, the technological development described by Moore’s law is reaching its limit, due to the impossibility of reducing the transistor's size further \cite{Khan2018}. Convergence in the chip size for a classical Central Processor Unit (\textsc{CPU}), expected in the next decade, demands a paradigm change \cite{Demirdjian2022,Burg2021}. Quantum Computers (\textsc{QC}) promise to overcome these obstacles with a potential not capable of being delivered by their classical counterparts \cite{Jaksch2023}.

The advantage of \textsc{QC} relies on the exponential growth capacity to store and process information by its basic component, the qubit \cite{Jaksch2023}. The use of \textsc{QC}s for solving initial or boundary value problems has been attempted previously. In this respect, two categories include either the direct encoding of the \textsc{PDE} solution in one large quantum circuit or the Variational Quantum Algorithm (\textsc{VQA}) that evaluates shallow circuits in a hybrid strategy using classical optimizers \cite{Suau2021}. 

%FRIST
For the first category, Quantum Linear Solvers (\textsc{QLS}) have been extensively applied to systems of algebraic equations derived from the discretization of linear \textsc{PDE}s. The pioneering work of \cite{Harrow2009} presents a quantum algorithm to estimate the solution of Linear System of Equations (\textsc{LSE}), i.e. $Ax=b$. The approach is exponentially faster than classical algorithms for small condition numbers $k$ of $A$\sout{, between $1/k$ and 1}. The so-called \textsc{HHL} \pover{what is HHl - introduce abbreviation} method can be interpreted as an exponential accelerator for solving \textsc{LSE}. In \cite{Montanaro2016} a modified \textsc{HHL} is applied to solve a \textsc{LSE} originating from a Finite-Element Method (\textsc{FEM}) while the investigation of \cite{Berry2014} approximates the complete temporal evolution of a linear \textsc{PDE} with the mentioned \textsc{QLS}. 

Within the applications on fluid dynamics, the proposal of \cite{Steijl2018} recovers the vorticity for incompressible flows by merging the classical particle-mesh method for the Helmholtz equation with a quantum Fourier solver for the Poisson equation. 
At this point, it is also worth mentioning the works of \cite{Gaitan2020} and \cite{Oz2021} where the compressible Navier-Stokes and the Burgers' equation for one-dimensional \pover{inviscid -  double check} flows are resolved. In this case, the differential form of the \textsc{PDE} is spatially discretized into a system of coupled \textsc{ODE}s and approximated via a Quantum Amplitude Algorithm Estimation (\textsc{QAEA}) proposed by \cite{Kacewicz2006}. 
Another example has also been combined with spectral methods for solving first-order linear Ordinary Differential Equations (\textsc{ODE})s and second-order elliptic \textsc{PDE}s in \cite{Childs2020} and \cite{Childs2020a}, respectively. Here, the solution is approximated with truncated Fourier or Chebyshev series, in which the unknown coefficients are determined by a \textsc{QLS}. 
This type of quantum algorithm has also been used in the study of \cite{Cao2013} where the \textsc{HHL} quantum algorithm approximates the Poisson equation appearing in the predictor-corrector method when solving the incompressible Navier-Stokes equation. 
\sout{In the case of compressible flows, as in the work of }\cite{Chen2021}\sout{, the \textsc{HHL} method can be directly applied as \textsc{QLS} to approximate the \textsc{LSE} resulting from the discretized Navier-Stokes equations with classical Finite Volumes.}

\sout{
In the direct method the quantum acceleration is achieved by outsourcing the most computationally demanding part, i.e. solving the \textsc{LSE}, to the \textsc{QC}.} To complete efficiently the task of solving the \textsc{PDE} problem, \pover{the references above commonly require a large number of qubits, devoted for error-correction, in the quantum computing substep. Hence all approaches are suitable for future fault-tolerant quantum machines and less appropriate for the current Noise Intermediate-Scale Quantum (\textsc{NISQ}) era \cite{Suau2021}. }\sout{the quantum sub-step requires \sbengoechea{a large number of} \sout{many} qubits with specific ones devoted to error-correction, making the approach more suitable for future fault-tolerant quantum machines and less appropriate for the current Noise Intermediate-Scale Quantum (\textsc{NISQ}) era }\cite{Suau2021}. 

%SECOND

The development of hybrid classical-quantum \textsc{VQA}s, as a second category, provide an alternative, allowing to solve non-trivial problems with state-of-the-art \textsc{NISQ} devices \cite{Peruzzo2014}. \sbengoechea{This type of noise-tolerant algorithm is} based on the inexpensive evaluation of a cost function by the \textsc{QC} while the classical part optimizes the parameterized ansatz circuit, encoding the solution and avoiding the direct measurement of the quantum register. \sout{For application, the \textsc{PDE} to solve formulated as an optimization problem needs to be given.} \sbengoechea{As a consequence, the \textsc{PDE} to solve requires to be reformulated as an optimization problem.} The main advantage of the approach is the use of a short number of gate operations, making it more robust to the decoherence effects of the quantum gates composing the circuits. \sbengoechea{Decoherence in gates or register? ask Nis}

Hybrid \textsc{VQA}s are used in many applications such as the finding of ground states \cite{Peruzzo2014}, simulation dynamics of quantum systems \cite{} \TODO{CITE}, or solving \textsc{LSE} \cite{Cerezo2021}. Concerning its application for \sout{\textsc{PDE}s} \sbengoechea{\textsc{CFD}}, the work of \cite{Demirdjian2022} reformulates the advection-diffusion Burger's equation as a \textsc{LSE}, containing the full time and space solutions. The sparse matrix can be then decomposed in a finite series of unitary operators and solved by the variational quantum linear solver proposed by \cite{BravoPrieto2019}. In \cite{Kyriienko2021}, quantum neural networks are trained with a hybrid \textsc{VQA} to fulfill systems of nonlinear differential equations by optimizing the spectral base function coefficients. The method is tested for the compressible Navier-Stokes equation modeling supersonic transition in a nozzle. The work of \cite{Sato2021} explores the ability of \textsc{VQA}s to solve the Poisson equation by minimizing the potential energy of this elliptic \textsc{PDE} to find the steady state solution. To this end, the dynamics of the Poisson equation can be linearly decomposed in a series of parameterized shallow quantum circuits. The idea of energy minimization by \cite{Sato2021} is extended in \cite{Leong2022,Leong2023} by including time domains through the implicit time-stepping of the Laplacian operator for arbitrary right-hand side in \sbengoechea{elliptic \textsc{PDE}s}. Additionally, the diffusion parts and the pressure correction of the reaction-diffusion and the incompressible Navier-Stokes equation are treated semi-implicit by the \textsc{VQA} and the non-linear terms with classical approaches. 
\pover{The above text is very rich in references! I like it. Sometimes I have trouble to read it , it seems like a long enumeration of facts. Maybe when reforming it , we can also shorten it by one paragraph. }

% OUR WORK:
The present study is a further step in the collective effort of bringing Computational Fluid Dynamics (\textsc{CFD}) applications to \textsc{QC}s. To this end, the quantum framework described in \cite{Lubasch2020} is extended to cover not only \pover{I think they also cover Least square opt in time!} specific eigenvalue problems of quantum mechanics but also elliptic \textsc{PDE}s \pover{with a variational framework derived from the Galerkin and Ritz theories of weighted residuals and variational caclus (given in Sec. \ref{sec:Mathematics}).} \pover{We achived to outline similtudes, between the engineered framework and the version described by \cite{Sato2021}, which closses the loop to common engineering applications.} \sout{with an adapted version of the variational method described by } \cite{Sato2021}. \pover{I would describe our work as a paralell to satos work from engineering point of view, not as a simple repetition.} The following section \ref{sec:Compilation} covers one distinct feature of the quantum algorithm, initially motivated by \cite{Lubasch2020}, which is the use of theas quantum supremacy task described, Hadamard test based structure \cite{Guseynov2023}. The capability of single-qubit measurements, avoids the \sout{exponential} sampling for the reading of the \sout{output} \pover{result} encoded in a quantum state, \sout{that could} potentially vanish the quantum advantage \cite{Berry2014,Kyriienko2021}. The expensive post-processing of the output is especially pronounced \sbengoechea{in \textsc{VQA}} for \textsc{CFD}, hence \textsc{I/O} between classic and quantum parts occurs for every time step of the temporal integration \cite{Chen2021}. Application to elliptic PDEs finalized, an extension to all types of linear PDEs, is achieved with small addition effort. Implicit discretization in time, as the tool for the merge to an elliptic framework, make the framework capable to solve parabolic and hyperbolic PDES, as described in \cite{Leong2022,Leong2023}. \sout{ Furthermore, based on the common Laplacian operator in all types of linear \textsc{PDE}s, the presented quantum algorithm can also be modified to approximate parabolic and hyperbolic \textsc{PDE}s applying implicit time-marching evolution, as described in }\cite{Leong2022,Leong2023}. 

The correct and robust treatment of boundary condition, not only crucial for industrial application, is another enhancement covered. 
\sout{The correct treatment of the boundary conditions is crucial in the solving of \textsc{PDE}s. }
Despite the importance, its implementation is not trivial in the context of \textsc{QC}, as the disparity of incomplete approaches proposed in the literature demonstrates. 
In the works of \cite{Cao2013} and \cite{Childs2020} only Dirichlet conditions are contemplated, while in the related study of \cite{Childs2020a} the solution is mirrored into the symmetric and antisymmetric sub-spaces for Neumann and Dirichlet cases, respectively. 
The mixed boundary conditions for the Burger's equation in \cite{Oz2021} can only be enforced classically. 
In the algorithm of \cite{Costa2019}, Dirichlet or Neumann conditions are imposed on the discrete wave equation previous to the derivation of the Hamiltonian operator, i.e. the solutions in the Hilbert space need to satisfy the boundaries. A modification of this approach is presented by \cite{Suau2021} where only Dirichlet boundaries are possible to calculate. 
For \textsc{VQA} cases, the boundary conditions in \cite{Kyriienko2021} are included either as a part of the cost function or as an additional constraint on the ansatz functions. 
On the other hand, Dirichlet and Neumann boundary operators in \cite{Sato2021} do not form unitary operators, which requires classical implementation or the measurement of the whole quantum register. 
Therefore, a focal point of this study refers to a novel treatment of the boundary conditions specialized to the unique properties of the \textsc{QC} hardware. In particular, a classical ghost-point technique from \textsc{CFD} is combined with the unitary decomposition of the boundaries, as for the \textsc{PDE} operators \cite{Sato2021}, then compiled into quantum gates, and finally included as a constraint in the cost function. The proposed approach permits the full-quantum implementation of arbitrary homogeneous and inhomogeneous boundaries for Dirichlet, Neumann and mixed conditions without putting additional constraints on the trial functions.  

The final goal of this investigation is to address the natural question of how feasible and accurate \textsc{VQA} methods work for homogeneous and inhomogeneous linear \textsc{PDE}s with arbitrary boundary conditions. For that, the presented quantum framework is emulated \pover{using a cotempory highly paralell toolbox based on }with \textsc{IBM}'s \textsc{qiskit} environment in this study, \pover{The implemententation of QC Hardware is out of scope of this research. An implementation is recommended to be subject of future projects.} \sout{ since the \textsc{QC} is not yet ready}. 

\sbengoechea{The algorithm is hybrid ablet to be adapted for error mitigation and it exploits the shallow Qcircuits which makes it possible to implement with current and near-term QC.}

\TODO{The manuscript is divided in ... }
\pover{ <- may it is possible to referece the sections already in the text above}
\pover{To see if this needs to be included in the goals: Sell it as a libary of quantum Software as a set of compiled classical CFD algorithms into the quantum framework.}
\clearpage

==> Container/C_OldSections/Math.tex <==
%###########################################
%       Mathematical Framework
%###########################################
\pover{IDEE: Introduce PDE in time and space, then formualte weak in time space and discretize time space ...  We have then a ODE (follow eplliptic framework in a second step) in space an can apply the same framework with an additional rigt hand side.   Try to embed variational problem into a time variational problem }

\section{Mathematical Framework}  \label{sec:Mathematics}
In this section, we want to outline the mathematical framework and the idea of solving PDEs as a variational problem designed to be executed on quantum hardware. Similar to \cite{Leong2022,Leong2023,Sato2021,Arrazola2019,Cao2013}, the to-be-presented problem is cast into a so-called ansatz method \cite{Grossmann2007}. All of these publications cover techniques shifted from classical CFD to a quantum computing environment, which the common goal to pave the road for QCFD. In contrast to the given-above references, the mathematical framework to-be-presented is capable of being applied to nonlinear problems as well as arbitrary combinations of boundary conditions. \pover{? Do we violate the v-elliptic setting}
We unveil the developed framework restricted to a one-dimensional ($d=1$) spatial domain $\bar{\O}$, where the internal domain $\O$ is subject to multiple dynamics. The boundary condition setting changes. As introduction, the state $y_{\Bar{\O}}(x): \mathbb{R}^d \to \mathbb{R}$ is defined in $\Bar{\O}$ with boundary $\B : = \Bar{\O}/\O$. The one-dimensional domain is the frequently covered unit interval. Here we introduce a second-order differential equation, in the homogeneous Dirichlet boundaries condition (BC) setting, given as
\begin{align}
\begin{split}
     -\nu \Delta y_{\Bar{\O}}(x) -\zeta y_{\Bar{\O}}(x)p(x) -\xi y_{\Bar{\O}}(x)^{r} &= f(x) \quad \text{in } \O : =  (0,1)\\
   y_{\Bar{\O}}(0) = y_{\Bar{\O}}(1)  &= 0  \qquad \;\, \text{on } \B \\
   \end{split}
        \label{eq:Generic_PDE}
\end{align}

The right-hand-side (RHS) is given by a known source term $f(x): \mathbb{R} \to \mathbb{R}$. For now, it is assumed, that $f \in C$. \pover{Which is the requirement to f?}. It represents effects on the dynamical system. The Greek $\xi\in\mathbb{N}$ denotes the scale of the $r$-th order nonlinearity. The product of an external potential $p(x)$ and the state $y_{\Bar{\O}}(x)$ is scaled by $\zeta\in \mathbb{R}$. The Greek letter $\nu>0$ is the diffusion coefficient. To generalize the complete two-point boundary-value problem, mention that the boundary conditions play an important role in the reformulation of a boundary-value problem to a variational problem \cite{Grossmann2007}. This is why we stay with the homogeneous Dirichlet setting for now. Later it is extended to Neumann- and mixed-boundary conditions (the interested reader is referred to Sec. \ref{sec:Discretization}). Furthermore, we assume in the beginning that $\zeta=0 \, \& \,\xi=0$, such that we recover the commonly known Poisson equation.

As a common computational strategy in engineering, we follow the weaker notation of the PDE in \Eq{eq:Generic_PDE}, given by the weighted residual technique with the weighting-function $z_{\Bar{\O}}(x) \in C\left(\Bar{\O}\right)$. Assuming the existence of a twice differentiable solution $\hat{y}_{\Bar{\O}} \in C^2\left(\O\right) $ solving \Eq{eq:Generic_PDE}, consecutive multiplication and integration results in the variational equation, for which every solution $\hat{y}_{\Bar{\O}}$ of \Eq{eq:Generic_PDE} satisfies
\begin{align}
 \int_{\O}  z_{\Bar{\O}}(x) R(\hat{y}_{\Bar{\O}}(x)) dx  = 0  \quad \forall z_{\Bar{\O}}(x), \quad \text{ with} \quad  R(\hat{y}_{\Bar{\O}}(x)) = -\nu \Delta \hat{y}_{\Bar{\O}} (x)- f(x) = 0. \label{equ:weighted_res}
\end{align}

Splitting the occurring order of the arguments of the variational equation, in a bilinear $a(y_{\Bar{\O}},z_{\Bar{\O}})$ and linear $F(z_{\Bar{\O}})$ form (omitting the arguments), the abstract setting $    a(y_{\Bar{\O}},z_{\Bar{\O}}) =  F(z_{\Bar{\O}})$ reads
\begin{align}
    a(y_{\Bar{\O}},z_{\Bar{\O}}): = - \nu\int_{\O} z_{\Bar{\O}} \Delta y_{\Bar{\O}} dx = \int_{\O} z_{\Bar{\O}} f dx = : F(z_{\Bar{\O}}).
        \label{eq:variational_eq}
\end{align}

The obtained variational equation is the starting point for the application of the most well-known approach to get a flexible numerical framework, viz. the \textit{Galerkin approach of weighted residuals} \cite{Ern2004}. The choice of $z_{\Bar{\O}}$, associated with a certain numerical method, makes it possible to derive a system of equations driving  the residual $R(y_{\Bar{\O}})$ at any point in time-space to zero.
Commonly, $z_{\Bar{\O}} \in C^1\left(\O\right)$, which allows integration by parts to derive a super weak formulation of the strong problem in \Eq{eq:Generic_PDE}. Despite, this last step is not applied here, which makes the framework only characterized by the property “weak in space”.


In the following, we want to present a universal optimization approach to solve \Eq{eq:Generic_PDE}. First mention, that the boundary conditions are limited to the definition of \Eq{eq:Generic_PDE}, viz. $y_{\Bar{\O}} \in W^{2,2}_0 \left(\O\right)$  and $z_{\Bar{\O}} \in W^{0,2}_0 \left(\O\right)$. Furthermore, it is assumed that the bilinear form $a(y_{\Bar{\O}},z_{\Bar{\O}}): W^{2,2}_0 \times W^{0,2} \to \mathbb{R}$ is continuous, elliptic  and symmetric, then $\hat{y}_{\Bar{\O}}$ is also a solution to the variational problem, \cite{Grossmann2007,Glowinski2015},
\begin{align}
    \min\limits_{y_{\Bar{\O}} \in H^2_0} \mathcal{J}(y_{\Bar{\O}}) \quad  \text{with} \quad \mathcal{J}(y_{\Bar{\O}}):= a(y_{\Bar{\O}},y_{\Bar{\O}}) - 2F(y_{\Bar{\O}}).
    \label{eq:Generic_Opt}
\end{align}

The functional $\mathcal{J}(y_{\Bar{\O}}): W^{2,2}_0 \to \mathbb{R} $ is referred to as the exact objective. We now apply the \textit{Ritz-method} to solve the problem given in \Eq{eq:Generic_Opt} approximately. Therefore, we choose a finite-dimensional subspace $Y \subset W^{2,2}_0$ and solve for the solution $\hat{y} \in Y$ characterized by, \cite{Grossmann2007},
\begin{align}
    \min\limits_{y \in Y} \mathcal{J}(y) \quad  \text{with} \quad \mathcal{J}(y):= a(y,y) - 2F(y).
    \label{eq:Generic_Opt_Approx}
\end{align}
The state $y$ approximates $y_{\Bar{\O}}$ and is commonly referred to as the ansatz function or test function. The ansatz function is assumed to be given by a known mapping $u(\lamb_{c}): \mathbb{R}^{c} \to Y$, where $c\in \mathbb{N}$ defines the number of control parameters $\lamb$.  At this point, it is important to mention, that the ability to represent an arbitrary state $y$ on the final hardware is limited. It is required to fulfill the partition of unity in the form of an isoperimetric condition, given by the $L^2$ scalar product as \cite{Troutman1996,Werner2005}
\begin{align}
    (y^*,y)_{L^2} = \int_{\O}  y^*(x) y(x) dx =  1.
    \label{eq:partition_of_unity}
\end{align}

With the restriction to the normalized subspace $(\|y\|_{Y} = 1)$, the problem relies on a constraint functional space.
%###########################################
%       Optimal Control Problem
\subsection{Optimal Control Problem} \label{sec:optimal_control}
Moving the variational framework designed previously into the constraint functional space, explicitly given by \textit{Lie groups}, reduces the computational complexity heavily by the variability in the corresponding parameter space \cite{Abrudan2005}. The function $y$ is here made variable by the control $\upb \in \mathbb{R}^{c+1}, \upb: = \left(\lambda_0, \lamb_c\right)^\intercal$, such that 
\begin{align}
    y(x)(\upb) = \lambda_{0} u(x)(\lamb_c).
        \label{eq:Generic_Ansatz}
\end{align} 
The ansatz, $(u(x)(\lamb_c) : (u(x)(\lamb_c)^*, u(x)(\lamb_c))_{L^2} = 1$ as a Lie group embedding, enforces the restriction of the solution $y(x)$. Mention the fact that the parameterization $\lamb_\text{c}$ makes the position $y(x)$ on a hyper-sphere surface variable. Consequently, the path between multiple controls $\lamb_\text{c}$ is always referred to a tangential direction on the hyper-surface of the functional space. Classically speaking, are all ansatz related to a specific Lie Group \cite{Hall2010}.

In the following, we assume that the state $y(x)$ can be represented uniquely by the control $\upb$, $ \upb \mapsto \yb$. This requirement to the ansatz is interpreted as classical equality constraint $e(y,\upb)) =  y(x) - \lambda_{0} u(x)(\lamb_{c}) = 0$. It is straightforward to augment the unconstrained minimization problem in \Eq{eq:Generic_Opt_Approx} by the equality constraint $e(y,\upb)$, to achieve the optimal control problem $  \min \limits_{y}  \mathcal{J}(y) \text{ s.t. } e(y,\upb) = 0.$
In terms of optimal control theory, the equality constraint $e(y,\upb)$ denotes a \textit{control-to-state operator}, which is essential in the later-to-be-presented framework \cite{Troutman1996}. As it is possible here, the constraint $e(y,\upb)$ is realized directly by substitution. Accordingly, we formulate the complete unconstrained optimization problem, given the reduced objective $J(\upb) : \mathbb{R}^{c+1} \to \mathbb{R}$, as 
\begin{align}
	\begin{split}
     \min \limits_{\upb} J(\upb)  \quad \text{with} \quad J(\upb) :=& a(y(\upb),y(\upb)) - 2F(\upb),\\
			 =&  - \nu\int_{\O} \lambda_{0}^2 u(x)(\lamb_{c}) \Delta u(x)(\lamb_{c}) dx - 2 \int_{\O} \lambda_{0} u(x)(\lamb_{c}) f(x) dx.
	\end{split}
\label{eq:Reduced_Opt}
\end{align}

The problem in \Eq{eq:Reduced_Opt} can of course be solved using zero-order approaches, e.g. sampling methods \cite{Nocedal2006, Dennis1996}. The framework presented applies first-order approaches. Despite, the problem highly depends on the choice of $u(x)(\lamb_c)$ and thus on \textit{Lie-Algebra} theory. Choosing problem appropriate $u(x)(\lamb_c)$'s shifts the problem \Eq{eq:Reduced_Opt} into a nonconvex setting, which of course is elaborated in detail given sec. \ref{sec:optimization} \cite{Bittel2021,Symons2023}.
\pover{May add https://doi.org/10.1007/978-3-031-00832-0}

Nevertheless, the optimal value coincide with a stationary point $\bar{\upb} : J(\upb)  \geq  J(\bar{\upb}) \quad \forall \upb$ \cite{Troutman1996}. Taking the Gâteaux derivative with respect to the argument of $J(\upb)$ the condition for an optimal point can be reformulated as a first-order optimality condition, which is \cite{Troutman1996}
\begin{align}
    \frac{\partial J}{\partial \upb} \delta \upb&= \begin{pmatrix}
            \nabla_{\lambda_0} J(\upb) \\ 
            \nabla_{\lamb_c} J(\upb) 
        \end{pmatrix} \cdot \begin{pmatrix}
            \delta \lambda_0\\
            \delta \lamb_c
        \end{pmatrix} =  0 \quad \forall \delta\upb, \\ 
    \begin{split} 
        &= -2\nu\int_{\O} \lambda_{0} u(\lamb_{c}) \Delta u(\lamb_{c}) \delta \lambda_{0} dx - 2 \int_{\O} u(\lamb_{c}) f \delta\lambda_{0} dx \\
        &\quad\,-\nu\int_{\O} \lambda_{0}^2 u'(\lamb_{c})\delta\lamb_{c}\Delta u(\lamb_{c}) dx-\nu\int_{\O} \lambda_{0}^2 u(\lamb_{c})
        \Delta u'(\lamb_{c}) \delta\lamb_{c} dx - 2 \int_{\O} \lambda_{0} u(\lamb_{c})' \delta\lamb_{c} f dx.
    \end{split}
    \label{eq:first_order_opt}
\end{align}
The dash "'“, indicates the derivative with respect to $\lamb_c$. The argument concerning the space in $u$ and $f$ has been neglected for clarity. 

\pover{ Is it the Riemanian Gradient  or  Euklidian Gradient /Derivative ?  }

Proceeding, a reformulation of the Gâteaux derivatives in the equation \Eq{eq:first_order_opt} by the application of Green's Second Identity, to isolate the variational terms, is performed. After two integrations by parts, the Gâteaux derivative with respect to the control gives
\begin{align}
\nabla_{\lambda_0} J(\upb) \delta \lambda_0 &= -2 \nu \lambda_{0} \int_{\O}  u(\lamb_{c}) \Delta u(\lamb_{c}) \delta \lambda_{0} dx -2 \int_{\O} u(\lamb_{c}) f \delta\lambda_{0} dx, \\
%\begin{split}
%\nabla_{\lamb_c} J(\upb) \delta \lamb_c&= -2\nu \lambda_{0}^2 \int_{\O}  u(\lamb_{c})' \delta\lamb_{c} \Delta u(\lamb_{c}) dx -\nu\lambda_{0}^2  \int_{\B}  u(\lamb_{c})' \frac{\partial u(\lamb_{c}) \delta\lamb_{c}}{\partial n} -  u(\lamb_{c})' \delta\lamb_{c} \frac{\partial u(\lamb_{c})}{\partial n}  ds \\
%&\quad \,- 2  \lambda_{0} \int_{\O}   u(\lamb_{c})' \delta\lamb_{c} f(x) dx.  \text{\pover{Reformulate to isolate delta  -  check next eq. }}
%\end{split}\\
\begin{split}
\nabla_{\lamb_c} J(\upb) \delta \lamb_c&= -2 \nu\lambda_{0}^2 \int_{\O}  \Delta u(\lamb_{c})  u(\lamb_{c})' \delta\lamb_{c}dx -\nu\lambda_{0}^2  \int_{\B}  u(\lamb_{c}) \frac{\partial u(\lamb_{c})' \delta\lamb_{c}}{\partial n} -  \frac{\partial u(\lamb_{c})}{\partial n} u(\lamb_{c})' \delta\lamb_{c}   ds \\
&\quad \,- 2  \lambda_{0} \int_{\O} f(x) u(\lamb_{c})' \delta\lamb_{c}  dx.
\end{split}
\end{align}
\pover{Reformulate to isolate delta commented equation -  check next eq. }
\pover{reformulate by pulling variations out  .. just state final solution}

As evident, by the chosen space $W^{2,2}_0$ and assuming bijectivity, vanishes, both $u(\lamb_{c})$ and $ u(\lamb_{c})' \delta\lamb_{c}$ on the boundary. Hence, the surface integral can be neglected \cite{Grossmann2007}. It is different for other boundary setting, since Section \ref{sec:Discretization} emphasizes on this in detail. However, in contrast to \cite{Sato2021,Leong2022} the first-order optimality condition for $\lambda_0$ is not substituted into the reduced functional $J(\upb)$. Of course, this is a valid approach, nevertheless showed our experience that having full control over $\lambda_0$ is beneficial.  The consistent approximation of the given theory (Sec. \ref{sec:Discretization}) introduces the compilation to quantum hardware (Sec. \ref{sec:Compilation}), which finalizes in the presentation of numerical results (Sec.\ref{sec:Applications}).
\clearpage

==> Container/C_OldSections/Math_old.tex <==
%###########################################
%       Mathematical Framework
%###########################################
%\pover{interpret ansatz as a switching to cylinder / spherical coordinates} 

\TODO{max 3 Pages}

\pover{IDEE: Introduce PDE in time and space, then formualte weak in time space and discretize time space ...  We have then a ODE (follow eplliptic framework in a second step) in space an can apply the same framework with an additional rigt hand side.   Try to embed variational problem into a time variational problem }

\section{Mathematical Framework}  \label{sec:Mathematics}
In this section, we want to outline the mathematical framework and the idea of solving PDEs as a variational problem designed to be executed on quantum hardware. Similar to \cite{Leong2022,Leong2023,Sato2021,Arrazola2019,Cao2013}, the to-be-presented problem is cast into a so-called ansatz method \cite{Grossmann2007}. All of these publications cover techniques shifted from classical CFD to a quantum computing environment, which the common goal to pave the road for QCFD. In contrast to the given-above references, the mathematical framework to-be-presented is capable of being applied to nonlinear problems as well as arbitrary combinations of boundary conditions. \pover{? Do we violate the v-elliptic setting}
We unveil the developed framework restricted to a one-dimensional ($d=1$) spatial domain $\bar{\O}$, where the internal domain $\O$ is subject to multiple dynamics. The boundary condition setting changes. As introduction, the state $y_{\Bar{\O}}(x): \mathbb{R}^d \to \mathbb{R}$ is defined in $\Bar{\O}$ with boundary $\B : = \Bar{\O}/\O$. The one-dimensional domain is the frequently covered unit interval. Here we introduce a second-order differential equation, in the homogeneous Dirichlet boundaries condition (BC) setting, given as
\begin{align}
\begin{split}
     -\nu \Delta y_{\Bar{\O}}(x) -\zeta y_{\Bar{\O}}(x)p(x) -\xi y_{\Bar{\O}}(x)^{N} &= f(x) \quad \text{in } \O : =  (0,1)\\
   y_{\Bar{\O}}(0) = y_{\Bar{\O}}(1)  &= 0  \qquad \;\, \text{on } \B \\
   \end{split}
        \label{eq:Generic_PDE}
\end{align}
\TODO{DECIDE WITH SERGIO if we introduce time up here or not!! and adjust linear and nonlinear terms}

The right-hand-side (RHS) is given by a known source term $f(x): \mathbb{R} \to \mathbb{R}$. For now, it is assumed, that $f \in C$. \pover{Which is the requirement to f?}. It represents effects on the dynamical system. The Greek $\xi\in\mathbb{N}$ denotes the scale of the $r$-th order nonlinearity. The product of an external potential $p(x)$ and the state $y_{\Bar{\O}}(x)$ is scaled by $\zeta\in \mathbb{R}$. The Greek letter $\nu>0$ is the diffusion coefficient. To generalize the complete two-point boundary-value problem, mention that the boundary conditions play an important role in the reformulation of a boundary-value problem to a variational problem \cite{Grossmann2007}. This is why we stay with the homogeneous Dirichlet setting for now. Later it is extended to Neumann- and mixed-boundary conditions (the interested reader is referred to Sec. \ref{sec:Discretization}). Furthermore, we assume in the beginning that $\zeta=0 \, \& \,\xi=0$, such that we recover the commonly known Poisson equation.

Implementation and approximation of the problem in \Eq{eq:Generic_PDE} above can become tedious, for example, introduce regularity problems in the solution process. As a common computational strategy in engineering, an alternative weaker notation of the PDE in its strong form is formulated following a weighted residual technique. Assuming the existence of a twice differentiable solution $\hat{y}_{\Bar{\O}} \in C^2\left(\O\right) $, solving \Eq{eq:Generic_PDE} and mention the consecutive multiplication with an arbitrary weighting-function $z_{\Bar{\O}}(x) \in C\left(\Bar{\O}\right)$ and integration results in the variational equation, for which every solution $\hat{y}_{\Bar{\O}}$ of \Eq{eq:Generic_PDE} satisfies
\begin{align}
 \int_{\O}  z_{\Bar{\O}}(x) R(\hat{y}_{\Bar{\O}}(x)) dx  = 0  \quad \forall z_{\Bar{\O}}(x), \quad \text{ with} \quad  R(\hat{y}_{\Bar{\O}}(x)) = -\nu \Delta \hat{y}_{\Bar{\O}} (x)- f(x) = 0. \label{equ:weighted_res}
\end{align}

Splitting the occurring order of the arguments of the variational equation, in a bilinear $a(y_{\Bar{\O}},z_{\Bar{\O}})$ and linear $F(z_{\Bar{\O}})$ form (omitting the arguments), the setting reads
\begin{align}
    a(y_{\Bar{\O}},z_{\Bar{\O}}): = - \nu\int_{\O} z_{\Bar{\O}} \Delta y_{\Bar{\O}} dx = \int_{\O} z_{\Bar{\O}} f dx = : F(z_{\Bar{\O}}).
        \label{eq:variational_eq}
\end{align}
For the sake of completeness, mention the variational equation in its abstract form $    a(y_{\Bar{\O}},z_{\Bar{\O}}) =  F(z_{\Bar{\O}})$.

The obtained variational equation is the starting point for the application of the most well-known approach to get a flexible numerical framework, e.g. the \textit{Galerkin approach of weighted residual} \cite{Ern2004}. As the residual $R(y_{\Bar{\O}})$ vanishes at any point in time-space, it also vanishes for an arbitrary weight function $z_{\Bar{\O}}$. Here, the choice of $z_{\Bar{\O}}$, associated with a certain numerical method, makes it possible to derive a system of equations. One common choice is $z_{\Bar{\O}} \in C^1\left(\O\right)$, which allows integration by parts to derive a super weak formulation of the strong problem in \Eq{eq:Generic_PDE}. However, this last step is not applied here, which makes the framework only characterized by the property “weak in space”. In addition to this, the solution to the problem of \Eq{eq:Generic_PDE} is intended to be obtained by optimization. 

In the following, we want to present a universal approach. To explicitly distinguish between the quantum state space $H^\square$ and the Sobolev space $W^{\square,\square}$ as the setting for the PDE solutions, we neglect the abbreviation $H^2 \leftrightarrow W^{2,2}$. However, mention that the boundary conditions are limited to the definition of \Eq{eq:Generic_PDE}, viz. $y_{\Bar{\O}} \in W^{2,2}_0 \left(\O\right)$  and $z_{\Bar{\O}} \in W^{0,2}_0 \left(\O\right)$. Furthermore, it is assumed that the bilinear form $a(y_{\Bar{\O}},z_{\Bar{\O}}): W^{2,2}_0 \times W^{0,2} \to \mathbb{R}$ is continuous, elliptic  and symmetric, then $\hat{y}_{\Bar{\O}}$ is also a solution to the variational problem, \cite{Grossmann2007,Glowinski2015},
\begin{align}
    \min\limits_{y_{\Bar{\O}} \in H^2_0} \mathcal{J}(y_{\Bar{\O}}) \quad  \text{with} \quad \mathcal{J}(y_{\Bar{\O}}):= a(y_{\Bar{\O}},y_{\Bar{\O}}) - 2F(y_{\Bar{\O}}).
    \label{eq:Generic_Opt}
\end{align}

The functional $\mathcal{J}(y_{\Bar{\O}}): W^{2,2}_0 \to \mathbb{R} $ is referred to as the exact cost function or more generally the exact objective. We now apply the \textit{Ritz-method} to solve the problem given in \Eq{eq:Generic_Opt} approximately. Therefore, we choose a finite-dimensional subspace $Y \subset W^{2,2}_0$ and solve for the solution $\bar{y} \in Y$ characterized by, \cite{Grossmann2007},
\begin{align}
    \min\limits_{y \in Y} \mathcal{J}(y) \quad  \text{with} \quad \mathcal{J}(y):= a(y,y) - 2F(y).
    \label{eq:Generic_Opt_Approx}
\end{align}
The state $y$ approximates $y_{\Bar{\O}}$ and is commonly referred to as the ansatz function or test function. This ansatz function is assumed to be given by a known mapping $u(\lamb_{c}): \mathbb{R}^{c} \to Y$, where $c\in \mathbb{N}$ defines the number of control parameters $\lamb$. 

At this point, it is important to mention, that the ability to represent an arbitrary state $y$ on the final hardware is limited. It is required to fulfill the partition of unity in the form of an isoperimetric condition, given by the $L^2$ scalar product as \cite{Troutman1996,Werner2005}
\begin{align}
    (y^*,y)_{L^2} = \int_{\O}  y^*(x) y(x) dx =  1.
    \label{eq:partition_of_unity}
\end{align}

With the restriction to the normalized subspace $(\|y\|_{Y} = 1)$, the problem operates on a constraint functional space. This fact is important to mention and requires to be taken into account in the ongoing derivation. With the variational framework in \Eq{eq:Generic_Opt_Approx} given, the next steps cover the optimization method and the discretization of the continues setting. The consistent approximation of the given theory finalizes in the presentation of numerical results (see Sec.\ref{sec:Applications}).

\subsection{Optimal Control Problem} \label{sec:optimal_control}
Moving the variational framework designed in the previous section into the domain of \textit{Lie groups} allows reducing the computational complexity heavily, given by the variability in the corresponding parameter space \cite{Abrudan2005}. The function $y$ is here made variable by the control $\upb \in \mathbb{R}^{c+1}, \upb: = \left(\lambda_0, \lamb_c\right)^\intercal$, such that 
\begin{align}
    y(x)(\upb) = \lambda_{0} u(x)(\lamb_c).
        \label{eq:Generic_Ansatz}
\end{align} 
The ansatz, $(u(x)(\lamb_c) : (u(x)(\lamb_c)^*, u(x)(\lamb_c))_{L^2} = 1$ as a Lie group embedding, enforces the restriction of the solution $y(x)$. Mention the fact that the parameterization $\lamb_\text{c}$ makes the position $y(x)$ on a hyper-sphere surface variable. Consequently, the path between multiple controls $\lamb_\text{c}$ is always referred to a tangential direction on the hyper-surface of the functional space. Classically speaking, are all ansatz related to a specific Lie Group \cite{Hall2010}.

In the following, we assume that the state $y(x)$ can be represented uniquely by the control $\upb$, $ \upb \mapsto \yb$. This requirement to the ansatz is interpreted as classical equality constraint $e(y,\upb)) =  y(x) - \lambda_{0} u(x)(\lamb_{c}) = 0$. It is straightforward to augment the unconstrained minimization problem in \Eq{eq:Generic_Opt_Approx} by the equality constraint $e(y,\upb)$. As result, mention the optimal control problem
\begin{align}
    \min \limits_{y}  \mathcal{J}(y) \text{ s.t. } e(y,\upb) = 0.
    \label{eq:Generic_OptimalControlProblem}
\end{align}

In terms of optimal control theory, the equality constraint $e(y,\upb)$ denotes a \textit{control-to-state operator}, which is essential in the later-to-be-presented framework \cite{Troutman1996}. Using an indirect approach, e.g. penalty method, to translate the constrained into an unconstrained problem is of small interest. As it is possible here, the constraint $e(y,\upb)$ is realized directly by substitution, which is the straightforward approach, knowing the ansatz $u(x)(\lamb_c)$. In other cases, a Lagrangian framework could be used to realize an unconstrained problem \cite{Nocedal2006}.

By substitution and the unique mapping of the \textit{control-to-state operator}, we formulate the complete  unconstrained optimization problem, given the reduced objective $J(\upb) : \mathbb{R}^{c+1} \to \mathbb{R}$, as 
\begin{align}
	\begin{split}
     \min \limits_{\upb} J(\upb)  \quad \text{with} \quad J(\upb) :=& a(y(\upb),y(\upb)) - 2F(\upb),\\
			 =&  - \nu\int_{\O} \lambda_{0}^2 u(x)(\lamb_{c}) \Delta u(x)(\lamb_{c}) dx - 2 \int_{\O} \lambda_{0} u(x)(\lamb_{c}) f(x) dx.
	\end{split}
\label{eq:Reduced_Opt}
\end{align}
 
The problem in \Eq{eq:Reduced_Opt} can of course be solved using zero-order approaches, e.g. Evolutionary Algorithms, Simulated Annealing, generally speaking sampling methods as they are given in \cite{Nocedal2006, Dennis1996}. The framework presented covers the application of first-order approaches.
Despite, the problem highly depends on the choice of $u(x)(\lamb_c)$ and thus on Lie-Algebra Theory. Choosing problem appropriate $u(x)(\lamb_c)$'s shifts the problem \Eq{eq:Reduced_Opt} into a nonconvex setting, which of course is elaborated in detail given sec. \ref{sec:optimization} \cite{Bittel2021}.\TODO{ADD ref for non convex opt.}

Nevertheless, in both cases, the optimal values coincide with a stationary point. The question of local or global optimum is of course unanswered, despite for the minimum points $\bar{\upb} : J(\upb)  \geq  J(\bar{\upb}) \quad \forall \upb$ \cite{Troutman1996}. Taking the Gâteaux derivative with respect to the argument of $J(\upb)$ the condition for an optimal point can be reformulated as a first-order optimality condition, which is \cite{Troutman1996}
\begin{align}
    \frac{\partial J}{\partial \upb} \delta \upb&= \begin{pmatrix}
            \nabla_{\lambda_0} J(\upb) \\ 
            \nabla_{\lamb_c} J(\upb) 
        \end{pmatrix}  \begin{pmatrix}
            \delta \lambda_0\\
            \delta \lamb_c
        \end{pmatrix} =  0 \quad \forall \delta\upb, \\ 
    \begin{split} 
        &= -2\nu\int_{\O} \lambda_{0} u(\lamb_{c}) \Delta u(\lamb_{c}) \delta \lambda_{0} dx - 2 \int_{\O} u(\lamb_{c}) f \delta\lambda_{0} dx \\
        &\quad\,-\nu\int_{\O} \lambda_{0}^2 u'(\lamb_{c})\delta\lamb_{c}\Delta u(\lamb_{c}) dx-\nu\int_{\O} \lambda_{0}^2 u(\lamb_{c})
        \Delta u(\lamb_{c})' \delta\lamb_{c} dx - 2 \int_{\O} \lambda_{0} u(\lamb_{c})' \delta\lamb_{c} f dx.
    \end{split}
    \label{eq:first_order_opt}
\end{align}
The dash "'“, indicates the derivative with respect to $\lamb_c$. The argument concerning the space in $u$ and $f$ has been neglected for clarity. 

\pover{ Is it the Riemanian Gradient  or  Euklidian Gradient /Derivative ?  }
Proceeding, a reformulation of the Gâteaux derivatives in the equation \Eq{eq:first_order_opt} by the application of Green's Second Identity, to isolate the variational terms, is performed. After two integrations by parts, the Gâteaux derivative with respect to the control gives
\begin{align}
\nabla_{\lambda_0} J(\upb) \delta \lambda_0 &= -2 \nu \lambda_{0} \int_{\O}  u(\lamb_{c}) \Delta u(\lamb_{c}) \delta \lambda_{0} dx -2 \int_{\O} u(\lamb_{c}) f \delta\lambda_{0} dx, \\
\begin{split}
\nabla_{\lamb_c} J(\upb) \delta \lamb_c&= -2\nu \lambda_{0}^2 \int_{\O}  u(\lamb_{c})' \delta\lamb_{c} \Delta u(\lamb_{c}) dx +\nu\lambda_{0}^2  \int_{\B}  u(\lamb_{c}) \frac{\partial u(\lamb_{c})' \delta\lamb_{c}}{\partial n} -  u(\lamb_{c})' \delta\lamb_{c} \frac{\partial u(\lamb_{c})}{\partial n}  ds \\
&\quad \,- 2  \lambda_{0} \int_{\O}   u(\lamb_{c})' \delta\lamb_{c} f(x) dx.  \text{\pover{Reformulate to isolate delta  -  check next eq. }}
\end{split}\\
\begin{split}
&= -2 \nu\lambda_{0}^2 \int_{\O}  \Delta u(\lamb_{c})  u(\lamb_{c})' \delta\lamb_{c}dx +\nu\lambda_{0}^2  \int_{\B}  u(\lamb_{c}) \frac{\partial u(\lamb_{c})' \delta\lamb_{c}}{\partial n} -  \frac{\partial u(\lamb_{c})}{\partial n} u(\lamb_{c})' \delta\lamb_{c}   ds \\
&\quad \,- 2  \lambda_{0} \int_{\O} f(x) u(\lamb_{c})' \delta\lamb_{c}  dx.
\end{split}
\end{align}
\pover{reformulate by pulling variations out  .. just state final solution}

As evident, by the chosen space $H^2_0$ and assuming bijectivity, vanishes, both $u(\lamb_{c})$ and $ u(\lamb_{c})' \delta\lamb_{c}$ on the boundary. Hence, the surface integral can be neglected \cite{Grossmann2007}. In case of a different boundary setting, this expression might need to be taken into account. Section \ref{sec:Discretization} emphasizes on this. However, in contrast to \cite{Sato2021,Leong2022} the first-order optimality condition for $\lambda_0$ is not substituted into the reduced functional $J(\upb)$. Of course, this is a valid approach, nevertheless showed our experience that having full control over $\lambda_0$ is beneficial. Consequently, the variational framework determines the optimal values $\hat{\upb} = \left(\hat{\lambda_0}, \hat{\lamb_c}\right)^\intercal$, which solve the problem in \Eq{eq:Reduced_Opt}. With the continuous formulations of the framework given, the next steps for the computation on quantum hardware are required. In the following, the discretization and hardware compilation of the domain and dynamics is introduced. 

==> Container/C_OldSections/NumericalResults.tex <==
%###########################################
%       Numerical Results
%###########################################
\section{Numerical Results} \label{sec:Applications}
The computational strategy is applied to the following three validation the Poisson Equation (Sec. \ref{sec:Application:Poisson}), the Heat Equation (Sec. \ref{sec:Application:Heat}), and the Wave Equation (Sec. \ref{sec:Application:Wave})\pover{Do we want to show the wave eq results}, respectively. The applications cover various boundary condition settings. For comparison, benchmarks are given by a classical analog to the presented toolbox, which is realized by solving a linear system of equations arising by discretization of the variational \Eq{eq:variational_eq}.
%Mention the counter $\#PAR$, which defines the number of parameters/degrees of freedom (DOF) per problem. To compare the results, references have been implied. 
In the context of this publication, we restrict the simulations to sampling-free idealized quantum devices, available via emulation. The library we present, of course, is subject to scaling effects and robustness when it comes to physical quantum hardware. 

\subsection{The Poisson Equation}
\label{sec:Application:Poisson}
As a first case, assume the temporal derivative in \Eq{eq:Generic_PDE} as vanished. Setting the diffusion coefficient $\nu=-1.0$, one recovers a classical diffusion problem, viz. the Poisson problem. The source term is assumed to be given by a constant $f(x) = 1.0$.

To generalize the complete two-point boundary-value problem in \Eq{eq:Generic_PDE-TR-2}, mention the extension to homogenous and inhomogeneous Dirichlet, Neumann boundary conditions introduced by $D,N$, c.f. Sec. \ref{sec:Discretization}. In common, all boundary value problems reduce to the optimal control problem \Eq{eq:Discrete_Opt_BC}. Here, the source term is augmented as $\Tilde{f}= f + f_\text{ghost}$ given by \Eq{eq:Ghost}. In case of a given value $D$ as Dirichlet Boundary Conditions mention
\begin{align}
     f_\text{ghost} = (\underbrace{-u_1 D \, \left(\frac{\nu \lambda_0^2}{\Delta x^2}\right)}_{\text{source-term modif.} \, f_1},0\hdots,0,
\end{align}

The application of the presented framework to the problem above is finalized in the results given in  \Fig{fig:Results:Poisson}. The rate of convergence is additionally given in \Fig{fig:Results:Poisson:Cost}.

\begin{figure}[H]
\centering
\input{Figures/Results/Legend.tex}\\
    \begin{subfigure}[t]{0.49\textwidth}
       \centering
        \input{Figures/Results/R_Poisson_Dirichlet_homogenous.tex}
        \caption{Dirichlet poison  -  constant RHS homogenous 0 setting} 
        \label{fig:Results:Poisson:homoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Neumann_homogenous.tex}
        \caption{Neumann poison  -  constant RHS homogenous 0 setting} 
        \label{fig:Results:Poisson:homoNeumann}
    \end{subfigure}  \\
     \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Poisson_Dirichlet_inhomogenous}
        \caption{Dirichlet poison  -  constant RHS inhomogenous 0.1 0.2 setting} 
        \label{fig:Results:Poisson:inhomoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
         \input{Figures/Results/R_Poisson_Neumann_inhomogenous.tex}
        \caption{Neumann poison  -  constant RHS inhomogenous 0.1 0.2 setting} 
    \label{fig:Results:Poisson:inhomoNeumann}
    \end{subfigure}  
    \caption{Results Poisson for n=2 and n=4 }
    \label{fig:Results:Poisson}
\end{figure}

\begin{minipage}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{example-image}
        \captionof{figure}{Costfunction }
        \label{fig:Results:Poisson:Cost}
\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
    \centering
    \begin{tabular}{@{}lll@{}}
    \toprule
    Case       & \multicolumn{2}{l}{Norm2 Error} \\ \midrule
               & n=2            & n=4            \\ \midrule
    Dirichlet homogeneous   &                &                \\
    Neumann homogeneous     &                &                \\
    Dirichlet inhomogeneous &                &                \\
    Neumann inhomogeneous   &                &                \\ \bottomrule
    \end{tabular}
    \captionof{table}{Errors Poisson}
    \label{tab:Results:Poisson:Errors}
\end{minipage}
As evident matches determined solution the reference, given by classical FD, perfectly. Quantifying, \Tab{tab:Results:Poisson:Errors} lists the relative error in the 2-Norm and $\infty-$Norm. 

\pover{Dirichlet inhomogeneous 0 with F=1 cost.  and UL =  ? UR= ?}
\pover{Neumann inhomogeneous 0 with \pover{F=1 cost} and  UL =  ? UR= ?}

 \TODO{Discuss results :  Wieso fehler größer 10-7? Ist immer der optimale punkt erreicht ?  Eventuell noch einmal die Laufzeit oder anzahl der Auswertungen aufschreiben. }

\subsection{The Heat Equation} \label{sec:Application:Heat}

\begin{itemize}
    \item 1. Dirichlet homogeneous 0 with F=1 (and u0=0)  
    \item 2. Neumann homogeneous 0 with dirac F=1 and u=0 
    \item 3. inhomogeneous left 10 and right 0 and u0=F=0 (final solution linear) 
    \item 4. Mixxed  -  neumann dirichlet inhomogeneous 
\end{itemize}


\begin{figure}[htbp]
\centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \input{Figures/Results/R_Heat_Dirichlet_homogenous.tex}
        \caption{Dirichlet Heat  -  constant RHS homogenous 0 setting initial const F} 
        \label{fig:Results:Heat:homoDirichlet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
         \centering
        \input{Figures/Results/R_Heat_Dirichlet_inhomogenous.tex}
        \caption{Dirichlet Heat  -  constant RHS homogenous 0 setting initial const F} 
        \label{fig:Results:Heat:inhomoDirichlet}
    \end{subfigure}  
    \caption{Heat RESULTS}
    \label{fig:Results:Heat}
\end{figure}

\begin{figure}[htbp]
    \centering
    \input{Figures/Results/R_Heat_Errors}
    \caption{Norm in all time steps \pover{add the erros of all Heat cases}}
    \label{fig:Results:Heat:Errors}
\end{figure}

\subsection{The Wave Equation } \label{sec:Application:Wave}
% Do similar to : https://people.maths.ox.ac.uk/trefethen/pdectb/wave1d2.pdf

mixxed left right 

\begin{itemize}
    \item 1 . dirac as initial U and 2 hills neumann homo
    \item  2.  dirac as initial U and 2 hills dirichlet homo
\end{itemize}

\begin{figure}
    \centering
    \input{Figures/Results/R_Wave_Dirichlet_homogenous}
    \caption{Numerical Reuslts for the Wave equation problem, using $N_\text{p}=18$ and homogenous dirichlet boundary conditions}
    \label{fig:Wave_Dirichlet}
\end{figure}


initial conditions an $e^{-x^2}$

Additional source terms in the wave eq open the possibilites to model other hyperbolic pdes like Klein Gordon and Sine Gordon equations 





==> Figures/Complexity/C_QNPU_new.tex <==
\tikzsetnextfilename{Complexity-QNPU_new}
\begin{tikzpicture}
\begin{semilogyaxis}[
tick pos=left,
xmajorgrids,
xlabel = $n$,
ylabel = number of gates,
xmin=2, xmax=14,
ymin=10,
ymax=2000,
ymajorgrids,
]

\addplot [solid,semithick]
table [col sep = comma , row sep=crcr]{%
2.0,  16 \\  
4.0,  92 \\  
6.0,  154 \\  
8.0,  216 \\
10.0, 278 \\
12.0, 340 \\
};
\node[above] at (13,280) {{$j_{L_k}$}};

%\addlegendentry{$Laplacian$}

\addplot [dotted,semithick]
table [col sep = comma , row sep=crcr]{%
2.0,  144 \\  
4.0,  288 \\  
6.0,  432 \\  
8.0,  576 \\
10.0, 720 \\
12.0, 864 \\
};
\node[above] at (13,700) {{$j_{S_k}$}};

%\addlegendentry{$Source$}

\addplot [dashed,semithick]
table [col sep = comma , row sep=crcr]{%
2.0,  30 \\  
4.0,  60 \\  
6.0,  90 \\  
8.0,  120 \\
10.0, 150 \\
12.0, 180 \\
};
%\addlegendentry{$Potential$}
\node[above] at (13,110) {{$j_{P_k}$}};


\addplot [dashdotted,semithick]
  table [col sep = comma , row sep=crcr]{% % New Gate scaling commented
 2.0, 77\\
 4.0,  305\\
 6.0,  505\\
 8.0,  705\\
 10.0, 905\\
 12.0, 1105\\
 };
 %\addlegendentry{$Dirichlet$}
 \node[above] at (13,1100) {{{$\tilde j_{DN_k}$}}};


\addplot [loosely dotted,semithick]
table [col sep = comma , row sep=crcr]{%
2.0,  30 \\  
4.0,  60 \\  
6.0,  90 \\  
8.0,  120 \\
10.0, 150 \\
12.0, 180 \\
};
%\addlegendentry{$Neumann$}
\node[above] at (13,150) {{$\tilde j_{N_k}$}};
\end{semilogyaxis}
\end{tikzpicture}


==> Figures/F_Laplace.tex <==
\tikzsetnextfilename{Laplace}
\begin{quantikz}[column sep=0.1cm,row sep=0.1cm]
{\text{CP}}& \vqw{1}&\vqw{1} & \\
\lstick[2]{IP, e.g. $\ket{\psi}$}  & \targ{} & \ctrl{1}& \qw  \rstick[2]{OP} \\
& \qw & \targ{}  & \qw  \\
\end{quantikz}

==> Figures/F_Nonlinear.tex <==
\tikzsetnextfilename{Nonlinear}
\begin{quantikz}[column sep=0.1cm,row sep=0.1cm]
                                 &[1.0cm]&                      {\text{CP}} &\vqw{1} &\vqw{2}&\vqw{4}& & & \vqw{6} & \vqw{7} &\vqw{9} \\
´\lstick[4]{IP$_1$ e.g  $\ket{\psi}^{\otimes^n}$}&[1.0cm]&\lstick{$\ket{\psi_1}$}& \targ{}& \qw   & \qw   &\qw  &&&\hdots&&\qw & \rstick[4]{OP$_1$}\\ 
                                 &[1.0cm]&\lstick{$\ket{\psi_2}$}& \qw    &\targ{}& \qw   &\qw&&&\hdots&&\qw &\\
                                 &[1.0cm]&                       & \vdots &       &       & &&&&&\vdots &\\
                                 &[1.0cm]&\lstick{$\ket{\psi_n}$}&  \qw   &  \qw  &\targ{}&\qw&&&\hdots&&\qw &\\
                                 &\vdots&                &        &       &\vdots &      & &  &  & &\vdots& \\
\lstick[4]{IP$_r$ e.g $\ket{\psi}^{\otimes^n}$}&[1.0cm]&\lstick{$\ket{\psi_1}$}&\qw   &\hdots&&&\qw &\targ{}& \qw  & \qw  & \qw & \rstick[4]{OP$_r$}\\
                                   &[1.0cm]&\lstick{$\ket{\psi_2}$}&\qw   &\hdots&&&\qw& \qw   &\targ{}& \qw  &\qw&\\
                                   &[1.0cm]&          & \vdots&       &       & &  &  &&&\vdots& \\
                                   &[1.0cm]&\lstick{$\ket{\psi_n}$}& \qw &  \hdots&&&\qw &  \qw   &  \qw  & \targ{}& \qw&\\
\end{quantikz}

==> Figures/F_ODRY_ansatz.tex <==
\tikzsetnextfilename{ODRY}
\begin{quantikz}[column sep=0.1cm,row sep=0.1cm]
    \qw&\gate{R_{y}\left(\lambda\right)}&\ctrl{1}&\gate{R_{y}\left(\lambda\right)}&\ctrl{1} &\gate{R_{y}\left(\lambda\right)}&\qw \\
    \qw&\gate{R_{y}\left(\lambda\right)}&\targ{}&\gate{R_{y}\left(\lambda\right)}&\targ{}&\gate{R_{y}\left(\lambda\right)}&\qw 
\end{quantikz}

==> Figures/F_direct_meas.tex <==
\tikzsetnextfilename{direct_meas}
\begin{quantikz}[column sep=0.15cm,row sep=0.1cm]
    \lstick{$\ket{0}^{\otimes n}$ \\Initialize} & \qwbundle{n\quad} & \gate{U} &\meter{Measure $^{\otimes n}$}
\end{quantikz}

==> Figures/F_indirect_meas.tex <==
\tikzsetnextfilename{indirect_meas}
 \begin{quantikz}[column sep=0.1cm,row sep=0.1cm]
    \lstick{$\ket{0}$}  & \gate{H} &  \ctrl{1} & \gate{H} &\meter{Measure}\\
    \lstick{$\ket{\psi}^{\otimes n}$ \\Initialize} & \qwbundle{n} & \gate{U} & \qw & \qw
\end{quantikz}

==> Figures/Results/R_Heat_Dirichlet_inhomogeneous.tex <==
\tikzsetnextfilename{Results-HeatDirichletInHomo}
\begin{tikzpicture}
\begin{axis}[
tick pos=left,
xmajorgrids,
xmin=0, xmax=1,
ymajorgrids,
width=0.75\textwidth,
height=0.45\textwidth,
]



\end{axis}
\end{tikzpicture}


==> highlights.tex <==
\begin{center}
    {\Large
Highlights
}
\end{center}

\begin{itemize}
    \item Variational Quantum algorithm to solve initial-boundary value problems. 
    
    \item Quantum Computing-ready implementations of Dirichlet, Neumann, and Robin conditions.
    
    \item Robust boundary treatment, without additional ansatz or framework requirements. 
    
    \item Excellent agreement with classical finite differences results for heat transfer. 
    
    \item A remarkable \textit{polylog} complexity in the number of grid points or corresponding qubits. 
\end{itemize}

